Dynamical mean-field analysis of adaptive Langevin diffusions: Propagation-of-chaos and convergence of the linear response

Motivated by an application to empirical Bayes learning in high-dimensional regression, we study a class of Langevin diffusions in a system with random disorder, where the drift coefficient is driven by a parameter that continuously adapts to the empirical distribution of the realized process up to the current time. The resulting dynamics take the form of a stochastic interacting particle system having both a McKean-Vlasov type interaction and a pairwise interaction defined by the random disorder. We prove a propagation-of-chaos result, showing that in the large system limit over dimension-independent time horizons, the empirical distribution of sample paths of the Langevin process converges to a deterministic limit law that is described by dynamical mean-field theory. This law is characterized by a system of dynamical fixed-point equations for the limit of the drift parameter and for the correlation and response kernels of the limiting dynamics. Using a dynamical cavity argument, we verify that these correlation and response kernels arise as the asymptotic limits of the averaged correlation and linear response functions of single coordinates of the system. These results enable an asymptotic analysis of an empirical Bayes Langevin dynamics procedure for learning an unknown prior parameter in a linear regression model, which we develop in a companion paper.

==> adaptiveprior.tex <==
\section{Analysis of adaptive dynamics}

In this section, we prove Theorem \ref{thm:adaptivealpha_dynamics} on the
adaptive empirical Bayes dynamics with time-varying prior parameter
$\widehat\alpha^t$, and discuss further the examples of Section
\ref{sec:examples}.

\subsection{General analysis under uniform LSI}

We introduce a few notational shorthands: Conditional on
$\X,\btheta^*,\beps$, let
\[q_\alpha(\btheta) \equiv \sP_{g(\cdot,\alpha)}(\btheta \mid \X,\y)\]
be the posterior law under the prior parameter $\alpha$.
We write $\langle \cdot \rangle_\alpha$ for its posterior expectation. Given
a posterior sample $\btheta \sim q_\alpha$, define
\begin{equation}\label{eq:barqalpha}
\bar \sP_{\btheta}=\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)},
\qquad \bar \sP_\alpha=\langle \bar \sP_{\btheta} \rangle_\alpha.
\end{equation}
Thus $\bar \sP_\alpha$ is a $(\X,\y)$-dependent joint law over variables
$(\theta^*,\theta)$ which satisfies
\begin{equation}\label{eq:barqalphaproperty}
\E_{(\theta^*,\theta) \sim \bar \sP_\alpha} f(\theta^*,\theta)
=\frac{1}{d}\sum_{j=1}^d \langle f(\theta_j^*,\theta_j) \rangle_\alpha
=\frac{1}{d}\sum_{j=1}^d \int f(\theta_j^*,\theta_j) q_\alpha(\btheta)\d\btheta.
\end{equation}
We write $\theta \sim \bar \sP_\alpha$ as shorthand for the $\theta$-marginal of
$(\theta^*,\theta) \sim \bar \sP_\alpha$.

%The following is a statement of the Gibbs variational representation of the
%marginal log-likelihood $\widehat F(\alpha)$.
%
%\begin{proposition}\label{prop:gibbsvariational}
%Suppose Assumption \ref{assump:prior} holds for $g=g(\cdot,\alpha)$.
%Let $\widehat F(\alpha)$ and $V(q,\alpha)$ be as defined in (\ref{eq:hatF}) and
%(\ref{eq:gibbsenergy}). Then
%\[\widehat F(\alpha)=\inf_{q \in \cP_2(\R)} V(q,\alpha).\]
%\end{proposition}
%\begin{proof}
%Note that $g(\cdot,\alpha)$ has finite second moment under Assumption
%\ref{assump:prior}, hence
%\[\int \|\btheta\|_2^2\,q_\alpha(\btheta)\d\btheta
%\leq \frac{1}{\sP_{g(\cdot,\alpha)}(\y \mid \X)}
%\int \|\btheta\|_2^2 \cdot
%(2\pi\sigma^2)^{-n/2}\prod_{j=1}^d g(\theta_j,\alpha)\d\btheta<\infty\]
%so also $q_\alpha \in \cP_2(\R^d)$.
%For any $q \in \cP_2(\R^d)$, by nonnegativity of KL-divergence,
%\[0 \leq \DKL(q \| q_\alpha)
%=\int \big[\log q(\btheta)-\log q_\alpha(\btheta) \big] q(\btheta)\d\btheta
%=d\big(V(q,\alpha)-\widehat F(\alpha)\big),\]
%hence $\widehat F(\alpha) \leq V(q,\alpha)$ with equality attained at
%$q=q_\alpha$.
%\end{proof}

We record the following basic observation, that the bound
(\ref{eq:posteriormeansq}) holds uniformly over compact subsets of $O$.

\begin{lemma}
Under Assumptions \ref{assump:prior} and \ref{assump:compactalpha}, 
for any compact subset $S \subset O$, there 
is a constant $C \equiv C(S)>0$ such that (for any realization of $\X,\y$)
\begin{equation}\label{eq:posteriormeansquniform}
\sup_{\alpha \in S} \langle \|\btheta\|_2^2 \rangle_\alpha
\leq Cd.
\end{equation}
\end{lemma}
\begin{proof}
Under Assumption \ref{assump:prior}, $\alpha \mapsto \log g(0,\alpha)$ and
$\alpha \mapsto \partial_\theta \log g(0,\alpha)$ are both
continuous over $\alpha \in \R^K$, and hence bounded above on $S$.
Then, applying
\[\log g(\theta,\alpha)=\log g(0,\alpha)+\theta \cdot \partial_\theta \log
g(0,\alpha)+\int_0^\theta \int_0^t \partial_\theta^2 \log g(s,\alpha)\d s\,
\d t,\]
under either condition (a) or (b) of Proposition \ref{prop:LSI} and
the uniform boundedness of $\partial_\theta^2 \log g(\theta,\alpha)$ ensured by
Assumption \ref{assump:prior}, we have
$\log g(\theta,\alpha) \leq C-c\theta^2$ for some constants $C,c>0$, all $\theta
\in \R$, and all $\alpha \in S$. This implies that the first and second moments
$\E_{g(\cdot,\alpha)} \theta$ and $\E_{g(\cdot,\alpha)} \theta^2$
are uniformly bounded over $\alpha \in S$. Then
(\ref{eq:posteriormeansquniform}) follows from the same argument as that of
(\ref{eq:posteriormeansq}) in Lemma \ref{lemma:elementarybounds}.
\end{proof}

We now prove Lemma \ref{lemma:gradalphaF} on the derivatives of
$F,\widehat F$ and uniform convergence of
$\widehat F,\nabla \widehat F$ over compact subsets of $O$.

\begin{proof}[Proof of Lemma \ref{lemma:gradalphaF}]
Let $O \subset \R^K$ be the open domain of
Assumption \ref{assump:compactalpha}, and define the $(\X,\y)$-event
\[\event(C_\LSI)=\{
\text{(\ref{eq:LSI}) holds for } q_\alpha(\btheta) \equiv
\sP_{g(\cdot,\alpha)}(\btheta \mid \X,\y) \text{ for every } \alpha \in O\}.\]
Assumption \ref{assump:compactalpha} ensures that for a large enough
constant $C_\LSI>0$, $\event(C_\LSI)$ holds a.s.\ for all large $n,d$.
Let $Q$ be a countable dense subset of $O$. Throughout the proof,
we restrict to the almost-sure event where the convergence statements of
Corollary \ref{cor:fixedalpha_dynamics} and Proposition
\ref{prop:mseconcentration} hold for every $\alpha \in Q$, and where
$\event(C_\LSI)$ holds for all large $n,d$.

For (a), differentiating
\[\widehat F(\alpha)={-}\frac{1}{d}\log
\int \Big(\frac{1}{2\pi\sigma^2}\Big)^{n/2}
\exp\Big({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+\sum_{j=1}^d \log g(\theta_j,\alpha)\Big)\d\btheta\]
and applying the property (\ref{eq:barqalphaproperty}), we have
\begin{equation}\label{eq:hatFderivcalculation}
\nabla \widehat F(\alpha)={-}\frac{1}{d}\sum_{j=1}^d \langle \nabla_\alpha
\log g(\theta_j,\alpha) \rangle_\alpha
=-\E_{\theta \sim \bar \sP_\alpha} \nabla_\alpha \log g(\theta,\alpha).
\end{equation}
For the form of $\nabla F(\alpha)$, define analogously to (\ref{eq:fomega})
\begin{equation}\label{eq:fomegaalpha}
f(\omega,\omega_*,\alpha)
={-}\E_{g_*,\omega_*}\log \sP_{g(\cdot,\alpha),\omega}(Y)
-\frac{1}{2}\left(2\delta+\log \frac{2\pi}{\omega}
-\delta \log \frac{\delta}{\omega\sigma^2}
+(1-\delta)\frac{\omega}{\omega_*}
+\omega\sigma^2\Big(\frac{\omega}{\omega_*}-2\Big)\right)
\end{equation}
where the dependence on $\alpha$ is in $\sP_{g(\cdot,\alpha),\omega}(Y)$.
For any
$\alpha \in O$, let $\omega(\alpha),\omega_*(\alpha)$ be the fixed points
$\omega,\omega_*$ of (\ref{eq:mmse}) corresponding to the DMFT system with fixed
prior $g \equiv g(\cdot,\alpha)$. (This DMFT system is regular and exponentially
convergent by Proposition \ref{prop:LSI} and Theorem
\ref{thm:fixedalpha_dynamics}, hence $\omega(\alpha),\omega_*(\alpha)$ are
well-defined.) Then
\begin{equation}\label{eq:Ffrelation}
F(\alpha)=f(\omega(\alpha),\omega_*(\alpha),\alpha)
+\frac{\delta}{2}(1+\log 2\pi\sigma^2).
\end{equation}
We recall from the calculations of (\ref{eq:omegastationarity}) that
at the fixed points $(\omega(\alpha),\omega_*(\alpha))$, we have
$\partial_\omega f(\omega(\alpha),\omega_*(\alpha),\alpha)=0$ and
$\partial_{\omega_*} f(\omega(\alpha),\omega_*(\alpha),\alpha)=0$. 
By Lemma \ref{lemma:mmse_lipschitz}, $\omega(\alpha),\omega_*(\alpha)$
are locally Lipschitz and hence absolutely continuous over $\alpha \in O$. Then,
differentiating by the chain rule,
\begin{align*}
\nabla F(\alpha)&=\nabla_\alpha
f(\omega,\omega_*,\alpha)\Big|_{(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))}\\
&={-}\nabla_\alpha\bigg[\E_{g_*,\omega_*}\log \sP_{g(\cdot,\alpha),\omega}
(Y)\bigg]\bigg|_{(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))}\\
&={-}\nabla_\alpha\bigg[\E_{g_*,\omega_*} \log\int
\Big(\frac{\omega}{2\pi}\Big)^{1/2}
\exp\Big({-}\frac{\omega}{2}(Y-\theta)^2+\log g(\theta,\alpha)\Big)\d\theta
\bigg]
\bigg|_{(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))}
\end{align*}
By definition $\sP_\alpha$ is the joint law of $(\theta^*,\theta)$ under the
generative process where $(\theta^*,Y)$ are drawn from the law defining
$\E_{g_*,\omega_*}$, and $\theta \sim P_{g(\cdot,\alpha),\omega}(\theta
\mid Y)$. Hence, evaluating $\nabla_\alpha$ above gives
\[\nabla F(\alpha)={-}\E_{\theta \sim \sP_\alpha} \nabla_\alpha \log g(\theta,\alpha).\]

For (b), consider any compact $S \subset O$. Let $C,C'>0$ denote constants
depending on $S$ changing from instance to instance.
Note that Corollary \ref{cor:fixedalpha_dynamics} shows
$\widehat F(\alpha) \to F(\alpha)$ for each $\alpha \in Q$. 
Assumption \ref{assump:prior} implies that 
$\partial_\theta \nabla_\alpha \log g(\theta,\alpha)$ is uniformly
bounded over $(\theta,\alpha) \in \R \times S$, so
\[\|\nabla_\alpha \log g(\theta,\alpha)\|_2 \leq 
\|\nabla_\alpha \log g(0,\alpha)\|_2+C|\theta|.\]
Then, since $\nabla_\alpha \log g(0,\alpha)$ must be bounded
over $\alpha \in S$, and $\sup_{\alpha \in S}
\langle \|\btheta\|_2^2 \rangle_\alpha \leq Cd$
by (\ref{eq:posteriormeansquniform}), we have
\begin{align}
\sup_{\alpha \in S}
\|\E_{\theta \sim \bar \sP_\alpha} \nabla_\alpha \log g(\theta,\alpha)\|_2
&\leq \sup_{\alpha \in S}
\frac{1}{d}\sum_{j=1}^d \langle\|\nabla_\alpha \log g(\theta_j,\alpha)\|_2
\rangle_\alpha\notag\\
&\leq \sup_{\alpha \in S}
\|\nabla_\alpha \log g(0,\alpha)\|_2
+\frac{C}{d}\sum_{j=1}^d \langle |\theta_j| \rangle_\alpha \leq C'.\label{eq:nablaFboundO}
\end{align}
This shows $\nabla \widehat F(\alpha)$ is bounded over compact
subsets of $O$. Then for any compact subset $S \subset O$,
the functions $\widehat F(\alpha)$ for all $n,d$ are equicontinuous in a
neighborhood of each point
$\alpha \in S$, and hence are uniformly equicontinuous over $S$ since a finite
number of such neighborhoods cover $S$. Then by Arzela-Ascoli, the
convergence $\widehat F(\alpha) \to F(\alpha)$ for each $\alpha \in Q$ implies
uniform convergence over $\alpha \in S$.

We next show the pointwise convergence $\nabla \widehat F(\alpha) \to \nabla
F(\alpha)$ for each $\alpha \in Q$. Recalling our definition of
$\bar \sP_{\btheta}$ in (\ref{eq:barqalpha}) and applying
the convexity $W_2(\lambda\sP+(1-\lambda)\sP',\sQ)^2 \leq 
\lambda W_2(\sP,\sQ)^2+(1-\lambda)W_2(\sP',\sQ)^2$ and Jensen's inequality,
\[W_2(\bar \sP_\alpha,\sP_\alpha)^2
\leq \langle W_2(\bar \sP_{\btheta},\sP_\alpha)^2 \rangle_\alpha.\]
For each $\alpha \in Q$, the right side converges to 0 as $n,d \to \infty$
by Corollary \ref{cor:fixedalpha_dynamics}(a). Thus
\[\lim_{n,d \to \infty} W_1(\bar \sP_\alpha,\sP_\alpha)
\leq \lim_{n,d \to \infty} W_2(\bar \sP_\alpha,\sP_\alpha)=0.\]
Assumption \ref{assump:prior} ensures that $\nabla_\alpha
\log g(\theta,\alpha)$ is Lipschitz in $\theta$,
so this Wasserstein-1 convergence implies
\[\lim_{n,d \to \infty} \nabla \widehat F(\alpha)
=\lim_{n,d \to \infty} \E_{\theta \sim \bar \sP_\alpha} \nabla_\alpha \log
g(\theta,\alpha)=\E_{\theta \sim \sP_\alpha} \nabla_\alpha \log
g(\theta,\alpha)=\nabla F(\alpha)\]
for each $\alpha \in Q$, as claimed.

To extend this to uniform convergence over any compact subset $S \subset O$,
we differentiate (\ref{eq:hatFderivcalculation}) a second time.
Writing $\Var_\alpha,\Cov_\alpha$ for the
variance and covariance under $\langle \cdot \rangle_\alpha$,
\begin{equation}\label{eq:hessF}
\nabla^2 \widehat F(\alpha)=
-\frac{1}{d}\bigg\langle\sum_{j=1}^d \nabla_\alpha^2 \log
g(\theta_j,\alpha)\bigg \rangle_\alpha
-\frac{1}{d}\Cov_\alpha\bigg[\sum_{j=1}^d \nabla_\alpha \log
g(\theta_j,\alpha)\bigg].
\end{equation}
The first term is uniformly bounded over $\alpha \in S$, by
the same argument as showing boundedness of $\nabla \widehat F(\alpha)$ above.
For the second term, on the event $\event(C_\LSI)$,
for every unit vector $v \in \R^K$ and $\alpha \in S$,
\[\Var_\alpha\bigg[\sum_{j=1}^d v^\top \nabla_\alpha \log
g(\theta_j,\alpha)\bigg]
\leq (C_\LSI/2)\bigg\langle
\sum_{j=1}^d \Big(v^\top \partial_\theta \nabla_\alpha \log
g(\theta_j,\alpha)\Big)^2\bigg \rangle_\alpha\]
by the Poincar\'e inequality for $q_\alpha$ implied by its LSI. Since
$\partial_\theta \nabla_\alpha \log g(\theta,\alpha)$ is
bounded over $\alpha \in S$, the second term of (\ref{eq:hessF}) is also
bounded on $\event(C_\LSI)$.
Thus $\nabla^2 \widehat F(\alpha)$ is uniformly bounded over $\alpha
\in S$ for all large $n,d$. This implies as above that for any compact $S
\subset O$, the functions $\nabla \widehat F(\alpha)$ for all large $n,d$ are
uniformly equicontinuous on $S$, and hence
$\nabla \widehat F(\alpha) \to \nabla F(\alpha)$ uniformly over $\alpha \in S$.
This shows part (b).

For part (c), note that if $g^*=g(\cdot,\alpha^*)$, then
\[\E_\y \widehat F(\alpha)-\E_\y \widehat F(\alpha^*)
=d^{-1}\DKL(\sP_{g(\cdot,\alpha^*)}(\y \mid \X) \|
\sP_{g(\cdot,\alpha)}(\y \mid \X)) \geq 0,\]
so $\alpha^*$ is a minimizer of $\alpha \mapsto \E_\y \widehat F(\alpha)$ over
$\R^K$. Applying the convergence $\widehat F(\alpha)-\E_\y \widehat
F(\alpha) \to 0$ for each $\alpha \in Q$ from Proposition
\ref{prop:mseconcentration}, we have also
$\E_\y \widehat F(\alpha) \to F(\alpha)$ for each $\alpha \in Q$. Note that
\[\nabla_\alpha \E_\y \widehat F(\alpha)
={-}\E_\y \E_{\theta \sim \bar \sP_\alpha}
\nabla_\alpha \log g(\theta,\alpha),\]
and that $\sup_{\alpha \in S} \E_\y \langle \|\btheta\|_2^2 \rangle_\alpha \leq
Cd$ for each compact $S \subset O$ since (\ref{eq:posteriormeansquniform}) holds for any realization of $\y$.
Then the argument (\ref{eq:nablaFboundO}) shows also that
$\nabla_\alpha \E_\y \widehat F(\alpha)$ is uniformly bounded over $\alpha \in
S$, hence
\[\lim_{n,d \to \infty} \sup_{\alpha \in S} |\E_\y \widehat
F(\alpha)-F(\alpha)|_2=0.\]
Since $\alpha^*$ is a minimizer of
$\E_\y \widehat F(\alpha)$, this implies that
$F(\alpha) \geq F(\alpha^*)$ for every $\alpha \in S$. Since this holds for any
compact $S \subset O$, this shows part (c).
\end{proof}

We proceed to prove Theorem \ref{thm:adaptivealpha_dynamics}.
Let $\{\btheta^t,\widehat\alpha^t\}_{t \geq 0}$ be the strong solution of the
SDE (\ref{eq:langevin_sde}--\ref{eq:gflow}) under the choice
of $\cG(\alpha,\sP)$ in (\ref{eq:FalphaEB}). Let $\{\alpha^t\}_{t \geq 0}$ be
the (deterministic) DMFT limit of $\{\widehat\alpha^t\}_{t \geq 0}$. Consider
the SDE
\begin{equation}\label{eq:tildethetaSDE}
\d\tilde\btheta^t=\nabla_{\tilde\btheta}\bigg({-}\frac{1}{2\sigma^2}\|\y-\X\tilde\btheta^t\|_2^2
+\sum_{j=1}^d \log g(\tilde \theta_j^t,\alpha^t)\bigg)\d t+\sqrt{2}\,\d\b^t
\end{equation}
which replaces $\widehat\alpha^t$ by $\alpha^t$, with the initial
conditions $\tilde\btheta^0=\btheta^0$ and $\alpha^0$ of Assumption
\ref{assump:model}, and defined by
the same Brownian motion $\{\b^t\}_{t \geq 0}$
as that of $\{\btheta^t,\widehat\alpha^t\}_{t \geq 0}$.

We write $q_t$ for the density of $\tilde\btheta^t$ conditional on
$\X,\btheta^*,\beps$, where $q_0=g_0^{\otimes d}$ is the initial density of
$\tilde\btheta^0=\btheta^0$. In parallel to (\ref{eq:barqalpha}), we denote
\begin{equation}\label{eq:barqt}
\bar \sP_{\tilde\btheta^t}=\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\tilde
\theta_j^t)},
\qquad \bar \sP_t=\E_{\tilde \btheta^t \sim q_t} \bar \sP_{\tilde\btheta^t}
\end{equation}
where $\E_{\tilde \btheta^t \sim q_t}$ is the expectation with respect to this
density $q_t$, i.e.\ over the law of
$\tilde\btheta^t$ conditional on $\X,\btheta^*,\beps$. We write
$\tilde \theta^t \sim \bar \sP_t$ for the $\tilde \theta^t$-marginal
of a sample $(\theta^*,\tilde \theta^t) \sim \bar \sP_t$.

\begin{lemma}\label{lemma:Vdecreasing}
Under Assumptions \ref{assump:model}, \ref{assump:prior}, and
\ref{assump:gradient}, there exists a unique strong solution
$\{\tilde\btheta^t\}_{t \geq 0}$ to (\ref{eq:tildethetaSDE}).
Letting $q_t$ be the above conditional density of $\tilde\btheta^t$, and
letting $V(q,\alpha)$ be the Gibbs free energy (\ref{eq:gibbsenergy}), then almost surely
\begin{equation}\label{eq:Vdecreasing}
\limsup_{n,d \to \infty}
\sup_{t \in [0,T]} \frac{\d}{\d t} \Big(V(q_t,\alpha^t)+R(\alpha^t)\Big) \leq 0.
\end{equation}
\end{lemma}
\begin{proof}
Fixing $C_0>0$ large enough, let
\[\event(C_0)=\{\|\X\|_\op \leq C_0,\;
\|\y\|_2^2 \leq C_0d,\;\|\btheta^0\|_2^2 \leq C_0d\}.\]
We restrict to the event where the almost-sure statements of
Theorem \ref{thm:dmft_approx} hold and where
$\event(C_0)$ holds for all large $n,d$.

By (\ref{eq:alphaconfined}), for any $T>0$, there exists a compact ball
$S_T$ depending on $C_0,T$ such that $\widehat\alpha^t \in S_T$ for all $t \in
[0,T]$. Since $\widehat\alpha^t \to \alpha^t$ as $n,d \to \infty$, this implies
also $\alpha^t \in S_T$ for all $t \in [0,T]$.
By Assumption \ref{assump:prior}, $(\theta,\alpha)
\mapsto \log \partial_\theta g(\theta,\alpha)$ restricted to $\alpha \in S_T$
is Lipschitz. Then the drift of (\ref{eq:tildethetaSDE}) is Lipschitz over
each time horizon $[0,T]$, so (\ref{eq:tildethetaSDE}) 
admits a unique strong solution $\{\tilde\btheta^t\}_{t \geq 0}$
(c.f.\ \cite[Theorem II.1.2]{kunita1984stochastic}). We note that
\[\frac{\d}{\d t}(\tilde \btheta^t-\btheta^t)
=\frac{1}{\sigma^2}\X^\top \X(\btheta^t-\tilde\btheta^t)
+\Big[\partial_\theta \log g(\tilde \theta_j^t,\alpha^t)-
\partial_\theta \log g(\theta_j^t,\widehat\alpha^t)\Big]_{j=1}^d.\]
Applying again the Lipschitz property of
$(\theta,\alpha) \mapsto \log g(\theta,\alpha)$
and the bound $\|\X\|_\op \leq C_0$, there is a constant $C>0$ depending on
$C_0,T$ such that
\[\bigg\|\frac{1}{\sqrt{d}}\frac{\d}{\d t}(\tilde \btheta^t-\btheta^t)\bigg\|_2
\leq \frac{C}{\sqrt{d}}
\|\tilde \btheta^t-\btheta^t\|_2+C\|\alpha^t-\widehat\alpha^t\|_2.\]
Since $\sup_{t \in [0,T]} \|\alpha^t-\widehat\alpha^t\|_2 \to 0$
by Theorem \ref{thm:dmft_approx}(a), a Gronwall argument implies
\begin{equation}\label{eq:tildethetaerror}
\lim_{n,d \to \infty}
\sup_{t \in [0,T]} \frac{1}{\sqrt{d}}\|\tilde\btheta^t-\btheta^t\|_2=0.
\end{equation}

By definition of the
DMFT equations, the evolution of $\alpha^t$ under the choice
of $\cG(\alpha,\sP)$ in (\ref{eq:FalphaEB}) is given by
\begin{equation}\label{eq:alphaflowEB}
\frac{\d}{\d t} \alpha^t=\E_{\theta^t \sim \sP(\theta^t)}
\nabla_\alpha \log g(\theta^t,\alpha^t)-\nabla R(\alpha^t)
\end{equation}
where $\sP(\theta^t)$ is the law of the DMFT variable $\theta^t$.
The law $q_t$ of $\tilde\btheta^t$ satisfies the Fokker-Planck equation
\begin{equation}\label{eq:FokkerPlanck}
\frac{\d}{\d t} q_t(\btheta)
=\nabla_{\btheta} \cdot \bigg[q_t(\btheta)\nabla_{\btheta}\bigg(
\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2-\sum_{j=1}^d
\log g(\theta_j,\alpha^t)+\log q_t(\btheta)\bigg)\bigg].
\end{equation}
Then, using (\ref{eq:alphaflowEB}) and (\ref{eq:FokkerPlanck}) to differentiate
$V(q_t,\alpha^t)+R(\alpha^t)$ by the chain rule,
\begin{align}
\frac{\d}{\d t} \Big(V(q_t,\alpha^t)+R(\alpha^t)\Big)
&={-}\frac{1}{d}\underbrace{\int
\bigg\|\nabla_{\btheta}\Big(\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2-\sum_{j=1}^d
\log g(\theta_j,\alpha^t)+\log q_t(\btheta) \Big)
\bigg\|_2^2 q_t(\btheta)\d\btheta}_{:=\FI_t}\label{eq:defFI}\\
&-\Big(\E_{\theta^t \sim \sP(\theta^t)}\nabla_\alpha \log
g(\theta^t,\alpha^t)-\nabla R(\alpha^t)\Big)^\top \Big(\int \frac{1}{d}\sum_{j=1}^d \nabla_\alpha
\log g(\theta_j,\alpha^t)q_t(\btheta)\d\btheta-\nabla R(\alpha^t)\Big).\notag
\end{align}
Here, the first term $\FI_t$ (the relative Fisher information) arises
from differentiation in $q_t$ and integration-by-parts in $\btheta$,
while the second term arises from differentiation in $\alpha^t$. 
Recalling the notation (\ref{eq:barqt}),
\[\int \frac{1}{d}\sum_{j=1}^d \nabla_\alpha
\log g(\theta_j,\alpha^t)q_t(\btheta)\d\btheta
=\E_{\tilde \theta^t \sim \bar \sP_t} \nabla_\alpha \log g(\tilde \theta^t,\alpha^t)\]
so we may write the above as 
\begin{equation}\label{eq:Gibbstimederiv}
\begin{aligned}
\frac{\d}{\d t} \Big(V(q_t,\alpha^t) + R(\alpha^t)\Big)
&={-}\frac{1}{d}\,\FI_t
-\Big\|\E_{\tilde \theta^t \sim \bar \sP_t} \nabla_\alpha \log
g(\tilde \theta^t,\alpha^t)-\nabla R(\alpha^t)\Big\|^2\\
&\hspace{0.5in}
+\underbrace{\Big(\E_{\tilde \theta^t \sim \bar \sP_t}
\nabla_\alpha \log g(\tilde \theta^t,\alpha^t)
-\E_{\theta^t \sim \sP(\theta^t)}
\nabla_\alpha \log g(\theta^t,\alpha^t)
\Big)^\top \Big(\E_{\tilde \theta^t \sim \bar \sP_t} \nabla_\alpha \log
g(\tilde \theta^t,\alpha^t)-\nabla R(\alpha^t)\Big)}_{:=\Delta_t}.
\end{aligned}
\end{equation}
By the convexity 
$W_2(\lambda\sP+(1-\lambda)\sP',\sQ)^2 \leq 
\lambda W_2(\sP,\sQ)^2+(1-\lambda)W_2(\sP',\sQ)^2$ and Jensen's inequality,
\[W_2(\bar \sP_t,\sP(\theta^*,\theta^t))^2
\leq \E_{\tilde \btheta^t \sim q_t} W_2(\bar \sP_{\tilde
\btheta^t},\sP(\theta^*,\theta^t))^2\]
where $\sP(\theta^*,\theta^t)$ is the joint law of the  DMFT variables
$(\theta^*,\theta^t)$.
By Theorem \ref{thm:dmft_approx}(b) and (\ref{eq:tildethetaerror}), for any
fixed $T>0$ we have
\[\sup_{t \in [0,T]}
W_2(\bar \sP_{\tilde \btheta^t},\sP(\theta^*,\theta^t))^2
\leq \sup_{t \in [0,T]} 2W_2(\bar \sP_{\tilde \btheta^t},\bar \sP_{\btheta^t})^2
+2W_2(\bar \sP_{\btheta^t},\sP(\theta^*,\theta^t))^2 \to 0\]
as $n,d \to \infty$.
Since $W_2(\bar \sP_{\tilde \btheta^t},\sP(\theta^*,\theta^t))^2
\leq Cd^{-1}(\|\btheta^*\|_2^2+\|\tilde \btheta^t\|_2^2
+\E (\theta^*)^2+\E(\theta^t)^2)$ which is uniformly
integrable under $\tilde \btheta^t \sim q_t$ for all $t \in [0,T]$
and all large $n,d$, the dominated convergence theorem then implies
\begin{equation}\label{eq:barqconvergence}
\lim_{n,d \to \infty} \sup_{t \in [0,T]}
W_2(\bar \sP_t,\sP(\theta^*,\theta^t))=0.
\end{equation}
Recalling that
$(\theta,\alpha) \mapsto \nabla_\alpha \log g(\theta,\alpha)$ is uniformly
Lipschitz over $\alpha \in S_T$, this Wasserstein-2 convergence implies
\[\lim_{n,d \to \infty}
\sup_{t \in [0,T]} \Big|\E_{\theta \sim \bar \sP_t}
\nabla_\alpha \log g(\theta,\alpha^t)
-\E_{\theta \sim \sP(\theta^t)}
\nabla_\alpha \log g(\theta,\alpha^t)\Big|=0,\]
hence $\lim_{n,d \to \infty} \sup_{t \in [0,T]} |\Delta_t|=0$ for the quantity
$\Delta_t$ of (\ref{eq:Gibbstimederiv}).
As the first two terms of (\ref{eq:Gibbstimederiv}) are non-positive, this shows
(\ref{eq:Vdecreasing}).
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:adaptivealpha_dynamics}]
Let $O \subset \R^K$ be the domain of
Assumption \ref{assump:compactalpha}.
Fixing sufficiently large constants $C_0,C_\LSI>0$, define
\[\event(C_0,C_\LSI)=\{\|\X\|_\op \leq C_0,\;
\|\y\|_2^2 \leq C_0d,\;\|\btheta^0\|_2^2 \leq C_0d,\;
\text{and (\ref{eq:LSI}) holds for } q_\alpha \text{ for every } \alpha \in O\}.\]
We restrict to the event where the almost-sure statements of
Assumption \ref{assump:model}(d), Theorem
\ref{thm:dmft_approx}, and Lemma \ref{lemma:gradalphaF} all hold, and where
$\event(C_0,C_\LSI)$ holds for all large $n,d$. Throughout, $C,C',c>0$
denote constants that may depend on $C_0,C_\LSI$ and change
from instance to instance.

We first show that for a constant $C>0$,
\[\int_0^\infty \|\nabla F(\alpha^t)+\nabla R(\alpha^t)\|_2^2 \d t<C.\]
We remind the reader that $q_t$ is the law of $\tilde\btheta^t$ (conditioned on
$\X,\btheta^*,\beps$) and $q_{\alpha^t}$ is the posterior law of $\btheta$ under
the prior $g \equiv g(\cdot,\alpha^t)$.
On $\event(C_0,C_\LSI)$, the LSI for $q_{\alpha^t}$ and its implied
$T_2$-transportation inequality
(c.f.\ \cite[Theorem 9.6.1]{bakry2014analysis}) imply
for the Fisher information term $\FI_t$ of (\ref{eq:defFI}) that
\[\FI_t \geq C_{\LSI}^{-1} \DKL(q_t\| q_{\alpha^t}) \geq 
C_{\LSI}^{-2} W_2(q_t,q_{\alpha^t})^2\]
for all $t \geq 0$. The average marginal
distribution of coordinates of $\tilde \btheta^t \sim q_t$ is the
$\tilde\theta^t$-marginal of $\bar \sP_t$ defined
in (\ref{eq:barqt}),
and that of $\btheta \sim q_{\alpha^t}$ is the $\theta$-marginal of
$\bar \sP_{\alpha^t}$ as defined in (\ref{eq:barqalpha}).
Considering the coordinatewise coupling of $\bar \sP_t,\bar \sP_{\alpha^t}$,
we see that
$W_2(\bar \sP_t, \bar \sP_{\alpha^t})^2 \leq d^{-1}W_2(q_t,q_{\alpha^t})^2$, so
\begin{equation}\label{eq:FIW2qbar}
d^{-1}\FI_t \geq C_{\LSI}^{-2}W_2(\bar \sP_t,\bar \sP_{\alpha^t})^2.
\end{equation}
Applying this and the uniform Lipschitz continuity of
$\theta \mapsto \nabla_\alpha \log g(\theta,\alpha)$ over $\alpha \in O$
guaranteed by Assumption \ref{assump:compactalpha},
\[\Big\|\E_{\tilde \theta^t \sim \bar \sP_t} \nabla_\alpha \log g(\tilde
\theta^t,\alpha^t)
-\E_{\theta \sim \bar \sP_{\alpha^t}} \nabla_\alpha \log g(\theta,\alpha^t)
\Big\|_2^2
\leq C'\,W_2(\bar \sP_t, \bar \sP_{\alpha^t})^2
\leq Cd^{-1}\FI_t.\]
Then applying this as a lower bound for $d^{-1}\FI_t$ in
(\ref{eq:Gibbstimederiv}), and applying also $C^{-1}(a-b)^2+b^2 \geq c_0a^2$
for a constant $c_0>0$ and all $a,b \in \R$, we get from
(\ref{eq:Gibbstimederiv}) that
\[\frac{\d}{\d t} \Big(V(q_t,\alpha^t)+R(\alpha^t)\Big)
\leq {-}c_0\Big\|\E_{\theta \sim \bar \sP_{\alpha^t}} \nabla_\alpha \log
g(\theta,\alpha^t)-\nabla R(\alpha^t)\Big\|^2+\Delta_t.\]
Now note from Lemma \ref{lemma:gradalphaF} that
\[\E_{\theta \sim \bar \sP_{\alpha^t}} \nabla_\alpha \log
g(\theta,\alpha^t)={-}\nabla \widehat F(\alpha^t).\]
Applying $\sup_{t \in [0,T]} \Delta_t \to 0$ and the uniform convergence
$\nabla \widehat F(\alpha) \to \nabla F(\alpha)$ over $\alpha \in S_T$
from Lemma \ref{lemma:gradalphaF} (where $S_T$ is a compact domain that contains
$\{\alpha^t\}_{t \in [0,T]}$), this shows a strengthening of
(\ref{eq:Vdecreasing}),
\[\limsup_{n,d \to \infty} \sup_{t \in [0,T]}
\frac{\d}{\d t} \Big(V(q_t,\alpha^t)+R(\alpha^t)\Big)
\leq {-}c_0\|\nabla F(\alpha^t)+\nabla
R(\alpha^t)\|_2^2.\]
Then for any $T>0$,
\[c_0\int_0^T \|\nabla F(\alpha^t)+\nabla R(\alpha^t)\|_2^2\,\d t
\leq \limsup_{n,d \to \infty}
V(q_0,\alpha^0)+R(\alpha^0)-V(q_T,\alpha^T)-R(\alpha^T).\]
Note that $V(q_0,\alpha^0)=V(g_0^{\otimes d},\alpha^0)$ is bounded above by a
constant on $\event(C_0,C_\LSI)$ for all large $n,d$, while
by the definition (\ref{eq:gibbsenergy}),
\[V(q_T,\alpha^T) \geq \frac{1}{d}\DKL(q_T\|g(\cdot,\alpha^T)^{\otimes d})
+\frac{n}{2d}\log 2\pi\sigma^2
\geq \frac{n}{2d}\log 2\pi\sigma^2\]
which is bounded below by a constant for all $T$ and all large $n,d$.
Then taking the limit $n,d \to \infty$ followed by
$T \to \infty$ shows, for some constant $C>0$,
\begin{equation}\label{eq:intgradFsquared}
\int_0^\infty \|\nabla F(\alpha^t)+\nabla R(\alpha^t)\|_2^2\,\d t<C
\end{equation}
as claimed.

Suppose now that all points of
\[\Crit:=\{\alpha \in O:\nabla F(\alpha)+\nabla R(\alpha)=0\}\]
are isolated. By compactness, $\{\alpha^t\}_{t \geq 0}$ has at least one limit
point $\alpha^\infty \in S$. Suppose by contradiction that
$\alpha^\infty \notin \Crit$. 
Lemma \ref{lemma:gradalphaF} implies that $\nabla F(\alpha)+\nabla R(\alpha)$
is continuous over $\alpha \in O$, so this implies
$\|\nabla F(\alpha)+\nabla R(\alpha)\|_2>\delta$ for all $\alpha \in
B_\delta(\alpha^\infty):=\{\alpha:\|\alpha-\alpha^\infty\|_2<\delta\}$
and some $\delta>0$. However, Assumption \ref{assump:prior} and the condition
$\alpha^t \in S$ imply
\begin{equation}\label{eq:dtalphabound}
\bigg\|\frac{\d}{\d t}\alpha^t\bigg\|_2
\leq \E_{\theta \sim \sP(\theta^t)}\|\nabla_\alpha \log g(\theta,\alpha^t)\|_2
+\|\nabla R(\alpha^t)\|_2
\leq C(1+\E|\theta^t|+\|\alpha^t\|_2) \leq C'
\end{equation}
for constants $C,C'>0$ and all $t \geq 0$. Then for each $t_0 \geq 0$ such that
\begin{equation}\label{eq:alphat0}
\alpha^{t_0} \in B_{\delta/2}(\alpha^\infty)
\end{equation}
we must have
$\alpha^t \in B_\delta(\alpha^\infty)$ for all $t \in [t_0-c\delta,t_0+c\delta]$
and some constant $c>0$. Then $\int_{t_0-c\delta}^{t_0+c\delta} \|\nabla
F(\alpha^t)+\nabla R(\alpha^t)\|_2^2\,\d t \geq 2c\delta^3$. The condition (\ref{eq:alphat0}) must
hold for infinitely many times $t_0$ because $\alpha^\infty$ is a limit point of
$\{\alpha^t\}_{t \geq 0}$,
but this contradicts (\ref{eq:intgradFsquared}). Thus we must have
$\alpha^\infty \in \Crit$. Since this holds for
every limit point $\alpha^\infty$ of $\{\alpha^t\}_{t \geq 0}$, and all points
of $\Crit$ are isolated, this implies that the limit point $\alpha^\infty$
of $\{\alpha^t\}_{t \geq 0}$ is unique, and
\[\lim_{t \to \infty} \alpha^t=\alpha^\infty.\]

For any $\eps>0$, choosing $T(\eps)$ such that
$\|\alpha^t-\alpha^\infty\|_2<\eps/2$ for all $t>T(\eps)$, we then have
$\limsup_{n,d \to \infty} \|\widehat\alpha^t-\alpha^\infty\|_2<\eps$
by Theorem \ref{thm:dmft_approx}(a), showing the first statement of
(\ref{eq:posteriorconverges}).
For the second statement of (\ref{eq:posteriorconverges}), we note from
(\ref{eq:Gibbstimederiv}) that
\[\frac{\d}{\d t}\Big(V(q_t,\alpha^t)+R(\alpha^t)\Big) \leq -\frac{1}{d}\FI_t
+\Delta_t.\]
Then, by the same arguments as above, for some constant $C>0$ and every $T>0$,
\[\limsup_{n,d \to \infty} \int_0^T d^{-1}\FI_t
\leq \limsup_{n,d \to \infty}
V(q_0,\alpha^0)+R(\alpha^0)-V(q_T,\alpha^T)-R(\alpha^T) \leq C.\]
Recalling (\ref{eq:FIW2qbar}), this implies
\begin{equation}\label{eq:integratedW2tmp}
\limsup_{n,d \to \infty} \int_0^T W_2(\bar \sP_t,\bar \sP_{\alpha^t})^2\d t
\leq C.
\end{equation}
For each fixed $t \geq 0$, we have
\begin{equation}\label{eq:barPapproximatesDMFT}
\lim_{n,d \to \infty} W_2(\bar \sP_t,\sP(\theta^*,\theta^t))=0
\end{equation}
by (\ref{eq:barqconvergence}). We have also by Jensen's inequality
and (\ref{eq:fixedalpha_equilibriumlaw}) of Corollary
\ref{cor:fixedalpha_dynamics}(a),
\begin{equation}\label{eq:barPconvergence}
\limsup_{n,d \to \infty} W_2(\bar \sP_{\alpha^t},\sP_{\alpha^t})^2
\leq \limsup_{n,d \to \infty} \E_{\btheta \sim q_{\alpha^t}}\big[
W_2(\bar \sP_{\btheta},\sP_{\alpha^t})^2\big]=0.
\end{equation}
Thus, for each $t \geq 0$,
$\lim_{n,d \to \infty} W_2(\bar \sP_t,\bar \sP_{\alpha^t})
=W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})$.
Then by Fatou's lemma and (\ref{eq:integratedW2tmp}),
$\int_0^T W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})^2 \d t
\leq C$. Since $T>0$ is arbitrary, taking $T \to \infty$ gives
\begin{equation}\label{eq:integratedW2bound}
\int_0^\infty W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})^2 \d t \leq C.
\end{equation}

For any $s \leq t$, considering the coordinatewise coupling gives
$W_2(\bar \sP_s,\bar \sP_t)^2
\leq d^{-1}\E[\|\tilde \btheta^s-\tilde \btheta^t\|_2^2 \mid
\X,\btheta^*,\beps] \leq C(t-s)$, the last inequality holding by \cite[Theorem
II.2.1]{kunita1984stochastic}. Also
\begin{equation}\label{eq:W2barPlipschitz}
W_2(\bar \sP_{\alpha^s},\bar \sP_{\alpha^t})^2
\leq d^{-1}W_2(q_{\alpha^s},q_{\alpha^t})^2 \leq C\|\alpha^t-\alpha^s\|_2
\leq C'|t-s|
\end{equation}
by the local $W_2$-Lipschitz continuity of $q_\alpha$
in $\alpha$ shown in (\ref{eq:W2locallylipschitz}) and 
the bound (\ref{eq:dtalphabound}) for $\d\alpha^t/\d t$. Then by
(\ref{eq:barPapproximatesDMFT}) and (\ref{eq:barPconvergence}), taking the limit
$n,d \to \infty$, this implies also that
\[|W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})^2
-W_2(\sP(\theta^*,\theta^s),\sP_{\alpha^s})^2| \leq C(t-s)\]
for all $s \leq t$, i.e.\ $t \mapsto
W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})^2$ is globally Lipschitz.
Thus (\ref{eq:integratedW2bound}) implies
\begin{equation}\label{eq:W2Pthetatalphat}
\lim_{t \to \infty}
W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^t})^2=0.\end{equation}
We have similarly to (\ref{eq:W2barPlipschitz}) that
$W_2(\bar \sP_{\alpha^t},\bar \sP_{\alpha^\infty})^2
\leq d^{-1}W_2(q_{\alpha^t},q_{\alpha^\infty})^2
\leq C\|\alpha^t-\alpha^\infty\|_2$. Hence by (\ref{eq:barPconvergence}), also
$W_2(\sP_{\alpha^t},\sP_{\alpha^\infty})^2 \leq C\|\alpha^t-\alpha^\infty\|_2$,
so
\begin{equation}\label{eq:W2alphatalphainfty}
\lim_{t \to \infty} W_2(\sP_{\alpha^t},\sP_{\alpha^\infty})^2=0.
\end{equation}
Combining (\ref{eq:W2Pthetatalphat}) and (\ref{eq:W2alphatalphainfty}),
for any $\eps>0$ there exists $T(\eps)>0$ such that
$W_2(\sP(\theta^*,\theta^t),\sP_{\alpha^\infty})<\eps$ for all $t \geq T(\eps)$.
The second statement of (\ref{eq:posteriorconverges}) follows from this and
$\lim_{n,d \to \infty} W_2(\frac{1}{d}\sum_j
\delta_{(\theta_j^*,\theta_j^t)},\sP(\theta^*,\theta^t))=0$ as ensured
by Theorem \ref{thm:dmft_approx}.
\end{proof}

\subsection{Analysis of examples}\label{sec:exampledetails}

\begin{proof}[Analysis of Examples \ref{ex:gaussianmean} and
\ref{ex:logconcave}]

We prove the claims in Example \ref{ex:logconcave} that Assumptions
\ref{assump:prior}, \ref{assump:gradient}, \ref{assump:compactalpha} hold,
and that $\Crit$ consists of the unique point $\alpha=\alpha^*$. (Then these
claims hold also in Example \ref{ex:gaussianmean} for the Gaussian prior,
which is a special case.)

Assumptions \ref{assump:prior} and \ref{assump:gradient} are immediate from the
given conditions for $f(x)$. For Assumption \ref{assump:compactalpha}, let us
first show that there exists a compact interval $S \subset \R$ for which
$\{\alpha^t\}_{t \geq 0}$ is confined to $S$ (for all $t \geq 0$):
By Lemma \ref{lemma:Vdecreasing}, for each fixed $t \geq 0$, almost surely
\begin{equation}\label{eq:Vdiffbound}
\limsup_{n,d \to \infty} V(q_t,\alpha^t)-V(q_0,\alpha^0) \leq 0.
\end{equation}
By the Gibbs variational principle (\ref{eq:gibbsvariational})
and the lower bound ${-}\log g(\theta,\alpha)=f(\theta-\alpha)
\geq f(0)+\frac{c_0}{2}(\theta-\alpha)^2$,
\begin{align*}
V(q_t,\alpha^t) &\geq \widehat F(\alpha^t)\\
&={-}\frac{1}{d}\log \int 
(2\pi\sigma^2)^{-n/2}
\exp\Big({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+\sum_{j=1}^d \log g(\theta_j,\alpha^t)\Big)\d\btheta\\
&\geq {-}\frac{1}{d}\log \int (2\pi\sigma^2)^{-n/2}
\exp\Big({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
-f(0)d-\sum_{j=1}^d \frac{c_0}{2}(\theta_j-\alpha^t)^2\Big)\d\btheta
\end{align*}
Applying $\|\X\|_\op \leq C$ a.s.\ for all large $n,d$,
it is readily checked by explicit evaluation of this integral over
$\btheta$ that
\[V(q_t,\alpha^t) \geq C+\frac{c_0}{2}(\alpha^t)^2
-\frac{1}{2d}\Big(\frac{\X^\top \y}{\sigma^2}+c_0\alpha^t\1\Big)^\top
\Big(\frac{\X^\top\X}{\sigma^2}+c_0\I\Big)^{-1}
\Big(\frac{\X^\top \y}{\sigma^2}+c_0\alpha^t\1\Big)\]
a.s.\ for all large $n,d$ and a constant $C \in \R$ depending on
$\sigma^2,\delta,f(0),c_0,\alpha^*$,
where here $\1$ denotes the all-1's vector in $\R^d$. We have
\[\lim_{n,d \to \infty}
\frac{1}{d}\,\1^\top\Big(\frac{\X^\top \X}{\sigma^2}+c_0\I\Big)^{-1}\1
=\sigma^2 G({-}\sigma^2 c_0)>\frac{1}{c_0}\]
strictly, where $G(z)=\lim d^{-1}\Tr (\X^\top \X-z\I)^{-1}$ denotes
the Stieltjes transform of the Marcenko-Pastur spectral limit of $\X^\top \X$.
Applying this to lower-bound the quadratic term in $\alpha^t$ above,
and applying Cauchy-Schwarz to lower-bound the linear term, we get
\[V(q_t,\alpha^t) \geq C'+c'(\alpha^t)^2\]
for some constants $C' \in \R$ and $c'>0$.
Now applying this and $V(q_0,\alpha^0)=V(g_0^{\otimes d},\alpha^0) \leq C$
to (\ref{eq:Vdiffbound}), we deduce that $(\alpha^t)^2$ is uniformly
bounded over all $t \geq 0$, i.e.\ there exists a compact interval $S$ 
for which $\alpha^t \in S$ for all $t \geq 0$, as claimed. By enlarging $S$, we
may assume without loss of generality $\alpha^* \in S$.
Then, taking $O$ to be any neighborhood of $S$, the
remaining LSI condition of Assumption \ref{assump:compactalpha} holds by
the strong convexity of $f(x)$ and Proposition \ref{prop:LSI}.

We now show that $F(\alpha)$ is strictly convex on $O$, by
showing convexity of the original negative log-likelihood $\widehat F(\alpha)$:
Fixing sufficiently large and small constants $C_0,c>0$,
let us restrict to the event
\[\event=\{\|\X\|_\op \leq C_0,\; \|\X\1\|_2 \geq c\sqrt{d}\}\]
which holds a.s.\ for all large $n,d$.
Recalling the form of $\nabla^2 \widehat F(\alpha)$ from (\ref{eq:hessF})
and applying this with ${-}\log g(\theta,\alpha)=f(\theta-\alpha)$,
\[\widehat F''(\alpha)=
\frac{1}{d}\bigg\langle\sum_{j=1}^d f''(\theta_j-\alpha) \bigg \rangle_\alpha
-\frac{1}{d}\Var_\alpha\bigg[\sum_{j=1}^d f'(\theta_j-\alpha)\bigg]\]
where $\langle \cdot \rangle_\alpha$ is the average under the posterior law
corresponding to $g(\cdot,\alpha)$, and $\Var_\alpha$ is its posterior
variance. Since $f(x)$ is strictly convex, the posterior density of $\theta$ is
strictly log-concave for each fixed $\alpha$. Then, denoting
\[\v_\alpha(\btheta)=\Big(f''(\theta_j-\alpha)\Big)_{j=1}^d \in \R^d,
\qquad \D_\alpha(\btheta)=\diag\Big(f''(\theta_j-\alpha)\Big)_{j=1}^d \in \R^{d
\times d},\]
the Brascamp-Lieb inequality \cite[Theorem 4.9.1]{bakry2014analysis} implies
\[\Var_\alpha\bigg[\sum_{j=1}^d f'(\theta_j-\alpha)\bigg]
\leq \bigg\langle \v_\alpha(\btheta)^\top \bigg(\D_\alpha(\btheta)
+\frac{\X^\top\X}{\sigma^2}\bigg)^{-1}\v_\alpha(\btheta)\bigg\rangle_\alpha\]
Observing also that $\sum_{j=1}^d f''(\theta_j-\alpha)
=\v_\alpha(\btheta)^\top\D_\alpha(\btheta)^{-1}\v_\alpha(\btheta)$,
this shows
\[\widehat F''(\alpha)
\geq \frac{1}{d}\,\bigg\langle \v_\alpha(\btheta)^\top 
\bigg[\D_\alpha(\btheta)^{-1}
-\bigg(\D_\alpha(\btheta)+\frac{\X^\top\X}{\sigma^2}\bigg)^{-1}\bigg]
\v_\alpha(\btheta)\bigg\rangle_\alpha.\]
Applying the Woodbury matrix identity
and $0 \preceq \sigma^2\I+\X\D_\alpha(\btheta)^{-1}\X^\top \preceq C'\,\I$
on the event $\event$ for some constant $C'>0$,
\begin{align*}
\widehat F''(\alpha)
&\geq \frac{1}{d}\,\bigg\langle \v_\alpha(\btheta)^\top 
\bigg[\D_\alpha(\btheta)^{-1}\X^\top
\bigg(\sigma^2\,\I+\X\D_\alpha(\btheta)^{-1}\X^\top\bigg)^{-1}
\X\D_\alpha(\btheta)^{-1}\bigg]\v_\alpha(\btheta)\bigg\rangle_\alpha\\
&\geq \frac{1}{C'd} \bigg\langle \v_\alpha(\btheta)^\top 
\D_\alpha(\btheta)^{-1}\X^\top \X\D_\alpha(\btheta)^{-1}\v_\alpha(\btheta)
\bigg\rangle_\alpha
=\frac{1}{C'd}\1^\top\X^\top\X\1 \geq c',
\end{align*}
the last inequality holding for some $c'>0$ on $\event$. Thus, on $\event$,
$\widehat F(\alpha)-(c'/2)\alpha^2$ is convex over $\alpha \in \R$.
Since $\event$ holds a.s.\ for all large $n,d$ and $F(\alpha)$ is the
almost-sure pointwise limit of $\widehat F(\alpha)$, this implies that
$F(\alpha)-(c'/2)\alpha^2$ is also convex \cite[Theorem
10.8]{rockafellar1997convex}, so $F(\alpha)$ is strongly convex as claimed.
Lemma \ref{lemma:gradalphaF}(c) implies that $\nabla F(\alpha^*)=0$, i.e.\
$\alpha^*$ is a point of $\Crit$, so by this convexity it is the unique point of
$\Crit$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:alphaconfined}]
By Lemma \ref{lemma:Vdecreasing}, for each fixed $t \geq 0$, almost surely
\begin{equation}\label{eq:VRdiffbound}
\limsup_{n,d \to \infty} \Big(V(q_t,\alpha^t)+R(\alpha^t)\Big)
-\Big(V(q_0,\alpha^0)+R(\alpha^0)\Big) \leq 0.
\end{equation}
By definition of $V(q,\alpha)$ in (\ref{eq:gibbsenergy}), we have
\begin{align*}
V(q_0,\alpha^0)=V(g_0^{\otimes d},\alpha^0)
&=\frac{1}{d}\int \frac{1}{2\sigma^2}\|\y-\X\btheta\|^2
\prod_{j=1}^d g_0(\theta_j)\d\theta_j
+\DKL(g_0\|g(\cdot,\alpha^0))+\frac{n}{2d}\log 2\pi\sigma^2,\\
V(q_t,\alpha^t)&=\frac{1}{d}\int \frac{1}{2\sigma^2}\|\y-\X\btheta\|^2
q_t(\btheta)\d\btheta
+\frac{1}{d}\DKL(q_t\|g(\cdot,\alpha^t)^{\otimes d})
+\frac{n}{2d}\log 2\pi\sigma^2.
\end{align*}
Let $\Pi_\X \in \R^{n \times n}$ be the projection orthogonal to the
column span of $\X$. Then, applying the above forms with
$\DKL(q_t\|g(\cdot,\alpha^t)^{\otimes d})
\geq 0$ and noting that
$\|(\I-\Pi_\X)(\y-\X\btheta)\|^2=\|(\I-\Pi_\X)\y\|^2$ which
does not depend on $\btheta$, we have
\begin{align*}
&V(q_0,\alpha^0)-V(q_t,\alpha^t)\\
&\leq \frac{1}{d}\int \frac{1}{2\sigma^2}\|\y-\X\btheta\|^2
\prod_{j=1}^d g_0(\theta_j)\d\theta_j
-\frac{1}{d}\int \frac{1}{2\sigma^2}\|\y-\X\btheta\|^2
q_t(\btheta)\d\btheta+\DKL(g_0\|g(\cdot,\alpha^0))\\
&=\frac{1}{d}\int \frac{1}{2\sigma^2}\|\Pi_\X(\y-\X\btheta)\|^2
\prod_{j=1}^d g_0(\theta_j)\d\theta_j
-\frac{1}{d}\int \frac{1}{2\sigma^2}\|\Pi_\X(\y-\X\btheta)\|^2
q_t(\btheta)\d\btheta+\DKL(g_0\|g(\cdot,\alpha^0))\\
&\leq \frac{1}{d}\int \frac{1}{2\sigma^2}\|\Pi_\X(\y-\X\btheta)\|^2
\prod_{j=1}^d g_0(\theta_j)\d\theta_j+\DKL(g_0\|g(\cdot,\alpha^0)).
\end{align*}
Let us apply
\[\|\Pi_\X(\y-\X\btheta)\|^2 \leq 2\|\Pi_\X\beps\|^2+
2\|\X(\btheta^*-\btheta)\|_2^2,\]
$\|\X\|_\op^2 \leq C(1+\delta)$, and $\|\Pi_\X \beps\|^2 \leq
C\min(n,d)\sigma^2$ for a universal constant $C>0$ a.s.\ for all large $n,d$.
Then, for a constant $C(g_*,g_0,\alpha^0)>0$ depending only on
$g_*,g_0,\alpha^0$,
\[\limsup_{n,d \to \infty}
V(q_0,\alpha^0)-V(q_t,\alpha^t)
\leq C(g_*,g_0,\alpha^0)\Big(\frac{1+\delta}{\sigma^2}+1\Big).\]
Applying this to (\ref{eq:VRdiffbound}) and noting that $R(\alpha^0)=0$ because
$\|\alpha^0\| \leq D$, for every $t \geq 0$ we get
\[R(\alpha^t) \leq C(g_*,g_0,\alpha^0)\Big(\frac{1+\delta}{\sigma^2}+1\Big).\]
The lemma follows from this bound and the condition
$R(\alpha) \geq \|\alpha\|-D$ whenever $\|\alpha\| \geq D+1$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:largedelta}]
Fixing any $s^2=\sigma^2/\delta>0$,
Proposition \ref{prop:alphaconfined} implies that
there exists a constant radius $D'>0$ (depending on $s^2$ but not on $\delta$)
such that for any $\delta>1$,
\[\alpha^t \in \ball(D') \text{ for all } t \geq 0.\]
Set $S=\overline{\ball(D')}$ and
$O=\ball(D'+1)$. Then for each fixed $\alpha \in O$,
Assumption \ref{assump:prior} implies
\begin{equation}\label{eq:loggunifbounds}
C_0 \geq
{-}\partial_\theta^2 \log g(\theta,\alpha) \geq \begin{cases} c_0 & \text{ for
} |\theta| \geq R\\
c_1 & \text{ for all } \theta \in \R \end{cases}
\end{equation}
for some $C_0,R,c_0>0$ and $c_1 \in \R$ depending on $\alpha$. Then, by
Lipschitz continuity
of $(\theta,\alpha) \mapsto \partial_\theta^2 \log g(\theta,\alpha)$ 
over $\alpha \in \overline{O}$ and
compactness of $\overline{O}$, these bounds (\ref{eq:loggunifbounds})
must also hold for some
uniform constants $C_0,R,c_0>0$ and $c_1 \in \R$ (depending on $s^2$ but
not $\delta$) and all $\alpha \in O$.
By this bound (\ref{eq:loggunifbounds}) and Proposition \ref{prop:LSI}(b),
for some sufficiently large $\delta_0=\delta_0(s^2)>0$, $\sigma^2=\delta s^2$,
and all $\delta \geq \delta_0$,
the LSI (\ref{eq:LSI}) must hold for $g=g(\cdot,\alpha)$ and each
$\alpha \in O$. This verifies Assumption \ref{assump:compactalpha}.

Throughout the remainder of the proof, let $C,C',c,c'>0$
denote constants that may depend on $\alpha^*$, $D$, $D'$, and
$s^2$ but not on $\delta$, and that may change from instance to
instance. We compare the optimization landscape of $F(\alpha)$ with that
of $G_{s^2}(\alpha)$ over $O$. Let
$\mse(\alpha)$, $\mse_*(\alpha)$, $\omega(\alpha)$, $\omega_*(\alpha)$ be as
defined by (\ref{eq:mmse}) and (\ref{eq:static_fixedpoint}) for the prior
$g=g(\cdot,\alpha)$. We first bound
$\mse(\alpha)$, $\mse_*(\alpha)$, $\omega(\alpha)$, $\omega_*(\alpha)$:
Write as shorthand $\langle \cdot \rangle=
\langle \cdot \rangle_{g(\cdot,\alpha),\omega(\alpha)}$ for the posterior
expectation in the scalar channel model (\ref{eq:scalarchannel}). We have
\[\langle (Y-\theta) \rangle^2
=\frac{1}{Z}\int (Y-\theta)^2 e^{-\frac{\omega(\alpha)}{2}(Y-\theta)^2}
g(\theta,\alpha) \d\theta,
\qquad Z=\int e^{-\frac{\omega(\alpha)}{2}(Y-\theta)^2}g(\theta,\alpha)\d\theta.\]
We separate the integrals over the sets
$\{\theta:e^{-\frac{\omega(\alpha)}{2}(Y-\theta)^2} \leq Z\}$
and $\{\theta:e^{-\frac{\omega(\alpha)}{2}(Y-\theta)^2}>Z\}$, and on the latter 
set apply the upper bound $(Y-\theta)^2<\max(0,{-}\frac{2}{\omega(\alpha)}\log Z)$.
This gives
\[\langle (Y-\theta) \rangle^2
\leq \int (Y-\theta)^2 \1\{e^{-\frac{\omega(\alpha)}{2}(Y-\theta)^2} \leq Z\}
g(\theta,\alpha)\d\theta+\max(0,{-}\tfrac{2}{\omega(\alpha)}\log Z)
\leq 2\int (Y-\theta)^2 g(\theta,\alpha)\d\theta,\]
the last inequality applying Jensen's inequality to bound $\log Z \geq
\int -\frac{\omega(\alpha)}{2}(Y-\theta)^2 g(\theta,\alpha)\d\theta$.
It is clear from the lower bounds of (\ref{eq:loggunifbounds}) and the
boundedness of $\log g(0,\alpha)$ and $\partial_\theta \log g(0,\alpha)$ over
$\alpha \in \overline{O}$ that $\int \theta^2 g(\theta,\alpha)\d\theta<C$ for
some constant $C>0$, for all $\alpha \in O$. Thus this inequality shows
\[\langle (Y-\theta) \rangle^2 \leq C(1+Y^2),\]
which implies also
\[\langle (\langle \theta \rangle-\theta) \rangle^2
\leq \langle (Y-\theta) \rangle^2 \leq C(1+Y^2),
\quad \langle \theta \rangle^2
\leq 2Y^2+2(Y-\langle \theta \rangle)^2
\leq 2Y^2+2\langle (Y-\theta)^2 \rangle
\leq C'(1+Y^2).\]
Taking expectations over $Y=\theta^*+z$ with $\theta^* \sim g_*$ and $z \sim
\N(0,\omega_*(\alpha)^{-1})$, we get $\mse(\alpha),\mse_*(\alpha)
\leq C(1+\omega_*(\alpha)^{-1})$. Then applying 
$\omega_*(\alpha)^{-1}=(\sigma^2+\mse_*(\alpha))/\delta
\leq s^2+C(1+\omega_*(\alpha)^{-1})/\delta$,
for all $\delta>\delta_0$ sufficiently large,
this implies $\omega_*(\alpha)^{-1} \leq C'$. This in turn shows
\begin{equation}\label{eq:msebounds}
\mse(\alpha),\mse_*(\alpha) \leq C.
\end{equation}
Let $o_\delta(1)$ denote a quantity that converges to 0 uniformly over
$\alpha \in O$ as $\delta \to \infty$ (fixing $s^2=\sigma^2/\delta$).
Then, applying (\ref{eq:msebounds}) to the fixed point equations
$\omega(\alpha)=\delta/(\sigma^2+\mse(\alpha))$ and
$\omega_*(\alpha)=\delta/(\sigma^2+\mse_*(\alpha))$,
\begin{equation}\label{eq:omegabounds}
\omega(\alpha)^{-1}=s^2+o_\delta(1),\qquad \omega_*(\alpha)^{-1}
=s^2+o_\delta(1).
\end{equation}

We recall from Lemma \ref{lemma:mmse_lipschitz} that
$\omega(\alpha),\omega_*(\alpha)$ must be
continuous functions of $\alpha \in O$. We now argue via the implicit function
theorem that for all $\delta>\delta_0$ sufficiently large, these are in
fact continuously-differentiable over $\alpha \in O$. For this,
fix any $\alpha \in O$ and consider the map
\begin{equation}\label{eq:fixedpointmap}
f_\alpha(\omega,\omega_*)=
\begin{pmatrix}
\omega^{-1}-\delta^{-1}(\sigma^2+\E_{g_*,\omega_*}[\langle (\theta-\langle
\theta \rangle_{g(\cdot,\alpha),\omega})^2\rangle_{g(\cdot,\alpha),\omega}]) \\
\omega_*^{-1}-\delta^{-1}(\sigma^2+\E_{g_*,\omega_*}[(\theta^*-
\langle \theta \rangle_{g(\cdot,\alpha),\omega})^2]\end{pmatrix}.
\end{equation}
Thus (\ref{eq:mmse}) and (\ref{eq:static_fixedpoint}) imply that
$0=f_\alpha(\omega(\alpha),\omega_*(\alpha))$. Let us momentarily write as
shorthand $\E=\E_{g_*,\omega_*}$ and $\langle \cdot \rangle=\langle \cdot
\rangle_{g(\cdot,\alpha),\omega}$. Expressing
$Y=\theta^*+\omega_*^{-1/2}z$,
$\E$ may be understood as the expectation over $\theta^* \sim g_*$ and $z \sim
\N(0,1)$. The expected posterior average $\E \langle \cdot \rangle$
is given explicitly by
\[\E \langle f(\theta) \rangle
=\E \frac{\int f(\theta) e^{H_\alpha(\theta,\omega,\omega_*)}\d\theta}
{\int e^{H_\alpha(\theta,\omega,\omega_*)}\d\theta},
\qquad H_\alpha(\theta,\omega,\omega_*)
=\omega(\theta^*+\omega_*^{-1/2}z)\theta-\frac{\omega}{2}\theta^2
+\log g(\theta,\alpha),\]
and the derivatives in
$(\omega,\omega_*)$ may be computed via differentiation of $H_\alpha$.
Let us denote by $\kappa_j(\cdot)$ the $j^\text{th}$ mixed cumulant associated
to the posterior mean $\langle \cdot \rangle=\langle \cdot
\rangle_{g(\cdot,\alpha),\omega}$, i.e.\
\[\kappa_1(f(\theta))=\langle f(\theta) \rangle,
\qquad \kappa_2(f(\theta),g(\theta))=\langle f(\theta)g(\theta) \rangle
-\langle f(\theta) \rangle\langle g(\theta) \rangle,\]
etc. Then 
$\E[\langle (\theta-\langle \theta \rangle)^2\rangle]
=\E[\kappa_2(\theta,\theta)]$ and
$\E[(\theta^*-\langle \theta \rangle)^2]
=\E[(\theta^*-\kappa_1(\theta))^2]$, and differentiating in
$(\omega,\omega_*)$ gives
\begin{align*}
\partial_\omega \E[\langle (\theta-\langle
\theta \rangle)^2\rangle]
&=\E[\kappa_3(\theta,\theta,\partial_\omega
H_\alpha(\theta,\omega,\omega_*))],\\
\partial_{\omega_*} \E[\langle (\theta-\langle
\theta \rangle)^2\rangle]
&=\E[\kappa_3(\theta,\theta,\partial_{\omega_*}
H_\alpha(\theta,\omega,\omega_*))],\\
\partial_\omega \E[(\theta^*-\langle \theta \rangle)^2]
&=\E[{-2}(\theta^*-\kappa_1(\theta))\kappa_2(\theta,
\partial_\omega H_\alpha(\theta,\omega,\omega_*))]\\
\partial_{\omega_*} \E[(\theta^*-\langle \theta \rangle)^2]
&=\E[{-2}(\theta^*-\kappa_1(\theta))\kappa_2(\theta,
\partial_{\omega_*} H_\alpha(\theta,\omega,\omega_*))]
\end{align*}
We note that each absolute moment $\E_{g_*,\omega_*(\alpha)}[\langle |\theta|^k
\rangle_{g(\cdot,\alpha),\omega(\alpha)}]$ is bounded by a constant over
$\alpha \in O$, by continuity of this quantity in $\alpha$ and compactness of
$\overline{O}$. Then it is direct to check that each of the above four
derivatives evaluated at $(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))$
is also bounded by a constant over $\alpha \in O$. This implies that
the derivative of the map $f_\alpha(\omega,\omega_*)$ in
(\ref{eq:fixedpointmap}) satisfies
\begin{equation}\label{eq:domegaf}
\d_{\omega,\omega_*}
f_\alpha(\omega,\omega_*)\Big|_{(\omega,\omega_*)=(\omega(\alpha),\omega(\alpha_*))}
=\begin{pmatrix} {-}\omega^{-2}+o_\delta(1) &
o_\delta(1) \\ o_\delta(1) & -\omega_*^{-2}+o_\delta(1) \end{pmatrix}
\bigg|_{(\omega,\omega_*)=(\omega(\alpha),\omega(\alpha_*))}
=-s^2\,\I+o_\delta(1).
\end{equation}
In particular, for $\delta>\delta_0$ sufficiently large, this derivative is
invertible. Since $f_\alpha(\omega,\omega_*)$ is continuously-differentiable
in $(\omega,\omega_*,\alpha)$ (where differentiability
in $\alpha$ is ensured by Assumption \ref{assump:prior} for
$\log g(\theta,\alpha)$), the implicit function theorem implies that for
each $\alpha_0 \in O$, there exists a unique continuously-differentiable
extension of the root $(\omega(\alpha_0),\omega_*(\alpha_0))$ of
$0=f_{\alpha_0}(\omega(\alpha_0),\omega_*(\alpha_0))$ to a solution of
$0=f_\alpha(\omega,\omega_*)$ in an open neighborhood of $\alpha_0$.
This extension must then coincide with $\omega(\alpha),\omega_*(\alpha)$,
because Lemma \ref{lemma:mmse_lipschitz} ensures that
$\omega(\alpha),\omega_*(\alpha)$ are continuous in $\alpha$.
Thus $\omega(\alpha),\omega_*(\alpha)$ are continuously-differentiable
in $\alpha \in O$, as claimed. The
implicit function theorem shows also that their first derivatives are given by
\[\begin{pmatrix} \nabla_\alpha \omega^\top \\ \nabla_\alpha \omega_*^\top
\end{pmatrix}=[\d_{\omega,\omega_*} f_\alpha]^{-1} \d_\alpha f_\alpha.\]
We may check as above that the $\alpha$-derivatives
\begin{align*}
\partial_{\alpha_j} \E[\langle (\theta-\langle
\theta \rangle)^2\rangle]
&=\E[\kappa_3(\theta,\theta,\partial_{\alpha_j}
H_\alpha(\theta,\omega,\omega_*))],\\
\partial_{\alpha_j} \E[(\theta^*-\langle \theta \rangle)^2]
&=\E[{-2}(\theta^*-\kappa_1(\theta))\kappa_2(\theta,
\partial_{\alpha_j} H_\alpha(\theta,\omega,\omega_*))]
\end{align*}
evaluated at $(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))$
are also both bounded by a constant over $\alpha \in \overline{O}$. By the
definition of $f_\alpha$, this implies
$\d_\alpha f_\alpha|_{(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))}
=o_\delta(1)$, so together with (\ref{eq:domegaf}), this shows also
\begin{equation}\label{eq:gradomegabounds}
\nabla_\alpha \omega(\alpha)=o_\delta(1),
\quad \nabla_\alpha \omega_*(\alpha)=o_\delta(1).
\end{equation}

Recall from Lemma \ref{lemma:gradalphaF} that
\[\nabla F(\alpha)={-}\E_{\theta \sim \sP_\alpha}
\nabla_\alpha \log g(\theta,\alpha)
=-\E_{g_*,\omega_*(\alpha)}\langle \nabla_\alpha \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega(\alpha)}.\]
Applying continuity of $(\omega,\omega_*) \mapsto
\E_{g_*,\omega_*}\langle \nabla_\alpha \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega}$ and the approximations
$\omega(\alpha)^{-1},\omega_*(\alpha)^{-1}=s^2+o_\delta(1)$ shown above,
we have
\begin{equation}\label{eq:gradFcompare}
\nabla F(\alpha)={-}\E_{g_*,s^{-2}}\langle \nabla_\alpha \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),s^{-2}}+o_\delta(1)
=\nabla G_{s^2}(\alpha),
\end{equation}
where $G_{s^2}(\alpha)={-}\E_{g_*,s^{-2}}[\log \sP_{g(\cdot,\alpha),s^{-2}}(Y)]$
is the negative population log-likelihood (\ref{eq:Galpha}) in the scalar
channel model with fixed noise variance $s^2$. 
[Note that fixing an arbitrary point $\alpha_0 \in O$ and integrating this
gradient approximation over $\alpha \in O$, this also implies
\[F(\alpha)=G(\alpha)+(F(\alpha_0)-G(\alpha_0))+o_\delta(1),\]
i.e.\ $F$ approximately coincides with $G$ up to an additive shift.]
Furthermore, the above
differentiability of $\omega(\alpha),\omega_*(\alpha)$ implies $F(\alpha)$ is
twice continuously-differentiable over $\alpha \in O$, and differentiating
$\nabla F(\alpha)$ by the chain rule gives
\begin{align}
\partial_{\alpha_i}\partial_{\alpha_j}
F(\alpha)&=-\partial_\omega\Big(\E_{g_*,\omega_*(\alpha)}\langle
\partial_{\alpha_i} \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega(\alpha)}\Big)
\cdot \partial_{\alpha_j} \omega(\alpha)\notag\\
&\hspace{1in}-\partial_{\omega_*} \Big(\E_{g_*,\omega_*(\alpha)}\langle
\partial_{\alpha_i} \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega(\alpha)}\Big)
\cdot \partial_{\alpha_j} \omega_*(\alpha)\notag\\
&\hspace{1in}-\partial_{\alpha_j} \Big(\E_{g_*,\omega_*(\alpha)}\langle
\partial_{\alpha_i} \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega(\alpha)}\Big).\label{eq:HessFform}
\end{align}
Writing again $\E=\E_{g_*,\omega_*}$, 
$\langle \cdot \rangle=\langle \cdot \rangle_{g(\cdot,\alpha),\omega}$,
and $\kappa_j$ for the cumulants with respect to $\langle \cdot \rangle$,
we have
\begin{align*}
\partial_\omega \E \langle \partial_{\alpha_i} \log g(\theta,\alpha) \rangle
&=\E[\kappa_2(\partial_{\alpha_i} \log g(\theta,\alpha),
\partial_\omega H_\alpha(\theta,\omega,\omega_*))]\\
\partial_{\omega_*}
\E \langle \partial_{\alpha_i} \log g(\theta,\alpha) \rangle
&=\E[\kappa_2(\partial_{\alpha_i} \log g(\theta,\alpha),
\partial_{\omega_*} H_\alpha(\theta,\omega,\omega_*))],
\end{align*}
and these are bounded at $(\omega,\omega_*)=(\omega(\alpha),\omega_*(\alpha))$
over all $\alpha \in O$. Furthermore
\[\partial_{\alpha_j} \E \langle
\partial_{\alpha_i} \log g(\theta,\alpha) \rangle
=\E \langle
\partial_{\alpha_i} \partial_{\alpha_j} \log g(\theta,\alpha)
\rangle+\E[\kappa_2(\partial_{\alpha_i} \log g(\theta,\alpha),
\partial_{\alpha_j} \log g(\theta,\alpha))].\]
Applying these and the bounds (\ref{eq:gradomegabounds}) to
(\ref{eq:HessFform}),
\begin{align*}
&\partial_{\alpha_i}\partial_{\alpha_j} F(\alpha)\\
&=-\E_{g_*,\omega_*(\alpha)} \langle
\partial_{\alpha_i} \partial_{\alpha_j} \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),\omega(\alpha)}
-\E_{g_*,\omega_*(\alpha)} \Cov_{\langle g(\cdot,\alpha),\omega(\alpha) \rangle}
(\partial_{\alpha_i} \log g(\theta,\alpha),
\partial_{\alpha_j} \log g(\theta,\alpha))+o_\delta(1)\\
&=\underbrace{-\E_{g_*,s^{-2}} \langle
\partial_{\alpha_i} \partial_{\alpha_j} \log g(\theta,\alpha)
\rangle_{g(\cdot,\alpha),s^{-2}}
-\E_{g_*,s^{-2}} \Cov_{\langle g(\cdot,\alpha),s^{-2} \rangle}
(\partial_{\alpha_i} \log g(\theta,\alpha),
\partial_{\alpha_j} \log g(\theta,\alpha))}_{=\partial_{\alpha_i}
\partial_{\alpha_j} G_{s^2}(\alpha)}+o_\delta(1)\\
\end{align*}
Thus we have shown
\begin{equation}\label{eq:hessFapprox}
\nabla^2 F(\alpha)=\nabla^2 G_{s^2}(\alpha)+o_\delta(1)
\end{equation}
where again $o_\delta(1)$ converges to 0 uniformly over $\alpha \in O$ as
$\delta \to \infty$.

The approximation (\ref{eq:gradFcompare}) implies that
$\nabla F+\nabla R$ converges uniformly to
$\nabla G_{s^2}+\nabla R$ over $\alpha \in O$,
as $\delta \to \infty$. Then for all $\delta>\delta_0$ sufficiently large and
for some
function $\iota:[\delta_0,\infty) \to (0,\infty)$ satisfying
$\iota(\delta) \to 0$ as $\delta \to \infty$, each
point of $\Crit \cap \,\ball(D)=\{\alpha \in \ball(D):\nabla F(\alpha)=0\}$
must fall within a ball of radius $\iota(\delta)$ around a point of
$\Crit_G=\{\alpha \in \ball(D):\nabla G_{s^2}(\alpha)=0\}$.
The approximation (\ref{eq:gradFcompare}) further
implies that for each such ball around a point $\alpha_0 \in \Crit_G$,
$\nabla^2 F$ converges uniformly to
$\nabla^2 G_{s^2}$ on this ball, as $\delta \to \infty$. If
$\nabla^2 G_{s^2}(\alpha_0)$ is non-singular, then for all $\delta>\delta_0$
sufficiently large, an argument via the topological degree shows that
there must be exactly one point of $\Crit$ in this ball (having the same index
as $\alpha_0$ as a critical point of $G_{s^2}$) --- see e.g.\ \cite[Lemma
5]{mei2018landscape}. This shows statements (1) and (2) of the proposition.

As a direct consequence of these statements, if
$\alpha^*$ is the unique point of $\Crit_G$ and $\nabla^2 G_{s^2}(\alpha^*)$
is non-singular, then there is a unique point of $\Crit \cap \,\ball(D)$.
If furthermore $g_*(\theta)=g(\theta,\alpha^*)$, then this point of
$\Crit \cap \,\ball(D)$ must be $\alpha^*$ itself, since
$\nabla F(\alpha^*)=0$ by Lemma \ref{lemma:gradalphaF}(c).
\end{proof}

\begin{proof}[Analysis of Example \ref{ex:gaussianmeanmixture}]
We verify Assumptions \ref{assump:prior} and \ref{assump:gradient}
for Example \ref{ex:gaussianmeanmixture} of the
Gaussian mixture model with varying means. Let $\iota \in \{1,\ldots,K\}$
denote the mixture component of $\theta$, and let
$\langle f(\iota,\theta) \rangle=\E[f(\iota,\theta) \mid \theta]$
denote the posterior average over $\iota$ given $\theta \sim
\N(\alpha_\iota,\omega_0^{-1})$ and prior $\iota \sim
\operatorname{Uniform}\{1,\ldots,K\}$. Let $\kappa_2(\cdot)$ denote the
covariance associated to $\langle \cdot \rangle$. Then, since
\[\log g(\theta,\alpha)=\log \sum_{k=1}^K p_k \sqrt{\frac{\omega_k}{2\pi}}
\exp\Big({-}\frac{\omega_k}{2}(\theta-\alpha_k)^2\Big),\]
the derivatives of $\log g(\theta,\alpha)$ up to order 2 are given by
\begin{equation}\label{eq:loggderivmeanmix}
\begin{aligned}
\partial_\theta \log g(\theta,\alpha)
&=\langle \omega_\iota(\alpha_\iota-\theta)\rangle,
\quad \partial_\theta^2 \log g(\theta,\alpha)
=\kappa_2\big(\omega_\iota(\alpha_\iota-\theta),\omega_\iota(\alpha_\iota-\theta)\big)-\langle
\omega_\iota \rangle\\
%\partial_\theta^3 \log g(\theta,\alpha)&=
%\kappa_3\big(\omega_\iota(\alpha_\iota-\theta),\omega_\iota(\alpha_\iota-\theta),\omega_\iota(\alpha_\iota-\theta)\big)
%-3\kappa_2\big(\omega_\iota(\alpha_\iota-\theta),\omega_\iota\big)\\
\partial_{\alpha_i} \log g(\theta,\alpha)
&=\omega_i(\theta-\alpha_i)\langle \1_{\iota=i} \rangle,
\quad \partial_{\alpha_i}\partial_\theta \log g(\theta,\alpha)
=\omega_i(\theta-\alpha_i)\kappa_2\big(\1_{\iota=i},\omega_\iota(\alpha_\iota-\theta)\big)+\omega_i\langle \1_{\iota=i} \rangle,\\
%\partial_{\alpha_i}\partial_\theta^2 \log g(\theta,\alpha)
%&=\omega_i(\theta-\alpha_i)\kappa_3\big(\1_{\iota=i},\omega_\iota(\alpha_\iota-\theta),\omega_\iota(\alpha_\iota-\theta)\big)
%+2\omega_i\kappa_2\big(\1_{\iota=i},\omega_\iota(\alpha_\iota-\theta)\big)\\
%&\hspace{1in}-\omega_i(\theta-\alpha_i)\kappa_2(\1_{\iota=i},\omega_\iota),\\
\partial_{\alpha_i}\partial_{\alpha_j} \log g(\theta,\alpha)
&=\omega_i\omega_j(\theta-\alpha_i)(\theta-\alpha_j)\kappa_2(\1_{\iota=i},\1_{\iota=j})-\1_{i=j}\omega_i\langle \1_{\iota=i} \rangle\\
%\partial_{\alpha_i}\partial_{\alpha_j}\partial_\theta \log g(\theta,\alpha)
%&=\omega_i\omega_j(\theta-\alpha_i)(\theta-\alpha_j)\kappa_3\big(\1_{\iota=i},\1_{\iota=j},\omega_\iota(\alpha_\iota-\theta)\big)
%+\omega_i\omega_j(2\theta-\alpha_i-\alpha_j)\kappa_2(\1_{\iota=i},\1_{\iota=j})\\
%&\hspace{1in}-\1_{i=j}\omega_i\kappa_2\big(\1_{\iota=i},\omega_\iota(\alpha_\iota-\theta)\big),\\
%\partial_{\alpha_i}\partial_{\alpha_j}\partial_{\alpha_k} \log g(\theta,\alpha)
%&=\omega_i\omega_j\omega_k(\theta-\alpha_i)(\theta-\alpha_j)(\theta-\alpha_k)
%\kappa_3(\1_{\iota=i},\1_{\iota=j},\1_{\iota=k})
%-\1_{i=k}\omega_i\omega_j(\theta-\alpha_j)\kappa_2(\1_{\iota=i},\1_{\iota=j})\\
%&\hspace{1in}-\1_{j=k}\omega_i\omega_j(\theta-\alpha_i)\kappa_2(\1_{\iota=i},
%\1_{\iota=j})
%-\1_{i=j}\omega_i\omega_k(\theta-\alpha_k)\kappa_2(\1_{\iota=i},\1_{\iota=k})
\end{aligned}
\end{equation}
In particular, $|\partial_{\alpha_i} \log g(\theta,\alpha)| \leq
C(1+|\theta|+|\alpha_i|)$, so Assumption \ref{assump:gradient}(a) holds.

To bound the high-order derivatives of $\log g(\theta,\alpha)$
locally over $\alpha \in \R^K$, 
let $k_{\max} \in \{1,\ldots,K\}$ be the (unique)
index corresponding to the smallest
value of $\omega_k$. For any compact subset $S \subset \R^K$, there exist
constants $B(S),c_0(S)>0$ depending on the fixed values $\{p_1,\ldots,p_K\}$,
$\{\omega_1,\ldots,\omega_K\}$ and $S$ such that for all $\alpha \in S$, we have
\[\frac{\omega_k}{2}(\theta-\alpha_k)^2 \geq \frac{\omega_{k_{\max}}}{2}
(\theta-\alpha_{k_{\max}})^2
+c_0(S)\theta^2 \text{ for any } \theta>B(S) \text{ and all } k \neq k_{\max}.\]
This implies there exists a constant $C(S)>0$ for which
\[\langle \1_{\iota \neq k_{\max}} \rangle \leq C(S)e^{-c_0(S)\theta^2}
\text{ for all } \theta>B(S) \text{ and } \alpha \in S.\]
Let $\iota'$ denote an independent copy of $\iota$ under its posterior law
given $\theta$. Then for any $\theta>B$, any $\alpha \in S$,
and any $k \in \{1,\ldots,K\}$,
the posterior variance of $\1_{\iota=k}$ is bounded as
\[\langle |\1_{\iota=k}-\langle \1_{\iota=k} \rangle|^2 \rangle
\leq \langle |\1_{\iota=k}-\1_{\iota'=k}|^2 \rangle
\leq 4 \langle \1_{\iota \neq k_{\max} \text{ or }
\iota' \neq k_{\max}} \rangle \leq C'(S)e^{-c_0(S)\theta^2},\]
and similarly
\[\langle |\omega_\iota(\theta-\alpha_\iota)-\langle
\omega_\iota(\theta-\alpha_\iota) \rangle|^2 \rangle
\leq C'(S)(1+\theta)e^{-c_0(S)\theta}.\]
Applying these bounds and H\"older's inequality, all posterior covariances in
(\ref{eq:loggderivmeanmix}) are exponentially small in
$\theta^2$ for $\theta>B(S)$, implying that all derivatives of order 2 in
(\ref{eq:loggderivmeanmix}) are bounded over $\alpha \in S$ and $\theta>B$.
Similarly they are bounded over $\alpha \in S$ and $\theta<-B$, and hence
also bounded uniformly over $\alpha \in S$ and $\theta \in \R$ since we may
bound the cumulants trivially by a constant for $\theta \in [-B,B]$.
The same argument bounds all mixed cumulants of $\1_{\iota=k}$ and
$\omega_\iota(\alpha_\iota-\theta)$ of orders 3 and 4, and hence also all
partial derivatives of $\log g(\theta,\alpha)$ of orders 3 and 4
over $\alpha \in S$ and $\theta \in \R$. This
implies Assumptions \ref{assump:prior}(a) and \ref{assump:gradient}(b). These
arguments show also, as $\theta \to \pm \infty$,
$\kappa_2(\omega_\iota(\alpha_\iota-\theta),\omega_\iota(\alpha_\iota-\theta))
\to 0$ and $\langle \omega_\iota \rangle \to \omega_{k_{\max}}$, so
$\partial_\theta^2[-\log g(\theta,\alpha)] \to \omega_{k_{\max}}>0$, verifying
Assumption \ref{assump:prior}(b). Thus Assumptions \ref{assump:prior} and
\ref{assump:gradient} hold.
\end{proof}

\begin{proof}[Analysis of Example \ref{ex:gaussianweightmixture}]
We verify Assumptions \ref{assump:prior} and \ref{assump:gradient}
in Example \ref{ex:gaussianweightmixture} for the
Gaussian mixture model with fixed mixture mean/variances and varying weights.
Again let $\iota \in \{0,\ldots,K\}$ denote the mixture component of $\theta$,
and let $\langle f(\iota,\theta) \rangle=\E[f(\iota,\theta) \mid \theta]$
denote the posterior average over $\iota$ given $\theta \sim
\N(\mu_\iota,\omega_\iota^{-1})$ and prior
$\P[\iota=k]=e^{\alpha_k}/(e^{\alpha_0}+\ldots+e^{\alpha_K})$.
Let $\kappa_2(\cdot)$ denote the
covariance associated to $\langle \cdot \rangle$, and
in addition, let $\langle \cdot \rangle_{\text{prior}}$ and
$\kappa_2^{\text{prior}}$ denote the mean and covariance
over $\iota$ drawn from the prior
$\P[\iota=k]=e^{\alpha_k}/(e^{\alpha_0}+\ldots+e^{\alpha_K})$.
Then, since
\[\log g(\theta,\alpha)=\log\sum_{k=0}^K e^{\alpha_k}
\sqrt{\frac{\omega_k}{2\pi}}\exp\Big({-}\frac{\omega_k}{2}(\theta-\mu_k)^2\Big)
-\log\sum_{k=0}^K e^{\alpha_k},\]
the derivatives of $\log g(\theta,\alpha)$ up to order 2 are given by
\begin{equation}\label{eq:gaussianmixturederivs}
\begin{gathered}
\partial_{\alpha_i} \log g(\theta,\alpha)=\langle \1_{\iota=i} \rangle
-\langle \1_{\iota=i}\rangle_{\text{prior}},
\quad \partial_{\alpha_i} \partial_{\alpha_j}
\log g(\theta,\alpha)=\kappa_2(\1_{\iota=i},\1_{\iota=j})
-\kappa_2^{\text{prior}}(\1_{\iota=i},\1_{\iota=j}),\\
\partial_\theta \log g(\theta,\alpha)
=\langle \omega_\iota(\mu_\iota-\theta) \rangle,
\quad \partial_{\alpha_i}\partial_\theta
\log g(\theta,\alpha)
=\kappa_2\big(\1_{\iota=i},\omega_\iota(\mu_\iota-\theta)\big),\\
%\partial_{\alpha_k}\partial_\theta^2 \log g(\theta,\alpha)
%=\kappa_3\big(\1_{\iota=k},\omega_\iota(\mu_\iota-\theta),
%\omega_\iota(\mu_\iota-\theta)\big)
%-\kappa_2(\1_{\iota=k},\omega_\iota),\\
\partial_\theta^2 \log g(\theta,\alpha)
=\kappa_2\big(\omega_\iota(\mu_\iota-\theta),
\omega_\iota(\mu_\iota-\theta)\big)-\langle \omega_\iota \rangle.
%\partial_\theta^3 \log g(\theta,\alpha)
%=\kappa_3\big(\omega_\iota(\mu_\iota-\theta),\omega_\iota(\mu_\iota-\theta),
%\omega_\iota(\mu_\iota-\theta)\big)
%-3\kappa_2\big(\omega_\iota(\mu_\iota-\theta),\omega_\iota\big)+2\theta
%\kappa_2(\omega_\iota,\omega_\iota).
\end{gathered}
\end{equation}
In particular, this shows $\sum_k \partial_{\alpha_k} \log
g(\theta,\alpha)=1-1=0$,
so $\nabla_\alpha \log g(\theta,\alpha)$ always belongs to the subspace
$E=\{\alpha \in \R^{K+1}:\alpha_0+\ldots+\alpha_K=0\}$. Furthermore,
$|\partial_{\alpha_i} \log g(\theta,\alpha)|$ is uniformly bounded,
so Assumption \ref{assump:gradient}(a) holds.

To bound the higher-order derivatives locally over $\alpha \in E$,
let $k_{\max} \in \{1,\ldots,K\}$ be the
index corresponding to the smallest $\omega_k$, and among these the largest
$\mu_k$ (if there are multiple $\omega_k$'s equal to the smallest value).
Then for some constants $B,c_0>0$ depending only on the fixed values
$\{\mu_0,\ldots,\mu_K\}$ and $\{\omega_0,\ldots,\omega_K\}$, we have
\[\frac{\omega_k}{2}(\theta-\mu_k)^2
\geq \frac{\omega_{k_{\max}}}{2}
(\theta-\mu_{k_{\max}})^2+c_0\theta \text{ for any } \theta>B \text{ and all }
k \neq k_{\max}.\]
This implies, for any compact subset $S \subset E$, there is a constant $C(S)>0$
for which
\[\langle \1_{\iota \neq k_{\max}} \rangle
\leq C(S)e^{-c_0\theta} \text{ for all } \theta>B \text{ and } \alpha \in S.\]
Then the same arguments as in the preceding example show
\[\langle |\omega_\iota-\langle \omega_\iota \rangle|^2 \rangle
\leq C'(S)e^{-c_0\theta}, \quad
\langle |\omega_\iota(\mu_\iota-\theta)-\langle \omega_\iota(\mu_\iota-\theta)
\rangle|^2 \rangle
\leq C'(S)(1+\theta)e^{-c_0\theta},\]
implying via Cauchy-Schwarz that each order-2 derivative in
(\ref{eq:gaussianmixturederivs}) is bounded over
$\alpha \in S$ and $\theta>B$. Similarly it is bounded over
$\alpha \in S$ and $\theta<-B$, hence also for all $\alpha \in S$
and $\theta \in \R$, and the same argument applies to bound the
higher order mixed cumulants of $\omega_\iota$ and
$\omega_\iota(\mu_\iota-\theta)$ and the partial
derivatives of $\log g(\theta,\alpha)$ of orders 3 and 4.
This implies Assumptions \ref{assump:prior}(a) and
\ref{assump:gradient}(b). This shows also
$\lim_{\theta \to \infty} \partial_\theta^2 [-\log g(\theta,\alpha)]
=\omega_{k_{\max}}>0$, and a similar argument holds for $\theta \to {-}\infty$,
establishing Assumption \ref{assump:prior}(b).
\end{proof}

\begin{proof}[Analysis of Example \ref{ex:expfamily}]
In the exponential family model of Example \ref{ex:expfamily}, we have
\[\partial_\theta^q \log g(\theta,\alpha)
=\sum_{k=1}^K \alpha_k T_k^{(q)}(\theta)+(\log h)^{(q)}(\theta),
\quad \partial_{\alpha_i} \partial_\theta^q \log g(\theta,\alpha)
=T_i^{(q)}(\theta) \text{ for all } q \geq 0,\]
\[\partial_{\alpha_{k_1}} \ldots \partial_{\alpha_{k_p}}
\log g(\theta,\alpha)=-\partial_{\alpha_{k_1}} \ldots \partial_{\alpha_{k_p}}
A(\alpha) \text{ for all } p \geq 2,\]
and all other mixed derivatives are 0. Then the stated conditions for
$T_k(\theta)$ and $\log h(\theta)$
imply Assumption \ref{assump:prior}. Furthermore, since
$\nabla_{\alpha}\partial_\theta \log g(\theta,\alpha)$ is globally bounded,
this implies also $\|\nabla_{\alpha} \log g(\theta,\alpha)\|_2
\leq C(1+|\theta|+\|\alpha\|_2)$, so Assumption \ref{assump:gradient}(a) holds.
The derivative bounds in Assumption \ref{assump:gradient}(b) follow from
the stated conditions for $T_k(\theta)$ and $\log h(\theta)$, together with
the fact that $A(\alpha)$ is analytic on all of $\R^K$ and hence has bounded
derivatives over compact subsets of $\R^K$. Thus
Assumptions \ref{assump:prior} and \ref{assump:gradient} hold in this example.
\end{proof}

%\begin{lemma}\label{lem:gibbs_G_general}
%Suppose $\cG$ is chosen as (\ref{eq:FalphaEB}). Suppose that $g(\theta;\alpha)$ satisfies (\ref{eq:prior_logcavity}), and uniformly over $(\theta, \alpha) \in \R\times S$ for any compact set $S\subset \R^K$, 
%\begin{align}\label{eq:smoothness_verify}
%\pnorm{\partial_\theta^{q_1} \nabla_{\alpha}^{q_2} \log g(\theta;\alpha)}{F} \leq M, \quad q_1 + q_2 \in \{2,3\}, \quad q_1,q_2 \in \Z_+,  
%\end{align}
%for some $M = M(S) > 0$, where $\partial_\theta^{q_1} \nabla_{\alpha}^{q_2} \log g(\theta;\alpha) = \big(\partial_\theta^{q_1} \partial_{\alpha_{i_1}}\ldots \partial_{\alpha_{i_{q_2}}} \log g(\theta;\alpha)\big)_{i_1,\ldots,i_{q_2} \in [K]}$ is understood as a tensor in $(\R^{K})^{q_2}$. Then Assumptions \ref{assump:prior} and \ref{assump:gradient} are satisfied. 
%\end{lemma}
%\begin{proof}
%To verify Assumption \ref{assump:gradient}-(a), we have
%\begin{align*}
%\pnorm{\cG(\alpha, \sP)}{} &= \pnorm{\E_{\sP} \nabla_{\alpha} \log g(\theta;\alpha)}{} \leq \sup_{\theta\in\R, \alpha\in S} \pnorm{\nabla_\alpha^2 \log g(\theta;\alpha)}{\op} \cdot \pnorm{\alpha}{} + \pnorm{\nabla_\alpha \log g(0;0)}{} + \E_{\sP}[\sup_{\theta\in \R, \alpha\in S} \pnorm{\partial_\theta \nabla_{\alpha} \log g(\theta;\alpha)}{}|\theta|]\\
%&\leq C(1+\pnorm{\alpha}{} + \E_{\sP} |\theta|),
%\end{align*}
%with $C = \pnorm{\nabla_\alpha \log g(0;0)}{} \vee M$. To verify (\ref{eq:G_smooth1}), we have
%\begin{align*}
%\pnorm{\cG(\alpha, \sP) - \cG(\alpha', \sP')}{} &\leq \E_{\sP} \pnorm{\nabla_\alpha \log (\theta;\alpha) - \nabla_\alpha \log (\theta;\alpha')}{} + \Big|(\E_{\sP} - \E_{\sP'}) \pnorm{ \nabla_\alpha \log (\theta;\alpha')}{}\Big|\\
%&\leq \sup_{\theta\in\R, \alpha \in S} \pnorm{\nabla_\alpha^2 \log g(\theta;\alpha)}{\op}\pnorm{\alpha - \alpha'}{} + MW_2(\sP, \sP') \leq M(\pnorm{\alpha - \alpha'}{} + W_2(\sP, \sP') ),
%\end{align*}
%where we use the fact that $\theta \mapsto \pnorm{\nabla_\alpha \log g(\theta;\alpha)}{}$ is $M$-Lipschitz uniformly over $(\theta,\alpha) \in \R \times S$ since
%\begin{align*}
%\Big|\pnorm{\nabla_\alpha \log g(\theta;\alpha)}{} - \pnorm{\nabla_\alpha \log g(\theta';\alpha)}{}\Big| \leq \sup_{\theta\in\R, \alpha \in S}\pnorm{\partial_\theta \nabla_\alpha \log g(\theta;\alpha)}{F} \cdot |\theta - \theta'| \leq M |\theta - \theta'|.  
%\end{align*}
%The claim (\ref{eq:G_smooth2}) is verified since
%\begin{align*}
%\nabla_{\alpha} \cG(\alpha, \Prob_n(\btheta)) = d^{-1} \sum_{j=1}^d \nabla_\alpha^2 \log g(\theta_j; \alpha),\quad \nabla_{\btheta}\nabla_{\alpha} \cG(\alpha, \Prob_n(\btheta)) = d^{-1} (\partial_\theta\nabla_\alpha \log g(\theta_j;\alpha))_{j=1}^d.
%\end{align*}
%The claim (\ref{eq:G_smooth3}) is verified by the formulas
%\begin{align*}
%[\nabla_{\btheta}^2 \cG(\alpha, \Prob_n(\btheta))]_{i,j,\cdot} &= \frac{1}{d}\bm{1}_{i=j} \partial_\theta^2 \nabla_\alpha \log g(\theta_i;\alpha), \quad i,j\in[d],\\
%[\nabla_{\btheta} \nabla_\alpha \cG(\alpha, \Prob_n(\btheta))]_{i,\cdot,\cdot} &= \frac{1}{d}\partial_\theta \nabla_\alpha^2 \log g(\theta_i;\alpha), \quad i\in[d], \\
%\nabla_\alpha^2 \cG(\alpha, \Prob_n(\btheta)) &= \frac{1}{d} \sum_{j=1}^d \nabla_{\alpha}^3 \log g(\theta_j;\alpha).
%\end{align*}
%\end{proof}
%
%%\todo{Example 1: $K$-component Gaussian mixture prior
%\[g(\theta;\alpha)=\frac{\sum_{k=1}^K e^{\alpha_k}\d\N(\theta;\mu_k,\tau_k^2)}
%{\sum_{k=1}^K e^{\alpha_k}}\]
%with fixed grid $\{(\mu_k,\sigma_k^2)\}_{k=1}^K$ and unknown mixture weights,
%where $\d\N(\theta;\mu,\tau^2)$ denotes the normal density. We may take
%\[\cF(\alpha,\cL)=\E_{\theta \sim \cL}[\nabla_\alpha \log g(\theta;\alpha)]
%=\bigg(\E_{\theta \sim \cL}\bigg[\frac{e^{\alpha_k}\d\N(\theta;\mu_k,\tau_k^2)}
%{\sum_{j=1}^K e^{\alpha_j}\d\N(\theta;\mu_j,\tau_j^2)}\bigg]
%-\frac{e^{\alpha_k}}{\sum_{j=1}^K e^{\alpha_j}}\bigg)_{k=1}^K\]}

%\begin{lemma}[Exponential family]
%Consider the exponential family density $g(\theta;\alpha) = h(\theta)\exp(\sum_{k=1}^K \alpha_k T_k(\theta) - A(\alpha))$ for some $h:\R\rightarrow\R_+$, $T_1,\ldots,T_K: \R\rightarrow \R$, and $A(\alpha) = \int h(\theta)\exp(\sum_{k=1}^K \alpha_k T_k(\theta)) \d\theta$. Suppose that
%\begin{enumerate}
%\item For any $\alpha \in \R^K$, it holds that $\liminf_{|\theta|\rightarrow\infty} -\partial_\theta^2 \log h(\theta) - \sum_{k=1}^K \alpha_k T_k''(\theta) > 0$.
%\item There exists some $L_1 > 0$ such that
%\begin{align*}
%\sup_{\theta\in\R}\Big[\max_{1\leq k\leq K} |T_k'(\theta)| \vee  |T_k''(\theta)| \vee  |T_k'''(\theta)| \vee |\partial_\theta^2 \log h(\theta)| \vee |\partial_\theta^3 \log h(\theta)|\Big] \leq L_1.
%\end{align*}
%\item For any $f:\R\rightarrow\R$, write $\av{f(\theta)} = \int f(\theta)h(\theta)\exp(\sum_{k=1}^K \alpha_k T_k(\theta))\d \theta/\int h(\theta)\exp(\sum_{k=1}^K \alpha_k T_k(\theta))\d \theta$. For any compact set $S\subset\R^K$, there exists some $L_2 = L_2(S) > 0$ such that
%\begin{align*}
%&\max_{i,j\in[K]} |\av{T_iT_j} - \av{T_i}\av{T_j} | \leq L_2,\\
%&\max_{i,j,k\in[K]} |\av{T_iT_jT_k} - \av{T_i}\av{T_jT_k} - \av{T_j}\av{T_iT_k} - \av{T_k}\av{T_iT_j} + 2 \av{T_i}\av{T_j}\av{T_k} | \leq L_2.
%\end{align*}
%\end{enumerate} 
%Then $g(\theta;\alpha)$ and $\cG(\cdot)$ chosen in (\ref{eq:FalphaEB}) satisfy Assumptions \ref{assump:prior} and \ref{assump:gradient}. 
%\end{lemma}
%\begin{remark}
%A concrete example of the above is $g(\theta;\alpha) = (2\pi\tau^2)^{-1/2}\exp(-(\theta - \alpha)^2/(2\tau^2))$, for which $K = 1$, $h(\theta) =  (2\pi\tau^2)^{-1/2}\exp(-\theta^2/(2\tau^2))$, $T_1(\theta) = \theta/\tau^2$.
%\end{remark}
%\begin{proof}
%This follows from the following direct calculation:
%\begin{align*}
%\partial_\theta^{(\ell)} \log g(\theta;\alpha) &= \partial_\theta^{(\ell)} \log h(\theta) + \sum_{k=1}^K \alpha_k T_k^{(\ell)}(\theta), \ell = 1,2,3,\\
%[\partial_\theta \nabla_{\alpha} \log g(\theta;\alpha)]_i &= T_i'(\theta), \quad [\partial_\theta^2 \nabla_{\alpha} \log g(\theta;\alpha)]_i = T_i''(\theta),\\
%[\nabla_\alpha^2 \log g(\theta;\alpha)]_{i,j} &= \partial_{\alpha_i}\partial_{\alpha_j} A(\alpha) = \av{T_iT_j} - \av{T_i}\av{T_j}, \quad \partial_\theta\nabla_\alpha^2 \log g(\theta;\alpha) = 0, \\
%[\nabla_\alpha^3 \log g(\theta;\alpha)]_{i,j,k} &= \partial_{\alpha_i}\partial_{\alpha_j}\partial_{\alpha_k} A(\alpha) = \av{T_iT_jT_k} - \av{T_i}\av{T_jT_k} - \av{T_j}\av{T_iT_k} - \av{T_k}\av{T_iT_j} + 2 \av{T_i}\av{T_j}\av{T_k}
%\end{align*}
%\end{proof}

%\begin{lemma}[Gaussian mixture]
%Fix $\tau^2 > 0$ and let $\mu_1,\ldots,\mu_K \in \R$ satisfy $\max_{1\leq i\leq K} |\mu_i| \leq B$ for some $B > 0$. Then $g(\theta;\alpha) = \sum_{k=1}^K e^{\alpha_k} \d \N(\theta; \mu_k, \tau^2)/\sum_{k=1}^K e^{\alpha_k}$ and $\cG(\cdot)$ chosen in (\ref{eq:FalphaEB}) satisfy Assumptions \ref{assump:prior} and \ref{assump:gradient}. 
%\end{lemma}
%\begin{proof}
%For simplicity we verify the conditions of Lemma \ref{lem:gibbs_G_general} for  $\tau^2 = 1$. Consider the model $\theta = \mu + Z$ where $\mu$ takes value $\mu_i$ with probability $e^{\alpha_i}/\sum_{k=1}^K e^{\alpha_k}$ and is independent of $Z \sim \N(0,1)$. For any $f:\R\rightarrow\R$, we use $\av{f(\mu)} = \sum_{k=1}^K f(\mu_k)\phi(\theta - \mu_k)/\sum_{k=1}^K \phi(\theta - \mu_k)$ to denote the posterior mean given observation $\theta$. Then direct calculation shows that
%\begin{align*}
%\partial_\theta \log g(\theta;\alpha) = -\theta + \av{\mu}, \quad \partial_\theta^2 \log g(\theta;\alpha) =  -1 + \av{\mu^2} - \av{\mu}^2, \quad \partial_\theta^2 \log g(\theta;\alpha) = \av{\mu^3} - 3\av{\mu^2}\av{\mu} + 2\av{\mu}^3,
%\end{align*}
%and
%\begin{align*}
%\partial_{\alpha_i} \av{\mu}&= \av{\bm{1}_{\mu = \mu_i}}(\mu_i - \av{\mu}) = \partial_\theta \av{\bm{1}_{\mu = \mu_i}} = \av{\bm{1}_{\mu = \mu_i}} (\mu_i - \av{\mu}),\\
%\partial_{\alpha_j} \av{\bm{1}_{\mu = \mu_i}} &= \bm{1}_{i=j}\av{\bm{1}_{\mu = \mu_i}} - \av{\bm{1}_{\mu = \mu_i}}\av{\bm{1}_{\mu = \mu_j}}, \quad \partial_{\alpha_j} \Prob(\mu = \mu_i) = \bm{1}_{i=j} \Prob(\mu = \mu_i) - \Prob(\mu = \mu_i)\Prob(\mu = \mu_j).
%\end{align*}
%From these we deduce
%\begin{align*}
%\partial_{\alpha_i}\partial_\theta \log g(\theta;\alpha) &= \partial_{\alpha_i} \av{\mu} = \av{\bm{1}_{\mu = \mu_i}}(\mu_i - \av{\mu}),\\
%\partial_{\alpha_i} \partial_\theta^2 g(\theta;\alpha) &= \partial_\theta \av{\bm{1}_{\mu = \mu_i}}\cdot (\mu_i - \av{\mu}) - \av{\bm{1}_{\mu = \mu_i}} \partial_\theta \av{\mu} = \av{\bm{1}_{\mu = \mu_i}}((\mu_i - \av{\mu})^2 - \av{\mu^2} + \av{\mu}^2),\\
%\partial_{\alpha_i} \log g(\theta;\alpha) &= \av{\bm{1}_{\mu=\mu_i}} - \Prob(\mu = \mu_i),\\
%\partial_{\alpha_i}\partial_{\alpha_j} \log g(\theta;\alpha) &= \av{\bm{1}_{\mu = \mu_i}}\bm{1}_{i=j} - \av{\bm{1}_{\mu = \mu_i}}\av{\bm{1}_{\mu = \mu_j}} - \Prob(\mu = \mu_i)\bm{1}_{i=j} +  \Prob(\mu = \mu_i)  \Prob(\mu = \mu_j),\\
%\partial_{\alpha_i}\partial_{\alpha_j}\partial_{\alpha_k} \log g(\theta;\alpha) &= \bm{1}_{i=j=k}\av{\bm{1}_{\mu = \mu_i}} - \bm{1}_{i=j} \av{\bm{1}_{\mu = \mu_i}}\av{\bm{1}_{\mu = \mu_k}} - \bm{1}_{i=k}\av{\bm{1}_{\mu = \mu_i}}\av{\bm{1}_{\mu = \mu_j}} - \bm{1}_{j=k}\av{\bm{1}_{\mu = \mu_j}}\av{\bm{1}_{\mu = \mu_i}}\\
%&\quad + 2\av{\bm{1}_{\mu = \mu_i}}\av{\bm{1}_{\mu = \mu_j}}\av{\bm{1}_{\mu = \mu_k}} - \bm{1}_{i=j=k}\Prob(\mu = \mu_i) + \bm{1}_{i=j}\Prob(\mu = \mu_i)\Prob(\mu = \mu_k)\\
%&\quad + \bm{1}_{i=k}\Prob(\mu = \mu_i)\Prob(\mu = \mu_j) + \bm{1}_{j=k}\Prob(\mu = \mu_i)\Prob(\mu = \mu_j) - 2 \Prob(\mu = \mu_i)\Prob(\mu = \mu_j)\Prob(\mu = \mu_k),
%\end{align*}
%and all of the above is bounded by some constant that only depends on $B$. This verifies (\ref{eq:smoothness_verify}). Lastly, note that $\liminf_{|\theta| \to \infty} {-}\partial_\theta^2 \log g(\theta,\alpha) = 1$, verifying (\ref{eq:prior_logcavity}).
%\end{proof}
%
%\todo{Example 2: $K$-parameter exponential family
%\[g(\theta;\alpha)=h(\theta)\exp\bigg(\sum_{k=1}^K \alpha_k T_k(\theta)-A(\alpha)\bigg),
%\qquad A(\alpha)=\log \int \exp\bigg(\sum_{k=1}^K \alpha_k T_k(\theta)\bigg)h(\theta)
%\d\theta\]
%We may take
%\[\cF(\alpha,\cL)=\E_{\theta \sim \cL}[\nabla_\alpha \log g(\theta;\alpha)]
%=\E_{\theta \sim \cL}[T(\theta)]-\nabla A(\alpha).\]}
%
%\begin{assumption}\label{assump:lipschitz}
%\begin{enumerate}[(a)]
%\item $\cA$ is an open subset of $\R^K$, and
%for some $C>0$ and all $\cL \in \cP_2(\R)$ and $\alpha_1,\alpha_2 \in \cA$,
%\begin{align}
%\|\cF(\alpha_1,\cL)-\cF(\alpha_2,\cL)\|_2 \leq C\|\alpha_1-\alpha_2\|_2,\label{eq:lip_F_1}\\
%\blue{\|\cF(\alpha,\cL_1)-\cF(\alpha,\cL_2)\|_2 \leq CW_2(\cL_1, \cL_2)}\label{eq:lip_F_2}.
%\end{align}
%\item $(\theta,\alpha) \mapsto \log g(\theta;\alpha)$ is differentiable on $\R
%\times \cA$. For each compact subset $S \subset \cA$, some $C(S)>0$,
%and all $\theta_1,\theta_2 \in \R$ and $\alpha \in S$,
%\begin{align}
%\sup_{\theta\in\R}|\partial^2_\theta \log g(\theta;\alpha)| &\leq C(S) \label{eq:theta_deriv_lip}\\
%\|\nabla_\alpha \log g(\theta_1;\alpha)
%-\nabla_\alpha \log g(\theta_2;\alpha)\|_2 &\leq C(S)|\theta_1-\theta_2|\label{eq:alpha_deriv_lip},\\
%\|\nabla_\alpha \partial_\theta\log g(\theta;\alpha)\| &\leq C|\theta|\label{eq:mix_deriv_lip}.
%\end{align}
%\end{enumerate}
%\end{assumption}
%
%\ys{We verify Assumption \ref{assump:lipschitz} for the two examples above. For example 1, (\ref{eq:lip_F_1}) holds since
%\begin{align*}
%\partial_{\alpha_k} \cF(\alpha, \cL) = \E_{\theta\sim \cL} \Big[\frac{e^{\alpha_k} \d N(\theta; \mu_j, \tau_j^2)}{\sum_{j=1}^K e^{\alpha_j} \d N(\theta; \mu_j, \tau_j^2)} - \Big(\frac{e^{\alpha_k} \d N(\theta; \mu_j, \tau_j^2)}{\sum_{j=1}^K e^{\alpha_j} \d N(\theta; \mu_j, \tau_j^2)}\Big)^2\Big] - \frac{e^{\alpha_K}}{\sum_{j=1}^K e^{\alpha_j}} + \Big(\frac{e^{\alpha_K}}{\sum_{j=1}^K e^{\alpha_j}}\Big)^2 \leq 4,
%\end{align*}
%and (\ref{eq:lip_F_2}) holds since $\pnorm{\cF(\alpha, \cL_1) - \cF(\alpha, \cL_2)}{} = \sqrt{\sum_{k=1}^K \big(\E_{\theta\sim \cL_1} f_k(\theta) - \E_{\theta\sim \cL_2} f_k(\theta)\big)^2}$, where
%\begin{align*}
%f_k(\theta) = \frac{e^{\alpha_k}\d \N(\theta; \mu_k; \tau_k^2)}{\sum_{j=1}^K e^{\alpha_j}\d \N(\theta; \mu_j; \tau_j^2)}
%\end{align*}
%is bounded and Lipschitz with constant depending on $(\mu_j, \tau_j)$. Direct calculation yields
%\begin{align*}
%\partial_\theta \log g(\theta;\alpha) = -\frac{\sum_{k=1}^K e^{\alpha_k} \frac{\theta - \mu_k}{\tau_k^2}\d \N(\theta;\mu_k,\tau_k^2)}{\sum_{k=1}^K e^{\alpha_k} \d \N(\theta;\mu_k,\tau_k^2)} = \E\Big[\frac{\mu-X}{\tau^2}|X = \theta\Big]
%\end{align*}
%and
%\begin{align*}
%\partial^2_\theta \log g(\theta;\alpha) &= -\frac{\sum_{k=1}^K e^{\alpha_k} \frac{1}{\tau_k^2}\d \N(\theta;\mu_k,\tau_k^2)}{\sum_{k=1}^K e^{\alpha_k} \d \N(\theta;\mu_k,\tau_k^2)} + \frac{\sum_{k=1}^K e^{\alpha_k} (\frac{\theta - \mu_k}{\tau_k^2})^2\d \N(\theta;\mu_k,\tau_k^2)}{\sum_{k=1}^K e^{\alpha_k} \d \N(\theta;\mu_k,\tau_k^2)} - \Big(\frac{\sum_{k=1}^K e^{\alpha_k} \frac{\theta - \mu_k}{\tau_k^2}\d \N(\theta;\mu_k,\tau_k^2)}{\sum_{k=1}^K e^{\alpha_k} \d \N(\theta;\mu_k,\tau_k^2)}\Big)^2\\
%&= -\E\Big[\frac{1}{\tau^2}|X = \theta\Big] + \Var\Big(\frac{\mu - X}{\tau^2}|X = \theta\Big),
%\end{align*}
%where the expectation is taken over the channel $X|\mu,\tau \sim \N(\mu,\tau^2)$ and $(\mu,\tau^2) \sim \sum_{k=1}^K (e^{\alpha_k}/\sum_{j=1}^K e^{\alpha_j}) \delta_{(\mu_k, \tau_k^2)}$.
%
%For example 2, 
%\begin{align*}
%\pnorm{\cF(\alpha_1,\cL) - \cF(\alpha_2, \cL)}{} = \pnorm{\nabla A(\alpha_1) - \nabla A(\alpha_2)}{} \leq \sup_{\alpha \in\R^K} \pnorm{\nabla^2 A(\alpha)}{\op} \pnorm{\alpha_1 - \alpha_2}{}
%\end{align*}
%and
%\begin{align*}
%\pnorm{\cF(\alpha,\cL_1) - \cF(\alpha, \cL_2)}{} = \sqrt{\sum_{k=1}^K \big(\E_{\theta\sim \cL_1} T_k(\theta) - \E_{\theta\sim \cL_2} T_k(\theta)\big)^2} \leq CW_2(\cL_1, \cL_2),
%\end{align*}
%provided that $\{T_k\}_{k\in[K]}$ are Lipschitz. Next we have $\log g(\theta;\alpha) = \log h(\theta) + \sum_{k=1}^K \alpha_k T_k(\theta) - A(\alpha)$, so 
%\begin{align*}
%\partial_\theta \log g(\theta;\alpha) &= \partial_\theta h(\theta) + \sum_{k=1}^K \alpha_k \partial_\theta T_k(\theta),\\
%\partial_\theta^2 \log g(\theta;\alpha) &= \partial_\theta^2 h(\theta) + \sum_{k=1}^K \alpha_k \partial_\theta^2 T_k(\theta),\\
%\nabla_\alpha \partial_\theta \log g(\theta;\alpha) &= \Big(\partial_\theta T_1(\theta), \ldots, \partial_\theta T_K(\theta)\Big).
%\end{align*}.
%}




==> auxiliary.tex <==
\section{Auxiliary results}
\begin{lemma}\label{lem:gronwall}
Let $T > 0$ and suppose $g: [0,T] \rightarrow \R_+$ is a bounded function satisfying
\begin{align*}
g(t) \leq C_1 + \int_0^t C_2 g(s)\d s, \quad t\in[0,T].
\end{align*}
Then
\begin{align*}
g(t) \leq C_1\exp(C_2t), \quad t\in[0,T]. 
\end{align*}
\end{lemma}
\begin{proof}
Iterating the growth condition yields
\begin{align*}
g(t) \leq C_1\sum_{k=0}^n \frac{(C_2t)^k}{k!} + C_2^{n+1}\int_0^t\int_0^{s_1}\ldots\int_0^{s_n} g(s_{n+1})\d_{s_{n+1}}\ldots \d s_1. 
\end{align*}
The second term satisfies
\begin{align*}
0 \leq C_2^{n+1}\int_0^t\int_0^{s_1}\ldots\int_0^{s_n} g(s_{n+1})\d_{s_{n+1}}\ldots \d s_1 \leq \frac{\pnorm{g}{\infty}(C_2t)^{n+1}}{(n+1)!} \rightarrow_{n\rightarrow\infty} 0
\end{align*}
uniformly over $t\in [0,T]$. The result follows by taking $n\rightarrow\infty$.
\end{proof}





==> dmftgaussian.tex <==
\section{Solution of the DMFT system for fixed Gaussian prior}\label{appendix:gaussian}

We specialize the hypothesized model to a Gaussian prior
$g=\N(0,\frac{1}{\lambda})$ with
\[f(\theta)=\frac{\lambda}{2}\theta^2,
\qquad f'(\theta)=\lambda \theta, \qquad f''(\theta)=\lambda.\]
(We do not need to assume that this is the true prior $g_\ast(\cdot)$ for
$\theta^\ast$, i.e.\ the prior may be misspecified.)
Under this specialization, since $f''(\theta^t)$ does not depend on $\theta^t$,
the three equations
\eqref{def:response_theta}--\eqref{def:derivative_langevin_ostar} are a closed
system of deterministic equations, and
$R_\theta(t,s), R_\eta(t,s), R_\eta(t,\ast)$ may be defined in
\eqref{def:dmft_R} without taking expectations.

For any $z < 0$, let $m(z)$ be the positive root of the quadratic equation
\begin{equation}\label{eq:MPquadratic}
m(z)=\frac{1}{1-\delta^{-1}-\delta^{-1}zm(z)-z}
\Leftrightarrow \big(1+zm(z)\big)\big(1+\delta^{-1}m(z)\big)=m(z)
\end{equation}
which is the Stieltjes transform $m(z)=\lim_{n,p \to \infty} \frac{1}{p}\Tr
(\delta^{-1}\X^\top \X-z)^{-1}$ of the Marcenko-Pastur limit spectral law of
$\delta^{-1}\X^\top \X$.

%\subsection{Solution of DMFT system}

We first solve for the response functions $R_\theta(t,s), R_\theta(t,\ast),
R_\eta(t,s)$. 

\begin{lemma}\label{lem:response_sol}
We have
\[R_\theta(t,s)=\alpha(t-s), \qquad
R_\eta(t,s)=\frac{\delta}{\sigma^2}\beta(t-s), \qquad
R_\eta(t,*)=\frac{\delta}{\sigma^2}\gamma(t)\]
where
\begin{align}
\alpha(t) &= \int e^{-(\lambda + \delta x/\sigma^2)t} \mu(\d x), \label{eq:alpha_sol}\\
\beta(t) &= -\frac{1}{\sigma^2}\int xe^{-(\lambda + \delta x/\sigma^2)t}
\mu(\d x), \label{eq:beta_sol}\\
\gamma(t) &= \frac{1}{\sigma^2}\int \frac{x}{\lambda + \delta x/\sigma^2}
\Big(1-e^{-(\lambda +\delta x/\sigma^2)t}\Big)\mu(\d x)\label{eq:gamma_sol}
\end{align}
and $\mu(\cdot)$ is the Marcenko-Pastur limit spectral law
of $\delta^{-1}\X^\top\X$.
\end{lemma}
\begin{proof}
We posit a solution to (\ref{def:response_theta})--(\ref{def:response_g}) 
of the form
\begin{equation}\label{eq:ansatz}
R_\theta(t,s)=\frac{\partial \theta^t}{\partial u^s}=\alpha(t-s), \qquad
R_\eta(t,s)=\frac{\delta}{\sigma^2}\frac{\partial \eta^t}{\partial w^s}
=\frac{\delta}{\sigma^2}\beta(t-s)
\end{equation}
for some functions $\alpha,\beta:\R_+ \to \R$.
Then (\ref{def:response_theta}) and (\ref{def:response_g}) become
\begin{equation}\label{eq:alpha_beta_bar_ridge_cont}
\begin{aligned}
\alpha'(t) &= -\bigg(\lambda + \frac{\delta}{\sigma^2}\bigg)
\alpha(t) - \frac{\delta}{\sigma^2}\int_0^t
\beta(t-s)\alpha(s) \d s,\\
\beta(t) &= {-}\frac{1}{\sigma^2}\Big[\int_0^t \beta(t-s)\alpha(s)\d s + \alpha(t)\Big].
\end{aligned}
\end{equation}
For any function $x:\R_+\rightarrow\R$, let $\mathcal{L}_x(s) = \int_0^\infty
e^{-st}x(t)\d t$ be its Laplace transform. We apply the Laplace transform
identities
\[f(t)=\int_0^t x(t-s)y(s)\d s
\Rightarrow \cL_f(s)=\cL_x(s)\cL_y(s),
\qquad f(t)=x'(t) \Rightarrow \cL_f(s)=s\cL_x(s)-x(0),\]
and the boundary condition $\alpha(0)=1$.
Then taking the Laplace transform of both equations
\eqref{eq:alpha_beta_bar_ridge_cont} gives
\begin{align*}
s\cL_{\alpha}(s)-1
&={-}\bigg(\lambda+\frac{\delta}{\sigma^2}\bigg)\cL_{\alpha}(s)
-\frac{\delta}{\sigma^2}\cL_{\beta}(s)\cL_{\alpha}(s),\\
\cL_{\beta}(s)&={-}\frac{1}{\sigma^2}\Big[\cL_{\beta}(s)\cL_{\alpha}(s)+\cL_{\alpha}(s)\Big].
\end{align*}
Solving the second equation for $\cL_{\beta}(s)$ and substituting into the
first, we get
\begin{align*}
\cL_{\beta}(s)={-}\frac{\cL_{\alpha}(s)}{\sigma^2+\cL_{\alpha}(s)},
\qquad
\frac{\lambda + s}{\sigma^2}\mathcal{L}^2_{\alpha}(s) + \Big(\lambda + s +
\frac{\delta-1}{\sigma^2}\Big)\mathcal{L}_{\alpha}(s) - 1=0.
\end{align*}
The latter quadratic equation can be solved as
\begin{align*}
\cL_{\alpha}(s) %= \frac{\delta^{-1}(1+zm(z))}{1-\delta^{-1} - \delta^{-1}zm(z)}
=\frac{\sigma^2}{\delta}m(z)=\int\frac{1}{\lambda+s+\delta x/\sigma^2}\,\mu(\d x),
\qquad z:=z(s)=-\frac{(\lambda+s)\sigma^2}{\delta}.
\end{align*}
This then gives
\[\cL_{\beta}(s)=-\frac{\delta^{-1}m(z)}{1+\delta^{-1}m(z)}
=-\delta^{-1}(1+zm(z))
=-\frac{1}{\sigma^2}\int\frac{x}{\lambda+s+\delta x/\sigma^2}\mu(\d x).\]
Inverting these transforms yields (\ref{eq:alpha_sol}) and
(\ref{eq:beta_sol}).\footnote{These
inversions may be checked by directly computing the Laplace
transforms of (\ref{eq:alpha_sol}) and (\ref{eq:beta_sol}). Since this
identifies a solution of 
(\ref{def:response_theta})--(\ref{def:response_g}), and we are
assuming that the solution of the DMFT equations is unique, this confirms the
correctness of our posited form \eqref{eq:ansatz}; we will appeal to this type
of reasoning throughout this note.}

Lastly, (\ref{def:derivative_langevin_ostar}) can be written as
\begin{align*}
\gamma(t):=\frac{\sigma^2}{\delta}
R_\eta(t,\ast) = -\frac{1}{\sigma^2}\int_0^t \alpha(t-s)(\gamma(s)-1)\d s,
\end{align*}
taking the Laplace transform of which yields
\[\cL_\gamma(s)=-\frac{1}{\sigma^2}\cL_{\alpha}(s)\Big(\cL_\gamma(s)-\frac{1}{s}\Big).\]
Thus
\begin{align*}
\mathcal{L}_\gamma(s) &=
\frac{\cL_{\alpha}(s)}{s(\sigma^2+\mathcal{L}_{\alpha}(s))}
=\frac{\delta^{-1}m(z)}{s(1+\delta^{-1}m(z))}
=\frac{1+zm(z)}{\delta s}
=\frac{1}{\sigma^2}\left(\int \frac{x}{s(\lambda+s+\delta x/\sigma^2)}
\mu(\d x)\right),
\end{align*}
and inverting this yields (\ref{eq:gamma_sol}).
\end{proof}

Next we solve for the main iterates $\theta^t$ and $\eta^t$. 
\begin{lemma}\label{lem:theta_eta_sol}
Let
\begin{align*}
\rho^t \equiv \bigg(\frac{\delta}{\sigma^2}-R_\eta(t,\ast)\bigg)\theta^\ast + u^t.
\end{align*}
Suppose $\theta^0=0$. Then we have
\begin{align}
\theta^t &= \int_0^t \alpha(t-s)\rho^s \d s + \sqrt{2}\int_0^t
\alpha(t-s)\,\d B^s,\label{eq:thetaform}\\
\eta^t&=\gamma(t)(w^\ast + e) + \int_0^t \beta(t-s)w^s \d s + w^t.\label{eq:etaform}
\end{align}
\end{lemma}
\begin{proof}
By definition, we have
\begin{equation}\label{eq:etadef_rewrite}
\eta^t = -\frac{1}{\sigma^2} \int_0^t \alpha(t-s)(\eta^s - w^\ast - e)\d s + w^t.
\end{equation}
We posit a solution of the form
\[\eta^t=c(t)(w^*+e)+\int_0^t K(t-s)w^s\d s+w^t.\]
Substituting this form in the right side of \eqref{eq:etadef_rewrite} gives
\begin{align*}
&-\frac{1}{\sigma^2}\int_0^t \alpha(t-s)\Big[c(s)(w^\ast + e)
+\int_0^s K(s-s')w^{s'}\d s' + w^s\Big]\d s
+ \frac{1}{\sigma^2} \int_0^t \alpha(s)\d s \cdot (w^\ast + e) + w^t\\
&= -\frac{1}{\sigma^2}\int_0^t w^s \Big[\Big(\int_s^t \alpha(t-s')K(s'-s)
\d s'\Big) + \alpha(t-s)\Big]\d s + \frac{1}{\sigma^2}\Big[\int_0^t \alpha(s)\d
s - \int_0^t \alpha(t-s)c(s)\d s\Big] \cdot (w^\ast + e) + w^t.
\end{align*}
By matching the coefficients of $w^\ast + e$ and $w^s$ with those on the left
side of \eqref{eq:etadef_rewrite}, we have
\begin{align}
c(t) &=\frac{1}{\sigma^2}\int_0^t \alpha(s) \d s
-\frac{1}{\sigma^2}\int_0^t \alpha(t-s)c(s)\d s,\label{eq:c_coef}\\
K(t) &= - \frac{1}{\sigma^2}\int_0^t \alpha(t-s)K(s)\d s
-\frac{1}{\sigma^2}\alpha(t).
\end{align}
Taking the Laplace transforms on both sides and rearranging,
\begin{align*}
\cL_c(s) &= \frac{\cL_{\alpha}(s)/s}{\sigma^2 + \cL_{\alpha}(s)} = \frac{m(z)/\delta
s}{1+m(z)/\delta} = \frac{1+zm(z)}{\delta s}=\cL_{\gamma}(s)\\
\cL_K(s) &= {-}\frac{\cL_{\alpha}(s)}{\sigma^2 + \cL_{\alpha}(s)}
= -\delta^{-1}(1 + zm(z))=\cL_{\beta}(s),
\end{align*}
so $c(t)=\gamma(t)$ and $K(t)=\beta(t)$ as claimed.

Next we compute the coefficients for $\theta^t$. By definition, we have
\begin{align}
\theta^t &=-\bigg(\lambda + \frac{\delta}{\sigma^2}\bigg)\int_0^t \theta^s\d s -
\int_0^t \Big(\int_0^s \frac{\delta}{\sigma^2}\beta(s-s')\theta^{s'}\d
s'\Big)\d s + \int_0^t \rho^s\d s + \int_0^t \sqrt{2}\,\d B^s\nonumber\\
&=-\bigg(\lambda+\frac{\delta}{\sigma^2}\bigg)\int_0^t \theta^s\d s -
\frac{\delta}{\sigma^2} \int_0^t \Big(\int_0^{t-s} \beta(s')\d s'
\Big)\theta^s \d s + \int_0^t \rho^s\d s + \int_0^t \sqrt{2}\,\d B^s.
\label{eq:thetadef_rewrite}
\end{align}
We posit a solution of the form
\[\theta^t=\int_0^t A(t-s)\rho^s\d s+\sqrt{2}\int_0^t C(t-s)\,\d B^s\]
and substitute this form in the right side of \eqref{eq:thetadef_rewrite},
applying the identities
\begin{align*}
\int_0^t \int_0^s A(s-s')\rho^{s'}\d s'\d s &= \int_0^t \Big(\int_0^{t-s} A(s')\d s'\Big)\rho^s \d s,\\
\int_0^t \int_0^s C(s-s')\d B^{s'} \d s &= \int_0^t \Big(\int_0^{t-s}
C(s')\d s'\Big)\d B^s,\\
\int_0^t \Big(\int_0^{t-s} \beta(s')\d s'\Big)\Big(\int_0^s
A(s-s')\rho^{s'}\d s'\Big)\d s &= \int_0^t \rho^s \Big[\int_0^{t-s}
\Big(\int_0^{t-s-s'} \beta(s'')\d s''\Big)A(s')\d s'\Big]\d s,\\
\int_0^t \Big(\int_0^{t-s} \beta(s')\d s'\Big)\Big(\int_0^s
C(s-s')\d B^{s'}\Big)\d s &= \int_0^t \Big[\int_0^{t-s} \Big(\int_0^{t-s-s'}
\beta(s'')\d s''\Big)C(s')\d s'\Big]\d B^s.
\end{align*}
Then matching the coefficients of $\rho^s\,\d s$ and $\d B^s$ with those on the left side, we have
\begin{align*}
A(t) &= -\bigg(\lambda + \frac{\delta}{\sigma^2}\bigg)
\int_0^t A(s)\d s - \frac{\delta}{\sigma^2} \int_0^t \Big(\int_0^{t-s} \beta(s')\d s'\Big) A(s)\d s + 1,\\
C(t) &= -\bigg(\lambda + \frac{\delta}{\sigma^2}\bigg)\int_0^t C(s)\d s -
\frac{\delta}{\sigma^2} \int_0^t \Big(\int_0^{t-s} \beta(s')\d
s'\Big)C(s)\d s + 1.
\end{align*}
Thus $A(t)=C(t)$, and taking the Laplace transform gives
\[\cL_A(s)=-\bigg(\lambda+\frac{\delta}{\sigma^2}\bigg)
\frac{\cL_A(s)}{s}-\frac{\delta}{\sigma^2}\cL_A(s)\frac{\cL_{\beta}(s)}{s}
+\frac{1}{s}.\]
Solving for $\cL_A(s)$,
\begin{align*}
\cL_A(s)=\frac{\sigma^2}{(\lambda+s)\sigma^2 + \delta + \delta
\cL_{\beta}(s)}=\frac{\sigma^2}{-\delta z+ \delta - 1-zm(z)} =
\frac{\sigma^2}{\delta}m(z)=\cL_{\alpha}(s),
\end{align*}
so $A(t)=C(t)=\alpha(t)$ as claimed.
\end{proof}

Finally, we may compute an explicit form for $C_\theta(t,s)$.
\begin{lemma}
Suppose $\theta^0=0$ and $\E[{\theta^*}^2]=\tau_*^2$. Then we have
\begin{align}
C_\theta(t,\ast)&=\delta\tau_*^2\gamma(t)\label{eq:Cthetastar}\\
C_\theta(t,s)&=\frac{1}{\sigma^4}\int
\frac{\delta^2 \tau_*^2 x^2+\delta \sigma^2 x}
{(\lambda+\delta x/\sigma^2)^2}\Big(1-e^{-(\lambda+\delta x/\sigma^2)t}\Big)
\Big(1-e^{-(\lambda+\delta x/\sigma^2)s}\Big) \mu(\d x)\notag\\
&\hspace{1in}+\int \frac{1}{\lambda+\delta x/\sigma^2}\Big(e^{-(\lambda+\delta
x/\sigma^2)|t-s|}-e^{-(\lambda+\delta x/\sigma^2)(t+s)}\Big)
\mu(\d x)\label{eq:Cthetats}
\end{align}
\end{lemma}
\begin{remark}
Writing the eigendecomposition $\delta^{-1}\X^\top\X=\V\bLambda\V^\top$
with $\bLambda=\diag(x_i)_{i=1}^p$, and defining the change-of-variables
$\bxi^t=\V^\top\btheta^t$, $\bxi^\ast=\V^\top\btheta^\ast$,
$\bzeta=\frac{1}{\sigma^2}\V^\top\X^\top\y$, and $\d\W^t=\V^\top\d\B^t$,
the Langevin diffusion SDE takes the form of $p$ decoupled Ornstein-Uhlenbeck
processes
\[\xi_i^t=\Big[\zeta_i-\big(\lambda+\delta x_i/\sigma^2\big)\xi_i^t\Big]\d t
+\sqrt{2}\,\d W_i^t,\]
whose explicit solutions are
\[\xi_i^t=\frac{\zeta_i}{\lambda+\delta x_i/\sigma^2}
\Big(1-e^{-(\lambda+\delta x_i/\sigma^2)t}\Big)
+\sqrt{2}\,\int_0^t e^{-(\lambda+\delta x_i/\sigma^2)(t-u)}\,\d W_i^u.\]
From this, the above expressions for $C_\theta(t,\ast)=\lim_{n,p \to
\infty} p^{-1}{\bxi^t}^\top \bxi^\ast$
and $C_\theta(t,s)=\lim_{n,p \to \infty} p^{-1}{\bxi^t}^\top \bxi^s$ may
be easily deduced. The proof below verifies that these forms of
$C_\theta(t,\ast)$ and $C_\theta(t,s)$ are consistent with a calculation from
the DMFT equations.

From here we may also compute $C_\eta(t,s)$ as
\begin{align}\label{def:C_eta}
\notag C_\eta(t,s) &= \frac{\delta}{\sigma^4}\lim_{n,p} \frac{1}{n}\iprod{\X\btheta^t - \y}{\X\btheta^s - \y}\\
&= \frac{1}{\sigma^4} \lim_{n,p} \frac{1}{p}\iprod{\X(\btheta^t - \btheta^\ast)}{\X(\btheta^s - \btheta^\ast)} - \frac{1}{\sigma^4} \lim_{n,p} \frac{1}{p}\iprod{\X(\btheta^t - \btheta^\ast)}{\z} - \frac{1}{\sigma^4} \lim_{n,p} \frac{1}{p}\iprod{\X(\btheta^s - \btheta^\ast)}{\z} + \frac{\delta}{\sigma^2},
\end{align}
where
\begin{align*}
\lim_{n,p} \frac{1}{p}\iprod{\X(\btheta^t - \btheta^\ast)}{\X(\btheta^s - \btheta^\ast)} &= \frac{1}{\sigma^4}\int \frac{\delta^3\tau_\ast^2x^3 + \delta^2\sigma^2x^2}{(\lambda + \delta x/\sigma^2)^2}\Big(1-e^{-(\lambda + \delta x/\sigma^2)t}\Big)\Big(1-e^{-(\lambda + \delta x/\sigma^2)s}\Big)\mu(\d x)\\
&\quad + \int \frac{\delta x}{\lambda + \delta x/\sigma^2}\Big(e^{-(\lambda + \delta x/\sigma^2)|t-s|} - e^{-(\lambda + \delta x/\sigma^2)(t+s)}\Big)\mu(\d x)\\
&\quad - \frac{1}{\sigma^2}\int \frac{\delta^2x^2\tau_\ast^2}{\lambda + \delta x/\sigma^2}\Big(1-e^{-(\lambda + \delta x/\sigma^2)t}\Big)\mu(\d x)\\
&\quad - \frac{1}{\sigma^2}\int \frac{\delta^2x^2\tau_\ast^2}{\lambda + \delta x/\sigma^2}\Big(1-e^{-(\lambda + \delta x/\sigma^2)s}\Big)\mu(\d x) + \delta \tau_\ast^2,
\end{align*}
and
\begin{align*}
\lim_{n,p} \frac{1}{p}\iprod{\X(\btheta^t - \btheta^\ast)}{\z} = \int \frac{\delta x}{\lambda + \delta x/\sigma^2}\Big(1-e^{-(\lambda + \delta x/\sigma^2)t}\Big)\mu(\d x).
\end{align*}
Consequently, in the correctly specified case $\lambda = 1/\tau_\ast^2$, for any fixed $r$,  
\begin{align*}
C^\infty_\eta(r)\equiv \lim_{t\rightarrow\infty} C_\eta(t+r,t) = \frac{1}{\sigma^4}\int \frac{\delta x}{\lambda + \delta x/\sigma^2}\Big(e^{-(\lambda + \delta x/\sigma^2)|r|} - 1\Big)\mu(\d x) + \frac{\delta}{\sigma^2},
\end{align*}
with $C^\infty_\eta(0) = \delta/\sigma^2$. Also note that for $r\geq 0$, $C^\infty_\eta(r) = -\frac{\delta}{\sigma^2}(\gamma(r)-1)$.
\end{remark}
\begin{proof}
Applying independence of $\theta^\ast$ with $\{u^t\}_{t \geq 0}$ and $\{B^t\}_{t
\geq 0}$,
the expression for $\theta^t$ in Lemma \ref{lem:theta_eta_sol} yields
\begin{align*}
C_\theta(t,\ast)=\E[\theta^t\theta^\ast]=\tau_*^2\int_0^t \alpha(t-t')
\bigg(\frac{\delta}{\sigma^2}-R_\eta(t',*)\bigg)\d t'.
\end{align*}
Setting as before $z=z(s)=-(\lambda+s)\sigma^2/\delta$ and
taking Laplace transforms,
\[\cL_{C_\theta^*}(s)=\frac{\delta\tau_*^2}{\sigma^2}
\cL_\alpha(s)\bigg(\frac{1}{s}-\cL_\gamma(s)\bigg)
=\tau_*^2 m(z)\bigg(\frac{1}{s}-\frac{1+zm(z)}{\delta s}\bigg)
=\tau_*^2\,\frac{1+zm(z)}{s}=\delta\tau_*^2\cL_\gamma(s).\]
Hence $C_\theta(t,\ast)=\delta\tau_*^2\gamma(t)$.

Applying independence of $\theta^\ast$, $\{u^t\}_{t \geq 0}$, and $\{B^t\}_{t
\geq 0}$, where $\E[u^tu^s]=C_\eta(t,s)$, the expression for $\theta^t$
in Lemma \ref{lem:theta_eta_sol} yields also
\begin{align*}
C_\theta(t,s)&=\E[\theta^t\theta^s]
=\tau_*^2\int_0^t \d t'\,
\alpha(t-t')\bigg(\frac{\delta}{\sigma^2}-R_\eta(t',*)\bigg)
\cdot \int_0^s \d s'\,
\alpha(s-s')\bigg(\frac{\delta}{\sigma^2}-R_\eta(s',*)\bigg)\\
&\hspace{1in}+\int_0^t \d t'\int_0^s \d s'\alpha(t-t')\alpha(s-s')C_\eta(t',s')
+2\int_0^{t \wedge s} \d r\,\alpha(t-r)\alpha(s-r)\\
&=\delta^2\tau_*^2\gamma(t)\gamma(s)
+\int_0^t \d t'\int_0^s \d s'\alpha(t-t')\alpha(s-s')C_\eta(t',s')
+2\int_0^{t \wedge s} \d r\,\alpha(t-r)\alpha(s-r).
\end{align*}
Let $\cL_x(a,b)=\int_0^\infty \int_0^\infty \d t\d s\,e^{-at-bs} x(t,s)$ be the
bivariate Laplace transform of $x(t,s)$. For any $f:\R \to \R$, observe that
\begin{equation}\label{eq:LaplaceBrownianterm}
\int_0^\infty \!\!\!\int_0^\infty \d t \d s\,e^{-at-bs}
\int_0^{t \wedge s} \d r\,f(t-r)f(s-r)
=\int_0^\infty\d r\int_0^\infty \!\!\! \int_0^\infty \d t \d s\,
f(t)f(s)e^{-at-bs-(a+b)r}
=\frac{\cL_f(a)\cL_f(b)}{a+b}.
\end{equation}
Then, applying this with $f(\cdot)=\alpha(\cdot)$, we have
\begin{equation}\label{eq:Cthetalaplace}
\cL_{C_\theta}(a,b)=\delta^2\tau_*^2\cL_\gamma(a)\cL_\gamma(b)
+\cL_\alpha(a)\cL_\alpha(b)\cL_{C_\eta}(a,b)+\frac{2}{a+b}
\cL_\alpha(a)\cL_\alpha(b).
\end{equation}

Applying independence of $e$ with $(w^*,\{w^t\}_{t \geq 0})$, where
$\E[w^tw^s]=C_\theta(t,s)$ and $\E[w^tw^*]=C_\theta(t,*)$ and
$\E[{w^*}^2]=\tau_*^2$, 
the expression for $\eta^t$ in Lemma \ref{lem:theta_eta_sol} yields 
\begin{align*}
C_\eta(t,s)&=\frac{\delta}{\sigma^4}\E[(\eta^t-w^*-e)(\eta^s-w^*-e)]\\
&=\frac{\delta}{\sigma^4}\Bigg[(\gamma(t)-1)(\gamma(s)-1)(\tau_*^2+\sigma^2)
+(\gamma(t)-1)\bigg(\int_0^s \d s'\,
\beta(s-s')C_\theta(s',\ast)+C_\theta(s,\ast)\bigg)\\
&\hspace{0.5in}+(\gamma(s)-1)\bigg(\int_0^t \d t'\,
\beta(t-t')C_\theta(t',\ast)+C_\theta(t,\ast)\bigg)
+\int_0^t \d t' \int_0^s \d s'\, \beta(t-t')\beta(s-s')C_\theta(t',s')\\
&\hspace{0.5in}+\int_0^t \d t'\,\beta(t-t')C_\theta(t',s)
+\int_0^s \d s'\,\beta(s-s')C_\theta(t,s')+C_\theta(t,s)\Bigg].
\end{align*}
Taking the bivariate Laplace transform and using
$\cL_{C_\theta^*}=\delta\tau_*^2 \cL_\gamma$ from above,
\begin{align*}
\cL_{C_\eta}(a,b)&=\frac{\delta}{\sigma^4}\Bigg[(\tau_*^2+\sigma^2)
\Big(\cL_\gamma(a)-\frac{1}{a}\Big)\Big(\cL_\gamma(b)-\frac{1}{b}\Big)
+\delta\tau_*^2\Big(\cL_\gamma(a)-\frac{1}{a}\Big)\Big(\cL_\beta(b)+1\Big)\cL_\gamma(b)\\
&\hspace{1in}
+\delta\tau_*^2\Big(\cL_\gamma(b)-\frac{1}{b}\Big)\Big(\cL_\beta(a)+1\Big)\cL_\gamma(a)
+\Big(\cL_\beta(a)+1\Big)\Big(\cL_\beta(b)+1\Big)\cL_{C_\theta}(a,b)\Bigg].
\end{align*}
We recall that for $z=z(s)=-(\lambda+s)\sigma^2/\delta$, we have
\begin{align*}
\cL_\alpha(s)&=\frac{\sigma^2}{\delta}m(z)\\
\cL_\beta(s)+1&=1-\delta^{-1}(1+zm(z))=\frac{1+zm(z)}{m(z)}
={-}\frac{\delta\cL_\beta(s)}{m(z)}\\
\cL_\gamma(s)-\frac{1}{s}&=\frac{1+zm(z)}{\delta s}-\frac{1}{s}
={-}\frac{1+zm(z)}{sm(z)}={-}\frac{\delta \cL_\gamma(s)}{m(z)}
\end{align*}
Hence
\begin{align*}
\cL_\alpha(a)\cL_\alpha(b)\cL_{C_\eta}(a,b)
&=\delta\Big[\cL_\gamma(a)\cL_\gamma(b)\Big(\tau_*^2+\sigma^2+\delta\tau_*^2\cL_\beta(a)+\delta\tau_*^2\cL_\beta(b)\Big)+\cL_\beta(a)\cL_\beta(b)\cL_{C_\theta}(a,b)\Big]
\end{align*}
Substituting this into \eqref{eq:Cthetalaplace} and solving for
$\cL_{C_\theta}(a,b)$,
\begin{equation}\label{eq:LCthetaclosed}
\cL_{C_\theta}(a,b)
=\frac{\delta\cL_\gamma(a)\cL_\gamma(b)(\tau_*^2[1+\delta+\delta\cL_\beta(a)+\delta\cL_\beta(b)]+\sigma^2)
+2\cL_\alpha(a)\cL_\alpha(b)/(a+b)}{1-\delta \cL_\beta(a)\cL_\beta(b)}.
\end{equation}

Introduce the shorthands $z_a=z(a)$, $z_b=z(b)$, $m_a=m(z(a))$, and
$m_b=m(z(b))$. We now verify the three relations
\begin{align}
\frac{\cL_\alpha(a)\cL_\alpha(b)}{1-\delta \cL_\beta(a)\cL_\beta(b)}
&=\frac{\sigma^4}{\delta^2}\int \frac{1}{(x-z_a)(x-z_b)}\mu(\d x),
\label{eq:MPrelation1}\\
\frac{\cL_\gamma(a)\cL_\gamma(b)}{1-\delta \cL_\beta(a)\cL_\beta(b)}
&=\frac{1}{\delta^2 ab}\int \frac{x}{(x-z_a)(x-z_b)}\mu(\d
x),\label{eq:MPrelation2}\\
\frac{\cL_\gamma(a)\cL_\gamma(b)[1+\delta+\delta\cL_\beta(a)
+\delta\cL_\beta(b)]}{1-\delta \cL_\beta(a)\cL_\beta(b)}
&=\frac{1}{\delta ab}\int \frac{x^2}{(x-z_a)(x-z_b)}
\mu(\d x).\label{eq:MPrelation3}
\end{align}
Observe first that for any $k \geq 0$, by the identity
$\delta^{-1} zm(z)^2=m(z)-\delta^{-1}m(z)-zm(z)-1$, we have
\begin{align}
[1-\delta \cL_\beta(a)\cL_\beta(b)]z_a^km_a
&=\Big[1-\delta^{-1}(1+z_am_a)(1+z_bm_b)\Big]z_a^km_a\notag\\
&=z_a^km_a-(\delta^{-1}z_a^km_a+z_a^k
\cdot \delta^{-1}z_am_a^2)(1+z_bm_b)\notag\\
&=z_a^k(1+z_am_a)(1+z_bm_b)-z_a^km_az_bm_b.\label{eq:Laplaceinversiontmp}
\end{align}
Thus
\begin{equation}\label{eq:Laplaceinversionidentity}
[1-\delta \cL_\beta(a)\cL_\beta(b)](z_a^km_a-z_b^km_b)
=(z_a^k-z_b^k)(1+z_am_a)(1+z_bm_b)-(z_a^{k-1}-z_b^{k-1})z_am_az_bm_b.
\end{equation}
Applying this with $k=0$,
\begin{align*}
[1-\delta \cL_\beta(a)\cL_\beta(b)]
\int \frac{1}{(x-z_a)(x-z_b)}\mu(\d x)
&=\frac{1-\delta \cL_\beta(a)\cL_\beta(b)}{z_a-z_b}
\int \bigg(\frac{1}{x-z_a}-\frac{1}{x-z_b}\bigg)\mu(\d x)\\
&=\frac{[1-\delta \cL_\beta(a)\cL_\beta(b)](m_a-m_b)}{z_a-z_b}\\
&=\frac{m_am_b(z_a-z_b)}{z_a-z_b}
=\frac{\delta^2}{\sigma^4}\cL_\alpha(a)\cL_\alpha(b),
\end{align*}
which shows \eqref{eq:MPrelation1}. Similarly, applying
\eqref{eq:Laplaceinversionidentity} with $k=1$,
\begin{align*}
[1-\delta \cL_\beta(a)\cL_\beta(b)]
\int \frac{x}{(x-z_a)(x-z_b)}\mu(\d x)
&=\frac{1-\delta \cL_\beta(a)\cL_\beta(b)}{z_a-z_b}
\int \bigg(\Big(1+\frac{z_a}{x-z_a}\Big)
-\Big(1+\frac{z_b}{x-z_b}\Big)\bigg)\mu(\d x)\\
&=\frac{[1-\delta \cL_\beta(a)\cL_\beta(b)](z_am_a-z_bm_b)}{z_a-z_b}\\
&=\frac{(z_a-z_b)(1+z_am_a)(1+z_bm_b)}{z_a-z_b}
=\delta^2ab\cL_\gamma(a)\cL_\gamma(b),
\end{align*}
which shows \eqref{eq:MPrelation2}. Finally, applying
\eqref{eq:Laplaceinversionidentity} with $k=2$,
\begin{align*}
&[1-\delta \cL_\beta(a)\cL_\beta(b)]
\int \frac{x^2}{(x-z_a)(x-z_b)}\mu(\d x)\\
&=\frac{1-\delta \cL_\beta(a)\cL_\beta(b)}{z_a-z_b}
\int \bigg(\Big(x+z_a+\frac{z_a^2}{x-z_a}\Big)
-\Big(x+z_b+\frac{z_b^2}{x-z_b}\Big)\bigg)\mu(\d x)\\
&=\frac{[1-\delta \cL_\beta(a)\cL_\beta(b)](z_a-z_b+z_a^2m_a-z_b^2m_b)}{z_a-z_b}\\
&=1-\delta\cL_\beta(a)\cL_\beta(b)+
\frac{(z_a^2-z_b^2)(1+z_am_a)(1+z_bm_b)-(z_a-z_b)z_am_az_bm_b}{z_a-z_b}\\
&=1-\delta^{-1}(1+z_am_a)(1+z_bm_b)
+(z_a+z_b)(1+z_am_a)(1+z_bm_b)-z_am_az_bm_b\\
&\overset{(*)}{=}
\delta^{-1}(1+z_am_a)(1+z_bm_b)[1+\delta-(1+z_am_a)-(1+z_bm_b)]\\
&=\delta ab\cL_\gamma(a)\cL_\gamma(b)[1+\delta+\delta \cL_\beta(a)+\delta
\cL_\beta(b)],
\end{align*}
where the step $(*)$ applies
the following consequence of \eqref{eq:Laplaceinversiontmp} (with $k=1$)
\[\delta^{-1}(1+z_am_a)(1+z_bm_b)(z_am_a+z_bm_b)
=z_am_a+z_bm_b-(z_a+z_b)(1+z_am_a)(1+z_bm_b)+2z_am_az_bm_b\]
together with some algebraic simplification. This shows \eqref{eq:MPrelation3}.

Now applying \eqref{eq:MPrelation1}--\eqref{eq:MPrelation3} into
\eqref{eq:LCthetaclosed}, we get
\begin{align*}
\cL_{C_\theta}(a,b)
&=\int \bigg(\frac{\tau_*^2x^2+(\sigma^2/\delta)x}{ab(x-z_a)(x-z_b)}
+\frac{2\sigma^4}{\delta^2(a+b)} \cdot \frac{1}{(x-z_a)(x-z_b)}\bigg)\mu(\d x)\\
&=\frac{1}{\sigma^4}\int \frac{\delta^2\tau_*^2x^2+\delta\sigma^2 x}
{ab(\lambda+a+\delta x/\sigma^2)(\lambda+b+\delta x/\sigma^2)}
\mu(\d x)
+\frac{2}{a+b}\int\frac{1}{(\lambda+a+\delta x/\sigma^2)(\lambda+b+\delta
x/\sigma^2)}\mu(\d x).
\end{align*}
Laplace inversion of this first term gives the first term of
\eqref{eq:Cthetats}, while Laplace inversion of this second term using
\eqref{eq:LaplaceBrownianterm} gives
\begin{equation}\label{eq:LaplaceInvII}
2\int\bigg(\int_0^{t \wedge s} \d r e^{-(\lambda+\delta x/\sigma^2)(t-r)}
e^{-(\lambda+\delta x/\sigma^2)(s-r)}\bigg)\mu(\d x).
\end{equation}
Substituting the explicit form
\[\int_0^{t \wedge s} \d r e^{2(\lambda+\delta x/\sigma^2)r}
=\frac{1}{2(\lambda+\delta x/\sigma^2)}\Big(e^{2(\lambda+\delta x/\sigma^2)(t
\wedge s)}-1\Big)\]
shows that \eqref{eq:LaplaceInvII} is equal to the second term
of \eqref{eq:Cthetats}, concluding the proof.
\end{proof}




==> fixedprior.tex <==
\section{Analysis of dynamics under a fixed prior}

Let us fix the prior density $g(\cdot)$ and the data $(\X,\y)$, and write
for convenience
\begin{equation}\label{eq:qshorthand}
q(\btheta)=\sP_g(\btheta \mid \X,\y)
\propto \exp\bigg({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+\sum_{j=1}^d \log g(\theta_j)\bigg)
\end{equation}
for the posterior density. The Langevin diffusion (\ref{eq:langevin_sde}) is
then
\begin{equation}\label{eq:langevin_fixedq}
\d \btheta^t=\nabla \log q(\btheta^t)+\sqrt{2}\,\d\b^t,
\end{equation}
corresponding to the $K=0$ case of (\ref{eq:joint_sde}).
We remind the reader of our notations
\begin{align*}
\langle f(\btheta) \rangle&=\E_{\btheta \sim q}[f(\btheta)]\\
\langle f(\btheta^t) \rangle&=\E[f(\btheta^t) \mid \X,\y,\btheta^0]
\end{align*}
where $\{\btheta^t\}_{t \geq 0}$ is the solution of (\ref{eq:langevin_fixedq})
with a given initial condition $\btheta^0$. To make explicit the dependence on
this initial condition, we will denote as in Section \ref{sec:response}
\[P_tf(\btheta)=\langle f(\btheta^t) \rangle_{\btheta^0=\btheta}
=\E[f(\btheta^t) \mid \X,\y,\btheta^0=\btheta].\]
We define the corresponding infinitesimal generator 
\[\L f(\btheta)=\nabla \log q(\btheta)^\top \nabla f(\btheta)+\Tr \nabla^2
f(\btheta).\]

\subsection{Additional properties of Langevin diffusion with fixed prior}

For a fixed prior $g(\cdot)$, the diffusion
(\ref{eq:langevin_fixedq}) is elliptic with stationary law given by
$q(\btheta)$. We establish a Bismut-Elworthy-Li formula for the
derivative of the semigroup and a fluctuation-dissipation relation for the
response function in this setting.

The following is a version of the Bismut-Elworthy-Li formula
\cite{bismut1984large,elworthy1994formulae} adapted to our class $\cA$ of
functions with bounded first and second derivatives; for completeness, we give
a proof following \cite[Theorem 2.1]{elworthy1994formulae}.

\begin{lemma}\label{lemma:BEL}
Suppose Assumptions \ref{assump:prior} holds with a fixed prior $g(\cdot)$.
Fix any $\btheta \in \R^d$ and consider the joint diffusion of
$(\btheta^t,\V^t) \in \R^d \times \R^{d \times d}$ given by
\begin{equation}\label{eq:matrixV_sde}
\d\btheta^t=\nabla \log q(\btheta^t)\d t+\sqrt{2}\,\d \b^t,
\qquad \d\V^t=[\nabla^2 \log q(\btheta^t)]\V^t
\end{equation}
with initial condition $(\btheta^0,\V^0)=(\btheta,\I)$. Then for any
$f \in \cA$ and any $t>0$,
\begin{align}
\nabla P_t f(\btheta)&=\langle \V^{t\top}\,\nabla f(\btheta^t)
\rangle\label{eq:BEL1}\\
&=\frac{1}{t\sqrt{2}}\bigg\langle f(\btheta^t)\int_0^t {\V^s}^\top \d\b^s
\bigg\rangle
\label{eq:BEL2}
\end{align}
\end{lemma}
\begin{proof}
The rows of $\V^t$ are the vectors $\v_i^t$ of (\ref{eq:firstsecondvar}),
specialized to $K=0$.
Then (\ref{eq:BEL1}) is the first identity of (\ref{eq:Ptspaceder}).
By Proposition \ref{prop:langevinsolution}(c),
$(s,\btheta) \mapsto P_{t-s}f(\btheta)$ belongs to
$C^{1,2}([0,t] \times \R^d)$, and $\partial_s P_{t-s}f(\btheta)={-}\L
P_{t-s}f(\btheta)$. Then It\^o's formula applied to $P_{t-s}f(\btheta^s)$ gives
\begin{align*}
f(\btheta^t)&=P_t f(\btheta)
+\int_0^t (\partial_s+\L)P_{t-s}f(\btheta^s)\d s
+\sqrt{2}\int_0^t \nabla P_{t-s}f(\btheta^s)^\top \d\b^s\\
&=P_t f(\btheta)+\sqrt{2}\int_0^t \nabla P_{t-s}f(\btheta^s)^\top \d\b^s.
\end{align*}
Here $\{\V^s\}_{s \in [0,t]}$ is bounded (c.f.\ Proposition
\ref{prop:langevinsolution}(b)) and adapted to the canonical filtration of
$\{\b^s\}$, so $\int_0^t {\V^s}^\top \d\b^s$ is a martingale. Then multiplying
both sides by $\int_0^t \V^{s\top} \d\b^s$ and taking expectations gives
\[\bigg\langle f(\btheta^t)\int_0^t {\V^s}^\top \d\b^s\bigg\rangle
=\sqrt{2}\int_0^t \big\langle {\V^s}^\top \nabla P_{t-s}f(\btheta^s)\big\rangle\d s.\]
Proposition \ref{prop:langevinsolution}(c) guarantees
$P_{t-s} f \in \cA$, so applying (\ref{eq:BEL1}) with $P_{t-s}f$ in place of
$f$,
\[\int_0^t \big\langle {\V^s}^\top \nabla P_{t-s}f(\btheta^s)\big\rangle\d s
=\int_0^t \nabla P_s(P_{t-s}f)(\btheta)\d s
=t \cdot \nabla P_t f(\btheta).\]
Substituting above and rearranging shows (\ref{eq:BEL2}).
\end{proof}

We recall the form of the response function
\begin{equation}\label{eq:responsenonadaptive}
R_{AB}(t,s)=P_s(\nabla B^\top \nabla
P_{t-s}A)(\btheta)=\langle (\nabla B^\top \nabla
P_{t-s}A)(\btheta^s) \rangle_{\btheta^0=\btheta}
\end{equation}
of Proposition \ref{prop:responseexists} given by (\ref{eq:explicitresponse})
specialized to $K=0$. The following is a version of the
fluctuation-dissipation theorem, relating this response to the
correlation function under an initialization from the
stationary law $q(\btheta)$.

\begin{lemma}\label{eq:langevin_fdt_equi}
Suppose Assumption \ref{assump:prior} holds with a fixed prior $g(\cdot)$.
Let $\{\btheta^t\}_{t \geq 0}$ be the solution of (\ref{eq:langevin_sde})
with initial condition $\btheta^0=\btheta \in \R^d$. For $A \in \cA$ and
$B:\R^{d+K} \to \R$ such that each $\partial_{\theta_j} B \in \cB$,
let $R_{AB}(t,s)[\btheta]=\langle (\nabla B^\top \nabla
P_{t-s}A)(\btheta^s) \rangle_{\btheta^0=\btheta}$
and $C_{AB}(t,s)[\btheta]=\langle A(\btheta^t)B(\btheta^s)
\rangle_{\btheta^0=\btheta}$, viewed as functions of the initial condition
$\btheta$. Then for any $t \geq s \geq 0$, averaging over an initial condition
$\btheta \sim q$ drawn from the posterior law (\ref{eq:qshorthand}),
\[\partial_t \E_{\btheta \sim q} C_{AB}(t,s)[\btheta]={-}\E_{\btheta \sim q}
R_{AB}(t,s)[\btheta].\]
\end{lemma}
\begin{proof}
Since $q$ is stationary under (\ref{eq:langevin_fixedq}),
$\E_{\btheta \sim q} C_{AB}(t,s)[\btheta]
=\E_{\btheta \sim q} \langle A(\btheta^{t-s})B(\btheta)
\rangle_{\btheta^0=\btheta}=\E_{\btheta \sim q} (B \cdot P_{t-s}A)[\btheta]$.
Proposition \ref{prop:langevinsolution}(c) shows 
$\nabla P_tA,\nabla^2 P_tA$ are uniformly bounded, and $\nabla B,\nabla \log q$
are Lipschitz under Assumption \ref{assump:prior} and the given condition
$\partial_{\theta_j} B \in \cB$.
Since $q$ has finite moments of all orders under Assumption \ref{assump:prior},
this implies $(B \cdot \L P_t A)[\btheta]$ is uniformly integrable
over $t \in [0,T]$ with respect to $\btheta \sim q$.
Then, applying $\partial_t P_t A=\L P_t A$
by Proposition \ref{prop:langevinsolution}(c), we have
\begin{align*}
\partial_t \E_{\btheta \sim q} C_{AB}(t,s)[\btheta]
=\partial_t \E_{\btheta \sim q} (B \cdot P_{t-s}A)[\btheta]
=\E_{\btheta \sim q}(B \cdot \L P_{t-s} A)[\btheta].
\end{align*}
On the other hand, we have by integration-by-parts
\begin{align*}
\E_{\btheta \sim q} R_{AB}(t,s)&=\E_{\btheta \sim q}(\nabla B^\top \nabla
P_{t-s}A)[\btheta] =
\int q(\btheta)(\nabla B^\top \nabla P_{t-s}A)[\btheta] = -\int B(\btheta)
\sum_{j=1}^d \partial_j [q\,\nabla(P_{t-s} A)](\btheta)\\
&= -\int B(\btheta)\,\big[q\,\Tr \nabla^2(P_{t-s} A) + \nabla (P_{t-s} A)^\top
\nabla q\big](\btheta) = -\E_{\btheta \sim q}(B \cdot \L P_{t-s} A)[\btheta].
\end{align*}
(This integration-by-parts is justified since both
$\nabla B^\top \nabla P_{t-s}A$ and $B \cdot \L P_{t-s}A$ are integrable
under $q$.)
\end{proof}

\subsection{Replica fixed-point predictions (Theorem \ref{thm:dmft_equilibrium})}

\subsubsection{Analysis of $\theta$-equation}

Let $M$ be some positive integer and $T_0, T \in \R_+$ to be chosen later. For a given $M$, define sequence $\{a_i\}_{i=1}^M = \{a_i^{(M)}\}_{i=0}^M$ as
\begin{align}\label{eq:a_grid}
a_0 = \iota, \quad a_M = \sqrt{M}, \quad a_i = a_0 + i\cdot \frac{a_M - a_0}{M}, \quad 1\leq i\leq M-1,
\end{align}
 and $\{c_i\}_{i=1}^M = \{c_i^{(M)}\}_{i=1}^M$ as $\frac{c_i^2}{a_i} = \mu_\eta([a_{i-1}, a_i))$. With $U(\theta,\theta^\ast) = -\frac{\delta}{\sigma^2}(\theta - \theta^\ast) + (\log g)'(\theta)$, recall that the DMFT process is
 \begin{align}\label{eq:dmft_theta}
 \d\theta^t = \Big[U(\theta^t,\theta^\ast) - \int_0^t R_\eta(t,s)(\theta^s - \theta^\ast) \d s + u^t\Big]\d t + \sqrt{2}\d B^t,
 \end{align}
 with initialization $\theta^0$.  
 \begin{assumption}\label{assump:prior_cvx_infty}
 Let
 \begin{align}\label{eq:cvx_infty}
 \kappa(r) := \inf\{-\frac{(\theta^1 - \theta^2)((\log g)'(\theta_1) - (\log g)'(\theta_2))}{(\theta^1-\theta^2)^2}: |\theta^1 - \theta^2| = r\}.
 \end{align}
 Suppose that $\kappa(r) > -K$ for all $r\geq 0$ and $\kappa(r) \geq 0$ for $r\geq R$. 
 \end{assumption}
 
 \textbf{Step 1: Construction of auxiliary process}
 \begin{lemma}\label{lem:auxiliary_V}
 For any fixed positive integer $M$, consider the following process on $[0,T_0+T]$:
  \begin{align}\label{eq:auxiliary_theta}
\d\tilde{\theta}^t_{(M)} &=
\begin{cases}
\Big[U(\tilde{\theta}^t_{(M)},\theta^\ast) - \int_0^t R_\eta(t,s)(\tilde{\theta}^s_{(M)} - \theta^\ast)\d s + u^t\Big] \d t + \sqrt{2}\d \tilde{B}^t, & 0\leq t\leq T_0,\\
[U(\tilde{\theta}^t_{(M)},\theta^\ast) + z - \sum_{m=1}^M c_m \tilde{V}^t_m] + \sqrt{2} \d \tilde{B}^t, & T_0\leq t\leq T_0 + T,
\end{cases},\\
\d \tilde{V}^t_m &= -[a_m \tilde{V}^t_m + c_m(\tilde{\theta}^t_{(M)} - \theta^\ast)]\d t + \sqrt{2} \d \tilde{B}^t_m, \quad 1\leq m\leq M, \quad t\in [0,T_0+T].
 \end{align}
%For any positive integer $M$, consider the joint process
% \begin{align}\label{eq:auxiliary_joint}
% \d \tilde{\theta}^t_{(M)} &= [U(\tilde{\theta}^t_{(M)},\theta^\ast) + z - \sum_{m=1}^M c_m V^t_m] + \sqrt{2} \d B^t,\\
% \d V^t_m &= -[a_m V^t_m + c_m(\tilde{\theta}^t_{(M)} - \theta^\ast)]\d t + \sqrt{2} \d B^t_m, \quad 1\leq m\leq M, 
% \end{align}
 where: (1) initialization is $\tilde{\theta}^0_{(M)} = \theta^0$ and $\tilde{V}^0_m = 0$ for $1\leq m\leq M$; (2) $\{u^t\}$ is a Gaussian process with the same covariance structure as in (\ref{eq:dmft_theta}); (3) $\{\tilde{B}^t\}$ and $\{\tilde{B}^t_m\}$, $1\leq m\leq M$ are independent standard Brownian motions; (4) $\theta^\ast\sim g^\ast$ is independent of $z\sim \N(0, c_\eta(\infty))$, and they are independent of $\{u^t\}$, $\{\tilde{B}^t\}$, and $\{\tilde{B}^t_m\}$. %Then the joint law of $(\tilde{\theta}^t_{(M)}, \theta^\ast)$ in (\ref{eq:auxiliary_joint}) is the same as that in (\ref{eq:auxiliary_theta}) for $t\in[T_0,T_0+T]$. 

Then for any $T_0, T > 0$, it holds that
 \begin{align*}
 \sup_{t\in[0,T_0+T]} W_1(\cL(\theta^t,\theta^\ast), \cL(\tilde{\theta}^t_{(M)},\theta^\ast)) \leq Ce^{-cT_0}T^{3/2} + \delta(M),
 \end{align*}
for some $\delta(M) \rightarrow 0$ as $M\rightarrow\infty$.
 \end{lemma}
 \begin{proof}
 Let us shorthand $\tilde{\theta}^t_{(M)}$ as $\tilde{\theta}^t$ and construct a coupling of $(\{\theta^t\}, \theta^\ast)$ and $(\{\tilde{\theta}^t,\theta^\ast\})$. First note that, for any realization of $\{\tilde{B}^t_m\}$, $\tilde{V}^t_m$ can be explicitly solved as
 \begin{align}\label{eq:V_sol}
 \tilde{V}^t_m = -c_m\int_0^t e^{-a_m(t-s)}(\tilde{\theta}^s - \theta^\ast)\d s + \sqrt{2}\int_0^t e^{-a_m(t-s)}\d \tilde{B}^s_m,
 \end{align}
 hence with $\tilde{u}^t := z - \sqrt{2}\sum_{m=1}^M c_m\int_0^t e^{-a_m(t-s)}\d \tilde{B}^s_m$, we have for $t\in [T_0,T_0+T]$
 \begin{align*}
 \d \tilde{\theta}^t &= \Big[U(\tilde{\theta}^t,\theta^\ast) + \sum_{m=1}^M c_m^2\int_0^t e^{-a_m(t-s)}(\tilde{\theta}^s - \theta^\ast)\d s + \tilde{u}^t\Big]\d t + \sqrt{2} \d \tilde{B}^t.
 \end{align*}
Let $\tilde{R}_\eta^{(M)}(t,s) = -\sum_{m=1}^M c_m^2e^{-a_m(t-s)}$, then $\{\tilde{\theta}^t\}$ can be coupled as as
 \begin{align}\label{eq:auxiliary_theta}
\d\tilde{\theta}^t =
\begin{cases}
\Big[U(\tilde{\theta}^t,\theta^\ast) - \int_0^t R_\eta(t,s)(\tilde{\theta}^s - \theta^\ast)\d s + u^t\Big] \d t + \sqrt{2}\d \tilde{B}^t, & 0\leq t\leq T_0,\\
\Big[U(\tilde{\theta}^t,\theta^\ast) - \int_0^t \tilde{R}^{(M)}_\eta(t,s)(\tilde{\theta}^s - \theta^\ast)\d s + \tilde{u}^t\Big] \d t + \sqrt{2}\d \tilde{B}^t, & T_0\leq t\leq T_0 + T,
\end{cases}
 \end{align}
 where:
 \begin{itemize}
 \item $\theta^\ast$ is the same in (\ref{eq:dmft_theta}) and (\ref{eq:auxiliary_theta});
 \item the Brownian motion $\{\tilde{B}^t\}_{t\in [T_0,T_0+T]}$ is defined by $B^t$ for $t\in[0,T_0]$ and $2B^{T_0} - B^t$ for $t\in[T_0,T_0+T]$ so that $\d\tilde{B}^t = -\d B^t$ for $t\in [T_0,T_0+T]$;
 \item since $\{\tilde{u}^t\}_{t\in[T_0,T_0+T]}$ has covariance $\E[\tilde{u}^t\tilde{u}^s] = \sum_{m=1}^M \frac{c_m^2}{a_m}(e^{-a_m|t-s|} - e^{-a_m(t+s)}) + c_\eta(\infty)$, we choose $(\{u^t\}_{t\in[T_0,T_0+T]}, \{\tilde{u}^t\}_{t\in[T_0,T_0+T]})$ as the coupling given by Lemma \ref{lem:GP_couple}, and conditioning on $\{u^t\}_{t\in[T_0,T_0+T]}$, $\{u^t\}_{t\in [0,T_0]}$ is the same in  (\ref{eq:dmft_theta}) and (\ref{eq:auxiliary_theta}) and is generated from the associated conditional distribution of the joint Gaussian process law $\{u^t\}_{t\in[0,T_0+T]}$.
 \end{itemize}
 
 By construction, we have $\theta^t = \tilde{\theta}^t$ for $t\in [0,T_0]$. We will now bound $\sup_{t\in[T_0,T_0+T]} \E|\theta^t-\tilde{\theta}^t|$.
% \end{proof}
% 
% 
%  \begin{lemma}\label{lem:dmft_replica_compare_1}
% Consider the following joint process of $\{\tilde{\theta}^t_{(M)}, (V^t_m)_{1\leq m\leq M}\}$ for $t\in[0,T_0+T]$:
% \begin{align}\label{eq:auxiliary_theta}
%\d\tilde{\theta}^t_{(M)} =
%\begin{cases}
%\Big[U(\tilde{\theta}^t_{(M)},\theta^\ast) - \int_0^t R_\eta(t,s)(\tilde{\theta}^s_{(M)} - \theta^\ast)\d s + u^t\Big] \d t + \sqrt{2}\d \tilde{B}^t, & 0\leq t\leq T_0,\\
%\Big[U(\tilde{\theta}^t_{(M)},\theta^\ast) - \int_0^t \tilde{R}^{(M)}_\eta(t,s)(\tilde{\theta}^s_{(M)} - \theta^\ast)\d s + \tilde{u}^t_{(M)}\Big] \d t + \sqrt{2}\d \tilde{B}^t, & T_0\leq t\leq T_0 + T,
%\end{cases}
% \end{align}
% where (1) the initialization is $\tilde{\theta}^0_{(M)} = \theta^0$; (2) the Gaussian process $\{\tilde{u}^t_{(M)}\}_{t\in[T_0, T_0+T]}$ has covariance $\E[\tilde{u}^t_{(M)}\tilde{u}^s_{(M)}] = \sum_{m=1}^M \frac{c_m^2}{a_m}(e^{-a_m|t-s|} - e^{-a_m(t+s)}) + c_\eta(\infty)$ and $(\{u^t\}_{t\in[0,T_0+T]}\{\tilde{u}^t_{(M)}\}_{t\in[T_0,T_0+T]})$ is generated as follows: $(\{u^t\}_{t\in[T_0,T_0+T]}, \{\tilde{u}^t\}_{t\in[T_0,T_0+T]})$ is given by the coupling in Lemma \ref{lem:GP_couple}, and conditioning on $\{u^t\}_{t\in[T_0,T_0+T]}$, $\{u^t\}_{t\in [0,T_0]}$ is generated from the associated conditional distribution of the joint law $\cL(\{\theta^t\}_{t\in[0,T_0+T]})$ ; (3) the Brownian motion $\{\tilde{B}^t\}_{t\in [T_0,T_0+T]}$ is defined by $B^t$ for $t\in[0,T_0]$ and $2B^{T_0} - B^t$ for $t\in[T_0,T_0+T]$ so that $\d\tilde{B}^t = -\d B^t$ for $t\in [T_0,T_0+T]$; (4) $\tilde{R}_\eta^{(M)}(t,s) = \tilde{R}_\eta^{(M)}(t-s) = -\sum_{m=1}^M c_m^2e^{-a_m(t-s)}$. \
% 
% By construction, it clearly holds that $\theta^t = \tilde{\theta}^t_{(M)}$ for $t\in[0,T_0]$. The following result bounds their distance on $t\in[T_0,T_0+T]$.
% 
%
% Let
% \begin{align}\label{eq:cvx_infty}
% \kappa(r) := \inf\{-\frac{(\theta^1 - \theta^2)((\log g)'(\theta_1) - (\log g)'(\theta_2))}{(\theta^1-\theta^2)^2}: |\theta^1 - \theta^2| = r\}.
% \end{align}
% Suppose that $\kappa(r) > -K$ for all $r\geq 0$ and $\kappa(r) \geq 0$ for $r\geq R$. Then for any $T_0, T > 0$, it holds that
% \begin{align*}
% \sup_{t\in[T_0,T_0+T]}\E|\theta^t - \tilde{\theta}^t_{(M)}| \leq Ce^{-cT_0}T^{3/2} + \delta(M),
% \end{align*}
% where $\delta(M) \rightarrow 0$ as $M\rightarrow\infty$.
%  \end{lemma}
% \begin{proof}
 We shorthand $\tilde{R}_\eta^{(M)}$ as $\tilde{R}_\eta$. Let $Z_t := \theta^t - \tilde{\theta}^t$, and
 \begin{align*}
 b_t := b_t(\{\theta^s\}_{s\in[0,t]}, \theta^\ast, u^t) := U(\theta^t,\theta^\ast) - \int_0^t R_\eta(t,s)(\theta^s - \theta^\ast) \d s + u^t,\\
 \tilde{b}_t := \tilde{b}_t(\{\tilde{\theta}^s\}_{s\in[0,t]}, \theta^\ast, \tilde{u}^t) := U(\tilde{\theta}^t,\theta^\ast) - \int_0^t \tilde{R}_\eta(t,s)(\tilde{\theta}^s - \theta^\ast) \d s + \tilde{u}^t.
 \end{align*}
 Then $Z_t = 0$ for $t\in [0,T_0]$, and for $t\in [T_0, T_0+T]$, Ito's formula yields $\d |Z_t| = \frac{Z_t}{|Z_t|}(b_t - \tilde{b}_t)\d t + 2\sqrt{2}\d B^t$. Let $A: \R_+\rightarrow\R_+$ be a differentiable function to be specified later, and $r_t := |Z_t| + \int_0^t A(t-s) |Z_s|\d s = |Z_t| + \int_{T_0}^t A(t-s) |Z_s|\d s$ for $t\in [T_0, T_0+T]$, where Ito's formula yields
 \begin{align*}
 \d r_t = \d |Z_t| + \Big[A(0)|Z_t| + \int_0^t A'(t-s)|Z_s|\d s\Big]\d t.
 \end{align*}
 Then for any twice differentiable $f: \R_+\rightarrow\R$ satisfying $f(0) = 0$ and $f'(r) \in [0,1]$ for $r\in\R_+$, we have
 \begin{align*}
 \d f(r_t) &= f'(r_t)\Big[\d |Z_t| + \Big(A(0)|Z_t| + \int_0^t A'(t-s)|Z_s|\d s\Big)\d t\Big] + 4f''(r_t) \d t\\
 &= \Big[f'(r_t)\Big(\frac{Z_t}{|Z_t|}(b_t - \tilde{b}_t) + A(0)|Z_t| + \int_0^t A'(t-s)|Z_s|\d s\Big) + 4f''(r_t)\Big]\d t + 2\sqrt{2}f'(r_t)\d B^t.
 \end{align*}
 With $\tilde{R}_\eta(t,\ast) := -\int_0^t \tilde{R}(t,s)\d s$ and using $f'(r) \in [0,1]$ for any $r\geq 0$, we have the bound
% \begin{align*}
% \d f(|Z_t|) = \Big(f'(|Z_t|)\frac{Z_t}{|Z_t|}(b_t - \tilde{b}_t) + 4f''(|Z_t|)\Big)\d t + 2\sqrt{2}f'(|Z_t|)\d B^t, 
% \end{align*}

 \begin{align*}
 \E\Big[f'(r_t)\Big(\frac{Z_t}{|Z_t|}(b_t - \tilde{b}_t)\Big] &= \E\Big[f'(r_t)\frac{Z_t}{|Z_t|}\Big(-\frac{\delta}{\sigma^2}Z_t + \big((\log g)'(\theta^t) - (\log g)'(\tilde{\theta}^t)\big) - \int_0^t \tilde{R}_\eta(t,s)(\theta^s - \tilde{\theta}^s)\d s\\
 &\quad -\int_0^t \big(R_\eta(t,s) - \tilde{R}_\eta(t,s)\big)\theta^s\d s - (R_\eta(t,\ast) - \tilde{R}_\eta(t,\ast))\theta^\ast + (u^t - \tilde{u}^t)\Big)\Big]\\
 &\leq -\frac{\delta}{\sigma^2}\E[f'(r_t)|Z_t|] - \E[\kappa(|Z_t|)|Z_t|f'(r_t)] + \E\Big[\int_0^t |\tilde{R}_\eta(t,s)||Z_s|\d s\Big] + \Delta_t\\
 &\leq -\frac{\delta}{\sigma^2}\E[f'(r_t)|Z_t|] + \E[\kappa_-(|Z_t|)|Z_t|f'(r_t)] + \E\Big[\int_0^t |\tilde{R}_\eta(t,s)||Z_s|\d s\Big] + \Delta_t,
 \end{align*}
 where, $\kappa_-$ is the negative part of $\kappa$, and
 \begin{align}\label{eq:Delta_t}
 \Delta_t :=  \int_0^t \big|R_\eta(t,s) - \tilde{R}_\eta(t,s)\big|\E|\theta^s|\d s + |R_\eta(t,\ast) - \tilde{R}_\eta(t,\ast)|\E|\theta^\ast| + \E|u^t - \tilde{u}^t|.
 \end{align}
 Consequently, we have
 \begin{align*}
 \frac{\d \E f(r_t)}{\d t} &= \E\Big[f'(r_t)\Big(\frac{Z_t}{|Z_t|}(b_t - \tilde{b}_t) + A(0)|Z_t| + \int_0^t A'(t-s)|Z_s|\d s\Big) + 4f''(r_t)\Big] + \Delta_t\\
 &\leq \E\Big[-\big(\frac{\delta}{\sigma^2} - A(0)\big)f'(r_t)|Z_t| + \kappa_-(|Z_t|)|Z_t|f'(r_t) + 4f''(r_t)\Big] + \E\Big[f'(r_t)\int_0^t \big(A'(t-s) + \tilde{R}_\eta(t-s)\big)|Z_s| \d s\Big] + \Delta_t.
 \end{align*}
For some small enough $c > 0$, let $A(0):= \delta/\sigma^2 - c$ and $A(t) = A(0)e^{-ct} + \int_0^t e^{-c(t-s)}|\tilde{R}_\eta(s)|\d s$ (so that $A'(t) + |\tilde{R}_\eta(t)| = -cA(t)$), then we have
\begin{align*}
\frac{\d \E f(r_t)}{\d t} \leq \E\Big[-cr_tf'(r_t) + \kappa_-(|Z_t|)|Z_t|f'(r_t) + 4f''(r_t)\Big] + \Delta_t.
\end{align*}
Recall the constant $K,R$ given in (\ref{eq:cvx_infty}). Let
\begin{align}\label{eq:g_choice}
g(r) := 
\begin{cases}
\sup_{t\geq 0} \E[|Z_t|\kappa_-(|Z_t|)|r_t = r], & r\leq 2KR/c,\\
0 & \text{otherwise},
\end{cases}
\end{align}
and $f(\cdot)$ be specified by $f(0) = 0$, and $f'(r) = e^{-\frac{1}{4}\int_0^r g(s)\d s}$. Since $\kappa(r) \geq 0$ for $r\geq R$ and $\kappa(r) \geq -K$ for all $r\geq 0$, we have $g(r)\leq KR$, and hence $\omega \leq f'(r) \leq 1$ for all $r\in\R_+$ with $\omega = \exp(-K^2R^2/(2c))$. Moreover, $f''(r) = -e^{-\frac{1}{4}\int_0^r g(s)\d s} \cdot g(r)/4 \leq 0$ so $f$ is concave. Then
\begin{align}\label{eq:exp_decay_f}
\notag&\E\Big[-cr_tf'(r_t) + \kappa_-(|Z_t|)|Z_t|f'(r_t) + 4f''(r_t)\Big]\\
\notag&= \E\Big[\Big(-cr_tf'(r_t) + \kappa_-(|Z_t|)|Z_t|f'(r_t) + 4f''(r_t)\Big)(\bm{1}_{r_t > 2KR/c} + \bm{1}_{r_t \leq 2KR/C})\Big]\\
\notag&\leq \E\Big[\Big(-cr_tf'(r_t) + KRf'(r_t) + 4f''(r_t)\Big)\bm{1}_{r_t > 2KR/c}\Big] +  \E\Big[\Big(-cr_tf'(r_t) + f'(r_t)\E [\kappa_-(|Z_t|)|Z_t| | r_t] + 4f''(r_t)\Big)\bm{1}_{r_t \leq 2KR/c}\Big]\\
\notag&\leq -\E\Big[\frac{c}{2}r_tf'(r_t)\bm{1}_{r_t > 2KR/c}\Big] + \E\Big[\Big(-cr_tf'(r_t) + f'(r_t)g(r_t) + 4f''(r_t)\Big)\bm{1}_{r_t \leq 2KR/c}\Big]\\
&\stackrel{(*)}{=} -\E\Big[\frac{c}{2}r_tf'(r_t)\bm{1}_{r_t > 2KR/c}\Big] - \E\Big[cr_tf'(r_t)\bm{1}_{r_t \leq 2KR/c}\Big] \leq -\frac{c}{2}\E[r_tf'(r_t)] \leq -\frac{c\omega}{2}\E[r_t] \leq -\frac{c\omega}{2}\E[f(r_t)],
\end{align}
where in $(*)$ we use $f'(r)g(r) + 4f''(r) = 0$. Hence we obtain
\begin{align*}
\frac{\d \E f(r_t)}{\d t} \leq -c'\E[f(r_t)] + \Delta_t.
\end{align*}
Since $f(r_{T_0})  = f(0) = 0$, the above differential inequality yields that $\E f(r_t) \leq C'\Delta_t$ for all $t\geq T_0$, which further implies $\E[|Z_t|] \leq \E[r_t] \leq \E[f(r_t)]/\omega \leq C''\Delta_t$. 

It remains to show the following bound on $\Delta_t$: for any $t\in[T_0, T_0+T]$,
\begin{align}\label{eq:Delta_bound}
\Delta_t \leq Ce^{-cT_0}T^{3/2} + \delta(M),
\end{align}
where $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$. To bound $\int_0^t \big|R_\eta(t,s) - \tilde{R}_\eta(t,s)\big|\E|\theta^s|\d s$, it suffices to bound $\int_0^t \big|R_\eta(t,s) - \tilde{R}_\eta(t,s)\big|\d s$ by Lemma \ref{lem:dmft_theta_uniform}. To this end, we have by property (\ref{eq:Retaapproxinvariant})
\begin{align*}
\int_0^t |R_\eta(t,s) - \tilde{R}_\eta(t-s)|\d s &\leq \int_0^t |R_\eta(t,s) - r^{\tti}_\eta(t-s)|\d s + \int_0^t |r_\eta^{\tti}(t-s) - \tilde{R}_\eta(t-s)|\d s\\
&\leq Cte^{-ct} + \int_0^t |r_\eta^{\tti}(t-s) - \tilde{R}_\eta(t-s)|\d s. 
\end{align*}
To bound the second term, note that
\begin{align*}
r_\eta^{\tti}(\tau) - \tilde{R}_\eta(\tau) = \int_\iota^\infty ae^{-a\tau}\mu_\eta(\d a) - \sum_{i=1}^M c_i^2e^{-a_i\tau} = \sum_{i=1}^M \int_{a_{i-1}}^{a_i} (ae^{-a\tau} - a_ie^{-a_i\tau})\mu_\eta(\d a) + \int_{a:a>a_M} ae^{-a\tau} \mu_\eta(\d a),
\end{align*}
hence using the fact that $h(a) := ae^{-a\tau}$ satisfies $|h'(a)| \leq 2e^{-a\tau/2}$ and $\Delta := \max_{i\leq M} |a_i - a_{i-1}| \leq 1/\sqrt{M}$,
\begin{align*}
\int_0^t \big|r_\eta^{\tti}(\tau) - \tilde{R}_\eta(\tau)\big|\d\tau &\leq \sum_{i=1}^M\int_{a_{i-1}}^{a_i} \Big(\int_0^t |ae^{-a\tau} - a_ie^{-a_i\tau}|\d \tau\Big) \mu_\eta(\d a) + \int_{a:a>a_M} \Big(\int_0^t ae^{-a\tau}\d\tau\Big) \mu_\eta(\d a)\\
&\leq \sum_{i=1}^M\int_{a_{i-1}}^{a_i} \Big(\int_0^t 2\Delta e^{-a_{i-1}\tau/2}\d \tau\Big) \mu_\eta(\d a) + \mu_\eta([\sqrt{M},\infty))\\
&\lesssim \Delta\sum_{i=1}^M \int_{a_{i-1}}^{a_i} \frac{1}{a_{i-1}} \mu_{\eta}(\d a) + \mu_\eta([\sqrt{M},\infty)) \leq \frac{\Delta}{\iota} \mu_\eta([0,\sqrt{M})) + \mu_\eta([\sqrt{M},\infty)) := \delta(M),
\end{align*}
where $\delta(M)\rightarrow 0$ as $M \rightarrow\infty$. Next, since $R_\eta(t,\ast) = -\int_0^t R_\eta(t,s)$ and $\tilde{R}_\eta(t,\ast) = \int_0^t \tilde{R}_\eta(t,s)\d s$, we have $|R_\eta(t,\ast) - \tilde{R}_\eta(t,\ast)| \leq \int_0^t|R_\eta(t,s) - \tilde{R}_\eta(t-s)|\d s$, as bounded above. Lastly, Lemma \ref{lem:GP_couple} yields that $\sup_{t\in[T_0,T_0+T]} \E|u^t - \tilde{u}^t|\leq \delta(M) + Ce^{-cT_0}T^{3/2}$. Combining the above bounds yields (\ref{eq:Delta_bound}) and thus completes the proof.
\end{proof}

  \begin{lemma}\label{lem:dmft_theta_uniform}
 Suppose $g(\cdot)$ satisfies Assumption \ref{assump:prior_cvx_infty}. Then there exists some $C > 0$ such that $\sup_{t\geq 0} \E |\theta^t|^4 \leq C$.
 \end{lemma}
 \begin{proof}
 Let $\bar{\theta}^t := \theta^t - \theta^\ast$, which satisfies
 \begin{align*}
 \d \bar{\theta}^t = \Big[-\frac{\delta}{\sigma^2} \bar{\theta}^t + (\log g)'(\theta^t) - \int_0^t R_\eta(t,s)\bar{\theta}^s \d s + u^t\Big]\d t + \sqrt{2}\d B^t.
 \end{align*}
  Let $A:\R_+\rightarrow \R_+$ be a differentiable function to be specified later, and $r_t = |\bar{\theta}^t| + \int_0^t A(t-s)|\bar{\theta}^s|\d s$. Then Ito's formula yields
 \begin{align*}
 \d|\bar{\theta}^t| &= \frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big[-\frac{\delta}{\sigma^2} \bar{\theta}^t + (\log g)'(\theta^t) - \int_0^t R_\eta(t,s)\bar{\theta}^s \d s + u^t\Big]\d t + \sqrt{2}\frac{\bar{\theta}^t}{|\bar{\theta}^t|}\d B^t,\\
 \d r_t &= \d |\bar{\theta}^t| + \Big[A(0)|\bar{\theta}^t| + \int_0^t A'(t-s)|\bar{\theta}^s|\d s\Big]\d t\\
 &= \Big[-\Big(\frac{\delta}{\sigma^2} - A(0)\Big)|\bar{\theta}^t| + \int_0^t \Big(-\frac{\bar{\theta}^t}{|\bar{\theta}^t|}R_\eta(t,s) + A'(t,s)\Big)|\bar{\theta}^s|\d s + \frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big((\log g)'(\theta^t)+ u^t\Big)\Big]\d t + \sqrt{2}\frac{\bar{\theta}^t}{|\bar{\theta}^t|}\d B^t.
 \end{align*}
 This further implies that
 \begin{align*}
 \d r_t^4 &= 4r_t^3\Big[-\Big(\frac{\delta}{\sigma^2} - A(0)\Big)|\bar{\theta}^t| + \int_0^t \Big(-\frac{\bar{\theta}^t}{|\bar{\theta}^t|}R_\eta(t,s) + A'(t-s)\Big)|\bar{\theta}^s|\d s + \frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big((\log g)'(\theta^t)+ u^t\Big)\Big]\d t\\
 &\quad + 12r_t^2 \d t + 4\sqrt{2}r_t^3\frac{\bar{\theta}^t}{|\bar{\theta}^t|}\d B^t,
 \end{align*}
 and hence
 \begin{align*}
\frac{\d \E r_t^4}{\d t} &\leq 4\E r_t^3\Big[-\Big(\frac{\delta}{\sigma^2} - A(0)\Big)|\bar{\theta}^t| + \int_0^t \Big(|r_\eta^{\tti}(t-s)| + A'(t-s)\Big)|\bar{\theta}^s|\d s + \frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big((\log g)'(\theta^t) - (\log g)'(\theta^\ast)\Big)\\
 &\quad + \int_0^t |R_\eta(t,s) - r_\eta^{\tti}(t-s)||\bar{\theta}^s|\d s + |(\log g)'(\theta^\ast)| + |u^t|\Big] + 12\E[r_t^2]\\
 &\leq 4\E r_t^3\Big[-\Big(\frac{\delta}{\sigma^2} - A(0)\Big)|\bar{\theta}^t| + \int_0^t \Big(|r_\eta^{\tti}(t-s)| + A'(t-s)\Big)|\bar{\theta}^s|\d s + |\bar{\theta}^t|\kappa_-(|\bar{\kappa}^t|)\Big)\\
 &\quad + \int_0^t |R_\eta(t,s) - r_\eta^{\tti}(t-s)||\bar{\theta}^s|\d s + |(\log g)'(\theta^\ast)| + |u^t|\Big] + 12\E[r_t^2]
 \end{align*}
 Using the same arguments that lead up to (\ref{eq:exp_decay_f}) with $\tilde{R}_\eta(t-s)$ there replaced by $r^{\tti}(t-s)$, and property (\ref{eq:Retaapproxinvariant}), we have
 \begin{align*}
 \frac{\d r_t^4}{\d t} \leq -c' \E r_t^4 + C\E\Big[r_t^3 e^{-c_0t}\int_0^t |\bar{\theta}^s|\d s\Big] + C\Big(\E r_t^3\Big[|(\log g)'(\theta^\ast)| + |u|^t + |\bar{\theta}^t|\kappa_-(|\bar{\theta}^t|)\Big] + \E [r_t^2]\Big).
 \end{align*}
  By choosing $c$ in the definition of $A(t)$ to be small enough, for large enough $t$ we have $C\E\Big[r_t^3 e^{-c_0t}\int_0^t |\bar{\theta}^s|\d s\Big] \leq (c'/4)\E r_t^4$. Moreover, for large enough $C'$, if $\E r_t^4 \geq C'$, it can be readily checked that (using $|\bar{\theta}^t|\kappa_-(|\bar{\theta}^t|) \leq KR$)
  \begin{align*}
  C\Big(\E r_t^3\Big[|(\log g)'(\theta^\ast)| + |u|^t + |\bar{\theta}^t|\kappa_-(|\bar{\theta}^t|)\Big] + \E [r_t^2]\Big) \leq \frac{c'}{4}\E r_t^4.
  \end{align*}
  Consequently, we have for all large enough $t$ that
  \begin{align*}
  \frac{\d \E r_t^4}{\d t} \leq -\frac{c'}{2} \E r_t^4 + C''\bm{1}_{\E|r_t|^4\leq C'},
  \end{align*}
  which implies that $\sup_{t\geq 0} \E r_t^4 \leq C'''$. This further implies $\sup_{t\geq 0} \E |\theta^t|^4 \leq C''''$ as desired.
 \end{proof}
 
 
 
% \begin{lemma}\label{lem:dmft_theta_uniform}
% Suppose $g(\cdot)$ satisfies Assumption \ref{assump:prior_cvx_infty}. Then there exists some $C > 0$ such that $\sup_{t\geq 0} \E|\theta^t| \leq C$.
% \end{lemma}
% \begin{proof}
% Let $\bar{\theta}^t := \theta^t - \theta^\ast$, which satisfies
% \begin{align*}
% \d \bar{\theta}^t = \Big[-\frac{\delta}{\sigma^2} \bar{\theta}^t + (\log g)'(\theta^t) - \int_0^t R_\eta(t,s)\bar{\theta}^s \d s + u^t\Big]\d t + \sqrt{2}\d B^t.
% \end{align*}
% Let $A:\R_+\rightarrow \R_+$ be a differentiable function to be specified later, and $r_t = |\bar{\theta}^t| + \int_0^t A(t-s)|\bar{\theta}^s|\d s$. Then Ito's formula yields
% \begin{align*}
% \d|\bar{\theta}^t| &= \frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big[-\frac{\delta}{\sigma^2} \bar{\theta}^t + (\log g)'(\theta^t) - \int_0^t R_\eta(t,s)\bar{\theta}^s \d s + u^t\Big]\d t + \sqrt{2}\d B^t,\\
% \d r_t &= \d |\bar{\theta}^t| + [A(0)|\bar{\theta}^t| + \int_0^t A'(t-s)|\bar{\theta}^s|\d s]\d t.
% \end{align*}
% Then for any twice differentiable $f:\R_+\rightarrow\R$ satisfying $f(0) = 0$ and $f'(r) \in [0,1]$ for $r\in\R_+$, we have
% \begin{align*}
% \d f(r_t) &= f'(r_t)\Big[\d |\bar{\theta}^t| + \Big(A(0)|\bar{\theta}^t| + \int_0^t A'(t-s)|\bar{\theta}^s|\d s\Big)\d t\Big] + f''(r_t) \d t\\
% &= \Big[f'(r_t)\Big(\frac{\bar{\theta}^t}{|\bar{\theta}^t|}\Big(-\frac{\delta}{\sigma}\bar{\theta}^t + (\log g)'(\theta^t) - \int_0^t R_\eta(t,s)\bar{\theta}^s \d s + u^t\Big) + A(0)|\bar{\theta}^t| + \int_0^t A'(t-s)|\bar{\theta}^s|\d s\Big) + f''(r_t)\Big]\d t\\
% &\quad + \sqrt{2}f'(r_t)\d B^t,
% \end{align*}
% which further implies that
% \begin{align*}
% \frac{\d \E f(r_t)}{\d t} &= -\big(\frac{\delta}{\sigma^2} - A(0)\big)\E[f'(r_t)|\bar{\theta}^t|] + \E[f'(r_t)\frac{\bar{\theta}^t}{|\bar{\theta}^t|}\big((\log g)'(\theta^t) - (\log g)'(\theta^\ast)\big)] + \E[|(\log g)'(\theta^\ast)|]\\
% &\quad + \E[f'(r_t)\int_0^t \big(|R_\eta(t,s)| + A'(t-s)\big)|\bar{\theta}^s|\d s + f''(r_t)]\\
%&\leq \E\Big[-\big(\frac{\delta}{\sigma^2} - A(0)\big)f'(r_t)|\bar{\theta}^t| + \kappa_-(|\bar{\theta}^t|)|\bar{\theta}^t|f'(r_t) + f''(r_t)\Big] + \E\Big[f'(r_t)\int_0^t \big(A'(t-s) + |r_\eta^{\tti}(t-s)|\big)|\bar{\theta}^s| \d s\Big]\\
%&\quad + \E\Big[f'(r_t) \int_0^t |R_\eta(t,s) - r^{\tti}_\eta(t-s)||\bar{\theta}^s|\d s\Big] + \E[|(\log g)'(\theta^\ast)|].
% \end{align*}
% Using the same arguments that lead up to (\ref{eq:exp_decay_f}) with $\tilde{R}_\eta(t-s)$ there replaced by $r^{\tti}(t-s)$, and property (\ref{eq:Retaapproxinvariant}), we have
% \begin{align*}
% \frac{\d \E f(r_t)}{\d t} \leq -c' \E f(r_t) + C\E\Big[e^{-c_0t}\int_0^t |\bar{\theta}^s|\d s\Big] + \E[|(\log g)'(\theta^\ast)|].
% \end{align*}
% By choosing $c$ in the definition of $A(t)$ to be small enough, there exists some large enough $T_0 = T_0(c_0,c,c')$ such that $C\E\Big[e^{-c_0t}\int_0^t |\bar{\theta}^s|\d s\Big] \leq (c'/2)\E f(r_t)$, so that for $t\geq T_0$, it holds that $\frac{\d \E f(r_t)}{\d t} \leq -\frac{c'}{2} \E f(r_t) + \E[|(\log g)'(\theta^\ast)|]$, which can be further solved as
% \begin{align*}
% \E f(r_t) \leq e^{-(c'/2)(t-T_0)}\E f(r_{T_0}) + \frac{2\E[|(\log g)'(\theta^\ast)|]}{c'} \leq e^{-(c'/2)(t-T_0)}\E r_{T_0} + \frac{2\E[|(\log g)'(\theta^\ast)|]}{c'}.
% \end{align*}
% On the other hand, it is easy to show that $\sup_{t\in [0,T_0]} \E |\bar{\theta}^t| \leq C$ for some $C = C(T_0) > 0$, hence there exists some $C'$ such that $\sup_{t\geq 0} \E|\theta^t| \leq \sup_{t\geq 0} \E|\bar{\theta}^t| + \E|\theta^\ast| \leq C'$, as desired. 
% \end{proof}
 
% \begin{lemma}\label{lem:auxiliary_V}
% For any positive integer $M$, consider the joint process
% \begin{align}\label{eq:auxiliary_joint}
% \d \tilde{\theta}^t_{(M)} &= [U(\tilde{\theta}^t_{(M)},\theta^\ast) + z - \sum_{m=1}^M c_m V^t_m] + \sqrt{2} \d B^t,\\
% \d V^t_m &= -[a_m V^t_m + c_m(\tilde{\theta}^t_{(M)} - \theta^\ast)]\d t + \sqrt{2} \d B^t_m, \quad 1\leq m\leq M, 
% \end{align}
% where: (1) initialization is $\tilde{\theta}^0_{(M)} = \theta^0$ and $V^0_m = 0$ for $1\leq m\leq M$; (2) $\{B^t\}$ and $\{B^t_m\}$, $1\leq m\leq M$ are independent standard Brownian motions; (3) $\theta^\ast\sim g^\ast$ is independent of $z\sim \N(0, c_\eta(\infty))$, and they are independent of $\{B^t\}$ and $\{B^t_m\}$. Then the joint law of $(\tilde{\theta}^t_{(M)}, \theta^\ast)$ in (\ref{eq:auxiliary_joint}) is the same as that in (\ref{eq:auxiliary_theta}) for $t\in[T_0,T_0+T]$.
% \end{lemma}
% \begin{proof}
% We shorthand $\tilde{\theta}^t_{(M)}$ as $\tilde{\theta}^t$. Note that $V^t_m$ can be explicitly solved as
% \begin{align*}
% V^t_m = -c_m\int_0^t e^{-a_m(t-s)}(\theta^s - \theta^\ast)\d s + \sqrt{2}\int_0^t e^{-a_m(t-s)}\d B^s_m,
% \end{align*}
% hence with $\tilde{u}^t := z - \sqrt{2}\sum_{m=1}^M c_m\int_0^t e^{-a_m(t-s)}\d B^s_m$, we have
% \begin{align*}
% \d \tilde{\theta}^t &= \Big[U(\tilde{\theta}^t,\theta^\ast) + \sum_{m=1}^M c_m^2\int_0^t e^{-a_m(t-s)}(\tilde{\theta}^s - \theta^\ast)\d s + \tilde{u}^t\Big]\d t + \sqrt{2} \d B^t.
% \end{align*}
% It remains to note that $\tilde{R}_\eta^{(M)}(t,s) = -\sum_{m=1}^M c_m^2e^{-a_m(t-s)}$, and $\{\tilde{u}^t\}$ has covariance $\E[\tilde{u}^t\tilde{u}^s] = \sum_{m=1}^M \frac{c_m^2}{a_m}(e^{-a_m|t-s|} - e^{-a_m(t+s)}) + c_\eta(\infty)$.
% \end{proof}
 
 \begin{lemma}\label{lem:GP_couple}
 For any positive integer $M$, consider the covariance $K^{(M)}(t,s) = \sum_{m=1}^M \frac{c_m^2}{a_m}(e^{-a_m|t-s|} - e^{-a_m(t+s)}) + c_\eta(\infty)$. There exists a coupling of Gaussian processes $\{\tilde{u}^t_{(M)}\}_{t\in[T_0,T_0+T]}$ and $\{\check{u}^t\}_{t\in[T_0,T_0+T]}$ with covariance $K^{(M)}$ and $C_\eta$ respectively, such that
 \begin{align*}
 \sup_{t\in[T_0,T_0+T]}\E(\tilde{u}^t_{(M)} - \check{u}^t)^2 \leq \delta(M) + Ce^{-cT_0}T^{3/2},
 \end{align*}
 where $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$, and $C,c > 0$ do not depend on $M,T$. 
 \end{lemma}
 \begin{proof}
Define the covariance kernel $K^{(\infty)}(t,s) := \int_{\iota}^\infty \big(e^{-a|t-s|} - e^{-a(t+s)}\big) \mu_\eta(\d a) + c_\eta(\infty)$. We will couple $(K^{(M)}, K^{(\infty)})$ and $(K^{(\infty)}, C_\eta)$ respectively.

\textbf{Coupling of $(K^{(M)}, K^{(\infty)})$} Let $M'$ be any positive integer larger than $M$, and for notation simplicity we denote $\{a_i^{(M')}\}_{i=0}^{M'}$ and $\{c_i^{(M')}\}_{i=1}^{M'}$ (resp. $\{a_i^{(M)}\}_{i=0}^M$ and $\{c_i^{(M)}\}_{i=1}^M$) as $\{\tilde{a}_i\}_{i=0}^{M'}$ and $\{\tilde{c}_i\}_{i=1}^{M'}$ (resp. $\{a_i\}_{i=0}^M$ and $\{c_i\}_{i=1}^M$). Consider
\begin{align}\label{eq:GP_M_prime}
\tilde{u}^t := z - \sqrt{2}\sum_{m=1}^{M'} \tilde{c}_m\int_0^t e^{-\tilde{a}_m(t-s)}\d \tilde{B}^s_m,
\end{align}
where $z \sim \N(0,c_\eta(\infty))$, $\{\tilde{B}^t_m\}_{t\geq 0}$, $1\leq m\leq M'$ are independent standard Brownian motions, and they are independent. It is easy to verify that $\{\tilde{u}^t\}$ has covariance $K^{(M')}$. Now let $I_j \equiv [a_{j-1}, a_j)$ for $1\leq j\leq M$, and
\begin{align*}
u^t := z - \sqrt{2}\sum_{m=1}^M c_m \int_0^t e^{-a_m(t-s)} \d B^s_m, 
\end{align*}
where $z$ is the same as in (\ref{eq:GP_M_prime}), and for $1\leq m\leq M$, $B^t_m = \sum_{i\leq M': \tilde{a}_i \in I_m} \tilde{c}_i \tilde{B}^t_i/\sqrt{\sum_{i\leq M': \tilde{a}_i \in I_j} \tilde{c}_i^2}$. It can be readily verified that $\{B^t_m\}$, $1\leq m\leq M$ are independent standard Brownian motions, and hence $u^t$ is a Gaussian process with covariance $K^{(M)}$. We may now bound
\begin{align*}
\E[(u^t - \tilde{u}^t)^2] \lesssim \E\Big[\Big(\sum_{i\leq M': \tilde{a}_i > a_m} \tilde{c}_m\int_0^t e^{-\tilde{a}_m(t-s)}\d \tilde{B}^s_m\Big)^2\Big] + \E\Big[\Big(\sum_{j=1}^M \sum_{i\in I_j} \tilde{c}_i \int_0^t e^{-\tilde{a}_i(t-s)}\d \tilde{B}^i_s - \sum_{j=1}^M c_j \int_0^t e^{-a_j(t-s)} \d B^s_j\Big)^2\Big].
\end{align*}
Since $a_m = \sqrt{M}$, the first term equals $2^{-1}\sum_{i\leq M': \tilde{a}_i > \sqrt{M}} \tilde{c}_i^2/\tilde{a}_i \leq \delta_1(M)$ for some $\delta_1(M)\rightarrow 0$ as $M\rightarrow\infty$, by the tightness of the measure $\mu_\eta$. The second term equals
\begin{align*}
&\E\Big[\Big(\sum_{j=1}^M \sum_{i\in I_j} \tilde{c}_i \int_0^t e^{-\tilde{a}_i(t-s)}\d \tilde{B}^s_i - \sum_{j=1}^M c_j \int_0^t e^{-a_j(t-s)} \d B^s_j\Big)^2\Big]\\
&= \E\Big[\Big(\sum_{j=1}^M \sum_{i\in I_j} \int_0^t \Big(\tilde{c}_i e^{-\tilde{a}_i(t-s)} - \frac{c_j\tilde{c}_i}{\sqrt{\sum_{\ell\in I_j} \tilde{c}_\ell^2}}e^{-a_j(t-s)}\Big) \d \tilde{B}^s_i\Big)^2\Big]\\
&= \sum_{j=1}^M\sum_{i\in I_j} \int_0^t \Big(\tilde{c}_i e^{-\tilde{a}_i(t-s)} - \frac{c_j\tilde{c}_i}{\sqrt{\sum_{\ell\in I_j} \tilde{c}_\ell^2}}e^{-a_j(t-s)}\Big)^2 \d s \leq (I) + (II),
\end{align*} 
where
\begin{align*}
(I) =  \sum_{j=1}^M\sum_{i\in I_j} \int_0^t \tilde{c}_i^2 \big(e^{-\tilde{a}_is} - e^{-a_js}\big)^2 \d s, \qquad (II) = \sum_{j=1}^M\sum_{i\in I_j} \int_0^t \tilde{c}_i^2\Big(1-\frac{c_j}{\sqrt{\sum_{\ell\in I_j} \tilde{c}_\ell^2}}\Big)^2e^{-2a_j s}\d s. 
\end{align*}
Let $\Delta = (\sqrt{M} - \iota)/M \leq 1/\sqrt{M}$ be the spacing of $\{a_i\}_{i=0}^M$. Then
\begin{align*}
(I) &\leq \sum_{j=1}^M \sum_{i\in I_j} \int_0^t \tilde{c}_i^2 s^2 e^{-2a_{j-1}s} \Delta^2 \d s \leq \sum_{j=1}^M  \int_0^t \Big(\sum_{i\in I_j} \frac{\tilde{c}_i^2}{\tilde{a}_i}\Big) a_j s^2 e^{-2a_{j-1}s} \Delta^2 \d s \stackrel{(*)}{=} \sum_{j=1}^M c_j^2\int_0^t s^2e^{-2a_{j-1}s}\d s\\
&\lesssim \Delta^2 \sum_{j=1}^M \frac{c_j^2}{a_{j-1}^3} \lesssim \frac{\Delta^2}{\iota^2} \sum_{j=1}^M \frac{c_j^2}{a_j} := \delta_2(M)
\end{align*}
for some $\delta_2(M) \rightarrow 0$ as $M\rightarrow\infty$, where we use $\sum_{i\in I_j} \frac{\tilde{c}_i^2}{\tilde{a}_i} = \mu_\eta(I_j) = c_j^2/a_j$ in $(\ast)$. For $(II)$, since $c_j^2 = \sum_{\ell\in I_j} \frac{a_j}{\tilde{a}_\ell} \tilde{c}_\ell^2$, we have $|c_j^2 - \sum_{\ell\in I_j} \tilde{c}_\ell^2| \leq \Delta \sum_{\ell\in I_j} \tilde{c}_\ell^2/\tilde{a}_\ell = \Delta c_j^2/a_j$, and hence
\begin{align*}
(II) \asymp \sum_{j=1}^M \sum_{i\in I_j} \frac{\tilde{c}_i^2}{a_j} \frac{(c_j - \sqrt{\sum_{\ell\in I_j} \tilde{c}_\ell^2})^2}{\sum_{\ell\in I_j} \tilde{c}_\ell^2} \lesssim \sum_{j=1}^M \frac{(c_j^2 - \sum_{\ell\in I_j} \tilde{c}_\ell^2)^2}{a_j c_j^2} \lesssim \Delta^2 \sum_{j=1}^M \frac{c_j^2}{a_j^3} \leq \frac{\Delta^2}{\iota^2} \sum_{j=1}^M \frac{c_j^2}{a_j} := \delta_3(M).
\end{align*}
In summary, we have shown that $\sup_{t\geq 0}\E[(u^t - \tilde{u}^t)^2] \leq \delta(M)$ for some $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$. Now note that for fixed $T_0, T$, $\{\tilde{u}^t\}_{t\in [T_0, T_0+T]}$ has covariance $K^{(\tilde{M})}$ that converges pointwise to $K^{(\infty)}$ as $\tilde{M}\rightarrow\infty$, so by Lemma \ref{lem:couple_general_cov}, there exists a coupling $(\{\tilde{u}^t\}, \{\bar{u}^t\})$ with covariance $K^{(\infty)}$ on $\{\bar{u}^t\}$ such that $\sup_{t\in [T_0,T_0 + T]} \E (\tilde{u}^t - \bar{u}^t)^2 \rightarrow 0$ as $\tilde{M} \rightarrow\infty$ (but for fixed $T$). Consequently, for any $\tilde{M}$,
\begin{align*}
\sup_{t\in [T_0,T_0+T]} \E(u^t - \bar{u}^t)^2 \leq 2\sup_{t\in [T_0,T_0+T]} \E(u^t - \tilde{u}^t)^2  + 2\sup_{t\in [T_0,T_0+T]} \E(\tilde{u}^t - \bar{u}^t)^2 \leq 2\delta(M) + 2\sup_{t\in [T_0,T_0+T]} \E(\tilde{u}^t - \bar{u}^t)^2.  
\end{align*}
By taking $\tilde{M}\rightarrow\infty$, we obtain a coupling $(\{u^t\}, \{\bar{u}^t\})$ with covariance $(K^{(M)}, K^{(\infty)})$ on $[T_0,T_0+T]$ such that $\sup_{t\in [T_0,T_0+T]} \E(u^t - \bar{u}^t)^2 \leq \delta(M)$ for some $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$.

\textbf{Coupling of $(K^{(\infty)}, C_\eta)$} By property (\ref{eq:Cetaapproxinvariant}), on $[T_0,T_0+T]$ this pair satisfies condition (\ref{eq:cov_point_diff}) of Lemma \ref{lem:couple_general_cov} with $\iota = Ce^{-cT_0}$, so there exists a coupling $(\{\bar{u}^t\}, \{\check{u}^t\})$ with covariance $(K^{(\infty)}, C_\eta)$ such that $\sup_{t\in [T_0,T_0+T]} \E(\bar{u}^t - \check{u}^t)^2 \leq Ce^{-cT_0}T^{3/2}$.
 \end{proof}
 
 \begin{lemma}\label{lem:couple_general_cov}
Let $\{K(t,s)\}_{t,s\in[0,T]}$ and $\{\tilde{K}(t,s)\}_{t,s\in[0,T]}$ be two covariance kernels such that for some $\iota > 0$ and $C_0 > 0$
\begin{align}\label{eq:cov_point_diff}
\sup_{t,s\in[0,T]} |K(t,s) - \tilde{K}(t,s)| \leq \iota,
\end{align}
and
\begin{align}\label{eq:GP_regularity}
\max_{\bar{K} \in \{K,\tilde{K}\}}\sup_{t,s\in[0,T]} \bar{K}(t,t) + \bar{K}(s,s) - 2\bar{K}(t,s) \leq C_0|t-s|.
\end{align}
Then there exist two centered Gaussian processes $\{u^t\}_{t\in[0,T]}$ and $\{\tilde{u}^t\}_{t\in[0,T]}$ such that
\begin{align*}
\sup_{t\in[0,T]} \E[(u^t - \tilde{u}^t)^2]  \leq 6C_0 \iota + 3T^{3/2}\iota^{1/2}.
\end{align*}
\end{lemma}
\begin{proof}
We first prove two coupling results:
\begin{enumerate}
\item Fix $\gamma > 0$ and let $\floor{t} = \max\{i\gamma: i\in \Z_+, i\gamma \leq t\}$. %Suppose $\{K(t,s)\}_{t,s\leq T}$ is a covariance kernel satisfying
%\begin{align*}
%\sup_{t,s\in[0,T]} K(t,t) + K(s,s) - 2K(t,s) \leq C_0(t-s)^2.
%\end{align*}
Then there exist two centered Gaussian processes $\{u^t\}_{t\in[0,T]}$ and $\{v^t\}_{t\in[0,T]}$ with covariance $\E[u^tu^s] = K(t,s)$ and $\E[v^tv^s] = K(\floor{t}, \floor{s})$ such that $\sup_{t\in [0,T]} \E[(u^t - v^t)^2] \leq C_0\gamma$.
\item For two $N \times N$ covariance matrices $\Sigma_1$ and $\Sigma_2$, there exist a coupling $(X,Y)$ with $X \sim \N(0,\Sigma_1)$ and $Y \sim \N(0,\Sigma_2)$ such that $\E\pnorm{X-Y}{}^2 \leq \sqrt{N}\pnorm{\Sigma_1 - \Sigma_2}{F}$.
\end{enumerate}
To see the first claim, let $\{u^t\}_{t\in[0,T]}$ be a centered Gaussian process with covariance $\E[u^tu^s] = K(t,s)$, and $v^t := u^{\floor{t}}$ so that $\E[v^tv^s] = K(\floor{t},\floor{s})$. Suppose  for simplicity $N = T/\gamma$ is an integer. Then by (\ref{eq:GP_regularity})
\begin{align*}
\sup_{t\in[0,T]} \E(u^t - v^t)^2 = \sup_{t\in[0,T]} \E(u^t - u^{\floor{t}})^2 \leq C_0\gamma.
\end{align*}
%\begin{align*}
%\int_0^T \E[(u^t - v^t)^2]\d t = \sum_{\ell=0}^{N-1} \int_{\ell\gamma}^{(\ell+1)\gamma} \E[(u^t - u^{\ell\gamma})^2] \d t \leq N \cdot C_0 \gamma^2 \cdot \gamma = C_0 T\gamma^2,
%\end{align*} 
as desired. For the second claim, let $Z \sim \N(0,I_N)$ and $X = \Sigma^{1/2}Z$, $Y = \Sigma^{1/2}Z$, then
\begin{align*}
\E\pnorm{X- Y}{}^2 = \pnorm{\Sigma_1^{1/2} - \Sigma_2^{1/2}}{F}^2 \stackrel{(*)}{\leq} \pnorm{\Sigma_1 - \Sigma_2}{1} \leq \sqrt{N}\pnorm{\Sigma_1 - \Sigma_2}{F},
\end{align*}
where $(*)$ follows from Bhatia Theorem X.1.3 and $\pnorm{\cdot}{1}$ denotes the Schatten-1 norm. 

Now we prove the lemma. Fix $\gamma > 0$, and assume for simplicity $N = T/\gamma$ is an integer. Let $\Sigma_1,\Sigma_2 \in \R^{N\times N}$ be two covariances matrices defined by $(\Sigma_1)_{ij} = K(i\gamma, j\gamma)$ and $(\Sigma_2)_{ij} = \tilde{K}(i\gamma, j\gamma)$. Let $X = (X_0, \ldots, X_{N-1})$ and $Y = (Y_0,\ldots, Y_{N-1})$ be the coupling given by the second claim above, so that $\E\pnorm{X - Y}{}^2 \leq \sqrt{N}\pnorm{\Sigma_1 - \Sigma_2}{F} \leq N^{3/2}\iota$ by (\ref{eq:cov_point_diff}). Define Gaussian process $\{u^t_\gamma\}_{t\in [0,T]}$ by $u^t_\gamma = X_\ell$ if $t\in [\ell\gamma, (\ell+1)\gamma)$, then $\E[u^t_\gamma u^s_\gamma] = \E[X_{\floor{t}/\gamma}X_{\floor{s}/\gamma}] = K(\floor{t}, \floor{s})$. Let $\{u^t,v^t\}_{t\in[0,T]}$ be a coupling of Gaussian processes given by the first claim with $\{v^t\}$ realized as $\{u^t_\gamma\}$, and $\{\tilde{u}^t_\gamma\}_{t\in[0,T]}, \{\tilde{u}^t\}_{t\in[0,T]}$ be defined similarly, so that $\{u^t\}$ (resp. $\{\tilde{u}^t\}$) has covariance $K$ (resp. $\tilde{K}$). Then we have
\begin{align*}
\sup_{t\in [0,T]} \E (u^t - \tilde{u}^t)^2 &\leq 3 \Big[\sup_{t\in [0,T]} \E (u^t - u_\gamma^t)^2 + \sup_{t\in [0,T]} \E (u^t_\gamma - \tilde{u}_\gamma^t)^2 + \sup_{t\in [0,T]} \E (\tilde{u}^t - \tilde{u}_\gamma^t)^2\Big]\\
&\leq 6C_0 \gamma + 3\gamma \cdot \sum_{\ell=0}^{N-1} \E[(X_\ell - Y_\ell)]^2 \leq 6C_0 \gamma + 3T^{3/2}\gamma^{-1/2} \iota.
\end{align*}
The conclusion follows by choosing $\gamma = \iota$.
\end{proof}

\textbf{Step 2: Property of auxiliary process}
\begin{lemma}\label{lem:aux_converge}
Fix positive integer $M$. With $\omega_\ast^{(M)} = (\delta/\sigma^2 - \sum_{m=1}^M c_m^2/a_m)^2/c_\eta(\infty)$ and $\omega^{(M)} = \delta/\sigma^2 - \sum_{m=1}^M c_m^2/a_m$, it holds that
\begin{align*}
W_1(\cL(\tilde{\theta}^{T_0+T}_{(M)}, \theta^\ast), \cL_{g_\ast,\omega_\ast^{(M)};g,\omega^{(M)}}) \leq C\sqrt{M}e^{-\omega T}
\end{align*}
for some constants $C,\omega > 0$.
\end{lemma}
\begin{proof}
Recall from (\ref{eq:dmft_theta}) that $U(\theta,\theta^\ast) = -\frac{\delta}{\sigma^2}(\theta - \theta^\ast) + (\log g)'(\theta)$. Consider the following process on $[T_0, T_0 + T]$:
\begin{align}\label{eq:auxiliary_stationary}
\notag\d \bar{\theta}^{t}_{(M)} &= \Big[U(\bar{\theta}^t_{(M)}, \theta^\ast) + z - \sum_{m=1}^M c_m \bar{V}^t_m\Big] \d t - \sqrt{2}\d \tilde{B}^t,\\
\d \bar{V}^t_m &= -[a_m\bar{V}^t_m + c_m(\bar{\theta}^t_{(M)} - \theta^\ast)]\d t - \sqrt{2}\d \tilde{B}^t_m, \quad 1\leq m \leq M, 
\end{align}
where $(\theta^\ast, z)$ and the Brownian motions $\{\tilde{B}^t\}, \{\tilde{B}^t_{m}\}, 1\leq m\leq M$ are the same as in Lemma \ref{lem:auxiliary_V}, and conditioning on $\theta^\ast, z$, the initialization $(\bar{\theta}^{T_0}, \{\bar{V}_m^{T_0}\}_{m=1}^M)$ is distributed as $\cL(\tilde{\theta}^\infty_{(M)}, \tilde{V}^\infty_{(M)}|\theta^\ast,z)$, which has density $e^{-H(\bar{\theta}, \{\bar{V}_m\}_{m=1}^M)}/Z$, where $Z = \int e^{-H(\bar{\theta}, \{\bar{V}_m\}_{m=1}^M} \d\bar{\theta}\d \bar{V}_1 \ldots \d \bar{V}_{M}$, and
\begin{align*}
H(\bar{\theta}, \{\bar{V}_m\}_{m=1}^M) &= H(\bar{\theta}, \{\bar{V}_m\}_{m=1}^M; \theta^\ast,z)\\
&= \frac{1}{2}\Big(\frac{\delta}{\sigma^2} - \sum_{m=1}^{M} \frac{c_m^2}{a_m}\Big)(\bar{\theta} - \theta^\ast)^2 - \log g(\tilde{\theta}) + z\theta + \sum_{m=1}^{M} \frac{a_m}{2}(\bar{V}_m + \frac{c_m}{a_m}(\bar{\theta} - \theta^\ast))^2.
\end{align*}
We shorthand $\tilde{\theta}^t_{(M)}$ (resp. $\bar{\theta}^t_{(M)}$) as $\tilde{\theta}^t$ (resp. $\bar{\theta}^t$). It can be readily checked that $(\bar{\theta}^t, \{\bar{V}^t_m\}_{m=1}^M)$ correspond to a Langevin diffusion with stationary distribution $\cL(\tilde{\theta}^\infty_{(M)}, \tilde{V}^\infty_{(M)}|\theta^\ast,z)$ (and quenched $\theta^\ast,z$), so the law $\cL(\bar{\theta}^t, \{\bar{V}^t\}_{m=1}^M|\theta^\ast,z)$ equals $\cL(\tilde{\theta}^\infty_{(M)}, \tilde{V}^\infty_{(M)}|\theta^\ast,z)$ for all $t\in[T_0,T_0+T]$. 

Let us now bound $\E|\tilde{\theta}^t - \bar{\theta}^t|$, for which the proof is similar to that of Lemma \ref{lem:auxiliary_V}. Let $\tilde{\Gamma}^t := (\tilde{\theta}^t, \{\tilde{V}^t_m\}_{m=1}^M) \in \R^{M+1}$ and $\bar{\Gamma}^t \in \R^{M+1}$ be defined similarly, and $Z_t := \tilde{\Gamma}^t - \bar{\Gamma}^t$, then
\begin{align*}
\d Z_t = \big[- L Z_t + v_t\big]\d t + 2\sqrt{2}\d W^t, 
\end{align*}
where $L = [\delta/\sigma^2, -c^\top;-c, A]$ with $c = (c_1,\ldots, a_M)$ and $A = \diag(a_1,\ldots, a_M)$, $W^t = (\tilde{B}^t, \tilde{B}^t_1,\ldots, \tilde{B}^t_{M})$ is a standard Brownian motion, and $v_t \in \R^{M+1}$ with $(v_t)_1 = (\log g)'(\tilde{\theta}^t) - (\log g)'(\bar{\theta}^t)$ and $(v_t)_i = 0$, $2\leq i\leq M+1$. Ito's formula then yields
\begin{align*}
\d \pnorm{Z_t}{} = \frac{Z_t^\top}{\pnorm{Z_t}{}}\d Z_t = -\frac{Z_t^\top L Z_t}{\pnorm{Z_t}{}} + \frac{1}{\pnorm{Z_t}{}}(\tilde{\theta}^t - \bar{\theta}^t)\big((\log g)'(\tilde{\theta}^t) - (\log g)'(\bar{\theta}^t)\big) + 2\sqrt{2}\frac{Z_t^\top}{\pnorm{Z_t}{}}\d W^t, 
\end{align*}
and for any twice differentiable $f:R_+\rightarrow\R$ satisfying $f(0) = 0$ and $f'(r) \geq 0$ for $r\in \R_+$,
\begin{align*}
\d f(\pnorm{Z_t}{}) = f'(\pnorm{Z_t}{})\Big[-\frac{Z_t^\top L Z_t}{\pnorm{Z_t}{}} + \frac{1}{\pnorm{Z_t}{}}(\tilde{\theta}^t - \bar{\theta}^t)\big((\log g)'(\tilde{\theta}^t) - (\log g)'(\bar{\theta}^t)\big) + 2\sqrt{2}\frac{Z_t^\top}{\pnorm{Z_t}{}}\d W^t\Big] + 4f''(\pnorm{Z_t}{}).
\end{align*}
Using the fact that $\lambda_{\min}(L) \geq \min\{\delta/\sigma^2 - \sum_{m=1}^M \frac{c_m^2}{a_m}, \min_{1\leq m\leq M} a_m\} := c$ and the condition on $g(\cdot)$, this further implies (here and below $\E^\circ$ denotes conditional expectation over $\theta^\ast,z$) 
\begin{align*}
\frac{\d \E^\circ f(\pnorm{Z_t}{})}{\d t} \leq -cf'(\pnorm{Z_t}{}) +f'(\pnorm{Z_t}{})|\tilde{\theta}^t - \bar{\theta}|\kappa_-(|\tilde{\theta}^t - \bar{\theta}^t|) + 4f''(\pnorm{Z_t}{}).
\end{align*}
Now let
\begin{align*}
g(r) := 
\begin{cases}
\sup_{t\geq 0} \E^\circ[|\tilde{\theta}^t - \bar{\theta}^t|\kappa_-(|\tilde{\theta}^t - \bar{\theta}^t|)|\pnorm{Z_t}{} = r], & r\leq 2KR/c,\\
0 & \text{otherwise},
\end{cases}
\end{align*}
and $f(\cdot)$ be specified by $f(0) = 0$, and $f'(r) = e^{-\frac{1}{4}\int_0^r g(s)\d s}$. Then using a similar argument to those after (\ref{eq:g_choice}), we have $\frac{\d}{\d t}\E^\circ f(\pnorm{Z_t}{}) \leq -\omega$ and $\omega r\leq f(r) \leq r$ for all $r\in\R_+$, which implies that for any $t\in[T_0,T_0+T]$, $\E^\circ \pnorm{Z_t}{} \leq Ce^{-\omega(t-T_0)} \E^\circ \pnorm{Z_{T_0}}{}$, and hence $\E \pnorm{Z_t}{} \leq Ce^{-\omega(t-T_0)} \E \pnorm{Z_{T_0}}{}$ after further expectation over $\theta^\ast,z$. Lastly note that $\E\pnorm{Z_{T_0}}{} \leq \E\big(|\tilde{\theta}^{T_0}| + \pnorm{\tilde{V}^{T_0}}{} + |\bar{\theta}^t| + \pnorm{\bar{V}^{T_0}}{}\big)$. Using Lemma \ref{lem:dmft_theta_uniform} and (\ref{eq:V_sol}), we have $\E\big(|\tilde{\theta}^{T_0}| + \pnorm{\tilde{V}^{T_0}}{}\big) \leq C\sqrt{M}$. On the other hand, since $\bar{V}^{T_0}_m | \bar{\theta}^{T_0}, \theta^\ast \sim \N(-\frac{c_m}{a_m}(\bar{\theta} - \theta^\ast), \frac{1}{a_m})$, it is easy to show that $\E\big(|\bar{\theta}^t| + \pnorm{\bar{V}^{T_0}}{}\big) \leq C\sqrt{M}$. So we conclude
\begin{align*}
W_1(\cL(\tilde{\theta}^{T_0+T}_{(M)}, \theta^\ast), \cL(\tilde{\theta}^{\infty}_{(M)}, \theta^\ast)) \leq W_1(\cL(\tilde{\theta}^{T_0+T}_{(M)}, \theta^\ast, \tilde{V}^{T_0+T}_{(M)}), \cL(\tilde{\theta}^{\infty}_{(M)}, \theta^\ast, \tilde{V}^{\infty}_{(M)})) \leq Ce^{-\omega T} \E\pnorm{Z_{T_0}}{} \leq C\sqrt{M}e^{-\omega T}.
\end{align*}
\end{proof}

\begin{lemma}\label{lem:aux_station_approx}
For any positive integer $M$, let
\begin{align*}
\omega^{(M)} &= \delta/\sigma^2 - \sum_{m=1}^M c_m^2/a_m, \quad\omega_\ast^{(M)} = (\omega^{(M)})^2/c_\eta(\infty), \\
\omega^{(\infty)} &= \delta/\sigma^2 - \int_\iota^\infty \mu_\eta(\d a), \quad \omega_\ast^{(\infty)} = (\omega^{(\infty)})^2/c_\eta(\infty).
\end{align*}
Then
\begin{align*}
W_1(\cL_{g_\ast,\omega_\ast^{(M)}; g, w^{(M)}}, \cL_{g_\ast,\omega_\ast^{(\infty)}; g, w^{(\infty)}} ) \leq \delta(M)
\end{align*}
for some $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$.
\end{lemma}
\begin{proof}
Let $\cL_{g,\omega}(Y)$ denote the posterior distribution given $Y$ of the channel $Y = \theta + \eps$ with $\theta \sim g$, $\eps \sim \N(0,1/\omega)$. We will first bound $W_1(\cL_{g,\omega^{(M)}}(Y), \cL_{g,\omega^{(\infty)}}(\tilde{Y}))$ for given $Y,\tilde{Y}$. Let $U_{(M)}(\theta; Y) = \frac{\omega^{(M)}}{2}(\theta - Y)^2 - (\log g)(\theta)$ and $U_{(\infty)}(\theta; \tilde{Y})$ be defined similarly, such that the density of $\cL_{g,\omega^{(M)}}(Y)$ (resp. $\cL_{g,\omega^{(\infty)}}(Y')$) is proportional to $e^{-U_{(M)}}$ (resp. $e^{-U_{(\infty)}}$). Consider two Langevin diffusions
\begin{align*}
\d \theta^t = -U'_{(M)}(\theta^t)\d t + \sqrt{2}\d B^t, \quad \d \tilde{\theta}^t = -U'_{(\infty)}(\tilde{\theta}^t)\d t - \sqrt{2}\d B^t,
\end{align*}
where $B^t$ is a standard Brownian motion, and we initialize $\theta^0 \sim \cL_{g,\omega^{(M)}}(Y)$ and $\tilde{\theta}^0 \sim \cL_{g,\omega^{(\infty)}}(\tilde{Y})$, so that the law of $\theta^t$ and $\tilde{\theta}^t$ remain the same for all $t\geq 0$. Using a similar argument as in the proof of Lemma \ref{lem:auxiliary_V}, we have for fixed $Y,\tilde{Y}$%(here $\E^\circ$ denotes expectation conditioning on $Y,\tilde{Y}$)
\begin{align}\label{eq:theta_cond_bound}
\E|\theta^t - \tilde{\theta}^0| \leq Ce^{-\omega t}\E|\theta^0 - \tilde{\theta}^0| + |\omega^{(M)} - \omega^{(\infty)}|\E|\tilde{\theta}^t - \tilde{Y}| + \omega^{\infty}|Y - \tilde{Y}|.
\end{align}
Now for a common $\theta^\ast \sim g_\ast$ and $Z \sim \N(0,1)$, let $Y = \theta^\ast + Z/\sqrt{\omega_\ast^{(M)}}$ and $\tilde{Y} = \theta^\ast + Z/\sqrt{\omega_\ast^{(\infty)}}$, then the total law of $\theta^t$ (resp. $\tilde{\theta}^t$) is $\cL_{g_\ast,\omega_\ast^{(M)}; g, w^{(M)}}$ (resp. $\cL_{g_\ast,\omega_\ast^{(\infty)}; g, w^{(\infty)}}$) for all $t\geq 0$, so (\ref{eq:theta_cond_bound}) implies
\begin{align*}
W_1(\cL_{g_\ast,\omega_\ast^{(M)}; g, w^{(M)}}, \cL_{g_\ast,\omega_\ast^{(\infty)}; g, w^{(\infty)}}) &\leq \liminf_{t\rightarrow\infty}\E|\theta^t - \tilde{\theta}^t| \leq |\omega^{(M)} - \omega^{(\infty)}|\E|\tilde{\theta}^t - \tilde{Y}| + \omega^{\infty}\E|Y - \tilde{Y}|\\
&\leq C(|\omega^{(M)} - \omega^{(\infty)}| + |\omega_\ast^{(M)} - \omega_\ast^{(\infty)}|),
\end{align*}
which converges to 0 as $M\rightarrow\infty$. Here we use the fact that $\omega_\ast^{(M)} \wedge \omega_\ast^{(\infty)} \geq c$ for large enough $M$ and $\sup_{t\geq 0}\E|\tilde{\theta}^t| \leq C$, which can be obtained similar to Lemma \ref{lem:dmft_theta_uniform}.
\end{proof}

\textbf{Step 3: Completion of analysis of $\theta$-equation}
\begin{lemma}\label{lem:theta_replica_eq}
Recall from Lemma \ref{lem:aux_station_approx} that $\omega^{(\infty)} = \delta/\sigma^2 - c_\eta^{\tti}(0)$ and $\omega_\ast^{(\infty)} = (\omega^{(\infty)})^2/c_\eta(\infty)$. It holds that
\begin{align}\label{eq:theta_replica}
c_\theta^{\tti}(0) + c_\theta(\infty) = \E_{g_\ast, \omega_\ast^{(\infty)}} \langle \theta^2\rangle_{g,\omega^{(\infty)}},\quad c_\theta(\infty) =  \E_{g_\ast, \omega_\ast^{(\infty)}} \langle \theta\rangle_{g,\omega^{(\infty)}}^2, \quad c_\theta(\ast) = \E_{g_\ast, \omega_\ast^{(\infty)}}[\langle \theta\rangle_{g,\omega^{(\infty)}}\theta^\ast].
\end{align}
\end{lemma}
\begin{proof}
By Lemmas \ref{lem:auxiliary_V}, \ref{lem:aux_converge}, and \ref{lem:aux_station_approx}, for any positive integer $M$ it holds that
\begin{align*}
W_1(\cL(\theta^{T_0+T},\theta^\ast), \cL_{g_\ast,w_\ast^{(\infty)}; g,w^{(\infty)}}) \leq Ce^{-cT_0}T^{3/2} + \delta(M) + C\sqrt{M}e^{-cT}.
\end{align*}
Hence by choosing $M$ large enough, followed by $T$ large enough and then $T_0$ large enough, we have $W_1(\cL(\theta^t,\theta^\ast), \cL_{g_\ast,w_\ast^{(\infty)}; g,w^{(\infty)}}) \rightarrow 0$ as $t\rightarrow \infty$. By Lemma \ref{lem:dmft_theta_uniform} and a similar finite fourth moment bound for $\cL_{g_\ast,w_\ast; g,w}$, we then have $W_2(\cL(\theta^t,\theta^\ast), \cL_{g_\ast,w_\ast^{(\infty)}; g,w^{(\infty)}}) \rightarrow 0$. This implies
\begin{align*}
c_\theta^{\tti}(0) + c_\theta(\infty) &= \lim_{t\rightarrow\infty} \E[(\theta^t)^2] = \E_{g_\ast, \omega_\ast^{(\infty)}} \langle \theta^2\rangle_{g,\omega^{(\infty)}},\\
c_\theta(\infty) &= \lim_{r\rightarrow\infty}\lim_{t\rightarrow\infty} \E[\theta^t\theta^{t+r}] = \E_{g_\ast, \omega_\ast^{(\infty)}} \langle \theta\rangle_{g,\omega^{(\infty)}}^2,\\
c_\theta(\ast) &= \lim_{t\rightarrow\infty} \E[\theta^t\theta^\ast] = \E_{g_\ast, \omega_\ast^{(\infty)}}[\langle \theta\rangle_{g,\omega^{(\infty)}}\theta^\ast].
\end{align*}
\end{proof}

\subsubsection{Analysis of $\eta$-equation}
Let $M$ be some positive integer and $T_0, T \in \R_+$ to be chosen later. For a given $M$, define sequence $\{a_i\}_{i=1}^M = \{a_i^{(M)}\}_{i=0}^M$ as in (\ref{eq:a_grid})
%\begin{align*}
%a_0 = \iota, \quad a_M = \sqrt{M}, \quad a_i = a_0 + i\cdot \frac{a_M - a_0}{M}, \quad 1\leq i\leq M-1,
%\end{align*}
 and $\{b_i\}_{i=1}^M = \{b_i^{(M)}\}_{i=1}^M$ as $\frac{b_i^2}{a_i} = \mu_\theta([a_{i-1}, a_i))$.

\textbf{Step 1: Construction of auxiliary process}
Let $\xi^t := \eta^t - w^\ast - \eps$ and $\bar{z}$ be a mean-zero Gaussian variable with variance $\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)$ that is independent of everything else. For any positive integer $M$, consider the following process on $[0,T_0+T]$:
\begin{align*}
\tilde{\xi}^t_{(M)} &= 
\begin{cases}
-\frac{1}{\sigma^2}\int_0^t R_\theta(t,s)\tilde{\xi}^s_{(M)} + w^t - w^\ast - \eps, & t\in[0,T_0),\\
\sum_{i=1}^M b_i \tilde{W}^t_i + \bar{z}, & t\in[T_0, T_0+T],
\end{cases}\\
\d \tilde{W}^t_i &= -[a_i \tilde{W}^t_i + b_i\tilde{\xi}^t_{(M)}/\sigma^2]\d t + \sqrt{2}\d \tilde{B}^t_i, \quad 1\leq i\leq M,
\end{align*}
with initialization $\tilde{W}^0_i = 0$ for $1\leq i\leq M$. Note that the process $\{\tilde{\xi}^t\}$ maybe discontinuous at $T_0$. 

\begin{lemma}\label{lem:eta_aux_approx}
It holds that $\sup_{t\in[0, T_0+T]}W_2(\cL(\xi^t, \xi^{t+r}), \cL(\tilde{\xi}_{(M)}^t, \tilde{\xi}_{(M)}^{t+r})) \leq Ce^{c'(T+r)}(\delta(M) + e^{-cT_0})T+r)^{3/2})$
\end{lemma}
\begin{proof}
We shorthand $\tilde{\xi}_{(M)}^t$ as $\tilde{\xi}^t$. For $t\in [T_0, T_0+T]$, $\{\W^t\} := \{W^t_1,\ldots,W^t_M\}$ satisfy the matrix Ornstein-Uhlenbeck process
\begin{align*}
\d \W^t = -[\Lambda\W^t + b\bar{z}/\sigma^2]\d t + \sqrt{2}\d \B^t, 
\end{align*}
where $b = (b_1,\ldots,b_M)$, $\Lambda = A + bb^\top/\sigma^2$ with $A = \diag(a_1,\ldots,a_M)$, and $\B^t = (B^t_1,\ldots,B^t_M)$, and hence can be solved by
\begin{align*}
\W^t = e^{-\Lambda(t-T_0)}\W^{T_0} + \frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda(t-T_0)} - I)b\bar{z} + \sqrt{2}\int_{T_0}^t e^{-\Lambda(t-s)}\d \B^s.
\end{align*}
Hence for $t\geq T_0$, we have $\tilde{\xi}^t = -\frac{1}{\sigma^2}\int_0^t \tilde{R}_\theta(t-s) \tilde{\xi}^s \d s + \tilde{w}^t_{(M)}$, where $\tilde{R}_\theta(t) = \sum_{i=1}^M b_i^2 e^{-a_it}$, and $\tilde{w}^t_{(M)} = \sqrt{2}\int_0^t \sum_{i=1}^M b_ie^{-a_i(t-s)}\d B^s_i + \bar{z}$. It can be checked that $\{\tilde{w}^t_{(M)}\}$ is a centered Gaussian process with covariance
\begin{align*}
\E[\tilde{w}^t_{(M)}\tilde{w}^s_{(M)}] = \sum_{i=1}^M \frac{b_i^2}{a_i}(e^{-a_i|t-s|} - e^{-a_i(t+s)}) + \E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast). 
\end{align*}
On the other hand, the process $\bar{w}^t = w^t - w^\ast - \eps$ has covariance $\E[\bar{w}^t\bar{w}^s] = C_\theta(t,s) + \E_{g_\ast}[\theta^2] + \sigma^2 - 2C_\theta(t,\ast)$, so analogous arguments to Lemma \ref{lem:GP_couple} yields a coupling $(\{\bar{w}^t\}_{t\in [T_0,T_0+T]}, \{\tilde{w}^t_{(M)}\}_{t\in[T_0,T_0+T]})$ such that $\sup_{t\in[T_0,T_0+T]}\E(\bar{w}^t - \tilde{w}^t_{(M)})^2 \leq \delta(M) + Ce^{-cT_0}T^{3/2}$. Now we have $\xi^t = \tilde{\xi}^t$ for $t\in[0,T_0)$, and for $t\in[T_0,T_0+T]$, 
\begin{align*}
\E(\xi^t - \tilde{\xi}^t)^2 \leq C\Big[\E\Big(\int_0^t |\tilde{R}_\theta(t-s)||\xi^s - \tilde{\xi}^s|\d s\Big)^2 + \E \Big(\int_0^t |R_\theta(t,s) - \tilde{R}_\theta(t-s)||\xi^s|\d s\Big)^2 + \E (\bar{w}^t - \tilde{w}^t_{(M)})^2\Big].
\end{align*}
The first term satisfies
\begin{align*}
\E\Big(\int_0^t |\tilde{R}_\theta(t-s)||\xi^s - \tilde{\xi}^s|\d s\Big)^2 = \E\Big(\int_{T_0}^t |\tilde{R}_\theta(t-s)||\xi^s - \tilde{\xi}^s|\d s\Big)^2 \leq C \int_{T_0}^t \E (\xi^s - \tilde{\xi}^s)^2\d s. 
\end{align*}
Following the bound of (\ref{eq:Delta_bound}), the second and third term are collectively bounded by $\delta(M) + Ce^{-cT_0}T^{3/2}$. Hence by Lemma \ref{lem:gronwall}, it holds that $\sup_{t\in [T_0,T_0+T]}\E(\xi^t - \tilde{\xi}^t)^2 \leq Ce^{c'T}(\delta(M) + e^{-cT_0}T^{3/2})$. A similar bound holds for $\sup_{t\in [T_0,T_0+T]}\E(\xi^{t+r} - \tilde{\xi}^{t+r})^2$, completing the proof.
\end{proof}

\textbf{Step 2: Property of auxiliary process}
\begin{lemma}\label{lem:eta_aux_converge}
Let $b = (b_1,\ldots,b_M)$, $A = \diag(a_1,\ldots,a_M)$, and $\Lambda = A + bb^\top/\sigma^2$. Let $\cL_\xi^{(M,r)}$ denote the 2-dimensional Gaussian law $\N(0,\Sigma^{(M,r)})$ with $\Sigma^{(M,r)} = [\rho^2_{(M)}, \kappa_{(M,r)};\kappa_{(M,r)}, \rho^2_{(M)}]$, where $\rho^2_{(M)} = \Var(\bar{z})\cdot \Big[1 - b^\top\Lambda^{-1}b/\sigma^2\Big]^2 +  b^\top  \Lambda^{-1}b$ and $\kappa_{(M,r)} = \Var(\bar{z})\cdot \Big[1 - b^\top\Lambda^{-1}b/\sigma^2\Big]^2 +  b^\top  \Lambda^{-1}e^{-\Lambda r}b$. Then there exists some $C>0$ independent of $T_0,M$ and $\delta(T)\rightarrow 0$ as $T\rightarrow\infty$ such that for any $T > 0$, $W_2(\cL(\tilde{\xi}^{T_0+T}_{(M)},\tilde{\xi}^{T_0+T+r}_{(M)}), \cL_\xi^{(M,r)})\leq \delta(T)$.
\end{lemma}
\begin{proof}
We shorthand $\tilde{\xi}_{(M)}^t$ as $\tilde{\xi}^t$. For $t\in [T_0, T_0+T]$, $\{\W^t\} := \{W^t_1,\ldots,W^t_M\}$ satisfy the matrix Ornstein-Uhlenbeck process
\begin{align*}
\d \W^t = -[\Lambda\W^t + b\bar{z}/\sigma^2]\d t + \sqrt{2}\d \B^t, 
\end{align*}
where $b = (b_1,\ldots,b_M)$, $\Lambda = A + bb^\top/\sigma^2$ with $A = \diag(a_1,\ldots,a_M)$, and $\B^t = (B^t_1,\ldots,B^t_M)$, and hence can be solved by
\begin{align*}
\W^t = e^{-\Lambda(t-T_0)}\W^{T_0} + \frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda(t-T_0)} - I)b\bar{z} + \sqrt{2}\int_{T_0}^t e^{-\Lambda(t-s)}\d \B^s.
\end{align*}
This implies that for $t\in[T_0,T_0+T]$, with $W^{T_0}_i = -\frac{b_i}{\sigma^2}\int_0^{T_0}e^{-a_i(T_0-s)} \tilde{\xi}^s \d s + \sqrt{2}\int_0^{T_0} e^{-a_i(T_0-s)}\d B^s_i$, $1\leq i\leq M$,
\begin{align*}
\tilde{\xi}^t = b^\top e^{-\Lambda(t-T_0)}\W^{T_0} + \bar{z}\Big[1 + b^\top\frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda(t-T_0)} - I)b\Big] + \sqrt{2}\int_{T_0}^t b^\top e^{-\Lambda(t-s)}\d \B^s.
\end{align*}
Consequently, $(\tilde{\xi}^{T_0+T}, \tilde{\xi}^{T_0+T+r}) \sim \N(0, \Sigma^{(r)}_{T_0+T})$, where $\Sigma_{T_0+T}^{(r)} = [\rho^2_{T_0+T}, \kappa_{T_0+T,r};  \kappa_{T_0+T,r}, \rho^2_{T_0+T+r}]$ with
\begin{align*}
\rho^2_{T_0+T} &= b^\top e^{-\Lambda T} \E[(\W^{T_0} \W^{T_0})^\top]e^{-\Lambda T}b + \Var(\bar{z})\cdot \Big[1 + b^\top\frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda T} - I)b\Big]^2 +  b^\top  \Lambda^{-1}(I - e^{-2\Lambda T})b,\\
\rho^2_{T_0+T + r} &= b^\top e^{-\Lambda (T+r)} \E[(\W^{T_0} \W^{T_0})^\top]e^{-\Lambda (T+r)}b + \Var(\bar{z})\cdot \Big[1 + b^\top\frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda (T+r)} - I)b\Big]^2 +  b^\top  \Lambda^{-1}(I - e^{-2\Lambda (T+r)})b,\\
\kappa_{T_0+T;r} &=  b^\top e^{-\Lambda T} \E[(\W^{T_0} \W^{T_0})^\top]e^{-\Lambda (T+r)}b + \Var(\bar{z})\cdot \Big[1 + b^\top\frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda (T+r)} - I)b\Big]\Big[1 + b^\top\frac{1}{\sigma^2}\Lambda^{-1}(e^{-\Lambda T} - I)b\Big]\\
&\quad + b^\top \Lambda^{-1}(e^{-\Lambda r} - e^{-\Lambda(2T+r)})b.
\end{align*}
By Lemma \ref{lem:2d_gau_coupling}, for the desired bound on $W_1(\cL(\tilde{\xi}^{T_0+T}, \tilde{\xi}^{T_0+T+r}), \cL_\xi^{(M,r)})$, it suffices to show
\begin{align*}
|\rho^2_{T_0+T} - \rho^2_{ (M)}| \vee |\rho^2_{T_0+T+r} - \rho^2_{ (M)}| \vee |\kappa_{T+T_0,r} - \kappa_{(M,r)}| \leq \delta(T)
\end{align*}
for some $\delta(T)\rightarrow 0$ as $T\rightarrow\infty$. We will bound the first quantity, and the other two will follow from similar arguments. Note that $\rho^2_{T_0+T} - \rho^2_{\infty, (M)} = (I) + (II) + (III)$, where
\begin{align*}
(I) &= b^\top e^{-\Lambda T} \E[(\W^{T_0} \W^{T_0})^\top]e^{-\Lambda T}b, \quad (II) = -b^\top \Lambda^{-1}e^{-2\Lambda T}b ,\\
(III) &= \Var(\bar{z})\cdot \Big[\frac{1}{\sigma^2}b^\top \Lambda^{-1}e^{-\Lambda T}b \cdot \Big(2 + \frac{b^\top}{\sigma^2}\Lambda^{-1}(e^{-\Lambda t} - 2I)b\Big)\Big].
\end{align*}
To bound (I), note that $\E[(\W^{T_0} \W^{T_0})^\top] = \E[UU^\top] + D$, where $U_i = \frac{b_i}{\sigma^2}\int_0^{T_0} e^{-a_i(T_0-s)} \tilde{\xi}^s \d s$ and $D = \diag(\{\frac{1}{a_i}(1-e^{-2a_iT_0})\}_{i=1}^M)$, so it suffices to bound $(I_1) = b^\top e^{-\Lambda T} D e^{-\Lambda T} b$ and $(I_2) := b^\top e^{-\Lambda T} \E[UU^\top]e^{-\Lambda T}b$. For $(I_1)$, we have 
\begin{align*}
(I_1)\leq \pnorm{\Lambda^{-1/2}b}{}^2 \pnorm{\Lambda^{1/2}e^{-\Lambda T}}{\op}^2 \pnorm{D}{\op} \leq \pnorm{A^{-1/2}b}{}^2 \pnorm{\Lambda^{1/2}e^{-\Lambda T}}{\op}^2 \pnorm{D}{\op}. 
\end{align*}
The first term is bounded by $\sum_{i=1}^M b_i^2/a_i$ which converges to $\mu_{\theta}((0,\infty))$ as $M\rightarrow\infty$, the second term is, with $\{\lambda_i\}_{i=1}^M$  denoting the eigenvalues of $\Lambda$, $\max_{\lambda_i} \lambda_i^{1/2}e^{-\lambda_i T} \leq \sqrt{\iota}e^{-\iota T}$ using the fact that $\lambda \mapsto \lambda^{1/2}e^{-\lambda T}$ is decreasing on $[\iota,\infty)$ for large enough $T$ and $\lambda_{\min}(\Lambda) \geq \lambda_{\min}(A) \geq \iota$, and the third term is bounded by $\iota^{-1}$, so we conclude that $(I_1) = \delta(T)$ for some $\delta(T) \rightarrow 0$ as $T\rightarrow\infty$. The term $(I_2)$ satisfies
\begin{align*}
(I_2) = \E (b^\top e^{-\Lambda T} U)^2 &\leq \pnorm{\Lambda^{-1/2}b}{}^2 \pnorm{\Lambda^{1/2}e^{-\Lambda T}}{\op}^2 \cdot \E\sum_{i=1}^M \frac{b_i^2}{\sigma^4}\Big(\int_0^{T_0} e^{-a_i(T_0-s)}\tilde{\xi}^s \d s\Big)^2\\
&\leq \pnorm{\Lambda^{-1/2}b}{}^2 \pnorm{\Lambda^{1/2}e^{-\Lambda T}}{\op}^2 \cdot \sum_{i=1}^M \frac{b_i^2}{\sigma^4} \int_0^{T_0} e^{-a_i(T_0-s)} \d s \cdot \int_0^{T_0} e^{-a_i(T_0-s)}\E[(\tilde{\xi}^s)^2] \d s\\
&\leq Ce^{-\iota T}, 
\end{align*}
using in the last step $\sup_{t\in[0,T_0]} \E[(\tilde{\xi}^t)^2] \leq C$ for some $T_0$-independent $C$ (this holds since $\E(\tilde{\xi}^t)^2 = \frac{\sigma^4}{\delta}C_\eta(t,t) \leq C$ by Assumption \ref{assump:equilibrium}). Similar arguments can be applied to bound $(II)$ and $(III)$, so we conclude that $|\rho^2_{T_0+T} - \rho^2_{(M)}| \leq \delta(T)$ for some $\delta(T)\rightarrow 0$ as $T\rightarrow\infty$, completing the proof.
\end{proof}

\begin{lemma}\label{lem:2d_gau_coupling}
Let $Z$ (resp. $\tilde{Z}$) be a 2-dim centered Gaussian variable with covariance $\Sigma = [\rho_1^2, \kappa; \kappa,\rho_2^2]$ (resp. $\Sigma = [\tilde{\rho}_1^2, \tilde{\kappa}; \tilde{\kappa},\tilde{\rho}_2^2]$). Then there exists some universal $C > 0$ such that
\begin{align*}
W_2^2(\cL(Z), \cL(\tilde{Z})) \leq C\Big(\frac{(\kappa - \tilde{\kappa})^2}{\kappa + \tilde{\kappa}} + \frac{(\rho_1^2 - \tilde{\rho}_1^2)^2 + (\kappa -\tilde{\kappa})^2}{(\rho_1^2 - \kappa) + (\tilde{\rho}_1^2 - \tilde{\kappa})} + \frac{(\rho_2^2 - \tilde{\rho}_2^2)^2 + (\kappa -\tilde{\kappa})^2}{(\rho_2^2 - \kappa) + (\tilde{\rho}_2^2 - \tilde{\kappa})}\Big),
\end{align*}
\end{lemma}
\begin{proof}
This follows from the coupling $Z = (Z_1,Z_2)$ with $Z_1 =  \sqrt{\kappa}g_1 + \sqrt{\rho_1^2 - \kappa}g_2$ and $Z_2 = \sqrt{\kappa}g_1 + \sqrt{\rho_2^2 - \kappa}g_3$, and $\tilde{Z} = (\tilde{Z}_1,\tilde{Z}_2)$ with $\tilde{Z}_1 =  \sqrt{\tilde{\kappa}}g_1 + \sqrt{\tilde{\rho}_1^2 - \tilde{\kappa}}g_2$ and $\tilde{Z}_2 = \sqrt{\tilde{\kappa}}g_1 + \sqrt{\tilde{\rho}_2^2 - \tilde{\kappa}}g_3$, where $g_1,g_2,g_3$ are independent standard Gaussian variables. %Then
%\begin{align*}
%W_2^2(\cL(Z), \cL(\tilde{Z})) &\leq \E(Z_1 - \tilde{Z}_1)^2 + \E(Z_2 - \tilde{Z}_2)^2\\
%&\leq C\Big(\frac{(\kappa - \tilde{\kappa})^2}{\kappa + \tilde{\kappa}} + \frac{(\rho_1^2 - \tilde{\rho}_1^2)^2 + (\kappa -\tilde{\kappa})^2}{(\rho_1^2 - \kappa) + (\tilde{\rho}_1^2 - \tilde{\kappa})} + \frac{(\rho_2^2 - \tilde{\rho}_2^2)^2 + (\kappa -\tilde{\kappa})^2}{(\rho_2^2 - \kappa) + (\tilde{\rho}_2^2 - \tilde{\kappa})}\Big),
%\end{align*}
%as desired.
\end{proof}

\begin{lemma}\label{lem:eta_aux_M_converge}
There exists some $\bar{\kappa}_{(\infty,r)} \rightarrow 0$ as $r\rightarrow\infty$ such that the following holds. Let $\cL_\xi^{(\infty,r)}$ denote the 2-dimensional Gaussian law $\N(0,\Sigma^{(\infty,r)})$ with $\Sigma^{(\infty,r)} = [\rho^2_{(\infty)}, \kappa_{(\infty,r)};\kappa_{(\infty,r)}, \rho^2_{(\infty)}]$, where 
\begin{align*}
\rho^2_{(\infty)} &= \frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{(1 + \sigma^{-2}\int_{\iota}^\infty \mu_\theta(\d a))^2} + \frac{\int_{\iota}^\infty \mu_\theta(\d a)}{1 + \sigma^{-2}\int_{\iota}^\infty \mu_\theta(\d a)},\\
\kappa_{(\infty, r)} &= \frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{(1 + \sigma^{-2}\int_{\iota}^\infty \mu_\theta(\d a))^2} + \bar{\kappa}_{(\infty,r)}.
\end{align*}
Then $W_2(\cL_\xi^{(M,r)}, \cL_\xi^{(\infty,r)}) \leq \delta(M)$ for some $\delta(M)\rightarrow 0$ as $M\rightarrow\infty$.
\end{lemma}
\begin{proof}
This follows from the fact that $b^\top \Lambda^{-1} b = \frac{\sum_{i=1}^M b_i^2/a_i}{1 + \sigma^{-2}\sum_{i=1}^M b_i^2/a_i}$ via Woodbury's identity, and $\sum_{i=1}^M b_i^2/a_i \rightarrow \int_{\iota}^\infty \mu_\theta(\d a)$ as $M\rightarrow\infty$. 
\end{proof}

\textbf{Step 3: Completion of analysis of $\eta$-equation}
\begin{lemma}\label{lem:eta_replica_eq}
It holds that
\begin{align}
c_\eta^{\tti}(0) + c_\eta(\infty) &= \frac{\delta}{\sigma^4}\Big[\frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{\big(1+ c_\theta^{\tti}(0)/\sigma^2\big)^2} + \frac{c_\theta^{\tti}(0)}{1+ c_\theta^{\tti}(0)/\sigma^2}\Big],\label{eq:eta_replica_1}\\
c_\eta(\infty) &= \frac{\delta}{\sigma^4}\frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{1+ c_\theta^{\tti}(0)/\sigma^2} \label{eq:eta_replica_2}.
\end{align}
\end{lemma}
\begin{proof}
By Lemmas \ref{lem:eta_aux_approx}, \ref{lem:eta_aux_converge}, \ref{lem:eta_aux_M_converge}, it holds that $W_2(\cL(\xi^{T_0+T}, \xi^{T_0+T+r}), \cL_\xi^{(\infty,r)}) \leq Ce^{c'(T+r)}(\delta(M) + e^{-cT_0}(T+r)^{3/2})$. Hence for any fixed $r\geq 0$, by choosing $T$ large enough, followed by $M$ and $T_0$ large enough, we have $W_2(\cL(\xi^{t}, \xi^{t+r}), \cL_\xi^{(\infty,r)}) \rightarrow 0$ as $t\rightarrow \infty$. This implies (recall that $c_\theta^{\tti}(0) = \int_\iota^\infty \mu_\theta(\d a)$)
\begin{align*}
\frac{\sigma^4}{\delta}\big(c_\eta^{\tti}(0) + c_\eta(\infty)\big) &= \lim_{t\rightarrow\infty}\E[(\xi^t)^2] = \rho^2_{(\infty)} = \frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{\big(1+ c_\theta^{\tti}(0)/\sigma^2\big)^2} + \frac{c_\theta^{\tti}(0)}{1+ c_\theta^{\tti}(0)/\sigma^2}, \\
\frac{\sigma^4}{\delta} c_\eta(\infty) &= \lim_{r\rightarrow\infty}\lim_{t\rightarrow\infty} \E[\xi^t\xi^{t+r}] = \lim_{r\rightarrow\infty}\kappa_{(\infty, r)} = \frac{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)}{\big(1+ c_\theta^{\tti}(0)/\sigma^2\big)^2},
\end{align*}
as desired.
\end{proof}

\subsubsection{Completing the proof}

By Lemmas \ref{lem:theta_replica_eq} and \ref{lem:eta_replica_eq}, we have five equations (\ref{eq:theta_replica}), (\ref{eq:eta_replica_1}), (\ref{eq:eta_replica_2}) for the five variables $c^{\tti}_\theta(0), c_\theta(\infty), c_\theta(\ast), c_\eta^{\tti}(0), c_\eta(\infty)$. Let us now show the reduction to the fixed-point equations involving $\mse, \mse_\ast, \omega, \omega_\ast$. First by identifying $\omega$ with $\omega^{(\infty)}$, we have
\begin{align*}
\omega = \frac{\delta}{\sigma^2} - c_\eta^{\tti}(0) = \frac{\delta}{\sigma^2 + c_\theta^{\tti}(0)} = \frac{\delta}{\sigma+\mse}. 
\end{align*}
Simimilarly, identifying $\omega_\ast$ with $\omega_\ast^{(\infty)}$, we have
\begin{align*}
\omega_\ast = \frac{(\delta/\sigma^2 - c_\eta^{\tti}(0))^2}{c_\eta(\infty)} = \frac{\delta}{\E_{g_\ast}[\theta^2] + \sigma^2 + c_\theta(\infty) - 2c_\theta(\ast)} = \frac{\delta}{\sigma^2 + \mse_\ast}.
\end{align*}
On the other hand, we have
\begin{align*}
\mse = c_\theta^{\tti}(0) = \E_{g_\ast,\omega_\ast}[\langle \theta^2\rangle_{g,\omega} -  \langle \theta\rangle_{g,\omega}^2] = \E_{g_\ast,\omega_\ast} \langle (\theta - \langle \theta \rangle_{g,\omega})^2\rangle_{g,\omega},
\end{align*}
and
\begin{align*}
\mse_\ast = \E_{g_\ast} [(\theta^\ast)^2] - 2\E_{g_\ast,\omega_\ast}[\theta^\ast\langle\theta\rangle_{g,\omega}] + \E_{g_\ast,\omega_\ast} \langle\theta\rangle_{g,\omega}^2 = \E_{g_\ast,\omega_\ast}(\theta^\ast - \langle\theta\rangle_{g,\omega})^2,
\end{align*}
as desired. \qed


\subsection{Log-Sobolev inequality}

We prove Proposition \ref{prop:LSI} on a log-Sobolev inequality for the prior
and posterior laws.

\begin{lemma}\label{lemma:univariateLSI}
Under either condition of Proposition \ref{prop:LSI},
the LSI for the prior (\ref{eq:LSIprior}) holds.
Furthermore, consider the law
\begin{equation}\label{eq:univariatetilt}
\sP(\theta)=\frac{g(\theta)e^{{-}\frac{a}{2}\theta^2+b\theta}}{Z},
\qquad Z=\int g(\theta)e^{{-}\frac{a}{2}\theta^2+b\theta}\d\theta.
\end{equation}
For any $a>0$ and $b \in \R$, this law satisfies the LSI
\begin{equation}\label{eq:univariateLSI}
\E[f(\theta)^2] \leq C_\LSI\,\E[f'(\theta)^2].
\end{equation}
for all $f \in C^1(\R)$.
The inequalities (\ref{eq:LSIprior}) and (\ref{eq:univariateLSI}) hold with
constant $C_\LSI=2/c_0$ under Proposition \ref{prop:LSI}(a)
and $C_\LSI=(4/c_0)\exp(8R^2(c_0-c_1)^2/(\pi c_0))$ under
Proposition \ref{prop:LSI}(b), where both constants are independent of
$a,b$ defining (\ref{eq:univariatetilt}).
\end{lemma}

\begin{proof}
Under condition (a), ${-}(\log g)''(\theta) \geq c_0$ and
${-}\partial_\theta^2 \log \sP(\theta)
=a-(\log g)''(\theta) \geq c_0$, hence (\ref{eq:LSIprior}) and
(\ref{eq:univariateLSI}) hold with $C_\LSI=2/c_0$ by the Bakry-Emery criterion.

We consider condition (b). Applying $x=\min(x,{-c_0})+\max(x+c_0,0)$, define
\begin{align*}
\ell_-(\theta)
&=\log g(0)+(\log g)'(0) \cdot \theta+\int_0^\theta \int_0^x
\min\Big((\log g)''(u),-c_0\Big)\d u\,\d x\\
\ell_+(\theta)&=\int_0^\theta \int_0^x \max\Big((\log g)''(u)+c_0,0\Big)
\d u\,\d x
\end{align*}
so that $\log g(\theta)=\ell_-(\theta)+\ell_+(\theta)$. Then set
\begin{align*}
\tilde \ell_-(\theta)&={-}\log Z-a\theta^2+b\theta+\ell_-(\theta)
\end{align*}
so that $\log \sP(\theta)=\tilde \ell_-(\theta)+\ell_+(\theta)$.
By definition we have
$\ell_-''(\theta)=\min((\log g)''(\theta),-c_0) \leq -c_0$ and also
$\tilde \ell_-''(\theta)=-a+\ell_-''(\theta) \leq -c_0$.
We have $(\log g)''(u)+c_0 \leq 0$
for all $|u|>R$ and $(\log g)''(u)+c_0 \leq c_0-c_1$ for all $|u| \leq R$.
Hence $|\ell_+'(\theta)| \leq R|c_0-c_1|$. Thus both $\log g(\theta)$ and
$\log \sP(\theta)$ are sums of a $c_0$-strongly-log-concave
potential $\ell_-(\theta)$ or $\tilde \ell_-(\theta)$ and a
$R|c_0-c_1|$-Lipschitz perturbation $\ell_+(\theta)$. Then
\cite[Lemma 2.1]{bardet2018functional} shows that both laws satisfy a LSI
with constant $C_\LSI=(4/c_0)\exp(8R^2(c_0-c_1)^2/(\pi c_0))$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:LSI}]
The prior LSI (\ref{eq:LSIprior}) has been shown in Lemma
\ref{lemma:univariateLSI}. For the posterior LSI (\ref{eq:LSI}), note
that under condition (a), the posterior density is strongly
log-concave, satisfying
\[{-}\nabla^2 \log \sP_g(\btheta \mid \X,\y)
=\frac{1}{\sigma^2}\X^\top \X-\diag\Big((\log g)''(\theta_j)\Big)_{j=1}^d
\succeq c_0\I.\]
Hence (\ref{eq:LSI}) with $C_{\LSI}=2/c_0$
follows from the Bakry-Emery criterion.

We proceed to show (\ref{eq:LSI}) under condition (b). The proof is an
adaptation of the argument of
\cite{bauerschmidt2019very}; see also \cite[Theorem 3.4]{fan2023gradient}
and \cite{montanari2024provably} for similar specializations to
the linear model. By the Bai-Yin law (\cite[Theorem 3.1]{yin1988limit}),
for any $\eps>0$,
\[(\sqrt{\delta}-1)_+^2-\eps \leq \lambda_{\min}(\X^\top \X) 
\leq \lambda_{\max}(\X^\top \X) \leq (\sqrt{\delta}+1)^2+\eps\]
a.s.\ for all large $n,d$ (where $\delta=\lim n/d$). Thus, choosing some
sufficiently small $\eps>0$ and setting
\[\kappa=(\sqrt{\delta}-1)_+^2-2\eps,
\quad
\tau^2=\sigma^2\Big([(\sqrt{\delta}+1)^2-(\sqrt{\delta}-1)_+^2+3\eps]^{-1}-\eps
\Big),
\quad \bSigma=\sigma^2(\X^\top\X-\kappa\,\I)^{-1}-\tau^2\,\I,\]
we have $\X^\top\X-\kappa\,\I \succeq \eps\,\I$,
$(\X^\top\X-\kappa\,\I)^{-1} \succeq (\frac{\tau^2}{\sigma^2}+\eps)\,\I$, and
hence $\bSigma \succ 0$ a.s.\ for all large $n,d$.
Since $\sigma^2(\X^\top\X-\kappa\,\I)^{-1}=\bSigma+\tau^2\I$,
we have the Gaussian convolution identity
\[e^{-\frac{1}{2\sigma^2}\btheta^\top (\X^\top \X-\kappa\I)\btheta}
\propto \int e^{-\frac{1}{2\tau^2}\|\btheta-\bvarphi\|_2^2}
e^{-\frac{1}{2}\bvarphi^\top \bSigma^{-1} \bvarphi}\d\bvarphi\]
Then the posterior density $\sP_g(\btheta \mid \X,\y)$
satisfies
\begin{align*}
\sP_g(\btheta \mid \X,\y) &\propto \exp\Big({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|^2\Big)
\prod_{j=1}^d g(\theta_j)\\
&\propto
\exp\Big({-}\frac{1}{2\sigma^2}\btheta^\top(\X^\top\X-\kappa\I)\btheta\Big)
\prod_{j=1}^d
g(\theta_j)\exp\Big({-}\frac{\kappa}{2\sigma^2}\theta_j^2+\frac{\x_j^\top\y}{\sigma^2}\theta_j\Big)\\
&\propto \int e^{-\frac{1}{2}\bvarphi^\top \bSigma^{-1}\bvarphi}
\prod_{j=1}^d g(\theta_j)\exp\Big({-}\frac{\kappa}{2\sigma^2}\theta_j^2
-\frac{1}{2\tau^2}(\theta_j-\varphi_j)^2+\frac{\x_j^\top
\y}{\sigma^2}\theta_j\Big)\d\bvarphi.
\end{align*}
Defining
\begin{align*}
q_{\varphi_j}(\theta_j)&=\frac{1}{Z_j(\varphi_j)}
g(\theta_j)\exp\Big({-}\frac{\kappa}{2\sigma^2}\theta_j^2
-\frac{1}{2\tau^2}(\theta_j-\varphi_j)^2+\frac{\x_j^\top
\y}{\sigma^2}\theta_j\Big),\\
Z_j(\varphi_j)&=\int g(\theta_j)\exp\Big({-}\frac{\kappa}{2\sigma^2}\theta_j^2
-\frac{1}{2\tau^2}(\theta_j-\varphi_j)^2+\frac{\x_j^\top
\y}{\sigma^2}\theta_j\Big)\d\theta_j,\\
\mu(\bvarphi)&=\frac{
e^{-\frac{1}{2}\bvarphi^\top\bSigma^{-1}\bvarphi}\prod_{j=1}^d Z_j(\varphi_j)}
{\int e^{-\frac{1}{2}{\bvarphi'}^\top\bSigma^{-1}\bvarphi'}
\prod_{j=1}^d Z_j(\varphi_j')\d\bvarphi'}
\end{align*}
this gives the mixture-of-products representation
\[\sP_g(\btheta \mid \X,\y)=\int \underbrace{\prod_{j=1}^d
q_{\varphi_j}(\theta_j)}_{:=q_{\bvarphi}(\btheta)}
\mu(\bvarphi) \d\bvarphi.\]
Then for any $f \in C^1(\R^d)$,
\begin{equation}\label{eq:entdecomp}
\Ent[f(\btheta)^2 \mid \X,\y]=\E_{\bvarphi \sim \mu} \Ent_{\btheta \sim
q_{\bvarphi}}f(\btheta)^2+\Ent_{\bvarphi \sim \mu} \E_{\btheta \sim
q_{\bvarphi}}f(\btheta)^2.
\end{equation}

For the first term of (\ref{eq:entdecomp}),
note that inside the exponential defining $q_{\varphi_j}(\theta_j)$ we have
$\kappa \geq -2\eps$ and $\tau^2 \leq \sigma^2((1+3\eps)^{-1}-\eps)$, so
the coefficient of $\theta_j^2$ is negative for sufficiently
small $\eps>0$. Then
by Lemma \ref{lemma:univariateLSI}, $q_{\varphi_j}(\theta_j)$ satisfies
the univariate LSI (\ref{eq:univariateLSI}) with constant
$C_\LSI:=(4/c_0)\exp(8R^2(c_0-c_1)^2/(\pi c_0))$. So the product law
$q_{\bvarphi}$ satisfies LSI with the same constant by tensorization, and
\begin{equation}\label{eq:entdecompbound1}
\E_{\bvarphi \sim \mu} \Ent_{\btheta \sim q_{\bvarphi}}f(\btheta)^2
\leq C_\LSI\,\E_{\bvarphi \sim \mu} \E_{\btheta \sim q_{\bvarphi}}
\|\nabla f(\btheta)\|_2^2=C_\LSI\,\E_{\btheta \sim q} \|\nabla f(\btheta)\|_2^2.
\end{equation}

For the second term of (\ref{eq:entdecomp}), note that
\begin{align*}
{-}\nabla_{\bvarphi}^2 \log \mu(\bvarphi)
=\bSigma^{-1}-\diag\Big((\log Z_j)''(\varphi_j)\Big)_{j=1}^d
=\bSigma^{-1}
+\diag\Big(\frac{1}{\tau^2}-\frac{1}{\tau^4}\Var_{\theta_j \sim
q_{\varphi_j}}[\theta_j]\Big)_{j=1}^d.
\end{align*}
The LSI for $q_{\varphi_j}$ implies
$\Var_{\theta_j \sim q_{\varphi_j}}[\theta_j] \leq (C_\LSI/2)$ by its implied
Poincar\'e inequality. Applying the given condition (\ref{eq:sigma0condition})
and $4\max(1,\sqrt{\delta}) \geq (\sqrt{\delta}+1)^2-(\sqrt{\delta}-1)_+^2$
for all $\delta>0$, we see that for a sufficiently small
choice of $\eps>0$, we have $\tau^2 \geq C_\LSI/[2(1-\eps)]$. Then this gives
${-}\nabla_{\bvarphi}^2 \log \mu(\bvarphi) \succeq (\eps/\tau^2)\I$.
Then by the Bakry-Emery criterion, $\mu$ satisfies the LSI $\Ent_{\bvarphi \sim
\mu} f(\bvarphi)^2 \leq (2\tau^2/\eps)\E_{\bvarphi \sim \mu}\|\nabla
f(\bvarphi)\|_2^2$, hence
\[\Ent_{\bvarphi \sim \mu} \E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2 \leq \frac{2\tau^2}{\eps}\,
\E_{\bvarphi \sim \mu} \|\nabla_{\bvarphi} (\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2)^{1/2}\|_2^2.\]
Denote by $q_{\bvarphi^{-j}}$ the product of components of $q_{\bvarphi}$
other than the $j^\text{th}$. We compute
\[\partial_{\varphi_j} (\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2)^{1/2}
=\frac{\partial_{\varphi_j}\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2}
{2(\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2)^{1/2}}
=\frac{\E_{\btheta^{-j} \sim q_{\bvarphi^{-j}}} \partial_{\varphi_j}\E_{\theta_j
\sim q_{\varphi_j}}f(\btheta)^2}{2(\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2)^{1/2}}
=\frac{\E_{\btheta^{-j} \sim q_{\bvarphi^{-j}}}
\Cov_{\theta_j \sim q_{\varphi_j}}[f(\btheta)^2,\theta_j]}
{2\tau^2(\E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2)^{1/2}}.\]
We apply \cite[Proposition 2.2]{ledoux2001logarithmic}:
For any law $\nu$ on $\R^d$ satisfying a LSI $\Ent_\nu f^2 \leq C_\LSI\,\E_\nu
\|\nabla f\|_2^2$, and for any smooth functions $f,g:\R^d \to \R$,
\[\Cov_\nu[f^2,g] \leq C \sup_{\btheta \in \R^d} \|\nabla g(\btheta)\|_2
\cdot (\E_\nu f^2)^{1/2}(\E_\nu \|\nabla f\|_2^2)^{1/2}\]
where $C$ depends only on the LSI constant $C_\LSI$ of $\nu$.
Applying this to the univariate law $\nu=q_{\varphi_j}$, followed by
Cauchy-Schwarz,
\[\E_{\btheta^{-j} \sim q_{\bvarphi^{-j}}} \Cov_{\theta_j \sim
q_{\varphi_j}}[f(\btheta)^2,\theta_j]
\leq C_1(\E_{\btheta \sim q_{\bvarphi}}f(\btheta)^2)^{1/2}(\E_{\btheta \sim
q_{\bvarphi}}(\partial_{\theta_j} f(\btheta))^2)^{1/2}\]
where $C_1$ depends only on the LSI constant $C_\LSI$ for $q_{\varphi_j}$. 
Summing over $j=1,\ldots,d$ gives
\begin{align*}
\|\nabla_{\bvarphi} (\E_{\btheta \sim q_{\bvarphi}}f(\btheta)^2)^{1/2}\|_2^2
&=\sum_{j=1}^d\big[\partial_{\varphi_j} (\E_{\btheta \sim q_{\bvarphi}}
f(\btheta)^2))^{1/2}\big]^2 \\
&\leq \sum_{j=1}^d \Big(\frac{C_1}{2\tau^2}\Big)^2
\E_{\btheta \sim q_{\bvarphi}}(\partial_{\theta_j} f(\btheta))^2
=\Big(\frac{C_1}{2\tau^2}\Big)^2 \E_{\btheta \sim
q_{\bvarphi}} \|\nabla f(\btheta)\|_2^2.
\end{align*}
Thus
\begin{equation}\label{eq:entdecompbound2}
\Ent_{\bvarphi \sim \mu} \E_{\btheta \sim q_{\bvarphi}} f(\btheta)^2
\leq \frac{2\tau^2}{\eps}
\Big(\frac{C_1}{2\tau^2}\Big)^2
\E_{\btheta \sim \mu} \E_{\btheta \sim q_{\bvarphi}} \|\nabla f(\btheta)\|_2^2
=\frac{C_1^2}{2\eps\tau^2} \E[\|\nabla f(\btheta)\|_2^2 \mid \X,\y].
\end{equation}
Applying (\ref{eq:entdecompbound1}) and (\ref{eq:entdecompbound2}) to
(\ref{eq:entdecomp}) completes the proof of (\ref{eq:LSI}), for a combined
log-Sobolev constant $C_\LSI'=C_\LSI+C_1^2/(2\eps \tau^2)$.
\end{proof}

\subsection{Properties of the correlation and response}

For constants $C_0,C_\LSI>0$, define the $(\X,\y)$-dependent event 
\begin{align}\label{eq:good_event}
\event(C_0,C_\LSI)=\Big\{\|\X\|_\op \leq C_0,\quad
\|\y\|_2^2 \leq C_0d,\quad
\Ent_{\btheta \sim q}f(\btheta)^2 \leq C_\LSI\,\E_{\btheta \sim q} \|\nabla
f(\btheta)\|^2 \text{ for all }
f \in C^1(\R^d)\Big\}.
\end{align}
Fixing $\X,\y$, recall the coordinate functions from (\ref{eq:coordfuncs})
\[e_j(\btheta)=\theta_j,
\qquad x_i(\btheta)=\frac{\sqrt{\delta}}{\sigma^2}([\X\btheta]_i-y_i)\]
and their associated correlation and response matrices
(\ref{eq:matrixcorrresponse}). In light of (\ref{eq:responsenonadaptive}) and
the definition of the Markov semigroup $\{P_t\}_{t \geq 0}$, these take the form
\[
\begin{gathered}
\bC_\theta(t,s)=\Big(\big\langle e_k(\btheta^s)P_{t-s}e_j(\btheta^s) \big\rangle
\Big)_{j,k=1}^d, \qquad
\bC_\eta(t,s)=\Big(\big\langle x_k(\btheta^s)P_{t-s}x_j(\btheta^s) \big\rangle
\Big)_{j,k=1}^n,\\
\bR_\theta(t,s)=\Big(\big\langle \nabla e_k(\btheta^s)^\top \nabla P_{t-s}
e_j(\btheta^s) \big\rangle\Big)_{j,k=1}^d,
\qquad
\bR_\eta(t,s)=\Big(\langle
\nabla x_k(\btheta^s)^\top \nabla P_{t-s}x_j(\btheta^s) \big\rangle
\Big)_{j,k=1}^n.
\end{gathered}\]
We proceed to show approximate time-translation invariance at large times
for $\bC_\theta,\bC_\eta,\bR_\theta,\bR_\eta$ on the event $\event(C_0,C_\LSI)$.

We recall our shorthand $\langle f(\btheta) \rangle=\E_{\btheta \sim q}
f(\btheta)$ for the posterior expectation.
We first record the following elementary bounds under the event
$\event(C_0,C_\LSI)$. All constants throughout this section
are independent of the dimension $(n,d)$ and
depend only on $C_0,C_{\text{LSI}}$, $\delta,\sigma^2$ and the fixed
prior $g(\cdot)$.

\begin{lemma}\label{lemma:elementarybounds}
Suppose Assumptions \ref{assump:prior} and \ref{assump:LSI}
hold for a fixed prior $g(\cdot)$. Then on the event
$\event(C_0,C_\LSI)$, there exist constants $C,L>0$ for which
\begin{equation}\label{eq:posteriormeansq}
\langle \|\btheta\|_2^2 \rangle \leq Cd, \qquad \langle \|\nabla \log
q(\btheta)\|_2^2 \rangle \leq Cd,
\end{equation}
\begin{equation}\label{eq:negativeCD}
\|\nabla^2 \log q(\btheta)\|_\mathrm{op} \leq L,
\end{equation}
\begin{equation}\label{eq:thirdder}
\|(\log g)'''\|_\infty \leq L.
\end{equation}
\end{lemma}
\begin{proof}
(\ref{eq:negativeCD}--\ref{eq:thirdder}) are immediate from the form of $\log
q$, the bound $\|\X\|_\op \leq C_0$, and Assumption \ref{assump:prior}.

For (\ref{eq:posteriormeansq}), write $\E_g,\P_g$ for the expectation
and probability over $\theta \sim g$ and $\theta_j \overset{iid}{\sim} g$.
Write $C,C',c>0$ for ($g$-dependent) constants changing from instance to
instance. Denoting
$\|\theta\|_{\psi_2}:=\inf\{K>0:\E_g e^{\theta^2/K^2} \leq 2\}$
the subgaussian norm of $\theta \sim g$, we have
$\|\theta\|_{\psi_2} \leq \|\E_g
\theta\|_{\psi_2}+\|\theta-\E_g\theta\|_{\psi_2}$ which 
is bounded above by a constant depending on $C_\LSI$ and $\E_g \theta$
under the LSI for $g$ in Assumption \ref{assump:LSI}(a).
Then (c.f.\ \cite[Eq.\ (3.1)]{vershynin2018high})
\begin{equation}\label{eq:priortail}
\E_g\|\btheta\|_2^2 \leq Cd,
\qquad \P_g[\|\btheta\|_2^2-\E_g\|\btheta\|_2^2 \geq d]
\leq Ce^{-cd\min(u^2,u)} \text{ for all } u \geq 0.
\end{equation}
Write
\[q(\btheta)=\frac{1}{Z}\exp\bigg({-}\frac{\|\y-\X\btheta\|_2^2}{2\sigma^2}\bigg)
\prod_{j=1}^d g(\theta_j),
\qquad Z=\E_g
\bigg[\exp\bigg({-}\frac{\|\y-\X\btheta\|_2^2}{2\sigma^2}\bigg)\bigg].\]
We have by Jensen's inequality
${-}\log Z \leq \E_g[\|\y-\X\btheta\|_2^2/2\sigma^2]
\leq C(d+\E_g \|\btheta\|_2^2)
\leq C'd$. Then for any $M>0$, also bounding the
exponential from above by 1,
\[\Big\langle\|\btheta\|_2^2 \1\{\|\btheta\|_2^2 \geq Md\}\Big\rangle
\leq \frac{1}{Z}\,\E_g\Big[\|\btheta\|_2^2 \1\{\|\btheta\|_2^2 \geq Md\}\Big]
\leq e^{C'd}\E_g\Big[\|\btheta\|_2^2 \1\{\|\btheta\|_2^2 \geq Md\}\Big].\]
Integrating the tail bound (\ref{eq:priortail}) shows this is less than $d$
for a sufficiently large constant $M>0$, and thus
\[\langle \|\btheta\|_2^2 \rangle
\leq Md+\Big \langle \|\btheta\|_2^2 \1\{\|\btheta\|_2^2 \geq Md\} \Big\rangle
\leq (M+1)d.\]
This shows the first statement of (\ref{eq:posteriormeansq}). Since
$\nabla \log q(\btheta)$ is $L$-Lipschitz by (\ref{eq:negativeCD}), and
$\|\nabla \log q(0)\|_2^2 \leq 2\|\X^\top\y/2\sigma^2\|_2^2
+2d \cdot (\log g)'(0)^2 \leq Cd$, the second statement of
(\ref{eq:posteriormeansq}) follows from the first.
\end{proof}

\begin{lemma}\label{lem:W2contraction}
Suppose Assumptions \ref{assump:prior} and \ref{assump:LSI}
hold for a fixed prior $g(\cdot)$. 
Let $\{\btheta^t\}_{t \geq 0}$ be the solution to (\ref{eq:langevin_sde}) with
any initialization $\btheta^0 \sim q_0$,
and let $q_t$ be the law of $\btheta^t$ conditional on $(\X,\y)$.
Then on the event $\event(C_0,C_\LSI)$,
there exists a constant $C>0$ such that
\begin{equation}\label{eq:W2decay}
W_2(q_t,q) \leq Ce^{-(2/C_\LSI)t}
\,W_2(q_0,q) \text{ for all } t \geq 0.
\end{equation}
\end{lemma}
\begin{proof}
For $t \in [0,1]$ we may apply a simple synchronous coupling and
Gr\"onwall argument: Let $\{\btheta^t\}_{t \geq 0}$ and
$\{\tilde\btheta^t\}_{t \geq 0}$ be the solutions of (\ref{eq:langevin_sde})
with initial conditions $\btheta^0$ and $\tilde\btheta^0 \sim q$,
coupled by the same Brownian motion. Then
$\frac{\d}{\d t}\|(\btheta^t-\tilde\btheta^t)\|_2 \leq \|\tfrac{\d}{\d t}(\btheta^t-\tilde\btheta^t)\|_2
=\|\nabla \log q(\btheta^t)-\nabla \log q(\tilde \btheta^t)\|_2
\leq L\|\btheta^t-\tilde \btheta^t\|_2$ by definition
of the Langevin equation (\ref{eq:langevin_sde}) and by (\ref{eq:negativeCD}).
Hence
\begin{equation}\label{eq:thetadiffbound}
\|\btheta^t-\tilde\btheta^t\|_2
\leq e^{Lt}\|\btheta^0-\tilde\btheta^0\|_2.
\end{equation}
Letting $(\btheta^0,\tilde\btheta^0)$ be the coupling of $(q_0,q)$ for which
$\E[\|\btheta^0-\tilde\btheta^0\|_2^2 \mid \X,\y]=W_2(q_0,q)^2$, we have that
$(\btheta^t,\tilde\btheta^t)$ is a coupling of $(q_t,q)$, so
\[W_2(q_t,q)^2 \leq \E[\|\btheta^t-\tilde\btheta^t\|_2^2 \mid \X,\y]
\leq e^{2Lt}\E[\|\btheta^0-\tilde \btheta^0\|_2^2 \mid \X,\y]
=e^{2Lt}W_2(q_0,q)^2.\]
Thus $W_2(q_t,q) \leq e^L W_2(q_0,q)$ for all $t \in [0,1]$, which implies
(\ref{eq:W2decay}) for $t \in [0,1]$ and some $C>0$.

For $t \geq 1$, under the curvature-dimension lower bound
$-\nabla^2 \log q(\btheta) \succeq {-}L\operatorname{Id}$
implied by (\ref{eq:negativeCD}), we recall from \cite[Lemma
4.2]{bobkov2001hypercontractivity} that
\begin{equation}\label{eq:smoothing}
\DKL(q_1\|q) \leq \left(\frac{1}{4\alpha}+\frac{L}{2}\right)
W_2(q_0,q)^2, \qquad \alpha=\frac{e^{2L}-1}{2L}.
\end{equation}
Under the LSI condition of $\event(C_0,C_\LSI)$,
we have the exponential contraction of
relative entropy (c.f.\ \cite[Theorem 5.2.1]{bakry2014analysis})
\begin{equation}\label{eq:entropycontraction}
\DKL(q_t\|q) \leq e^{-2(t-1)/C_\LSI}\DKL(q_1\|q)
\text{ for all } t \geq 1.
\end{equation}
We have also the $T_2$-transportation inequality
(c.f.\ \cite[Theorem 9.6.1]{bakry2014analysis})
\begin{equation}\label{eq:T2}
W_2(q_t,q)^2 \leq C_\LSI\,\DKL(q_t\|q),
\end{equation}
and (\ref{eq:W2decay}) for $t \geq 1$ follows
follows from combining (\ref{eq:smoothing}), (\ref{eq:entropycontraction}), and
(\ref{eq:T2}).
\end{proof}

The following lemma now establishes approximate time-translation invariance of
$\bC_\theta,\bC_\eta,\bR_\theta,\bR_\eta$.

\begin{lemma}\label{lemma:TTI}
Suppose Assumptions \ref{assump:prior} and \ref{assump:LSI}
hold with a fixed prior $g(\cdot)$.
Let $\{\btheta^t\}_{t \geq 0}$ be the solution to (\ref{eq:langevin_fixedq})
with a fixed initialization $\btheta^0 \in \R^d$ satisfying $\|\btheta^0\|_2^2
\leq C_0d$, and set
\[\begin{gathered}
\bC_\theta^\infty(\tau)=\Big(\big\langle e_k(\btheta)P_\tau e_j(\btheta) \rangle
\Big)_{j,k=1}^d,\qquad
\bC_\eta^\infty(\tau) = \Big(\big\langle x_k(\btheta)
P_\tau x_j(\btheta) \big\rangle \Big)_{j,k=1}^n,\\
\qquad \bR_\theta^\infty(\tau)=\Big(\big\langle \nabla e_k(\btheta)^\top \nabla P_\tau
e_j(\btheta)\big\rangle\Big)_{j,k=1}^d,
\qquad \bR_\eta^\infty(\tau) = \Big(\big\langle \nabla x_k(\btheta)^\top
\nabla P_\tau x_j(\btheta)\big\rangle\Big)_{j,k=1}^n
\end{gathered}\]
where $\langle \cdot \rangle$ denotes expectation under the posterior law
$q(\cdot)$ of (\ref{eq:qshorthand}).
Then on the event $\event(C_0,C_\LSI)$, there exist constants $C,c>0$
such that for all $t \geq s \geq 0$,
\begin{align}
|\Tr \bC_\theta(t,s)-\Tr \bC_\theta^\infty(t-s)|
&\leq Cde^{-cs}\label{eq:Cthetacompare}\\
|\Tr \bR_\theta(t,s)-\Tr \bR_\theta^\infty(t-s)|
&\leq Cde^{-cs}\label{eq:Rthetacompare}\\
|\Tr \bC_\eta(t,s)-\Tr \bC_\eta^\infty(t-s)|
&\leq Cde^{-cs}\label{eq:Cetacompare}\\
|\Tr \bR_\eta(t,s)-\Tr \bR_\eta^\infty(t-s)|
&\leq Cde^{-cs}\label{eq:Retacompare}
\end{align}
\end{lemma}

\begin{proof}
We write $C,C',c,c'>0$ for constants that may change from instance to instance. 

Let $q_t$ be the law of $\btheta^t$ conditional on $(\X,\y)$ with a
fixed initial condition $\btheta^0=\x$. For any fixed $t \geq 0$, denote by
$\bvarphi^t \sim q$ a random vector such that
$(\btheta^t,\bvarphi^t)$ is a coupling of $(q_t,q)$ for which
$\langle \|\btheta^t-\bvarphi^t\|_2^2 \rangle=W_2(q_t,q)^2$.
Then observe that for any $M$-Lipschitz function $f$, we have
\begin{equation}\label{eq:Lipschitzcouplingbound}
\langle \|f(\btheta^t)-f(\bvarphi^t)\|_2^2 \rangle \leq
M^2\langle \|\btheta^t-\bvarphi^t\|_2^2\rangle =M^2W_2(q_t,q)^2.
\end{equation}
Furthermore $W_2(q_t,q)^2 \leq Ce^{-ct}W_2(\delta_\x,q)^2
\leq 2Ce^{-ct}(\|\x\|_2^2+\langle \|\btheta\|_2^2 \rangle)$
for all $t \geq 0$ by Lemma \ref{lem:W2contraction}.
Then, applying (\ref{eq:Lipschitzcouplingbound})
with $f(\x)=\x$ and $f(\x)=\nabla \log q(\x)$ and
(\ref{eq:posteriormeansq}--\ref{eq:negativeCD}) on the event
$\event(C_0,C_\LSI)$, we have the basic estimates
\begin{equation}\label{eq:W2contraction}
\begin{gathered}
\langle \|\btheta^t-\bvarphi^t\|_2^2\rangle \leq Ce^{-ct}(\|\x\|_2^2+d),
\quad \langle \|\nabla \log q(\btheta^t)-\nabla \log q(\bvarphi^t)\|_2^2\rangle
 \leq Ce^{-ct}(\|\x\|_2^2+d),\\
\langle \|\btheta^t\|_2^2\rangle \leq C(\|\x\|_2^2+d),
\quad \langle \|\nabla \log q(\btheta^t)\|_2^2\rangle \leq
C(\|\x\|_2^2+d)\\
\langle \|\bvarphi^t\|_2^2 \rangle=\langle \|\btheta\|_2^2 \rangle \leq Cd,
\quad \langle \|\nabla \log q(\bvarphi^t)\|_2^2 \rangle
=\langle \|\nabla \log q(\btheta)\|_2^2\rangle \leq Cd.
\end{gathered}
\end{equation}
We note that also
\begin{align}
\|P_t(\x)-P_t(\tilde\x)\|_2^2 &\leq e^{2Lt}\|\x-\tilde\x\|_2^2,\label{eq:PtLipschitz}\\
\|P_t(\x)-P_t(\tilde\x)\|_2^2 &\leq Ce^{-ct}(\|\x\|_2^2+\|\tilde\x\|_2^2+d).\label{eq:Ptlongtime}
\end{align}
Indeed, (\ref{eq:PtLipschitz}) follows from (\ref{eq:thetadiffbound}) and
Jensen's inequality. Also by Jensen's inequality and (\ref{eq:W2contraction}),
\begin{align}\label{eq:mean_concentrate}
\|P_t(\x)-\langle \btheta \rangle\|_2^2=\|\langle \btheta^t
-\bvarphi^t \rangle\|_2^2 \leq Ce^{-ct}(\|\x\|_2^2+d),
\end{align}
and applying this bound for
both $P_t(\x)$ and $P_t(\tilde\x)$ yields (\ref{eq:Ptlongtime}).

For (\ref{eq:Cthetacompare}), note that for any $s,\tau \geq 0$,
\begin{equation}\label{eq:Cthetasemigroupform}
\Tr \bC_\theta(s+\tau,s)
=\sum_{j=1}^d \langle e_j(\btheta^s)P_\tau e_j(\btheta^s) \rangle.
\end{equation}
Let $q_s$ be the law of $\btheta^s$ conditional on $(\X,\y)$
with the given initial condition $\btheta^0$ satisfying $\|\btheta^0\|_2^2 \leq
C_0d$, and let
$(\btheta^s,\bvarphi^s)$ be the optimal Wasserstein-2 coupling of $(q_s,q)$
as above. Then
\begin{align}
|\Tr \bC_\theta(s+\tau,s)-\Tr \bC_\theta^\infty(\tau)|
&\leq \sum_{j=1}^d \big\langle\big|e_j(\btheta^s)P_\tau e_j(\btheta^s)
-e_j(\bvarphi^s)P_\tau e_j(\bvarphi^s)\big|\big\rangle\notag\\
&\leq \sum_{j=1}^d \big\langle\big|(\theta_j^s-\varphi_j^s)P_\tau
e_j(\btheta^s)\big|\big\rangle
+\big\langle\big|\varphi_j^s(P_\tau e_j(\btheta^s)-P_\tau
e_j(\bvarphi^s))\big|\big\rangle\notag\\
&\leq \underbrace{\big\langle \|\btheta^s-\bvarphi^s\|_2^2\big\rangle^{1/2}
\big\langle\|P_\tau(\btheta^s)\|_2^2\big\rangle^{1/2}}_{\mathrm{I}}
+\underbrace{\big\langle\|\bvarphi^s\|_2^2\big\rangle^{1/2}
\big\langle\|P_\tau(\btheta^s)-P_\tau(\bvarphi^s)\|_2^2\big\rangle^{1/2}}_{\mathrm{II}}
\label{eq:Cthetacomparedecomp}
\end{align}
where we write as shorthand
$P_t(\x)=\langle\btheta^t \rangle_{\btheta^0=\x}
=(P_t e_1,\ldots,P_t e_d)[\x] \in \R^d$.

We have $\mathrm{I} \leq Cde^{-cs}$ for all $s \geq 0$ by
(\ref{eq:W2contraction}) and 
$\langle \|P_\tau(\btheta^s)\|_2^2 \rangle \leq \langle
\|\btheta^{s+\tau}\|_2^2 \rangle$
which follows from Jensen's inequality. For $\mathrm{II}$,
by (\ref{eq:PtLipschitz}) and (\ref{eq:W2contraction}), we have
\[\big\langle\|P_\tau(\btheta^s)-P_\tau(\bvarphi^s)\|_2^2 \big\rangle
\leq e^{2L\tau}\langle \|\btheta^s-\bvarphi^s\|_2^2 \rangle
\leq e^{2L\tau} \cdot Cde^{-cs}.\]
Choosing a large enough constant $s_0>0$, for $\tau \leq s/s_0$, this gives
$\langle \|P_\tau(\btheta^s)-P_\tau(\bvarphi^s)\|_2^2 \rangle \leq C'de^{-c's}$.
For $\tau>s/s_0$, applying instead
(\ref{eq:Ptlongtime}) and (\ref{eq:W2contraction}), we have
$\langle \|P_\tau(\btheta^s)-P_\tau(\bvarphi^s)\|_2^2 \rangle
\leq Ce^{-c\tau}(\langle \|\btheta^s\|_2^2 \rangle+\langle \|\bvarphi^s\|_2^2
\rangle+d) \leq C'de^{-c's}$. Thus, for some $C,c>0$,
\[\big\langle\|P_\tau(\btheta^s)-P_\tau(\bvarphi^s)\|_2^2 \big\rangle
\leq Cde^{-cs} \text{ for all } s,\tau \geq 0.\]
Thus also $\mathrm{II} \leq Cde^{-cs}$, and applying these bounds for
$\mathrm{I}$ and $\mathrm{II}$ to (\ref{eq:Cthetacomparedecomp})
shows (\ref{eq:Cthetacompare}).

For (\ref{eq:Rthetacompare}), note that
\begin{equation}\label{eq:Rthetaform}
\Tr \bR_\theta(s+\tau,s)=\sum_{j=1}^d \langle (\partial_j P_\tau
e_j)[\btheta^s]\rangle,
\qquad \Tr \bR_\theta^\infty(\tau)=\sum_{j=1}^d \langle (\partial_j P_\tau
e_j)[\btheta] \rangle.
\end{equation}
Let $\d P_t(\x) \in \R^{d\times d}$ be the Jacobian of the vector map
$\x \mapsto P_t(\x)$. By (\ref{eq:BEL1}) of Lemma \ref{lemma:BEL} applied
with $f=e_j$ for each $j=1,\ldots,d$, we have
\begin{equation}\label{eq:Ptjac1}
\d P_t(\x) = \langle \V^t \rangle_{\btheta^0=\x}
\end{equation}
where $\{\btheta^t,\V^t\}_{t \geq 0}$ is the solution of
(\ref{eq:matrixV_sde}) with initial condition $(\btheta^0,\V^0)=(\x,\I)$.
For $t \geq 1$, let us write also $\nabla P_t e_j(\x)=\nabla P_1 f(\x)$ with
$f=P_{t-1}e_j$. Noting that $f \in \cA$
by Proposition \ref{prop:langevinsolution}(c),
we may apply (\ref{eq:BEL2}) of Lemma \ref{lemma:BEL} with this $f$.
Doing so for each $j=1,\ldots,d$ gives
\begin{align}\label{eq:Ptjac2}
\d P_t(\x) = \frac{1}{\sqrt{2}}
\bigg\langle P_{t-1}(\btheta^1) \bigg(\int_0^1 (\V^s)^\top \d
\b^s\bigg)^\top\bigg\rangle_{\btheta^0=\x} \text{ for } t \geq 1.
\end{align}
In particular,
\begin{equation}\label{eq:tracePtjac}
\sum_{j=1}^d (\partial_j P_\tau e_j)[\x]
=\langle \Tr \V^\tau \rangle_{\btheta^0=\x}=\frac{1}{\sqrt{2}}
\bigg\langle P_{\tau-1}(\btheta^1)^\top \int_0^1 (\V^s)^\top \d
\b^s\bigg\rangle_{\btheta^0=\x}
\end{equation}
with the second equality holding for $\tau \geq 1$.

Now let $\{\btheta^t,\V^t\}_{t \geq 0}$ and $\{\tilde\btheta^t,\tilde \V^t\}_{t
\geq 0}$ be the solutions to (\ref{eq:matrixV_sde})
with initial conditions $(\btheta^0,\V^0)=(\x,\I)$ and
$(\tilde \btheta^0,\tilde \V^0)=(\tilde\x,\I)$,
coupled by the same Brownian motion $\{\b^t\}_{t \geq 0}$. By the form of
(\ref{eq:matrixV_sde}) and by (\ref{eq:negativeCD}),
$\frac{\d}{\d t}\|\V^t\|_\op
\leq \|\nabla^2 \log q(\btheta^t) \cdot \V^t\|_\op
\leq L\|\V^t\|_\op$, so
\begin{align}\label{eq:V_op_bound}
\|\V^t\|_\op \leq e^{Lt}\|\V^0\|_\op=e^{Lt}.
\end{align}
Then also
\begin{align*}
\frac{\d}{\d t}\|\V^t-\tilde\V^t\|_F &\leq
\|[\nabla^2 \log q(\btheta^t)-\nabla^2 \log q(\tilde \btheta^t)]\V^t\|_F
+\|[\nabla^2 \log q(\tilde \btheta^t)](\V^t-\tilde \V^t)\|_F\\
&\leq \|\nabla^2 \log q(\btheta^t)-\nabla^2 \log q(\tilde \btheta^t)\|_F
\|\V^t\|_\op+\|\nabla^2 \log q(\tilde \btheta^t)\|_\op \|\V^t-\tilde\V^t\|_F.
\end{align*}
Applying $\nabla^2 \log q(\btheta^t)-\nabla^2 \log q(\tilde \btheta^t)
=\diag((\log q)''(\theta^t_j)-(\log q)''(\tilde \theta^t_j))$,
(\ref{eq:negativeCD}-\ref{eq:thirdder}), and (\ref{eq:thetadiffbound}),
\[\frac{\d}{\d t}\|\V^t-\tilde\V^t\|_F 
\leq L\|\btheta^t-\tilde\btheta^t\|_2\|\V^t\|_\op
+L\|\V^t-\tilde\V^t\|_F
\leq Le^{Lt}\|\x-\tilde\x\|_2 \cdot e^{Lt}+L\|\V^t-\tilde\V^t\|_F.\]
Integrating this bound,
\[\|\V^t-\tilde\V^t\|_F \leq C\|\x-\tilde\x\|_2 \text{ for all } t \in [0,1].\]
So it follows from the first equality of (\ref{eq:tracePtjac})
that for $\tau \in [0,1]$,
\[\left|\sum_{j=1}^d \partial_j P_\tau e_j(\x)
-\partial_j P_\tau e_j(\tilde\x)\right|
=\Big|\big\langle \Tr (\V^\tau-\tilde \V^\tau) \big\rangle\Big|
\leq \sqrt{d}\,\big\langle \|\V^\tau-\tilde \V^\tau\|_F\big\rangle
\leq C\sqrt{d}\|\x-\tilde\x\|_2.\]
Hence by (\ref{eq:Rthetaform}) and (\ref{eq:W2contraction}), for $\tau \in [0,1]$,
\begin{align}\label{eq:response_bound_1}
|\Tr \bR_\theta(s+\tau,s)-\Tr \bR_\theta^\infty(\tau)|
\leq C\sqrt{d}\,\langle\|\btheta^s-\bvarphi^s\|_2 \rangle \leq C'de^{-cs}.
\end{align}
For $\tau \geq 1$, we apply instead the second equality of (\ref{eq:tracePtjac}) and Cauchy-Schwarz to obtain
\begin{align}\label{eq:response_bound_2}
\notag&\sqrt{2}\left|\sum_{j=1}^d \partial_j P_\tau e_j(\x)
-\partial_j P_\tau e_j(\tilde\x)\right|\\
\notag&\leq \bigg|\bigg\langle P_{\tau-1}(\btheta^1)^\top\int_0^1 (\V^s)^\top\d\b^s
-P_{\tau-1}(\tilde \btheta^1)^\top\int_0^1 (\tilde
\V^s)^\top\d\b^s\bigg\rangle\bigg|\\
\notag&\leq \Big\langle \Big\|P_{\tau-1}(\btheta^1)
-P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2 \Big\rangle^{1/2}
\bigg\langle \bigg\|\int_0^1 (\V^s)^\top\d\b^s\bigg\|_2^2\bigg\rangle^{1/2}+
\Big\langle \Big\|P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2 \Big\rangle^{1/2}
\bigg\langle \bigg\|\int_0^1
(\V^s-\tilde\V^s)^\top\d\b^s\bigg\|_2^2\bigg\rangle^{1/2}\\
\notag&=\Big\langle \Big\|P_{\tau-1}(\btheta^1)
-P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2 \Big\rangle^{1/2}
\bigg\langle \int_0^1 \|\V^s\|_F^2\d s\bigg\rangle^{1/2}+
\Big\langle \Big\|P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2 \Big\rangle^{1/2}
\bigg\langle \int_0^1 \|\V^s-\tilde\V^s\|_F^2\d s\bigg\rangle^{1/2}\\
&\leq C\sqrt{d}\Big\langle \Big\|P_{\tau-1}(\btheta^1)
-P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2 \Big\rangle^{1/2}
+C\|\x-\tilde\x\|_2\Big\langle \Big\|P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2
\Big\rangle^{1/2}.
\end{align}
Note that $\langle \|P_{\tau-1}(\tilde \btheta^1)\|_2^2 \rangle \leq \langle
\|\tilde \btheta^\tau\|_2^2 \rangle \leq C(\|\tilde\x\|_2^2+d)$ by (\ref{eq:W2contraction}).
Applying (\ref{eq:PtLipschitz}--\ref{eq:Ptlongtime}),
(\ref{eq:thetadiffbound}), and (\ref{eq:W2contraction}),
\begin{align*}
\Big\langle\Big\|P_{\tau-1}(\btheta^1)-P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2
\Big\rangle
&\leq e^{2L(\tau-1)}\langle \|\btheta^1-\tilde\btheta^1\|_2^2 \rangle
\leq Ce^{2L\tau}\|\x-\tilde\x\|_2^2 \text{ for all } \tau \geq 1,\\
\Big\langle \Big\|P_{\tau-1}(\btheta^1)-P_{\tau-1}(\tilde\btheta^1)\Big\|_2^2
\Big \rangle
&\leq Ce^{-c(\tau-1)}(\langle \|\btheta^1\|_2^2 \rangle+\langle
\|\tilde\btheta^1\|_2^2 \rangle+d)
\leq C'e^{-c\tau}(\|\x\|_2^2+\|\tilde\x\|_2^2+d) \text{ for all } \tau \geq 2.
\end{align*}
Choosing a large enough constant $s_0>0$, if $\tau \in [1,s/s_0]$, then we may
apply the former bound, (\ref{eq:W2contraction}), and Cauchy-Schwarz
to (\ref{eq:response_bound_2}) to get
\begin{align}\label{eq:response_bound_3}
|\Tr \bR_\theta(s+\tau,s)-\Tr \bR_\theta^\infty(\tau)|
&\leq \bigg\langle\bigg|\sum_{j=1}^d \partial_j P_\tau e_j(\btheta^s)
-\partial_j P_\tau e_j(\bvarphi^s)\bigg|\bigg\rangle\notag\\
&\leq Ce^{L\tau}\sqrt{d}\,\langle \|\btheta^s-\bvarphi^s\|_2 \rangle
+C\,\Big\langle\|\btheta^s-\bvarphi^s\|_2(\|\bvarphi^s\|_2+\sqrt{d})\Big\rangle\notag\\
&\leq C'd(e^{L\tau}+1)e^{-cs} \leq C''de^{-c's}.
\end{align}
If $\tau \geq s/s_0$, applying instead the latter bound to
(\ref{eq:response_bound_2}),
\begin{align}\label{eq:response_bound_4}
|\Tr \bR_\theta(s+\tau,s)-\Tr \bR_\theta^\infty(\tau)| &\leq
Ce^{-c\tau}\sqrt{d}\,\big(\langle
\|\btheta^s\|_2^2\rangle+\langle\|\bvarphi^s\|_2^2\rangle+d\big)^{1/2}
+C\,\Big\langle \|\btheta^s-\bvarphi^s\|_2(\|\bvarphi^s\|_2+\sqrt{d})\Big
\rangle\notag\\
&\leq C'de^{-c's}.
\end{align}
Combining these bounds for $\tau \in [0,1]$, $\tau \in [1,s/s_0]$, and
$\tau \geq s/s_0$ in (\ref{eq:response_bound_1}), (\ref{eq:response_bound_3}),
and (\ref{eq:response_bound_4}) shows (\ref{eq:Rthetacompare}).

The arguments for $\bC_\eta$ and $\bR_\eta$ in
(\ref{eq:Cetacompare}--\ref{eq:Retacompare}) are similar:
For (\ref{eq:Cetacompare}), recall the definitions (\ref{eq:coordfuncs})
and note that
\begin{align*}
&\Big|\Tr \bC_\eta(s+\tau,s) - \Tr \bC_\eta^\infty(\tau)\Big|\\
&\leq \sum_{i=1}^n \Big\langle\Big|x_i(\btheta^s)P_\tau
x_i(\btheta^s)-x_i(\bvarphi^s)P_\tau x_i(\bvarphi^s)\Big|\Big\rangle\\
&\leq \sum_{i=1}^n \Big\langle\Big|\big(x_i(\btheta^s) - x_i(\bvarphi^s)\big)
P_\tau x_i(\btheta^s)\Big|\Big\rangle + \Big\langle\Big|x_i(\bvarphi^s)\big(P_\tau x_i(\btheta^s) -
P_\tau x_i(\bvarphi^s)\big)\Big|\Big\rangle\\
&\leq \frac{\delta}{\sigma^4}\Big\langle \pnorm{\X(\btheta^s - \bvarphi^s)}{2}^2\Big\rangle^{1/2}
\Big\langle \pnorm{\X P_\tau (\btheta^s)-\y}{2}^2\Big\rangle^{1/2}
+\frac{\delta}{\sigma^4}\Big\langle \pnorm{\X\bvarphi^s-\y}{2}^2\Big\rangle^{1/2}
\Big\langle \pnorm{\X P_\tau (\btheta^s) - \X P_\tau
(\bvarphi^s)}{2}^2\Big\rangle^{1/2}.
\end{align*}
The desired (\ref{eq:Cetacompare}) follows the conditions $\|\X\|_\op \leq C_0$,
$\|\y\|_2^2 \leq C_0d$, and the preceding bounds for
(\ref{eq:Cthetacomparedecomp}).

For (\ref{eq:Retacompare}), note that
\begin{equation}\label{eq:Retaform}
\Tr \bR_\eta(s+\tau, s) = \frac{\delta}{\sigma^4}\big\langle\Tr \X[\d P_\tau(\btheta^s)]\X^\top\big\rangle,
\qquad \Tr \bR_\eta^\infty(\tau) = \frac{\delta}{\sigma^4}\big\langle\Tr \X[\d
P_\tau(\btheta)]\X^\top\big\rangle.
\end{equation}
Let $\{\btheta^t,\V^t\}_{t \geq 0}$ and $\{\tilde\btheta^t,\tilde \V^t\}_{t\geq
0}$ be the solutions of (\ref{eq:matrixV_sde}) with initial conditions
$(\x,\I)$ and $(\tilde \x,\I)$. If $\tau \in [0,1]$, we apply
(\ref{eq:Ptjac1}) to obtain
\[|\Tr \X[\d P_\tau(\x)]\X^\top-\Tr \X[\d P_\tau(\tilde \x)]\X^\top|
\leq \big\langle \pnorm{\V^\tau - \tilde{\V}^\tau}{F}\big\rangle
\cdot \pnorm{\X^\top \X}{F}
\leq \sqrt{d}\,\pnorm{\X}{\op}^2 \cdot \big\langle\pnorm{\V^\tau -
\tilde{\V}^\tau}{F}\big\rangle,\]
which leads to the bound (\ref{eq:response_bound_1}) up to a different constant
depending on the bound $C_0$ for $\pnorm{\X}{\op}$. If $\tau \geq 1$, we apply
(\ref{eq:Ptjac2}) to obtain 
\begin{align*}
&\sqrt{2}\,\Big|\Tr \X[\d P_\tau(\x)]\X^\top - \Tr \X[\d
P_\tau(\tilde\x)]\X^\top\Big|\\
&\leq \Big\langle\Big|\Big(P_{\tau-1}(\btheta^1) -
P_{\tau-1}(\tilde{\btheta}^1)\Big)^\top \X^\top \X \Big(\int_0^1 (\V^s)^\top \d
\b^s\Big)\Big|\Big\rangle + \Big\langle\Big|\Big(P_{\tau-1}(\tilde{\btheta}^1)\Big)^\top \X^\top \X
\Big(\int_0^1 (\V^s - \tilde{\V}^s)^\top \d \b^s\Big)\Big|\Big\rangle\\
&\leq \pnorm{\X}{\op}^2 \bigg[\Big\langle\pnorm{P_{\tau-1}(\btheta^1) -
P_{\tau-1}(\tilde{\btheta}^1)}{}^2\Big\rangle^{1/2} \bigg\langle \int_0^1
\|\V^s\|_F^2 \d s\bigg\rangle^{1/2} +
\Big(\Big\langle\pnorm{P_{\tau-1}(\tilde{\btheta}^1)}{}^2\Big\rangle^{1/2}
\bigg\langle \int_0^1 \|\V^s - \tilde{\V}^s\|_F^2 \d s\bigg\rangle^{1/2}\bigg].
\end{align*}
This can be bounded in the same way as (\ref{eq:response_bound_2}),
(\ref{eq:response_bound_3}), and (\ref{eq:response_bound_4})
up to different constants depending on the bound $C_0$ for $\pnorm{\X}{\op}$.
This shows (\ref{eq:Retacompare}).
\end{proof}

\begin{lemma}\label{lem:CRexpdecay}
Suppose Assumptions \ref{assump:prior} and \ref{assump:LSI}
hold for a fixed prior $g(\cdot)$.
Let $\{\btheta^t\}_{t \geq 0}$ be the solution to
(\ref{eq:langevin_sde}) with a fixed initial condition
$\btheta^0 \in \R^d$ satisfying $\|\btheta^0\|_2^2 \leq C_0d$.
Then on the event
$\event(C_0,C_\LSI)$, there exist constants $C,c>0$
such that for all $t \geq s \geq 0$,
\begin{align}
\big|\Tr \bC_\theta(t,s)-\langle\btheta^s \rangle^\top\langle\btheta \rangle\big|
&\leq Cde^{-c(t-s)}\label{eq:Cthetadecay}\\
|\Tr \bR_\theta(t,s)| &\leq
Cde^{-c(t-s)}\label{eq:Rthetadecay}\\
\bigg|\Tr \bC_\eta(t,s)-
\frac{\delta}{\sigma^4}(\X\langle\btheta^s\rangle-\y)^\top(\X\langle\btheta\rangle-\y)\bigg|
&\leq Cde^{-c(t-s)}\label{eq:Cetadecay}\\
|\Tr \bR_\eta(t,s)| &\leq
Cde^{-c(t-s)}\label{eq:Retadecay}
\end{align}
and furthermore
\begin{align}
\big|\langle\btheta^s \rangle^\top \langle\btheta
\rangle-\|\langle\btheta\rangle\|_2^2\big|
&\leq Cde^{-cs}\label{eq:Cthetainitdecay}\\
\big|(\X\langle\btheta^s\rangle-\y)^\top
(\X\langle\btheta\rangle-\y)-\|\X\langle\btheta\rangle-\y\|_2^2
\big| &\leq Cde^{-cs}\label{eq:Cetainitdecay}
\end{align}
\end{lemma}
\begin{proof}
For (\ref{eq:Cthetadecay}) and (\ref{eq:Cthetainitdecay}), observe that
\begin{align*}
\big|\Tr \bC_\theta(s+\tau,s)-\langle\btheta^s\rangle^\top \langle\btheta\rangle\big|
&=\big|\big\langle \btheta^{s\top}(P_\tau
\btheta^s-\langle\btheta\rangle)\big\rangle\big|\\
&\leq \big\langle\|\btheta^s\|_2^2\big\rangle^{1/2}
\big\langle\|P_\tau \btheta^s-\langle\btheta\rangle\|_2^2\big\rangle^{1/2}
\leq Cde^{-c\tau},
\end{align*}
the last inequality applying (\ref{eq:W2contraction}) and
(\ref{eq:mean_concentrate}). Similarly
\[\big|\langle\btheta^s\rangle^\top \langle\btheta\rangle-\|\langle\btheta
\rangle\|_2^2\big|
=\big|(P_s\btheta^0-\langle\btheta \rangle)^\top \langle\btheta \rangle\big|
\leq \|\langle\btheta\rangle\|_2 \cdot \|P_s\btheta^0-\langle\btheta\rangle\|_2
\leq Cde^{-cs}.\]

For (\ref{eq:Rthetadecay}), recall from (\ref{eq:Rthetaform}) that
$\Tr \bR_\theta(s+\tau,s)=\sum_{j=1}^d \langle (\partial_j P_\tau
e_j)[\btheta^s]\rangle$.
Then by the first equality of (\ref{eq:tracePtjac}) and (\ref{eq:V_op_bound}),
we have $|\Tr \bR_\theta(s+\tau,s)| \leq C\sqrt{d}$ for any $\tau \in [0,1]$.
For $\tau \geq 1$, we apply instead the second equality of (\ref{eq:tracePtjac}) where
$\int_0^t (\V^s)^\top \d \B^s$ is a martingale. Then
$\langle \langle \btheta\rangle^\top \int_0^1 (\V^s)^\top \d \B^s\rangle=0$,
so for any $\tau \geq 1$,
\begin{align*}
\left|\sum_{j=1}^d \partial_j P_\tau e_j(\x)\right|
&=\left|\bigg\langle\Big(P_{\tau-1}(\btheta^1)-\langle\btheta\rangle\Big)^\top
\int_0^1 (\V^s)^\top \d \B^s\bigg\rangle\right|\\
&\leq \big\langle\pnorm{P_{\tau-1}(\btheta^1) -
\langle\btheta\rangle}{}^2\rangle^{1/2}
\bigg\langle\int_0^1 \|\V^s\|_F^2 \d s\bigg\rangle^{1/2}
\leq Ce^{-c\tau}\sqrt{d}(\|\x\|_2+\sqrt{d}),
\end{align*}
the last inequality
using the estimates (\ref{eq:mean_concentrate}) and (\ref{eq:V_op_bound}). Then
by (\ref{eq:W2contraction}) and Jensen's inequality,
\begin{align*}
|\Tr \bR_\theta(s+\tau,s)| \leq
\bigg\langle\bigg|\sum_{j=1}^d (\partial_j P_\tau
e_j)[\btheta^s]\bigg|\bigg\rangle
\leq C'de^{-c'\tau}.
\end{align*}
Combining these cases $\tau \in [0,1]$ and $\tau \geq 1$ gives
(\ref{eq:Rthetadecay}).

The arguments for (\ref{eq:Cetadecay}), (\ref{eq:Retadecay}), and
(\ref{eq:Cetainitdecay}), are analogous to the above, and we omit these
for brevity.
\end{proof}

\subsection{The DMFT system is regular and exponentially convergent}

We now prove Theorem \ref{thm:fixedalpha_dynamics}, that the DMFT system
satisfies the conditions of Definition \ref{def:regular}.

\begin{lemma}\label{lem:fixedalpha_C}
Under Assumptions \ref{assump:model}, \ref{assump:prior}, and
\ref{assump:LSI} for a fixed prior $g(\cdot)$, the DMFT
system prescribed by Theorem \ref{thm:dmft_approx} satisfies the conditions of
Definition \ref{def:regular}(1).
\end{lemma}

\begin{proof}
We restrict to the almost sure event where the
convergence statements of Theorem \ref{thm:dmft_approx} hold, and where
$\event(C_0,C_\LSI)$ holds for all large $n,d$.

Consider first the statements for $C_\theta(t,s)$. Under Assumption
\ref{assump:model} we have $\|\btheta^0\|_2^2 \leq C_0d$ a.s.\ for
a large enough constant $C_0>0$ and all large $n,d$. Then
(\ref{eq:Cthetadecay}) of Lemma \ref{lem:CRexpdecay} implies,
for some constants $C,c>0$,
\begin{equation}\label{eq:Cthetalimsmalls}
\limsup_{n,d \to \infty} \big|d^{-1}\Tr \bC_\theta(t,s)
-d^{-1}\langle\btheta^s\rangle^\top \langle\btheta \rangle\big|
\leq Ce^{-ct} \text{ for all } s \leq t/2.
\end{equation}
By Theorem \ref{thm:dmft_approx}, 
$\lim_{n,d \to \infty} d^{-1} \Tr \bC_\theta(t,s)=C_\theta(t,s)$ for all
$t \geq s \geq 0$. Then, for each $s \geq 0$ and $t \geq 2s$,
\[\limsup_{n,d \to \infty} d^{-1}
\langle\btheta^s\rangle^\top\langle\btheta\rangle
\leq C_\theta(t,s)+Ce^{-ct},
\qquad \liminf_{n,d \to \infty} d^{-1}
\langle\btheta^s \rangle^\top\langle\btheta \rangle
\geq C_\theta(t,s)-Ce^{-ct}.\]
Taking $t \to \infty$ on the right side of both statements
shows that for each $s \geq 0$, there exists a limit
\begin{equation}\label{eq:cthetainit}
\tilde c_\theta(s):=\lim_{n,d \to \infty} d^{-1}
\langle \btheta^s \rangle^\top \langle \btheta \rangle
=\lim_{t \to \infty} C_\theta(t,s).
\end{equation}
Next, (\ref{eq:Cthetainitdecay}) of Lemma \ref{lem:CRexpdecay} implies
for some $C,c>0$,
\begin{equation}\label{eq:tildecsbound}
\limsup_{n,d \to \infty} \big|d^{-1}\langle\btheta^s\rangle^\top
\langle\btheta\rangle
-d^{-1}\|\langle\btheta\rangle\|_2^2\big| \leq Ce^{-cs} \text{ for all } s \geq 0.
\end{equation}
Then
\[\limsup_{n,d \to \infty} d^{-1}\|\langle\btheta\rangle\|_2^2
\leq \tilde c_\theta(s)+Ce^{-cs},
\qquad \liminf_{n,d \to \infty} d^{-1}\|\langle\btheta\rangle\|_2^2
\geq \tilde c_\theta(s)-Ce^{-cs}.\]
Taking $s \to \infty$ on the right side of both statements shows that there
exists a limit
\begin{equation}\label{eq:cthetainfty}
c_\theta(\infty):=\lim_{n,d \to \infty} d^{-1}\|\langle\btheta\rangle\|_2^2
=\lim_{s \to \infty} \tilde c_\theta(s).
\end{equation}
Setting $c_\theta^\init(s)=\tilde c_\theta(s)-c_\theta(\infty)$, the bounds
(\ref{eq:Cthetalimsmalls}) and (\ref{eq:tildecsbound}) then imply
\begin{equation}\label{eq:Cthetaapproxsmalls}
|C_\theta(t,s)-(c_\theta^\init(s)+c_\theta(\infty))|
\leq Ce^{-ct} \text{ for all } s \leq t/2,
\qquad |c_\theta^\init(s)| \leq Ce^{-cs} \text{ for all } s \geq 0.
\end{equation}

To approximate $C_\theta(t,s)$ for $s \geq t/2$,
consider $\bC_\theta^\infty(\tau)$ as defined in Lemma \ref{lemma:TTI}.
Let ${-}\L=\int_0^\infty a\,\d E_a$ be the spectral decomposition of ${-}\L$
as a positive, self-adjoint operator on $L^2(q)$
(c.f.\ \cite[Theorem A.4.2]{bakry2014analysis}), where $\{E_a\}_{a \geq 0}$ is a
family of orthogonal projections onto an increasing family of closed linear
subspaces of $L^2(q)$. In particular, $E_0f=\langle f(\btheta) \rangle$
is the projection onto the constant functions.
For each $\tau \geq 0$ and all $f,g \in L^2(q)$, we then have
\begin{equation}\label{eq:spectraldecomp}
\langle f(\btheta)P_\tau g(\btheta) \rangle=\int_0^\infty e^{-a \tau}\d \langle
f(\btheta)E_a g(\btheta) \rangle
\end{equation}
understood as a Stieltjes integral with respect to the bounded-variation
function $a \mapsto \langle f(\btheta)E_a g(\btheta) \rangle$
(c.f.\ \cite[Proposition 3.1.6(iii)]{bakry2014analysis}).
The LSI defining $\event(C_0,C_\LSI)$ implies a Poincar\'e inequality and
spectral gap, i.e.\ the spectrum of ${-}\L$ is included in
$\{0\} \cup [1/C_\LSI,\infty)$
(c.f.\ \cite[Proposition 5.1.3]{bakry2014analysis}).
Thus, fixing any constant $\iota \in (0,1/C_\LSI)$, we have
\begin{align*}
d^{-1}\Tr \bC_\theta^\infty(\tau)
=d^{-1}\sum_{j=1}^d \langle e_j(\btheta)P_\tau e_j(\btheta) \rangle
&=d^{-1}\sum_{j=1}^d \langle e_j(\btheta)E_0e_j(\btheta) \rangle
+d^{-1}\sum_{j=1}^d \int_\iota^\infty e^{-a\tau} \d\langle e_j(\btheta)E_a
e_j(\btheta) \rangle\\
&=d^{-1}\|\langle \btheta\rangle\|_2^2
+d^{-1}\sum_{j=1}^d \int_\iota^\infty e^{-a\tau} \d\langle e_j(\btheta)E_a
e_j(\btheta) \rangle,
\end{align*}
the first equality applying (\ref{eq:spectraldecomp}), and
the second equality applying $\sum_j \langle e_j(\btheta)E_0e_j(\btheta)
\rangle=\sum_j \langle \theta_j\langle \theta_j\rangle\rangle
=\|\langle \btheta\rangle \|^2$.
Define $(n,d,\X,\y)$-dependent scalars $c_{\theta,d},m_{\theta,d}>0$
and a positive measure $\mu_{\theta,d}$ on $[\iota,\infty)$ by
\begin{equation}\label{eq:muddef}
c_{\theta,d}=d^{-1}\|\langle \btheta \rangle\|_2^2, \quad 
m_{\theta,d}=d^{-1}\sum_{j=1}^d \int_\iota^\infty \d\langle e_j(\btheta)E_a e_j(\btheta)
\rangle, \quad
\mu_{\theta,d}(S)=d^{-1}\sum_{j=1}^d \int_S \d\langle e_j(\btheta)E_a e_j(\btheta)
\rangle,
\end{equation}
noting that $a \mapsto d^{-1}\sum_{j=1}^d
\langle e_j(\btheta)E_a e_j(\btheta) \rangle$ is nondecreasing and hence
defines a valid distribution function for $\mu_{\theta,d}$. Then
\begin{equation}\label{eq:Cthetamuexpr}
d^{-1}\Tr \bC_\theta^\infty(\tau)
=c_{\theta,d}+\int_\iota^\infty e^{-a\tau} \mu_{\theta,d}(\d a),
\qquad m_{\theta,d}=\mu_{\theta,d}([\iota,\infty)).
\end{equation}

Applying (\ref{eq:Cthetamuexpr}) with $\tau=0$,
\begin{equation}\label{eq:cmtheta}
c_{\theta,d}+m_{\theta,d}=d^{-1}\Tr \bC_\theta^\infty(0)=d^{-1}\langle \|\btheta\|_2^2\rangle
\leq C.
\end{equation}
In particular, $\mu_{\theta,d}$ is finite and uniformly bounded in total
variation norm for all $(n,d)$.
We claim that $\tau \mapsto d^{-1}\Tr \bC_\theta^\infty(\tau)$ is uniformly
equicontinuous over all $(n,d)$: Observe that
\begin{align}
\Big|d^{-1}\Tr \bC_\theta^\infty(\tau)-d^{-1}\Tr \bC_\theta^\infty(\tau')\Big|
&=\Big|d^{-1}\big\langle \btheta^\top [P_\tau-P_{\tau'}](\btheta)\big\rangle\Big|\notag\\
&\leq d^{-1}\langle\|\btheta\|_2^2\rangle^{1/2} \cdot
\langle\|[P_\tau-P_{\tau'}](\btheta)\|_2^2\rangle^{1/2}\notag\\
&=d^{-1}\langle\|\btheta\|_2^2\rangle^{1/2} \cdot
\langle\|\btheta-P_{|\tau-\tau'|}(\btheta)\|_2^2\rangle^{1/2}.\label{eq:equicontinuous}
\end{align}
Since $\nabla \log q(\btheta)$ is $L$-Lipschitz by (\ref{eq:negativeCD}),
\cite[Theorem II.2.1]{kunita1984stochastic} implies
$\|P_t(\x)-\x\|_2^2 \leq C(1+\|\x\|_2^2)t$ for 
all $t \in [0,1]$ and a constant $C>0$ depending only on $L$.
This and (\ref{eq:W2contraction}) imply
that the right side of (\ref{eq:equicontinuous}) is at most
$C'|\tau-\tau'|$ for a constant $C'>0$ and all $|\tau-\tau'| \leq 1$,
so $\tau \mapsto d^{-1}\Tr \bC_\theta^\infty(\tau)$ is uniformly
equicontinuous as claimed. We note that for any $M>0$, by the relation
(\ref{eq:Cthetamuexpr}),
$c_{\theta,d}+\mu_{\theta,d}([0,M))+e^{-M\tau}\mu_{\theta,d}([M,\infty))
\geq d^{-1}\Tr \bC_\theta^\infty(\tau)$. Then setting $\tau=1/M$ and rearranging
yields
\[(1-e^{-1})\mu_{\theta,d}([M,\infty)) \leq c_{\theta,d}+m_{\theta,d}-d^{-1}\Tr
\bC_\theta^\infty(1/M)=d^{-1}\Tr \bC_\theta^\infty(0)-d^{-1}\Tr
\bC_\theta^\infty(1/M).\]
So this uniform equicontinuity implies 
that the measures $\mu_{\theta,d}$ are uniformly tight.

Then, there exists a subsequence $\{(n_k,d_k)\}_{k \geq 1}$ of $(n,d)$ along
which $\mu_{\theta,d} \Rightarrow \mu_\theta$ weakly, for some finite
positive measure $\mu_\theta$ on $[\iota,\infty)$. Recalling also that
$c_{\theta,d}=d^{-1}\|\langle\btheta\rangle\|_2^2 \to c_\theta(\infty)$ as $n,d \to \infty$
by the definition (\ref{eq:cthetainfty}), and setting
\begin{equation}\label{eq:cthetadef}
c_\theta^\tti(\tau)=\int_\iota^\infty e^{-a\tau}\mu_\theta(\d a),
\end{equation}
this weak convergence applied to (\ref{eq:Cthetamuexpr}) implies
$\lim_{k \to \infty} d_k^{-1}\Tr \bC_\theta^\infty(\tau)=c_\theta^\tti(\tau)
+c_\theta(\infty)$.
Combining this with the convergence
$\lim_{k \to \infty} d_k^{-1}\Tr \bC_\theta(s+\tau,s)=C_\theta(s+\tau,s)$
by Theorem \ref{thm:dmft_approx}, for any $s,\tau \geq 0$ we have
\[\Big|C_\theta(s+\tau,s)-(c_\theta^\tti(\tau)+c_\theta(\infty))\Big|
\leq \limsup_{k \to \infty} \Big|d_k^{-1}\Tr \bC_\theta(s+\tau,s)
-d_k^{-1}\Tr \bC_\theta^\infty(\tau)\Big| \leq Ce^{-cs},\]
where the last inequality holds by (\ref{eq:Cthetacompare}).
In particular, for any $t \geq 0$,
\begin{equation}\label{eq:Cthetaapproxlarges}
|C_\theta(t,s)-(c_\theta^\tti(t-s)+c_\theta(\infty))|
\leq Ce^{-c't} \text{ for all } s \in [t/2,t].
\end{equation}
Since $C_\theta(t,s)-c_\theta(\infty)$ does not depend on $(\X,\y)$,
this implies that $c_\theta^\tti(\tau)$ does not depend on $(\X,\y)$ for every
$\tau \geq 0$, and thus also the measure $\mu_\theta$ does not depend on
$(\X,\y)$.
Together, (\ref{eq:Cthetaapproxsmalls}) and (\ref{eq:Cthetaapproxlarges})
imply (\ref{eq:Cthetaapproxinvariant}).

The statement (\ref{eq:Cetaapproxinvariant}) follows analogously:
By arguments parallel to (\ref{eq:cthetainit}), (\ref{eq:cthetainfty}), and
(\ref{eq:Cthetaapproxsmalls}),
Theorem \ref{thm:dmft_approx} and (\ref{eq:Cetadecay}) and
(\ref{eq:Cetainitdecay}) imply that there exist limits
\begin{align}
\tilde c_\eta(s)&:=\lim_{n,d \to \infty}
\frac{\delta}{n\sigma^4} (\X\langle \btheta^s \rangle-\y)^\top
(\X\langle \btheta \rangle-\y)=\lim_{t \to \infty} C_\eta(t,s),
\label{eq:cetainit}\\
c_\eta(\infty)&:=\lim_{n,d \to \infty} \frac{\delta}{n\sigma^4}
\|\X\langle \btheta \rangle-\y\|_2^2=\lim_{s \to \infty} \tilde c_\eta(s),
\label{eq:cetainfty}
\end{align}
which satisfy
\begin{equation}\label{eq:Cetaapproxsmalls}
|C_\eta(t,s)-(c_\eta^\init(s)+c_\eta(\infty))| \leq Ce^{-ct}
\text{ for all } s \leq t/2,
\qquad |c_\eta^\init(s)| \leq Ce^{-cs} \text{ for all } s \geq 0.
\end{equation}
To approximate $C_\eta(t,s)$ for $s \geq t/2$, note that
\[n^{-1}\Tr \bC_\eta^\infty(\tau)
=n^{-1}\sum_{i=1}^n
\big\langle x_i(\btheta)P_\tau x_i(\btheta)\big\rangle
=\frac{\delta}{n\sigma^4}\|\X\langle \btheta \rangle-\y\|_2^2
+\frac{1}{n}\sum_{i=1}^n \int_\iota^\infty
e^{-a\tau}\d\langle x_i(\btheta)E_a x_i(\btheta) \rangle.\]
Defining
\begin{equation}\label{eq:cetamuexpr}
c_{\eta,n}=\frac{\delta}{n\sigma^4}\|\X\langle \btheta \rangle-\y\|_2^2,
\quad \mu_{\eta,n}(S)=\frac{1}{n}\sum_{i=1}^n \int_S
\d\langle x_i(\btheta)E_a x_i(\btheta) \rangle,
\quad m_{\eta,n}=\mu_{\eta,n}([\iota,\infty)),
\end{equation}
we have
\begin{equation}\label{eq:cmeta}
c_{\eta,n}+m_{\eta,n}=n^{-1}\Tr \bC_\eta^\infty(0)
=\frac{\delta}{n\sigma^4}\langle \|\X\btheta-\y\|_2^2 \rangle \leq C.
\end{equation}
So along some subsequence $\{(n_k,d_k)\}_{k \geq 1}$, we have
$c_{\eta,n} \to c_\eta(\infty)$, $\mu_{\eta,n} \Rightarrow \mu_\eta$
weakly for a finite positive measure $\mu_\eta$ on $[\iota,\infty)$, and
$\lim_{k \to \infty} n_k^{-1}\Tr \bC_\eta^\infty(\tau)
=c_\eta^\tti(\tau)+c_\eta(\infty)$ for the quantity
\[c_\eta^\tti(\tau)=\int_\iota^\infty e^{-a\tau}\mu_\eta(\d a).\]
By an argument parallel to (\ref{eq:Cthetaapproxlarges})
using Theorem \ref{thm:dmft_approx} and (\ref{eq:Cetacompare}), this shows
\begin{equation}\label{eq:Cetaapproxlarges}
|C_\eta(t,s)-(c_\eta^\tti(t-s)+c_\eta(\infty))| \leq Ce^{-ct}
\text{ for all } s \in [t/2,t],
\end{equation}
and (\ref{eq:Cetaapproxsmalls}) and (\ref{eq:Cetaapproxlarges})
establish (\ref{eq:Cetaapproxinvariant}).

Finally, for (\ref{eq:Cthetastarlim}), observe that by Theorem
\ref{thm:dmft_approx}, $\lim_{n,d \to \infty} d^{-1}\langle\btheta^t\rangle^\top
\btheta^*=C_\theta(t,*)$. Noting that
\[\limsup_{n,d \to \infty}
d^{-1}\big|(\langle\btheta^t\rangle-\langle\btheta\rangle)^\top \btheta^*\big|
\leq \limsup_{n,d \to \infty}
d^{-1}\|P_t \btheta^0-\langle\btheta \rangle\|_2 \cdot \|\btheta^*\|_2
\leq Ce^{-ct}\]
by (\ref{eq:mean_concentrate}), this implies the existence of the limit
\begin{equation}\label{eq:cthetastar}
c_\theta(*):=\lim_{n,d \to \infty} d^{-1}\langle\btheta \rangle^\top \btheta^*
=\lim_{t \to \infty} C_\theta(t,*),
\end{equation}
which satisfies $|C_\theta(t,*)-c_\theta(*)| \leq Ce^{-ct}$.
This shows (\ref{eq:Cthetastarlim}).
\end{proof}

\zf{Move the below lemma to the DMFT section.}
\begin{lemma}\label{lem:Reta_ast_id}
For any $t \geq 0$, it holds that $R_\eta(t,\ast) = -\int_0^t R_\eta(t,s)\d s$.
\end{lemma}
\begin{proof}
Recall $\bar{R}^\gamma_\eta(t,\ast), \bar{R}^\gamma_\eta(t,s)$ in (\ref{eq:dmft_response}), $R^\gamma_\eta(t,\ast), R^\gamma_\eta(t,s)$ in (\ref{def:dmft_piecelinear_Rg}), and that for any $\gamma > 0$, $[t] = \floor{t}/\gamma$ with $\floor{t}$ given in (\ref{eq:t_floor_ceil}). Then 
\begin{align*}
R_\eta^\gamma(\floor{t}, \ast) \stackrel{(i)}{=} \bar{R}_\eta^\gamma([t],\ast) \stackrel{(ii)}{=} -\sum_{\ell=0}^{[t]-1} \bar{R}_\eta^\gamma([t],\ell) \stackrel{(iii)}{=} -\gamma\cdot\sum_{\ell=0}^{[t]-1} R_\eta^\gamma(\floor{t},\ell\gamma) \stackrel{(iv)}{=} -\int_0^t R_\eta^\gamma(\floor{t},s)\d s, 
\end{align*}
where $(i),(iii)$ follow from the correspondence (\ref{eq:induction_piecelinear_eta1})-(\ref{eq:induction_piecelinear_eta2}), $(ii)$ follows from Lemma \ref{lem:eta_response_id}, and $(iv)$ follows from the fact that $(t,s) \mapsto R_\eta^\gamma(t,s)$ is piecewise constant, i.e., $R_\eta^\gamma(t,s) = R_\eta^\gamma(\floor{t},\floor{s})$. Hence using the discretization bound in Lemma \ref{eq:eta_response_discre_error}, the conclusion follows by
\begin{align*}
\Big|R_\eta(t,\ast) + \int_0^t R_\eta(t,s)\d s\Big| \leq \Big|R_\eta(t,\ast) - R_\eta^\gamma(\floor{t},\ast)\Big| + \Big|\int_0^t R_\eta^\gamma(\floor{t},s)\d s - \int_0^t R_\eta^\gamma(\floor{t},s)\d s\Big|
\end{align*}
and taking $\gamma \rightarrow 0$.
\end{proof}

\begin{lemma}\label{lem:fixedalpha_R}
Under Assumptions \ref{assump:model}, \ref{assump:prior}, and
\ref{assump:LSI} for a fixed prior $g(\cdot)$, the DMFT
system prescribed by Theorem \ref{thm:dmft_approx} satisfies the conditions of
Definition \ref{def:regular}(2).
\end{lemma}
\begin{proof}
We again restrict to the almost sure event where the convergence statements of
Theorem \ref{thm:dmft_approx} hold, and where $\event(C_0,C_\LSI)$ holds for all
large $n,d$.

Consider first $R_\theta(t,s)$. By
(\ref{eq:Rthetadecay}) of Lemma \ref{lem:CRexpdecay} and the convergence
$R_\theta(t,s)=\lim_{n,d \to \infty} d^{-1}\bR_\theta(t,s)$ of Theorem
\ref{thm:dmft_approx},
\begin{equation}\label{eq:Rthetaapproxsmalls}
|R_\theta(t,s)| \leq Ce^{-ct} \text{ for all } s \leq t/2.
\end{equation}
For $s \geq t/2$, note that
the forms of (\ref{eq:Cthetamuexpr}) and (\ref{eq:cthetadef}) imply that both
$d^{-1}\Tr \bC_\theta^\infty(\tau)$ and $c_\theta^\tti(\tau)+c_\theta(\infty)$
are convex and differentiable in $\tau \geq 0$. Then, 
along the subsequence $\{(n_k,d_k)\}_{k \geq 1}$
of the preceding proof, the pointwise convergence
$\lim_{k \to \infty} d_k^{-1}\Tr
\bC_\theta^\infty(\tau)=c_\theta^\tti(\tau)+c_\theta(\infty)$  implies also
$\lim_{k \to \infty} d_k^{-1} \partial_\tau \Tr \bC_\theta^\infty(\tau)
=\partial_\tau c_\theta^\tti(\tau)$
for each $\tau \geq 0$ (c.f.\ \cite[Theorem 25.7]{rockafellar1997convex}). By
the fluctuation-dissipation relation of Lemma \ref{eq:langevin_fdt_equi}
applied with $A=B=e_j$ for each $j=1,\ldots,d$, we have
$\partial_\tau \Tr \bC_\theta^\infty(\tau)={-}\Tr \bR_\theta^\infty(\tau)$.
Then, defining $r_\theta^\tti(\tau)={-}\partial_\tau c_\theta^\tti(\tau)$,
this shows $\lim_{k \to \infty} d_k^{-1} \Tr \bR_\theta^\infty(\tau)
=r_\theta^\tti(\tau)$. Combining with
$\lim_{k \to \infty} d_k^{-1} \Tr \bR_\theta(s+\tau,s)=R_\theta(s+\tau,s)$
from Theorem \ref{thm:dmft_approx}, for any $s,\tau \geq 0$ we have that
\[\Big|R_\theta(s+\tau,s)-r_\theta^\tti(\tau)\Big|
\leq \limsup_{k \to \infty}
\Big|d_k^{-1}\Tr \bR_\theta(s+\tau,s)-d_k^{-1}\Tr \bR_\theta^\infty(\tau)\Big|
\leq Ce^{-cs},\]
where the last inequality applies (\ref{eq:Rthetacompare}).
In particular, for any $t \geq 0$,
\begin{equation}\label{eq:Rthetaapproxlarges}
|R_\theta(t,s)-r_\theta^\tti(t-s)| \leq Ce^{-c't}
\text{ for all } s \in [t/2,t].
\end{equation}
Together, (\ref{eq:Rthetaapproxsmalls}) and (\ref{eq:Rthetaapproxlarges})
imply (\ref{eq:Rthetaapproxinvariant}).

The statement (\ref{eq:Retaapproxinvariant}) follows analogously, and we omit
this for brevity.

Finally, for the statement (\ref{eq:Retastarlim}), recall from
Lemma \ref{lem:Reta_ast_id} that
$R_\eta(t,\ast) = -\int_0^t R_\eta(t,s)\d s$. Then, setting
\[r_\eta(*)={-}\int_0^\infty r_\eta^\tti(\tau)\d \tau
=\lim_{\tau \to \infty} c_\eta^\tti(\tau)-c_\eta^\tti(0)
={-}c_\eta^\tti(0),\]
we have
\[|R_\eta(t,*)-r_\eta(*)|
\leq \left|\int_0^t (R_\eta(t,s)-r_\eta^\tti(t-s))\d s\right|
+\left|\int_t^\infty r_\eta^\tti(\tau)\d \tau\right|
\leq t \cdot Ce^{-ct}+c_\eta^\tti(t)
\leq C'e^{-c't}.\]
\end{proof}

Together, Lemmas \ref{lem:fixedalpha_C} and \ref{lem:fixedalpha_R} prove
Theorem \ref{thm:fixedalpha_dynamics}.

\subsection{Limit MSE and free energy}

We now show Corollary \ref{cor:fixedalpha_dynamics} on the limit values of
MSE, YMSE, and free energy. We use the additional LSI assumption for
the true prior $g_*$ to establish the following concentration statements.

\begin{proposition}\label{prop:mseconcentration}
Let $\YMSE_*$ and the marginal likelihood
$\sP_g(\y \mid \X)$ be as defined in Theorem \ref{thm:fixedalpha_dynamics}.
Let $\E_\y$ denote the expectation with respect to $\theta_j^*
\overset{iid}{\sim} g_*$ and $\eps_i \overset{iid}{\sim} \N(0,\sigma^2)$
conditioning on $\X$. Under the conditions of Corollary
\ref{cor:fixedalpha_dynamics}, almost surely 
\begin{equation}\label{eq:mseconcentration}
\lim_{n,d \to \infty}
d^{-1}\log \sP_g(\y \mid \X)-d^{-1}\E_\y \log \sP_g(\y \mid \X)=0,
\qquad \lim_{n,d \to \infty} \YMSE_*-\E_\y\YMSE_*=0.
\end{equation}
\end{proposition}
\begin{proof}
Let $C,C',c>0$ be $(g_*,\sigma^2)$-dependent constants changing from instance
to instance. We restrict to the almost sure event (\ref{eq:good_event}) where $\event(C_0,C_\LSI)$
holds for all large $n,d$.

For the first statement, write $\bar \btheta^*=\btheta^*-\E\btheta^*$, and note
\begin{align*}
&\log \sP_g(\y \mid \X)\\
&=\log \int (2\pi\sigma^2)^{-n/2}
\exp\bigg({-}\frac{1}{2\sigma^2}\|\X\bar\btheta^*+\beps+\X(\E\btheta^*-\btheta)\|_2^2
+\sum_{j=1}^d \log g(\theta_j)\bigg)\d\btheta\\
&={-}\frac{n}{2}\log 2\pi\sigma^2
-\underbrace{\frac{\|\X\bar\btheta^*+\beps\|_2^2}{2\sigma^2}}_{:=\mathrm{I}}
+\underbrace{\log \int \exp\bigg({-}\frac{1}{\sigma^2}(\X\bar\btheta^*
+\beps)^\top\X(\E\btheta^*-\btheta)
-\frac{1}{2\sigma^2}\|\X(\E\btheta^*-\btheta)\|_2^2+\sum_{j=1}^d \log
g(\theta_j)\bigg)\d\btheta}_{:=\mathrm{II}}.
\end{align*}
For the concentration of $\mathrm{I}$ we have
\[\mathrm{I}=\begin{pmatrix} \bar\btheta^* \\ \beps
\end{pmatrix}^\top \M \begin{pmatrix} \bar\btheta^* \\ \beps \end{pmatrix},
\qquad \M=\frac{1}{2\sigma^2}\begin{pmatrix} \X^\top \X & \X^\top \\
\X & \I \end{pmatrix}.\]
The condition that $g_*$ satisfies the LSI (\ref{eq:LSIprior})
implies that the entries of $(\bar\btheta^*,\beps)$ are
independent, mean-0, and subgaussian, so
\begin{equation}\label{eq:concentrationI}
\P[|\mathrm{I}-\E_\y\mathrm{I}| \geq t]
\leq 2e^{-c\min(t^2/\|\M\|_F^2,\,t/\|\M\|_\op)}
\end{equation}
by the Hanson-Wright inequality (c.f.\ \cite[Theorem 6.2.1]{vershynin2018high}).
We have $\|\X\|_\op \leq C_0$ for all large $n,d$, hence $\|\M\|_\op \leq
C'$ and $\|\M\|_F^2 \leq C'd$ for some $C'>0$. This shows, for any $t>0$,
\[\P[|\mathrm{I}-\E_\y\mathrm{I}| \geq td]
\leq 2e^{-cd\min(t^2,t)}.\]
For the concentration of $\mathrm{II}$ we have
\[\nabla_{\bar \btheta^*}\mathrm{II}
={-}\frac{1}{\sigma^2}\X^\top \X(\E\btheta^*-\langle \btheta \rangle),
\qquad \nabla_{\beps}\mathrm{II}
={-}\frac{1}{\sigma^2}\X(\E\btheta^*-\langle \btheta \rangle).\]
Then the bound $\langle \|\btheta\|_2^2 \rangle \leq Cd$ from
(\ref{eq:posteriormeansq}) \ys{the bound here should be independent of $\beps, \btheta^\ast$} and $\|\X\|_\op \leq C_0$ imply
$\|\nabla_{\bar \btheta^*}\mathrm{II}\|_2,
\|\nabla_{\beps}\mathrm{II}\|_2 \leq C\sqrt{d}$, so $\mathrm{II}$ is
$C'\sqrt{d}$-Lipschitz in $(\bar\btheta^*,\beps)$. Since the law of
$(\bar\btheta^*,\beps)$ satisfies LSI by tensorization, this implies the
concentration
\begin{equation}\label{eq:concentrationII}
\P[|\mathrm{II}-\E_\y\mathrm{II}| \geq td] \leq 2e^{-cdt^2}.
\end{equation}
(\ref{eq:concentrationI}), (\ref{eq:concentrationII}), and the Borel-Cantelli
lemma show the first statement of (\ref{eq:mseconcentration}).

For the second statement, we have
\[n\YMSE=\big\langle \|\X\btheta\|_2^2\big\rangle
-\|\X\langle \btheta\rangle\|_2^2
=\frac{\int \|\X\btheta\|_2^2\exp(\mathrm{II})\d\btheta}
{\int \exp(\mathrm{II})\d\btheta}
-\bigg\|\frac{\int \X\btheta \exp(\mathrm{II})\d\btheta}{
\int \exp(\mathrm{II})\d\btheta}\bigg\|_2^2.\]
Momentarily writing $\Var,\Cov$ for the variance and covariance of $\btheta$
under the posterior law $\sP_g(\btheta \mid \X,\y)$,
differentiating in $(\bar\btheta^*,\beps)$ gives, for any unit vector $\v$ (of
the appropriate dimension $d$ or $n$)
\begin{align*}
\v^\top \nabla_{\bar\btheta^*}[n\YMSE]
&=\frac{1}{\sigma^2}\Cov\big[
\|\X\btheta\|_2^2,\,\v^\top \X^\top \X\btheta\big]
-\frac{2}{\sigma^2}\Cov\big[\langle \btheta \rangle^\top \X^\top \X\btheta,
\v^\top \X^\top \X\btheta\big],\\
\v^\top \nabla_{\beps^*}[n\YMSE]
&=\frac{1}{\sigma^2}\Cov\big[
\|\X\btheta\|_2^2,\,\v^\top \X\btheta\big]
-\frac{2}{\sigma^2}\Cov\big[\langle \btheta \rangle^\top \X^\top \X\btheta,
\v^\top \X\btheta\big].
\end{align*}
The Poincar\'e inequality implied by the assumed LSI for
$\sP_g(\btheta \mid \X,\y)$ shows
\[\Var[\|\X\btheta\|_2^2] \leq C\langle \|\X^\top \X \btheta\|_2^2 \rangle,
\quad \Var[\langle \btheta \rangle^\top \X^\top \X\btheta]
\leq C\|\X^\top \X\langle \btheta \rangle\|_2^2,
\quad \Var[\v^\top \X^\top \X\btheta] \leq C\|\X^\top \X\v\|_2^2.\]
Then applying $\langle \|\btheta\|_2^2 \rangle \leq Cd$ from
(\ref{eq:posteriormeansq}), $\|\X\|_\op \leq C_0$, and Cauchy-Schwarz, we obtain
$|\v^\top \nabla_{\bar\btheta^*}[n\YMSE]| \leq C\sqrt{d}$ and
$|\v^\top \nabla_{\beps^*}[n\YMSE]| \leq C\sqrt{d}$. So $n\YMSE$ is also
$C'\sqrt{d}$-Lipschitz in $(\bar\btheta^*,\beps)$, and the second statement of
(\ref{eq:mseconcentration}) follows from the same concentration argument as
above.
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:fixedalpha_dynamics}(a)]
We restrict to the almost sure event where the convergence statements of
Theorem \ref{thm:dmft_approx} hold, and where $\event(C_0,C_\LSI)$ 
and $\|\btheta^0\|_2^2 \leq C_0d$ also hold for all large $n,d$.

Observe that by (\ref{eq:muddef}) and (\ref{eq:cmtheta}),
\[\MSE=d^{-1}\langle \|\btheta-\langle \btheta \rangle\|_2^2 \rangle
=d^{-1}\big(\langle\|\btheta\|_2^2\rangle-\|\langle\btheta\rangle\|_2^2\big)
=m_d=\mu_d([\iota,\infty)),\]
so $\lim_{n,d \to \infty} \MSE=\mu_\theta([\iota,\infty))=c_\theta^\tti(0)$
by (\ref{eq:cthetadef}). Also
\[\MSE_*=d^{-1}\|\btheta^*-\langle \btheta \rangle\|_2^2
=d^{-1}\big(\|\btheta^*\|_2^2
-2\langle \btheta \rangle^\top \btheta^*+\|\langle \btheta \rangle\|_2^2\big),\]
so
$\lim_{n,d \to \infty} \MSE_*=\E[{\theta^*}^2]
-2c_\theta(*)+c_\theta(\infty)$ by Assumption \ref{assump:model} and the
definitions (\ref{eq:cthetainfty}) and (\ref{eq:cthetastar}).
Thus $\MSE \to \mse$ and $\MSE_* \to \mse_*$ for the quantities
$\mse,\mse_*$ defined in (\ref{eq:mmse}).

Similarly
\[\YMSE=n^{-1}\big\langle\|\X\btheta-\X\langle \btheta \rangle\|_2^2 \big\rangle
=n^{-1}\big(\langle\|\X\btheta-\y\|_2^2\rangle-\|\X\langle\btheta\rangle-\y\|_2^2\big).\]
Then by (\ref{eq:cetamuexpr}) and (\ref{eq:cmeta}),
$\lim_{n,d \to \infty} \YMSE=\frac{\sigma^4}{\delta}\mu_{\eta,n}([\iota,\infty))
=\frac{\sigma^4}{\delta}\,c_\eta^\tti(0)=\ymse$
as defined in (\ref{eq:mmse}). For $\YMSE_*$,
writing $\E_\y$ for the expectation over $(\btheta^*,\beps)$ as in
Proposition \ref{prop:mseconcentration}, observe first that
\begin{align*}
n^{-1}\E_\y\|\X\langle \btheta \rangle-\y\|_2^2
&=n^{-1}\E_\y\|\X\langle \btheta \rangle-\X\btheta^*\|_2^2
-2n^{-1}\E_\y\beps^\top(\X\langle \btheta \rangle-\X\btheta^*)+\sigma^2,
\end{align*}
and Gaussian integration-by-parts gives
\begin{align*}
\E_\y\beps^\top(\X\langle \btheta \rangle-\X\btheta^*)
&=\E_\y\beps^\top \X\langle \btheta \rangle
=\E_\y\langle \|\X\btheta-\X\btheta^*\|_2^2 \rangle
-\E_\y\|\X\langle \btheta \rangle-\X\btheta^*\|_2^2\\
&=\E_\y\langle \|\X\btheta-\X\langle \btheta \rangle\|_2^2 \rangle
=n\,\E_\y\YMSE.
\end{align*}
Thus
\begin{equation}\label{eq:YMSErelation}
\E_\y\YMSE_*=n^{-1}\E_\y\|\X\langle \btheta \rangle-\X\btheta^*\|_2^2
=n^{-1}\E_\y\|\X\langle \btheta \rangle-\y\|_2^2
+2\E_\y\YMSE-\sigma^2.
\end{equation}
We remark that $n^{-1}\|\X\langle \btheta \rangle-\y\|_2^2$ and $\YMSE$ are
bounded for all large $n,d$, by the
bound for $\langle \|\btheta\|_2^2 \rangle \leq C$ from (\ref{eq:posteriormeansq}).
Thus, applying $\YMSE \to \ymse$ and
$n^{-1}\|\X\langle\btheta \rangle-\y\|_2^2 \to
\frac{\sigma^4}{\delta}c_\eta(\infty)$ as argued above and dominated
convergence, the right side of (\ref{eq:YMSErelation}) converges to
$\ymse_*=\frac{\sigma^4}{\delta}(c_\eta(\infty)+2c_\eta^\tti(0))-\sigma^2$
as defined in (\ref{eq:mmse}). Then the concentration of $\YMSE_*$ established
in Proposition \ref{prop:mseconcentration} and (\ref{eq:YMSErelation})
show $\lim_{n,d \to \infty} \YMSE_*=\ymse_*$.

To show the last statement (\ref{eq:fixedalpha_equilibriumlaw}), conditional on
$\X,\btheta^*,\beps$ and the initialization $\btheta^0$,
consider a coupling of a posterior sample $\btheta \sim q$ with $\btheta^t$
such that
$\langle \|\btheta^t-\btheta\|_2^2 \rangle=W_2(q_t,q)^2$, where $\langle \cdot
\rangle$ denotes the expectation under this coupling and $q_t$ is the
conditional law of $\btheta^t$.
For a given realization of $(\btheta^t,\btheta)$, considering the
coordinatewise coupling of $\frac{1}{d}\sum_{j=1}^d
\delta_{(\theta_j^*,\theta_j^t)}$ with
$\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)}$ shows
\[W_2\left(\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j^t)},
\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)} \right)^2
\leq \frac{1}{d}\sum_{j=1}^d (\theta_j^t-\theta_j)^2
=\frac{1}{d}\|\btheta^t-\btheta\|_2^2.\]
Then
\[\Bigg\langle
W_2\Bigg(\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j^t)},
\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)}\Bigg)^2 \Bigg\rangle
\leq \frac{1}{d}\big\langle \|\btheta^t-\btheta\|_2^2 \big\rangle
=\frac{1}{d} W_2(q_t,q)^2.\]
Applying Lemmas \ref{lemma:elementarybounds} and \ref{lem:W2contraction},
$W_2(q_t,q)^2 \leq Ce^{-ct}(\langle
\|\btheta\|_2^2\rangle+\|\btheta^0\|_2^2) \leq C'de^{-ct}$
for some constants $C,C',c>0$ and all large $n,d$. So
\begin{equation}\label{eq:equilibriumlaw_tmp1}
\limsup_{n,d \to \infty}
\Bigg\langle
W_2\Bigg(\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j^t)},
\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)}\Bigg)^2
\Bigg\rangle \leq C'e^{-ct}.
\end{equation}
Theorem \ref{thm:dmft_approx}(b) implies that almost-surely over the
realization of $\{\btheta^t\}_{t \geq 0}$, for each fixed $t \geq 0$,
\[\lim_{n,d \to \infty} W_2\Bigg(\frac{1}{d}\sum_{j=1}^d
\delta_{(\theta_j^*,\theta_j^t)},\;\sP(\theta^*,\theta^t)\Bigg)^2=0\]
where $\sP(\theta^*,\theta^t)$ is the law of $(\theta^*,\theta^t)$ in
the DMFT system. We have
$W_2(\frac{1}{d}\sum_{j=1}^d
\delta_{(\theta_j^*,\theta_j^t)},\sP(\theta^*,\theta^t))^2
\leq C(1+d^{-1}\|\btheta^*\|_2^2+\|\btheta^t\|_2^2)$ for a constant $C>0$
not depending on $n,d$, and this is uniformly integrable under $\langle \cdot
\rangle$ for large $n,d$. Then dominated convergence implies
\begin{equation}\label{eq:equilibriumlaw_tmp2}
\lim_{n,d \to \infty} \Bigg\langle W_2\Bigg(\frac{1}{d}\sum_{j=1}^d
\delta_{(\theta_j^*,\theta_j^t)},\;\sP(\theta^*,\theta^t)\Bigg)^2\Bigg\rangle=0.
\end{equation}
By Theorem \ref{thm:dmft_equilibrium}, we have
\begin{equation}\label{eq:equilibriumlaw_tmp3}
\lim_{t \to \infty} W_2\Big(\sP(\theta^*,\theta^t),\;
\sP_{g_*,\omega_*;g,\omega}\Big)^2=0.
\end{equation}
Combining (\ref{eq:equilibriumlaw_tmp1}),
(\ref{eq:equilibriumlaw_tmp2}), and (\ref{eq:equilibriumlaw_tmp3}) shows
\[\lim_{t \to \infty} \limsup_{n,d \to \infty}
\Bigg\langle W_2\Bigg(\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^*,\theta_j)},
\sP_{g_*,\omega_*;g,\omega}\Bigg)^2 \Bigg\rangle=0.\]
Since the quantity in the $t \to \infty$ limit on the left side does not depend
on $t$, this implies (\ref{eq:fixedalpha_equilibriumlaw}).
\end{proof}

To show Corollary \ref{cor:fixedalpha_dynamics}(b) on the limit free
energy, we will apply an I-MMSE argument, together with the following
proposition which guarantees continuity of $\mse,\mse_*$ in the noise
variance $\sigma^2$ under either condition of Proposition \ref{prop:LSI}.
In the later proof of Theorem \ref{thm:adaptivealpha_dynamics}, we will require 
also continuity in the prior parameter $\alpha$; thus we establish both
statements here.

\begin{lemma}\label{lemma:mmse_lipschitz}
Fix any open subset $O \subset \R^K$, and suppose
Assumptions \ref{assump:model}, \ref{assump:prior}, and \ref{assump:LSI}
hold for each $\alpha \in O$ and $g=g(\cdot,\alpha)$ where the constant
$C_\LSI>0$ of Assumption \ref{assump:LSI} is uniform over $\alpha \in O$.
Consider the linear model with some noise variance $s^2 \geq \sigma^2$,
the Langevin dynamics with fixed $\alpha \in O$ (i.e.\ with $K=0$ and
$\cG \equiv 0$) corresponding to this model,
and let $\mse(s^2,\alpha),\mse_*(s^2,\alpha)$ be as defined by
(\ref{eq:sigma0condition}) for the DMFT limit of these dynamics, viewed as
functions of $(s^2,\alpha)$

Then for any compact interval
$I \subset [\sigma^2,\infty)$ and compact subset $S \subset O$,
$\mse(s^2,\alpha),\mse_*(s^2,\alpha)$ are Lipschitz functions of
$(s^2,\alpha) \in I \times S$.
\end{lemma}
\begin{proof}
Let us first bound the $W_2$-distance between the posterior laws
$\sP_g(\btheta \mid \X,\y)$ in a model with noise/prior parameters
$(s^2,\alpha)$ and a model with
noise/prior parameters $(\tilde s^2,\tilde \alpha)$.

In general, let $q(\btheta)=Z^{-1}e^{U(\btheta)}$ and $\tilde q(\btheta)=\tilde
Z^{-1}e^{\tilde U(\btheta)}$ be two densities satisfying the
log-Sobolev inequality (\ref{eq:LSI}) for a constant $C_\LSI>0$. Consider the
Langevin diffusion
\[\d\btheta^t=\nabla U(\btheta^t)+\sqrt{2}\,\d \b^t\]
with stationary law $q$ and a random initialization $\btheta^0 \sim q_0$,
and let $q_t$ be the density of $\btheta^t$. Then
\begin{align*}
\frac{\d}{\d t} \DKL(q_t\|\tilde q)
&=\frac{\d}{\d t} \int q_t(\log q_t-\log \tilde q)\\
&=\int \Big(\frac{\d}{\d t} q_t\Big)(\log q_t-\log \tilde q)
+\underbrace{\int \frac{q_t}{q_t}\Big(\frac{\d}{\d t} q_t\Big)}_{=0}
=\int \Big(\frac{\d}{\d t} q_t\Big)(\log q_t-\tilde U+\log \tilde Z).
\end{align*}
Substituting the Fokker-Planck equation
\[\frac{\d}{\d t} q_t=\nabla \cdot [q_t\nabla(\log q_t-U)]\]
and integrating by parts, we obtain
\begin{align*}
\frac{\d}{\d t} \DKL(q_t\|\tilde q)
&={-}\int q_t\,\nabla(\log q_t-U)^\top \nabla(\log q_t-\tilde U)\\
&={-}\int q_t\,\|\nabla(\log q_t-\tilde U)\|_2^2
-\int q_t\,\nabla(\tilde U-U)^\top \nabla(\log q_t-\tilde U)\\
&\leq {-}(1/2)\int q_t\,\|\nabla(\log q_t-\tilde U)\|_2^2
+(1/2)\int q_t\|\nabla(\tilde U-U)\|_2^2,
\end{align*}
the last step applying Cauchy-Schwarz for the second term. By the LSI for
$\tilde q$, the first term (the relative Fisher information) is lower bounded as
\[\int q_t\,\|\nabla(\log q_t-\tilde U)\|_2^2
=\int q_t\,\Big\|\nabla \log \frac{q_t}{\tilde q}\Big\|_2^2
\geq \frac{1}{2C_\LSI}\,\DKL(q_t\|\tilde q).\]
Thus we arrive at
\[\frac{\d}{\d t} \DKL(q_t\|\tilde q)
\leq {-}\frac{1}{4C_\LSI}\,\DKL(q_t\|\tilde q)
+\underbrace{\frac{1}{2} \E \|\nabla \tilde U(\btheta^t)-\nabla
U(\btheta^t)\|_2^2}_{:=\Delta(t)}.\]
Integrating this inequality gives
\begin{equation}\label{eq:KLcomparison}
\DKL(q_T\|\tilde q) \leq \int_0^T e^{-(1/4C_\LSI)(T-t)}\Delta(t)\d t
+e^{-(1/4C_\LSI)T}\DKL(q_0\|\tilde q)
\leq C\Big(\sup_{t \in [0,T]} \Delta(t)+e^{-cT}\DKL(q_0\|\tilde q)\Big)
\end{equation}
for constants $C,c>0$ depending only on $C_\LSI$.

Applying this in our setting, set $\y=\X\btheta^*+s\z$
and $\tilde\y=\X\btheta^*+\tilde s\z$ where $\z \sim \N(0,\I)$.
Conditioning on $\X,\btheta^*,\z$, define
\[U(\btheta)={-}\frac{1}{2s^2}\|\X\btheta^*+s \z
-\X\btheta\|_2^2+\sum_{j=1}^d \log g(\theta_j;\alpha)\]
so that $q(\btheta) \propto e^{U(\btheta)}$ is the posterior law given $(\X,\y)$
under parameters $(s^2,\alpha)$. Define similarly $\tilde U(\btheta)$ 
with $(\tilde s^2,\tilde \alpha)$ in place of $(s^2,\alpha)$,
and $\tilde q(\btheta)\propto e^{\tilde U(\btheta)}$
as the posterior law given $(\X,\tilde\y)$.
Let $\{\btheta^t\}_{t \geq 0}$ be a
Langevin diffusion defined by (\ref{eq:langevin_fixedq}) with
the law $q(\btheta)$, and a random initialization
$\btheta^0 \sim q_0 \equiv \tilde q$. Then
\[\Delta(t) \leq \E\Bigg[\bigg\|\frac{1}{s^2}\X^\top(\X\btheta^*+s
\z-\X\btheta^t)-\frac{1}{\tilde s^2}\X^\top(\X\btheta^*+\tilde s\z
-\X\btheta^t)\bigg\|_2^2+\sum_{j=1}^d \Big(\partial_\theta
\log g(\theta_j^t;\alpha)-\partial_\theta
\log g(\theta_j^t;\tilde \alpha)\Big)^2\;\Bigg|\;\X,\btheta^*,\z\Bigg].\]
Let $C,C'$ etc.\ be constants depending on the compact sets $S,I$ and changing
from instance to instance. For $\alpha,\tilde\alpha \in S$ and
$s^2,\tilde s^2 \in I$,
\[|s^{-2}-\tilde s^{-2}| \leq C|s^2-\tilde s^2|,
\quad |s^{-1}-\tilde s^{-1}| \leq C|s^2-\tilde s^2|,
\quad |\partial_\theta \log g(\theta;\alpha)-\partial_\theta \log g(\theta;\tilde\alpha)|
\leq C\|\alpha-\tilde\alpha\|_2,\]
the last inequality holding by Assumption \ref{assump:prior}. Thus
\[\Delta(t) \leq
C\Big[\|\X\|_\op^4(\|\btheta^*\|_2^2+\E[\|\btheta^t\|_2^2 \mid \X,\btheta^*,\z])
+\|\X\|_\op^2\|\z\|_2^2\Big](s^2-\tilde s^2)^2
+Cd\|\alpha-\tilde\alpha\|_2^2.\]
Applying $\E[\|\btheta^t\|_2^2 \mid \X,\btheta^*,\z,\btheta^0] \leq
C(\|\btheta^0\|_2^2+d)$ and $\E_{\btheta^0 \sim \tilde q}[\|\btheta^0\|_2^2]
\leq Cd$ by (\ref{eq:W2contraction}),
and the bounds $\|\X\|_\op \leq C$,
$\|\btheta^*\|_2^2 \leq Cd$, and $\|\z\|_2^2 \leq Cd$ a.s.\ for all
large $n,d$, we have
\[\sup_{t \geq 0}
\Delta(t) \leq C'd(s^2-\tilde s^2)^2+C'd\|\alpha-\tilde\alpha\|_2^2.\]
Then applying this to (\ref{eq:KLcomparison}) and noting that $\DKL(q_0\|\tilde
q)=0$, we get
\[\sup_{t \geq 0} \DKL(q_t\|\tilde q)
\leq Cd(s^2-\tilde s^2)^2+Cd\|\alpha-\tilde\alpha\|_2^2.\]
By lower-semicontinuity of KL-divergence and the $T_2$-transportation
inequality for $\tilde q$ implied by the LSI
(c.f.\ \cite[Theorem 9.6.1]{bakry2014analysis}),
\begin{equation}\label{eq:W2locallylipschitz}
W_2(q,\tilde q)^2 \leq C\DKL(q\|\tilde q)
\leq C\liminf_{t \to \infty} \DKL(q_t\|\tilde q)
\leq C'd(s^2-\tilde s^2)^2+C'd\|\alpha-\tilde\alpha\|_2^2.
\end{equation}
This gives our desired bound on the $W_2$-distance between $q$ and $\tilde q$.

Now let $\langle f(\btheta) \rangle_q$ and $\langle f(\btheta) \rangle_{\tilde
q}$ be the posterior expectations under $q$ (given $\y$) and $\tilde q$ (given
$\tilde \y$). Then by Jensen's inequality,
\[\|\langle \btheta \rangle_q-\langle \btheta \rangle_{\tilde q}\|_2 \leq
W_2(q,\tilde q).\]
Applying $|\|\x\|_2^2-\|\y\|_2^2| \leq \|\x-\y\|_2 \cdot \|\x+\y\|_2$ and
Cauchy-Schwarz, also
\[|\langle \|\btheta\|_2^2 \rangle_q-\langle \|\btheta\|_2^2 \rangle_{\tilde q}|
\leq W_2(q,\tilde q) \cdot \sqrt{2\langle \|\btheta\|_2^2 \rangle_q
+2\langle \|\btheta\|_2^2 \rangle_{\tilde q}}
\leq C\sqrt{d}\,W_2(q,\tilde q).\]
Applying these bounds, $\langle \|\btheta\|_2 \rangle_q \leq
\langle \|\btheta\|_2^2 \rangle_q^{1/2} \leq C\sqrt{d}$
by (\ref{eq:W2contraction}), and similarly for $\tilde q$, we get
\begin{align*}
\big|d^{-1}\langle \|\btheta-\langle \btheta\rangle_q\|_2^2\rangle_q
-d^{-1}\langle \|\btheta-\langle \btheta\rangle_{\tilde q}\|_2^2\rangle_{\tilde
q}\big|
&\leq d^{-1}\big|\langle \|\btheta\|_2^2 \rangle_q
-\langle \|\btheta\|_2^2 \rangle_{\tilde q}\big|
+d^{-1}\big|\|\langle \btheta \rangle_q\|_2^2
-\|\langle \btheta \rangle_{\tilde q}\|_2^2\big|\\
&\leq \frac{C'W_2(q,\tilde q)}{\sqrt{d}}
\leq C|s^2-\tilde s^2|+C\|\alpha-\tilde \alpha\|_2.
\end{align*}
Similarly
\begin{align*}
\big|d^{-1}\|\btheta^*-\langle \btheta\rangle_q\|_2^2
-d^{-1}\|\btheta^*-\langle \btheta\rangle_{\tilde q}\|_2^2\big|
&\leq 2d^{-1}\|\btheta^*\|_2\|\langle \btheta\rangle_q-
\langle \btheta\rangle_{\tilde q}\|_2
+d^{-1}\big|\|\langle \btheta \rangle_q\|_2^2
-\|\langle \btheta \rangle_{\tilde q}\|_2^2\big|\\
&\leq \frac{C'W_2(q,\tilde q)}{\sqrt{d}}
\leq C|s^2-\tilde s^2|+C\|\alpha-\tilde \alpha\|_2.
\end{align*}
Thus $\MSE$ and $\MSE_*$ are Lipschitz over $(s^2,\alpha) \in I \times S$
a.s.\ for all large $n,d$. By Corollary \ref{cor:fixedalpha_dynamics}(a)
already shown, $\lim_{n,d \to \infty} \MSE=\mse$ and $\lim_{n,d \to \infty}
\MSE_*=\mse_*$ a.s.\ for each $(s^2,\alpha) \in I \times S$,
so this implies the Lipschitz continuity of $\mse(s^2,\alpha)$ and
$\mse_*(s^2,\alpha)$.
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:fixedalpha_dynamics}(b)]
We apply Corollary \ref{cor:fixedalpha_dynamics}(a) and an
I-MMSE relation for mismatched Gaussian channels. 
Write $\E_\y$ for the expectation over $(\btheta^*,\beps)$ as in Proposition
\ref{prop:mseconcentration}. Let
\[I(\y,\btheta^* \mid \X)
=\E_\y \log \frac{P_{g_*}(\y \mid \btheta^*,\X)}{P_{g_*}(\y \mid \X)}
={-}\E_\y\log P_{g_*}(\y \mid \X)
-\frac{n}{2}(1+\log 2\pi\sigma^2)\]
be the signal-observation mutual information. Then
\begin{align}
\E_\y \log P_g(\y \mid \X)&={-}\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid \X))
+\E_\y \log P_{g_*}(\y \mid \X)\notag\\
&={-}\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid \X))
-I(\y,\btheta \mid \X)-\frac{n}{2}(1+\log 2\pi\sigma^2).
\label{eq:freeenergyIMMSE}
\end{align}

We denote the noise variance $\sigma^2=s^{-1}$, and write
\[E(s,g)=\E_\y\YMSE_*
=n^{-1}\E_\y\|\X\langle \btheta \rangle-\X\btheta^*\|^2\]
for the expected $\YMSE_*$ in a model with assumed prior $g$ and noise variance
$\sigma^2=s^{-1}$. We clarify that this means $\langle \cdot \rangle$ is the
posterior expectation under the law
\[\sP_g(\btheta \mid \X,\y) \propto \exp\bigg({-}\frac{1}{2\sigma^2}
\|\y-\X\btheta\|_2^2+\sum_{j=1}^d \log g(\theta_j)\bigg)\]
defined by $g$ and $\sigma^2=s^{-1}$, and $\E_\y$ is
the expectation over $(\btheta^*,\beps)$ defining $\y$, where 
$\beps$ also has variance $\sigma^2=s^{-1}$. We write
$I[s],\DKL[s]$ for the above quantities $I(\y,\btheta^* \mid \X)$ and
$\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid \X))$ in a model with noise variance
$\sigma^2=s^{-1}$. Then
\cite[Theorem 2]{guo2005mutual} and \cite[Eq.\ (24)]{verdu2010mismatched} show
the I-MMSE relations
\[\frac{\d}{\d s}I[s]=\frac{n}{2}E(s,g_*), \qquad
\frac{\d}{\d s}\DKL[s]=\frac{n}{2}\big(E(s,g)-E(s,g_*)\big).\]
In the limit $s=\sigma^{-2} \to 0$, it is direct to check that
$I[s] \to 0$ and $\DKL[s] \to 0$. Thus, for
$I(\y,\btheta^* \mid \X)=I[\sigma^{-2}]$ and
$\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid \X))=\DKL[\sigma^{-2}]$ in our
original model with noise variance $\sigma^2$, integrating these I-MMSE
relations shows
\[\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid \X))+I(\y,\btheta^* \mid \X)
=\frac{n}{2}\int_0^{\sigma^{-2}} E(s,g)\d s.\]
Note that Assumption \ref{assump:LSI} ensures the posterior LSI holds in the
model with any noise variance $s^{-1} \in [\sigma^2,\infty)$. Then
applying Corollary \ref{cor:fixedalpha_dynamics}(a) already shown and the
concentration of $\YMSE_*$ in Proposition \ref{prop:mseconcentration},
we have $E(s,g) \to \ymse_*(s)$ for each $s^{-1} \in (\sigma^2,\infty)$,
where $\ymse_*(s)$ is defined by (\ref{eq:mmse}) under the assumed prior
$g$ and noise variance $\sigma^2=s^{-1}$. We remark that by definition,
$E(s,g)$ is uniformly bounded a.s.\ for all large $n,d$. Then taking the limit
$n,d \to \infty$ and applying the bounded convergence theorem,
\begin{equation}\label{eq:IMMSE}
\lim_{n,d \to \infty}
\frac{1}{d}\Big(\DKL(P_{g_*}(\y \mid \X) \| P_g(\y \mid
\X))+I(\y,\btheta^* \mid \X)\Big)
=\frac{\delta}{2}\int_0^{\sigma^{-2}} \ymse_*(s)\d s.
\end{equation}

Let $(\omega(s),\omega_*(s))$ be defined by
(\ref{eq:mmse}--\ref{eq:static_fixedpoint}) when the noise variance is
$\sigma^2=s^{-1}$. Recall the marginal density $\sP_{g,\omega}(Y)$ of the
scalar channel model (\ref{eq:scalarchannelmarginal}), and define
\begin{align}
f(\omega,\omega_*,s)
&={-}\E_{g_*,\omega_*} \log \sP_{g,\omega}(Y)
-\frac{1}{2}\left(2\delta+\log \frac{2\pi}{\omega}
-\delta \log \frac{\delta s}{\omega}
+(1-\delta)\frac{\omega}{\omega_*}
+\frac{\omega}{s}\Big(\frac{\omega}{\omega_*}-2\Big)\right)\label{eq:fomega}\\
&=\frac{\omega}{2}\E \theta^{*2}
-\E\log \int \exp\Big(\omega
\theta(\theta^*+z)-\frac{\omega}{2}\theta^2\Big)g(\theta)\d\theta
-\frac{1}{2}\Big(2\delta-\delta\log\frac{\delta
s}{\omega}-\frac{\delta\omega}{\omega_*}+\frac{\omega}{s}\Big(\frac{\omega}{\omega_*}-2\Big)\Big)\notag
\end{align}
where $\theta^* \sim g_*$ and $z \sim \N(0,\omega_*^{-1})$.
Here, the second line applies the explicit form of
$\sP_{g,\omega}(Y)$, evaluates $\E_{g_*,\omega_*}$ under
the true model $Y=\theta^*+z$ with
$\theta^* \sim g_*$ and $z \sim \N(0,\omega_*^{-1})$, and applies some algebraic
simplification. We now claim that
\begin{equation}\label{eq:IMMSEalt}
\frac{\delta}{2}\int_0^s \ymse_*(t)\d t=f(\omega(s),\omega_*(s),s)
\end{equation}
for all $s \in (0,\sigma^{-2})$. To show this, it suffices to check that
$\lim_{s \to 0} f(\omega(s),\omega_*(s),s)=0$ and $\frac{\d}{\d
s}f(\omega(s),\omega_*(s),s)=\frac{\delta}{2}\ymse_*(s)$,
which we may do as follows:
\begin{itemize}
\item In the limit $s \to 0$, we have that $\mse(s),\mse_*(s)$ are bounded, so
$\omega(s),\omega_*(s) \sim \delta s$. Then
$\omega(s) \to 0$, $\omega_*(s) \to 0$, $\omega(s)/s \to \delta$, and
$\omega(s)/\omega_*(s) \to 1$. This shows $\lim_{s \to 0}
f(\omega(s),\omega_*(s),s)=0$.
\item Differentiating in $\omega,\omega_*$ and applying
Gaussian integration-by-parts with respect to $z \sim \N(0,\omega_*^{-1})$, we
may check that at $(\omega,\omega_*)=(\omega(s),\omega_*(s))$, we have
\begin{align*}
&\partial_\omega\bigg[\frac{\omega}{2}\E_{g_*,\omega_*} \theta^{*2}
-\E_{g_*,\omega_*}\log \int \exp\Big(\omega
\theta(\theta^*+z)-\frac{\omega}{2}\theta^2\Big)g(\theta)\d\theta\bigg]\\
&\hspace{1in}=\frac{1}{2}\E_{g_*,\omega_*} \langle (\theta^*-\theta)^2 \rangle_{g,\omega}
-\frac{\omega}{\omega_*}\E_{g_*,\omega_*} \langle (\theta-\langle \theta \rangle_{g,\omega})^2
\rangle_{g,\omega}=\frac{1}{2}(\mse+\mse_*)-\frac{\omega}{\omega_*}\mse,\\
&\partial_{\omega_*}\bigg[\frac{\omega}{2}\E_{g_*,\omega_*} \theta^{*2}
-\E_{g_*,\omega_*}\log \int \exp\Big(\omega
\theta(\theta^*+z)-\frac{\omega}{2}\theta^2\Big)g(\theta)\d\theta\bigg]\\
&\hspace{1in}=\frac{\omega^2}{2\omega_*^2}\E_{g_*,\omega_*} \langle (\theta-\langle \theta
\rangle_{g,\omega})^2\rangle_{g,\omega}=\frac{\omega^2}{2\omega_*^2}\mse.
\end{align*}
Applying $\mse=\delta/\omega-\sigma^2$ and $\mse_*=\delta/\omega_*-\sigma^2$ by
(\ref{eq:static_fixedpoint}) and comparing with the derivatives of the last term
of $f(\omega,\omega_*,s)$, this verifies
\begin{equation}\label{eq:omegastationarity}
\partial_\omega f(\omega(s),\omega_*(s),s)=0,
\qquad \partial_{\omega_*} f(\omega(s),\omega_*(s),s)=0.
\end{equation}
Furthermore, direct calculation shows that at
$(\omega,\omega_*)=(\omega(s),\omega_*(s))$,
\[\partial_s f(\omega(s),\omega_*(s),s)=\frac{\delta\sigma^2}{2}
+\frac{\omega\sigma^4}{2}\Big(\frac{\omega}{\omega_*}-2\Big)
=\frac{\delta}{2}\ymse_*(s),\]
the second equality using (\ref{eq:ymmseomega}).
Lemma \ref{lemma:mmse_lipschitz} and the definitions of $\omega,\omega_*$ in
(\ref{eq:static_fixedpoint}) imply that $\omega(s),\omega_*(s)$ are locally
Lipschitz, and hence absolutely continuous, over $s \in (0,\sigma^{-2})$. Then
so is $f(\omega(s),\omega_*(s),s)$, and
\begin{align*}
\frac{\d}{\d s} f(\omega(s),\omega_*(s),s)
&=\partial_\omega f(\omega(s),\omega_*(s),s)
\cdot \omega'(s)+\partial_{\omega_*} f(\omega(s),\omega_*(s),s)
\cdot \omega_*'(s)+\partial_s f(\omega(s),\omega_*(s),s)\\
&=\partial_s f(\omega(s),\omega_*(s),s)=\frac{\delta}{2}\,\ymse_*(s).
\end{align*}
\end{itemize}
This verifies the claim (\ref{eq:IMMSEalt}).

Applying (\ref{eq:IMMSE}) and (\ref{eq:IMMSEalt}) to (\ref{eq:freeenergyIMMSE})
and writing
$(\omega,\omega_*)=(\omega(\sigma^{-2}),\omega_*(\sigma^{-2}))$ for the
fixed points at the original noise variance $\sigma^2$, this shows
\[\lim_{n,d \to \infty} d^{-1}\E_\y
\log P_g(\y \mid \X)=-f(\omega,\omega_*,\sigma^{-2})
-\frac{\delta}{2}(1+\log 2\pi\sigma^2).\]
Applying concentration of $d^{-1}\log P_g(\y \mid \X)$ with respect to $\E_\y$
which is established in Propostion \ref{prop:mseconcentration}, and
substituting the form of $f$ in (\ref{eq:fomega}), this
shows Corollary \ref{cor:fixedalpha_dynamics}(b).
\end{proof}




==> introduction_old.tex <==
\section{Introduction}

Consider the linear model
\begin{align}\label{eq:linearmodel}
\y = \X\btheta^\ast + \beps \in \R^n, 
\end{align}
where $\X \in \R^{n\times d}$ is a random design matrix with i.i.d. entries, the signal $\btheta^\ast \in \R^d$ have i.i.d. entries $\theta^\ast_1,\ldots, \theta^\ast_d$ drawn from one-dimensional distribution $g_\ast$, $\beps \sim \N(0,\sigma^2 I_n)$ for some $\sigma^2 > 0$ is the error, and they are mutually independent. The model (\ref{eq:linearmodel}), also known as the Bayesian linear model in statistics (since $\btheta^\ast$ is random), has been widely applied in e.g.,  genetics for estimating effect size distributions and genetic architectures of complex traits, and we refer to
\cite{zhang2018estimation, oconnor2021distribution, spence2022flexible, morgante2023flexible} for examples of methods developed in this context.

The central statistical task of posterior inference in model (\ref{eq:linearmodel}) revolves around the posterior distribution of $\btheta^\ast$ given the observed data $(\X,\y)$. For any proposed prior distribution with Lesbesgue density $g$ on the components of $\btheta$, this takes the form
\begin{align}\label{eq:posterior_fixed_g}
\P_g(\btheta | \X,\y) = \frac{1}{Z(\X,\y)} \exp\bigg({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+\sum_{j=1}^d \log g(\theta_j)\bigg), 
\end{align}
where
\begin{align}\label{eq:partition_func}
Z(\X,\y) = \int_{\R^d}  \exp\bigg({-}\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+\sum_{j=1}^d \log g(\theta_j)\bigg) \d \btheta
\end{align}
is the normalizing constant, also known as the partition function. Since the normalizing constant $Z(\X,\y)$ is hard to compute when the signal dimension $d$ is large, people often resort to Monte Carlo Markov Chain (MCMC) sampling methods or other approximate inferential tools, such as variational inference. When the true prior distribution $g_\ast$ is known, one popular sampling technique is the so-called Langevin Monte Carlo \cite{roberts1996exponential}, whose continuous-time dynamic is the solution to the following stochastic differential equation (SDE), also known as the Langevin diffusion:
\begin{align}\label{eq:langevin_diff}
\d\btheta^t = \Big[\nabla_{\btheta}\Big(-\frac{1}{2\sigma^2}\|\y-\X\btheta\|_2^2
+ \sum_{j=1}^d \log g_\ast(\theta_j)\Big)\Big]\d t + \sqrt{2}\d \b^t \in \R^d, 
\end{align} 
where $\{\b^t\}_{t\geq 0}$ is a standard Brownian motion in $\R^d$. Under appropriate assumptions on the prior distribution $g_\ast$, it is well-known that the SDE (\ref{eq:langevin_diff}) admits a strong solution, and the law of $\{\btheta^t\}_{t\geq 0}$ converges exponentially fast to its stationary distribution, which is the posterior distribution (\ref{eq:posterior_fixed_g}). By repeatedly simulating the Langevin diffusion (\ref{eq:langevin_diff}), we obtain approximately i.i.d. draws from the posterior distribution (\ref{eq:posterior_fixed_g}), based on which we may compute summary statistics (e.g., posterior mean) as the estimator for the signal $\btheta^\ast$

In practice, however, it is often the case that the true prior density $g_\ast$ is unknown to the statistician, so we are facing with the coupled tasks of estimating the prior distribution and sampling from the posterior. This is known as the \emph{empirical Bayes} problem in statistics with a long history dating back to the 1950's \cite{Robbins51, Robbins56}, which, in the current context (\ref{eq:linearmodel}), has witnessed profound progress both in theory and computation, but primarily on the identity design case $\X = I$ with $n = p$. For general design matrices $\X$, there still remain significant statistical and computational challenges:
\begin{itemize}
\item From a statistical theory point of view, at the moment it is not completely clear under what conditions (on the design matrix $\X$, the sample dimension regime $(n,p)$, and other problem parameters) is consistent estimation of the prior density $g_\ast$ possible. Some sufficient conditions are provided in the recent work \cite{mukherjee2023mean, fan2023gradient} focusing on the nonparametric maximum likelihood estimator (NPMLE), and a more detailed discussion will be given in Section \ref{sec:result} below. 
\item From a computational point of view, estimating the prior density incurs significant additional challenges to sampling from the posterior distribution. One natural idea is to maximize, with respect to the prior density $g$, the data likelihood, which equals, up to some multiplicative constant, the partition function in (\ref{eq:partition_func}). This likelihood function is typically non-convex in terms of the prior density $g$ when viewed as a functional on the space of distributions, and its optimization landscape is largely unclear (in fact, even evaluating this likelihood will be computationally hard when the signal dimension $d$ is large). 
\end{itemize}
The main goal of this paper is to make progress towards these challenges. 

Concretely, in this paper we consider the so-called mean-field setting where $\X$ has i.i.d. entries following $\N(0,1/d)$, and the proportional regime where $n/d \rightarrow \delta \in (0,\infty)$. Such assumptions, although ideal, has been widely made in many previous work in statistics, machine learning, and probability to enable precise understanding of the inference procedure [ADD REF]. We also assume the prior $g_\ast$ takes the parametric form $g(\cdot,\alpha_\ast)$ indexed by some fixed-dimensional unknown parameter $\alpha_\ast \in \R^K$ in the parametric family $\{g(\cdot,\alpha),\alpha \in \R^K\}$, which we aim to estimate aside from sampling from the corresponding posterior distribution (\ref{eq:posterior_fixed_g}) with $g = g(\cdot,\alpha_\ast)$.  To address the computational issue mentioned above, we study a class of adaptive Langevin dynamic of the form (a slightly more general version is considered in Section \ref{sec:result} below):
\begin{align}
\d\btheta^t&=\bigg[\nabla_{\btheta} \Big({-}\frac{1}{2\sigma^2}\|\y-\X\btheta^t\|_2^2 + \sum_{j=1}^d \log g(\theta^t_j, \hat\alpha^t)\Big)\bigg]\d t+\sqrt{2}\,\d\b^t,
\label{eq:theta_dynamic}\\
\d\widehat\alpha^t&=\cG\Big(\widehat\alpha^t,\frac{1}{d}\sum_{j=1}^d
\delta_{\theta_j^t}\Big)\d t \label{eq:alpha_dynamic},
\end{align}
initialized from some $\btheta^0 \in \R^d$ and $\hat\alpha^0 \in \R^K$. Compared to (\ref{eq:langevin_diff}), the new component is the $\hat\alpha$-dynamic in (\ref{eq:alpha_dynamic}), which, with $\mathcal{P}(\R)$ denote the class of distributions on $\R$, is driven by the gradient function $\cG(\cdot, \cdot): \R^K \times \mathcal{P}(\R) \rightarrow \R^K$ that depends on the current state $\hat\alpha^t$ and the empirical distribution of the current $\btheta^t$. The joint evolution (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}) can be understood as a McVean-Vlasov-type SDE widely studied in interacting particle systems \cite{chaintron2022propagation, chaintron2021propagation}, with an additional mean-field interaction brought by $\X^\top(\X\btheta^t - \y)$ in the potential of $\btheta^t$. It will be clear in Section \ref{sec:result} below that with the choice $\cG\big(\alpha,\sP\big)
=\E_{\theta \sim \sP}[\nabla_\alpha \log g(\theta,\alpha)]$, the coupled evolution of $(\btheta^t,\hat\alpha^t)$ in (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}) may be understood as simulating a gradient flow in $\cP_2(\R) \times \R^K$ for maximizing the marginal likelihood of $\y$ over the prior parameter $\alpha$.

Our main theoretical results provide a precise distributional characterization - both in an average sense over the coordinates of $\btheta$ and in the sense of individual coordinates - of the joint dynamic (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}), in the prescribed mean-field setting. We summarize our contributions as follows:
\begin{enumerate}
\item We give a rigorous proof for the dynamic mean-field limit of $(\btheta^t, \hat\alpha^t)$ in (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}) along with $\bbeta^t = (\eta^t_1,\ldots,\eta^t_n) := \X\bbeta^t$, over any fixed time horizon $T$. More precisely, we show that, almost surely as $n,d\rightarrow\infty$ with $n/d\rightarrow\delta$, 
\begin{align}\label{intro:avg_dmft}
\frac{1}{d}\sum_{j=1}^d \delta_{(\theta_j^t)_{t \in [0,T]}}
\overset{W_2}{\to} \sP((\theta^t)_{t \in [0,T]}), \quad \frac{1}{n}\sum_{i=1}^n \delta_{(\eta_i^t)_{t \in [0,T]}} \overset{W_2}{\to} \sP((\eta^t)_{t \in [0,T]}), \quad (\widehat \alpha^t)_{t \in [0,T]} \to (\alpha^t)_{t \in [0,T]}, 
\end{align}
where three random elements on the left are understood as stochastic processes on $C([0,T], \R)$, $C([0,T], \R)$, and $C([0,T], \R^K)$ respectively, and $\overset{W_2}{\to}$ denotes convergence in the Wasserstein-2 distance (over suitable distributional classes on $C([0,T], \R)$). Moreover, $\sP((\theta^t)_{t \in [0,T]})$ and $\sP((\eta^t)_{t \in [0,T]})$ denote the laws of corresponding limiting processes $(\theta^t)_{t\in[0,T]}$ and $(\eta^t)_{t\in[0,T]}$ on $C([0,T], \R)$, whose joint evolution with the deterministic process $(\alpha^t)_{t\in[0,T]}$ is given by the so-called dynamic mean-field equations:
\begin{align}
\d\theta^t &= \Big[{-}\frac{\delta}{\sigma^2}(\theta^t-\theta^*) +
\partial_\theta \log g(\theta^t,\alpha^t)
+\int_0^t R_\eta(t, s)(\theta^{s} - \theta^\ast)\d s + u^t\Big]\d t + \sqrt{2}\,\d b^t\label{def:dmft_langevin_cont_theta}\\
\eta^t &= -\frac{1}{\sigma^2}\int_0^t R_\theta(t,s)\big(\eta^s + w^* -
\eps\big)\d s - w^t\label{def:dmft_langevin_cont_eta}\\
\frac{\d}{\d t} \alpha^t &= \cG(\alpha^t,
\sP(\theta^t))\label{def:dmft_langevin_alpha}, 
\end{align}
initialized from $(\theta^0,\alpha^0)$, where $\theta^0$ is drawn from the limiting empirical distribution of $\btheta^0$, and (deterministic) $\alpha^0$ is given by the almost sure limit $\lim_{n,d\rightarrow\infty} \hat\alpha^0$. Here $\{b^t\}_{t\geq 0}$ is a standard Brownian motion on $\R$, $\theta^\ast$ and $\eps$ are drawn independently from the weak limit of the empirical distribution $d^{-1}\sum_{j=1}^d \delta_{\theta^\ast_j}$ and $n^{-1}\sum_{i=1}^n \delta_{\eps_i}$ respectively, $\{u^t\}_{t\geq 0}$ and $\{(w^t)_{t\geq 0}, w^\ast\}$ are two independent mean-zero Gaussian processes with covariance structure 
\begin{align}\label{intro:covariance}
 \quad C_\theta(t,s) := \E[w^tw^s] = \E[\theta^t\theta^s], \quad C_\theta(t,\ast) := \E[w^tw^\ast] = \E[\theta^t\theta^\ast],\\
 C_\eta(t,s) := \E[u^tu^s] = \frac{\delta}{\sigma^4}\E[(\eta^t + w^\ast - \eps)(\eta^s + w^\ast - \eps )],
\end{align}
and $R_\theta(t,s)$, $R_\eta(t,s)$ are deterministic response functions whose definitions are self-consistently given by (\ref{def:response_theta})-(\ref{def:response_g}) below. 

\item We provide a novel interpretation of the covariance function $C_\theta(t,s)$ and response function $R_\theta(t,s)$ as the mean-field limit of certain ``high-dimensional" covariance and response functions. More precisely, we construct two matrices $\bC_\theta(t,s)$ and $\bR_\theta(t,s)$ in $\R^{d\times d}$ and show that, in some appropriate sense of convergence,
\begin{align*}
\frac{1}{d}\Tr\bC_\theta(t,s) \rightarrow C_\theta(t,s), \qquad \frac{1}{d}\Tr \bR_\theta(t,s) \rightarrow R_\theta(t,s),
\end{align*}
where $\Tr$ denotes the trace of a matrix. A similar statement holds for $C_\theta(t,\ast)$, $C_\eta(t,s)$, and $R_\eta(t,s)$. The above two interpretations, especially that of the response, have at least two important consequences: (i) they allow us to strengthen the average-case characterization (\ref{intro:avg_dmft}) to one that holds for each individual coordinate; (ii) they play a key role in establishing the so-called fluctuation-dissipation relation \cite{agarwal1972fluctuation} between $C_\theta(t,s)$ and $R_\theta(t,s)$. We discuss (i) momentarily and defer (ii), which plays a further role in the long-term analysis of (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}), to a companion paper.

\item Building on the interpretations of covariance and response functions as above, we further obtain a coordinate-wise analogue of (\ref{intro:avg_dmft}) with the form (see Theorem \ref{thm:dmft_entrywise} for precise statements): For any fixed coordinate $j\in[d]$ and $i\in[n]$, in some appropriate sense of convergence, 
\begin{align*}
\sP\big((\theta_j^t)_{t \in [0,T]}\big) \rightarrow \sP((\theta^t)_{t \in [0,T]}), \quad \sP\big((\eta_i^t)_{t \in [0,T]}\big) \rightarrow \sP((\eta^t)_{t \in [0,T]}),
\end{align*}
where the laws on the right side are again given by (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}). Compared with (\ref{intro:avg_dmft}), the additional technical components are a careful entrywise discretization of the dynamic (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}) and an entrywise expansion of $\btheta^t$ with respect to the previous iterates, with the discretization step further relying on a careful leave-two-out error analysis of (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}).

%By the definition of covariance in (\ref{intro:covariance}), the natural high-dimensional analogue of $C_\theta(t,s)$ is the matrix $\bC_\theta(t,s) \in \R^{d\times d}$, whose $(i,j)$-th entry is given by $[\bC_\theta(t,s)]_{i,j} = \langle (\btheta^t)_i (\btheta^s)_j \rangle$ with $\langle \cdot \rangle$ denoting expectation over the Brownian motion $\{\b^t\}$ in (\ref{eq:theta_dynamic}). In fact, it follows as a direct corollary of (\ref{intro:avg_dmft}) that almost surely as $n,d\rightarrow\infty$, 

\end{enumerate}

Aside from independent interest, these results also pave the way to the long-time (i.e., $T\rightarrow\infty$) analysis of the joint evolution (\ref{eq:theta_dynamic})-(\ref{eq:alpha_dynamic}), which allows us to address, e.g., the consistency of learning the prior parameter $\alpha$ in the statistical empirical Bayes context. Due to space constraints, we will present the details of such analysis in a companion paper.

\subsection{Related work}

\textbf{Dynamic mean-field theory (DMFT)} DMFT is first developed by physicists to study the performance of Langevin dynamics for disordered systems (e.g., spin glasses), using non-rigorous methods such as field theoretical methods and the dynamical cavity method \cite{mezard1987spin, crisanti1992spherical, cugliandolo1993analytical}. In the context of spin glass, the first rigorous proof appears in \cite{benarous1995large, benarous1997symmetric, guionnet1997averaged} (for continuous spins and Langevin dynamic) and \cite{grunwald1996sanov} (for Ising spins and Glauber dynamic), where the authors applied large deviation techniques and weak convergence theory; see also \cite{benarous2001aging, benarous2006cugliandolo} for results in the setting of spherical spin glass. In contrast, the proof technique in the current paper is more in line with the recent breakthrough paper \cite{celentano2021high}, which developed a reduction technique to the state evolution analysis of the approximate message passing (AMP) algorithm \cite{bolthausen2014iterative, bayati2011dynamics, javanmard2013state}; see also \cite{gerbelot2024rigorous} for a related but more direct analysis via the Gaussian conditioning technique. In addition to being conceptually simple, this proof technique has the benefit of inheriting well-established properties of the AMP dynamic, e.g., universality \cite{bayati2015universality, chen2021universality} and non-asymptotic analysis \cite{han2024entrywise}; see also \cite{dembo2021diffusions, dembo2021universality} for more direct proofs on the universality of DMFT. 

Building on the developments mentioned above, DMFT has been applied, in both rigorous and non-rigorous manners, to a wide range of problems in statistics, probability, and machine learning, including but not limited to matrix/tensor principal component analysis \cite{sarao2020marvels, liang2023high}, mixture model analysis \cite{mignacco2021dynamical}, generalized linear models \cite{agoritsas2018out, mignacco2021stochasticity}, inference of first-order methods \cite{patil2024failures, han2024gradient}, neural networks \cite{bordelon2022self}, stochastic gradient descent algorithms (SGD) \cite{}

\textbf{Empirical Bayes and posterior inference}

\subsection{Notation}

Throughout this paper, in the context of the posterior law
(\ref{eq:posterior}) with a fixed and given prior $g$, we will write
\[\langle f(\btheta) \rangle=\E_g[\btheta \mid \X,\y]\]
for the posterior expectation, conditioning on the ``quenched'' variables
$\X,\btheta^*,\beps$. In the context of the dynamics
(\ref{eq:langevin_sde}--\ref{eq:gflow}), we consider also
the initial conditions $\btheta^0,\widehat\alpha^0$ as quenched variables,
and write
\[\langle f(\btheta^t,\widehat \alpha^t) \rangle\]
for the expectation conditioned on
$\X,\btheta^*,\beps,\btheta^0,\widehat\alpha^0$. We use $\E$ for the full
expectation over also $\X,\btheta^*,\beps,\btheta^0,\widehat\alpha^0$.

For a random variable $\xi$ in a normed vector space $\cM$, we write
$\sP(\xi)$ to denote its law. $\cP_\infty(\cM)$ is the set of probability
distributions $\sP$ on $\cM$ for which $\E_{\xi \sim \sP} \|\xi\|^p<\infty$ for any integer $p > 0$,
and $W_2(\cdot,\cdot)$ is the Wasserstein-2 metric on $\cP_\infty(\cM)$.

$C([0,T],\R^d)$ is the space of continuous functions $f:[0,T] \to \R^d$
equipped with the norm $\|f\|=\sup_{t \in [0,T]} \|f(t)\|_2$.
$C^k(\R^d,\R^m)$ is the space of functions $f:\R^d \to \R^m$
that are $k$-times continuously-differentiable.



==> replica.tex <==
\section{Replica-symmetric predictions for the posterior overlaps}\label{appendix:replica}

Suppose that $n/d = \delta$, $X_{ij} \sim_{i.i.d.} \N(0, \frac{1}{d})$, the true prior of $\btheta^\ast$ is $g^\ast$, and the nominal prior is $g$ in the following posterior distribution:
\begin{align*}
P_g(\btheta|\X,\y) = \frac{(2\pi\sigma^2)^{-n/2}e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}\prod_{j=1}^d g(\theta_j)}{Z_n},
\end{align*}
where with $\Xi_n = \int (2\pi\sigma^2)^{-\frac{n}{2}}e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}g(\btheta) \d\btheta$, 
\begin{align*}
Z_n = Z_n(\X,\y) = \int (2\pi\sigma^2)^{-\frac{n}{2}}e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}\prod_{j=1}^d g(\theta_j) \d\btheta = (2\pi\sigma^2)^{-\frac{n}{2}}\Xi_n.
\end{align*}
The goal is to compute the limiting free energy
\begin{align*}
\lim_{d\rightarrow \infty} \frac{1}{d}\E_{g^\ast} \log Z_n = -\frac{\delta}{2}\log(2\pi\sigma^2) + \lim_{d\rightarrow \infty} \frac{1}{d}\E_{g^\ast} \log \Xi_n,
\end{align*}
where the expectation is taken over the model $\y = \X\btheta^\ast + \beps$ with $\btheta^\ast \sim_{iid} g^\ast$. The replica trick applies the formula
\begin{align}\label{ineq:replica_3}
\lim_{d\rightarrow\infty} \frac{1}{d}\E_{g^\ast} \log \Xi_n = \lim_{k\downarrow 0}\partial_k\big[\lim_{d\rightarrow\infty} \frac{1}{d}\log\E_{g^\ast} \Xi_n^k\big], 
\end{align}
where we treat $k$ as an integer. We have 
\begin{align*}
\E_{g^\ast} \Xi_n^k &= \E_{g^\ast} \int g(\btheta^1)\ldots g(\btheta^k) e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k \pnorm{\y - \X\btheta^a}{}^2} \d\btheta^1\ldots\d\btheta^k\\
&= \E_{\X}\int g^\ast(\btheta^0) (2\pi\sigma^2)^{-\frac{n}{2}}e^{-\frac{\pnorm{\y - \X\btheta^0}{}^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k \pnorm{\y - \X\btheta^a}{}^2} \d\btheta^0\d\btheta^1\ldots\d\btheta^k\d \y\\
&= \E_{\X}\int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \prod_{i=1}^n \Big[\int(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y_i - \x_i^\top\btheta^0)^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k (y_i - \x_i^\top\btheta^a)^2}\d y_i\Big]\d\btheta^0\d\btheta^1\ldots\d\btheta^k\\
&= \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \Big[\int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - \x^\top\btheta^0)^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k (y - \x^\top\btheta^a)^2}}\d y\Big]^n\d\btheta^0\d\btheta^1\ldots\d\btheta^k,
\end{align*}
where $\x \sim \N(0, d^{-1}I_d)$, and we use overline to denote the average with respect to $\x$. Let
\begin{align*}
v^0 \equiv \x^\top \btheta^0, v^a \equiv \x^\top \btheta^a, \quad a\in[k],
\end{align*}
we have $(v^0,v^1,\ldots,v^k) \sim \N(0, Q)$ conditioning on $(\btheta^0,\btheta^k)$, where $Q_{ab} = d^{-1}\iprod{\btheta^a}{\btheta^b}$. Hence we have
\begin{align}\label{ineq:replica_1}
\notag\E_{g^\ast}\Xi_n^k &= \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \Big[\int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y\Big]^n\d\btheta^0\d\btheta^1\ldots\d\btheta^k\\
&= \int_{[-M,M]^{\frac{(k+1)(k+2)}{2}}} e^{n\mathcal{G}(Q)} \mu_k(Q) \prod_{0\leq a\leq b \leq k}\d Q_{ab}, 
\end{align}
where
\begin{align*}
\mathcal{G}(Q) = \log \int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y,
\end{align*}
and
\begin{align*}
\mu_k(Q) = \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k)\prod_{0\leq a\leq b \leq k} \delta(\iprod{\btheta^a}{\btheta^b} - dQ_{ab})\d\btheta^0\ldots\d\btheta^k
\end{align*}
is the probability weight of the shell
\begin{align*}
\mathcal{S}(Q) = \{(\btheta^0,\ldots,\btheta^k): d^{-1}\iprod{\btheta^a}{\btheta^b} = Q_{a,b}, 0\leq a\leq b\leq k\}.
\end{align*}
Suppose $-d^{-1}\log \mu_k(Q) \rightarrow_{d\rightarrow\infty} \mathcal{I}(Q)$ for some rate function $\mathcal{I}(Q)$, then applying the Laplace method to (\ref{ineq:replica_1}) yields
\begin{align}\label{ineq:replica_2}
\lim_{d\rightarrow\infty} \frac{1}{d}\log\E_{g^\ast} \Xi_n^k = \sup_{Q} \big[\delta \mathcal{G}(Q) - \mathcal{I}(Q)\big]. 
\end{align}
By the replica-symmetric ansatz, the optimal $Q$ takes the form
\begin{align*}
Q = 
\begin{bmatrix}
r & m & m & m & \ldots & m\\
m & p & q & q & \ldots & q\\
m & q & p & q & \ldots & q\\
\ldots\\
m & q & q & q & \ldots & p
\end{bmatrix}.
\end{align*}
Let us now evaluate $\mathcal{G}(Q)$ and $\mathcal{I}(Q)$ under this ansatz. Denote
\begin{align*}
v^0 = u\sqrt{r-\frac{m^2}{q}} - t\frac{m}{\sqrt{q}}, \quad v^a = z^a\sqrt{p-q} - t\sqrt{q},
\end{align*}
where $u,t,\{z^a\}_{a=1}^k$ are standard normal variables. Then
\begin{align*}
e^{\mathcal{G}(Q)} &= \int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y\\
&= (2\pi\sigma^2)^{-1/2}\E_{u,t,z^a}\int e^{-\frac{r-m^2/q}{2\sigma^2}\big[u - (r-m^2/q)^{-1/2}(y + tm/\sqrt{q})\big]^2} e^{-\frac{p-q}{2\sigma^2}\sum_{a=1}^k\big[z^a - (p-q)^{-1/2}(y + t\sqrt{q})\big]^2} \d y\\
&= (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{1}{2(\sigma^2 + r-m^2/q)}\big[y + \frac{tm}{\sqrt{q}}\big]^2}e^{-\frac{k}{2(\sigma^2 + p-q)}\big[y + t\sqrt{q}\big]^2}\d y\\
&\equiv (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{\mathsf{A_1}}{2}y^2 - \frac{\mathsf{A}_2}{2}t^2 - \mathsf{B}t}\\
&= (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{\mathsf{A_1}}{2}y^2} e^{-\frac{\mathsf{A}_2}{2}(t + \frac{\mathsf{B}}{\mathsf{A}_2})^2} e^{\frac{\mathsf{B}^2}{2\mathsf{A}_2}}\d y,
\end{align*}
where with $\mathsf{U} = 1 + \sigma^{-2}(r-m^2/q)$ and $\mathsf{V} = 1 + \sigma^{-2}(p-q)$, 
\begin{align*}
\mathsf{A}_1 &= \frac{\sigma^{-2}}{\mathsf{U}} + \frac{k\sigma^{-2}}{\mathsf{V}},\\
\mathsf{A}_2 &= \frac{\sigma^{-2}}{\mathsf{U}}\frac{m^2}{q} + \frac{k\sigma^{-2}}{\mathsf{V}}q,\\
\mathsf{B} &= \frac{\sigma^{-2}}{\mathsf{U}}\frac{ym}{\sqrt{q}} + \frac{k\sigma^{-2}}{\mathsf{V}}y\sqrt{q}. 
\end{align*}
Consequently,
\begin{align*}
e^{\mathcal{G}(Q)} &= (2\pi\sigma^2)^{-1/2}V^{-\frac{k-1}{2}}\big[(1+\sigma^{-2}r)\mathsf{V} + kq\sigma^{-2}\mathsf{U}\big]^{-1/2} \int e^{-\frac{\mathsf{A}_1}{2}y^2 + \frac{\mathsf{B}^2}{2(\mathsf{A}_2 + 1)}}\d y\\
&= (2\pi\sigma^2)^{-1/2}V^{-\frac{k-1}{2}}\big[(1+\sigma^{-2}r)\mathsf{V} + kq\sigma^{-2}\mathsf{U}\big]^{-1/2} \int e^{-\frac{y^2}{2}\frac{\sigma^{-2}\mathsf{V} + k\sigma^{-2}\big[1+\sigma^{-2}(r-2m+q)\big]}{(1+r\sigma^{-2})\mathsf{V} + kq\sigma^{-2}\mathsf{U}}}\d y\\
&= \mathsf{V}^{-\frac{k-1}{2}}\big[\mathsf{V} + k(1+\sigma^{-2}(r-2m+q))\big]^{-1/2}.
\end{align*}
Next we evaluate the rate function $\mathcal{I}(Q)$. Since $d^{-1}\iprod{\btheta^a}{\btheta^b}$ is a set of sample means of $d$ i.i.d. variables with law $\mu = \mathcal{L}(\{\theta^a_1\theta^b_1\}_{0\leq a, b\leq k})$ on $\R^{(k+1)^2}$, Cramer's theorem yields that
\begin{align}\label{eq:rate_func}
\mathcal{I}(Q) = \sup_{\{\tilde{Q}_{ab}\}_{0\leq a, b\leq k}} \big[\iprod{\tilde{Q}}{Q} - M(\tilde{Q})\big],
\end{align}
where $M = M_\mu$ is the cumulant generating function of law $\mu$ evaluated as
\begin{align*}
M(\tilde{Q}) = \log \E_{\{Q_{ab}\}_{0\leq a, b\leq k} \sim \mu} e^{\iprod{\tilde{Q}}{Q}} = \log \int g^{\ast}(\theta^0)g(\theta^1)\ldots g(\theta^k) e^{\sum_{0\leq a,b\leq k} \tilde{Q}_{ab}\theta^a\theta^b} \d\theta^0\ldots \d\theta^k.
\end{align*}
Again by the RS ansatz, the optimal $\tilde{Q}$ in (\ref{eq:rate_func}) takes the form
\begin{align*}
\tilde{Q} = 
\begin{bmatrix}
c & d & d & d & \ldots & d\\
d & g & f & f & \ldots & f\\
d & f & g & f & \ldots & f\\
\ldots\\
d & f & f & f & \ldots & g
\end{bmatrix}.
\end{align*}
Hence with $\btheta = (\theta^0,\ldots, \theta^k) \in \R^{k+1}$,
\begin{align*}
M(\tilde{Q}) = M(c,d,f,g) &= \E e^{\iprod{\tilde{Q}}{\btheta\btheta^\top}}\\
&=\E \exp\Big[c(\theta^0)^2 + 2d\theta^0 \cdot \sum_{a=1}^k \theta^a + g \sum_{a=1}^k (\theta^a)^2 + f\sum_{1\leq a\neq b\leq k} \theta^a\theta^b\Big]\\
&=\E \exp\Big[\Big(\frac{d}{\sqrt{f}}\theta^0 + \sqrt{f}\sum_{a=1}^k \theta^a\Big)^2 + (c - \frac{d^2}{f})(\theta^0)^2 + (g-f)(\sum_{a=1}^k \theta^a)^2\Big]\\
&= \E_{\btheta}\E_{z\sim \N(0, \frac{f}{2d^2})}\exp\Big[\frac{2d}{\sqrt{f}}z\Big(\frac{d}{\sqrt{f}}\theta^0 + \sqrt{f}\sum_{a=1}^k \theta^a\Big)+ (c - \frac{d^2}{f})(\theta^0)^2 + (g-f)(\sum_{a=1}^k \theta^a)^2\Big]\\
&= \E_z \E_{\theta^0 \sim g^\ast}\Big(e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k,
\end{align*}
and therefore
\begin{align*}
\mathcal{I}(Q) = \sup_{c,d,f,g} \bigg\{rc + kpg + 2kmd + k(k-1)qf - \log\Big(\E_z \E_{\theta^0 \sim g^\ast}\bigg[e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k\bigg]\bigg\}.
\end{align*}
Combining (\ref{ineq:replica_3}), (\ref{ineq:replica_2}), and (\ref{eq:rate_func}), the RS ansatz yields that
\begin{align}\label{eq:replica_4}
\lim_{d\rightarrow\infty} \frac{1}{d}\E_{g^\ast}\log \Xi_n = \sup_{r,m,p,q}\inf_{c,d,f,g} \partial_k|_{k\downarrow 0}\big[f^{RS}(c,d,f,g, r,m,p,q;k)\big],
\end{align}
where
\begin{align*}
f^{RS} &= -\frac{(k-1)\delta}{2}\log[1+\sigma^{-2}(p-q)] - \frac{\delta}{2}\log\big[1+\sigma^{-2}(p-q)+k(1+\sigma^{-2}(r-2m+q))\big]\\
&\quad - (rc + kpg + 2kmd + k(k-1)qf) + \log\Big(\E_z \E_{\theta^0 \sim g^\ast}\bigg[e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k\bigg]\bigg\}.
\end{align*}
We first represent the optimal $(c,d,f,g)$ in $(r,m,p,q)$ for $k\downarrow 0$. To this end, we have
\begin{align}\label{eq:critical_1}
\notag\partial_r f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow c = 0,\\
\notag\partial_m f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow d = \frac{\delta\sigma^{-2}}{2\big[1+\sigma^{-2}(p-q)\big]},\\
\notag\partial_q\partial_k f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow f = \frac{\delta\sigma^{-2}\big[1+\sigma^{-2}(r-2m+q)\big]}{2\big[1+\sigma^{-2}(p-q)\big]^2},\\
\partial_p\partial_kf^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow g = f - d. 
\end{align}
Plugging these into $M(\cdot)$, we have
\begin{align}\label{eq:mgf_critical}
\notag M(c,d,f,g) &= \E_{z\sim \N(0,\frac{f}{2d^2})} \E_{\theta^0 \sim g^\ast}\Big(e^{\frac{2d^2}{f}z\theta^0 -\frac{d^2}{f}(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2d z\theta -d\theta^2}\Big)\Big]^k\\
&= \sqrt{\frac{\eta}{2\pi}} \int \E_{g^\ast} e^{-\frac{\eta}{2}(z-\theta^0)^2} \Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k \d z,
\end{align}
where we define $(\eta,\xi)$ as
\begin{align}\label{def:eta_xi}
\eta = \frac{2d^2}{f},\quad 2d = \xi.
\end{align}
Let us now represent $(r,m,p,q)$ in $(\xi, \eta)$. From (\ref{eq:rate_func}), the critical $(Q,\tilde{Q})$, denoted by $(Q^\ast,\tilde{Q}^\ast)$ (parametrized under the RS ansatz by $p,q,r,m,c,d,f,g$), satisfies
\begin{align*}
Q^\ast = \frac{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big]}{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\big]} = \frac{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big]}{M(\tilde{Q}^\ast)} \stackrel{k\downarrow 0}{\longrightarrow}\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big],
\end{align*}
where the last step follows since $M(\tilde{Q}^\ast) \rightarrow 1$ as $k\downarrow 0$ from (\ref{eq:mgf_critical}). As an example, let us compute $Q^\ast_{01} = m$, where
\begin{align*}
\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\theta^0\theta^1\big] &= \sqrt{\frac{\eta}{2\pi}}\int \E_{\theta^0\sim g^\ast}\Big[\theta^0 e^{-\frac{\eta}{2}(z - \theta^0)^2}\Big] \cdot \frac{\E_{\theta \sim g^\ast}\Big[\theta e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]}{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]} \cdot \Big\{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]\Big\}^k \d z\\
&\stackrel{k\downarrow 0}{\longrightarrow}\sqrt{\frac{\eta}{2\pi}}\int \E_{\theta^0\sim g^\ast}\Big[\theta^0 e^{-\frac{\eta}{2}(z - \theta^0)^2}\Big] \cdot \frac{\E_{\theta \sim g^\ast}\Big[\theta e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]}{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]} \d z\\
&= \E_{(g^\ast;\eta^{-1})} \big[\theta\av{\theta}_{(g;\xi^{-1})}\big].
\end{align*}
Here we introduce the scalar channel indexed by prior $g$ and noise level $\sigma^2$: 
\begin{align}\label{eq:scalar_channel}
Y = \theta + \eps, \quad \theta \sim g, \eps \sim \N(0,\sigma^2), 
\end{align}
and use $\E_{(g;\sigma^2)}$ to denote the expectation under this channel, and
\begin{align*}
\av{f(\theta)}_{(g;\sigma^2)} = \E[f(\theta)| Y = y] = \frac{\int f(\theta) e^{-\frac{(y-\theta)^2}{2\sigma^2}}g(\d\theta)}{\int  e^{-\frac{(y-\theta)^2}{2\sigma^2}}g(\d\theta)}
\end{align*}
to denote the posterior average. A similar calculation yields that
\begin{align}\label{eq:replica_parameter}
r &= Q^\ast_{00} = \E_{(g_\ast;\eta^{-1})}\big[\theta^2\big],\\
p &= Q^\ast_{11} = \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{(g;\xi^{-1})}\big],\\
q &= Q^\ast_{12} = \E_{(g_\ast;\eta^{-1})}\big[\av{\theta}^2_{(g;\xi^{-1})}\big],
\end{align}
from which we obtain
\begin{align}\label{eq:consistent_1}
\notag r-2m+q &= \E_{(g_\ast;\eta^{-1})}\big[(\theta - \av{\theta}_{g;\xi^{-1}})^2\big],\\
p - q &= \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align}
On the other hand, (\ref{eq:critical_1}) yields
\begin{align}\label{eq:consistent_2}
r-2m+q = \delta\eta^{-1} - \sigma^2, \quad p - q = \delta\xi^{-1} - \sigma^2.
\end{align}
Combining (\ref{eq:consistent_1}) and (\ref{eq:consistent_2}) yields the self-consistent equation for the critical $(\eta_\star, \xi_\star)$:
\begin{align}\label{eq:replica_consistent}
\notag\delta \eta^{-1} &= \sigma^2 + \E_{(g_\ast;\eta^{-1})}\big[(\theta - \av{\theta}_{g;\xi^{-1}})^2\big],\\
\delta \xi^{-1} &= \sigma^2 + \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align}
Lastly, note that (recall (\ref{eq:mgf_critical}))
\begin{align*}
\partial_k|_{k\downarrow 0} \log M(\tilde{Q}^\ast) &= \partial_k|_{k\downarrow 0} \log \Big[\sqrt{\frac{\eta}{2\pi}} \int \E_{g^\ast} e^{-\frac{\eta}{2}(z-\theta^0)^2} \Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k \d z\Big]\\
&= \partial_k|_{k\downarrow 0} \log \E_{z\sim(g^\ast;\eta^{-1})}\big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\big]^k\\
&= \partial_k|_{k\downarrow 0} \E_{z\sim(g^\ast;\eta^{-1})}\Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k\\
&\stackrel{(*)}{=} \E_{z\sim(g^\ast;\eta^{-1})} \log\Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]\\
&= \frac{\xi}{2}(\E_{g^\ast}[\theta^2] + \eta^{-1}) + \frac{1}{2}\log(2\pi\xi^{-1}) + \E_{z\sim(g^\ast;\eta^{-1})}\log p_{(g;\xi^{-1})}(z),
\end{align*}
where we use $p_{(g;\xi)}(\cdot)$ to denote the density of $Y$ in the scalar channel (\ref{eq:scalar_channel}). Then by plugging the critical $(r,m,p,q,c,d,f,g)$ into (\ref{eq:replica_4}), we have
\begin{align*}
\lim_{d} d^{-1}\E_{g^\ast} \log \Xi_n &= -\frac{\delta}{2}\log\big[1+\sigma^{-2}(p-q)\big] - \frac{\delta}{2}\frac{1+\sigma^{-2}(r-2m+q)}{1+\sigma^{-2}(p-q)} - (pg + 2md-qf) + \partial_k|_{k\downarrow 0} \log M(\tilde{Q}^\ast)\\
&= -\frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta\xi}{2\eta} - \xi\sigma^2 + \frac{\xi^2}{2\eta}\sigma^2 + \frac{\delta}{2} + \frac{\xi}{2\eta} + \frac{1}{2}\log(2\pi\xi^{-1}) + \E_{z\sim(g^\ast;\eta^{-1})}\log p_{(g;\xi^{-1})}(z),
\end{align*}
where $(\xi,\eta)$ are given by (\ref{eq:replica_consistent}).

\begin{remark}[Correctly specified case]
In this case, the RS ansatz posits that $d = f$ so $\eta = \xi$, and hence the above RS formula implies that
\begin{align*}
\lim_d d^{-1}I(\y; \btheta) &= \lim_d -d^{-1}\E_{\btheta^\ast \stackrel{i.i.d.}{\sim} g} \log \int e^{-\frac{\pnorm{\X(\btheta - \btheta^\ast)}{}^2}{2\sigma^2} + \frac{\beps^\top \X(\btheta - \btheta^\ast)}{\sigma^2}} \prod_{j=1}^p g(\theta_j)\d\btheta\\
&= -\lim_d d^{-1}\E_{g^\ast} \log \Xi_n - \frac{\delta}{2}\\
&= \frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta}{2} + \frac{\xi\sigma^2}{2} - \frac{1}{2}\log(2\pi\xi^{-1}) - \frac{1}{2} + H(Y;g,\xi^{-1}), 
\end{align*}
where $H(Y;g,\xi^{-1})$ denotes the differential entropy of the law of $Y$ in the channel (\ref{eq:scalar_channel}) with prior $g$ and noise variance $\xi^{-1}$, and $\xi$ solves the equation
\begin{align*}
\delta \xi^{-1} &= \sigma^2 + \E_{(g;\xi^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align*}
This is previously proved in, e.g., Theorem 3.2 of \cite{barbier2020mutual} (with the change of variable $E = \delta\xi^{-1} - \sigma^2$ therein), as
\begin{align*}
\lim_d d^{-1}I(\y; \btheta) = \inf i^{RS}(\xi^{-1}),
\end{align*}
where
\begin{align*}
i^{RS}(\xi^{-1}) = \frac{1}{2}\Big(\delta\log(\frac{\delta}{\sigma^2\xi}) - \delta + \frac{\sigma^2}{\xi^{-1}}\Big) + i_{(g;\xi^{-1})}(Y;\theta)
\end{align*}
with $i_{(g;\xi^{-1})}(Y;\theta)$ denotes the mutual information of the scalar channel (\ref{eq:scalar_channel}).
\end{remark}

\begin{remark}[Gaussian prior with mismatched variance]
Suppose $g^\ast = \N(0,\tau^2_\ast)$ and $g = \N(0,\tau^2)$, then 
\begin{align*}
&\lim_d d^{-1}\E_{g^\ast} \log \int e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2} - \frac{\pnorm{\btheta}{}^2}{2\tau^2}}\d\btheta\\
&= \frac{1}{2}\log(2\pi\tau^2) + \lim_d d^{-1}\E_{g^\ast} \log \Xi_n\\
&= -\frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta\xi}{2\eta} - \xi\sigma^2 + \frac{\xi^2}{2\eta}\sigma^2 + \frac{\delta}{2} + \frac{\xi}{2\eta} + \frac{1}{2}\log(\xi^{-1}) -\frac{1}{2}\log\big(\tau^2+\xi^{-1}) - \frac{\tau^2_\ast + \eta^{-1}}{2(\tau^2+\xi^{-1})} + \frac{1}{2}\log(2\pi\tau^2), 
\end{align*}
where we use $p_{g;\xi^{-1}}(y) = (2\pi (\tau^2 + \xi^{-1}))^{-1/2} e^{-\frac{y^2}{2(\tau^2 + \xi^{-1})}}$, and hence $\E_{y\sim (g^\ast;\eta^{-1})} \log p_{g;\xi^{-1}}(y) = -\frac{1}{2}\log\big[2\pi(\tau^2+\xi^{-1})\big] - \frac{\tau^2_\ast + \eta^{-1}}{2(\tau^2+\xi^{-1})}$. Next note that $\av{\theta}_{(g;\xi^{-1})} = \frac{\tau^2}{\tau^2 + \xi^{-1}}y$ and $\av{\theta^2}_{(g;\xi^{-1})} = \Big(\frac{\tau^2}{\tau^2 + \xi^{-1}}y\Big)^2 + \frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}$, so the consistent equation for $\xi$ reads
\begin{align}\label{eq:consistent_xi}
\delta \xi^{-1} = \sigma^2 + \frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}. 
\end{align}
Then the above RS formula can be further simplified as
\begin{align*}
&=\frac{\delta}{2}\log\Big(\frac{\sigma^2\xi}{\delta}\Big) + \frac{1}{2}\log\Big(\frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}\Big) + \frac{1}{2}\log(2\pi) - \frac{\tau_\ast^2}{2(\tau^2+\xi^{-1})} + \frac{\delta}{2} -\sigma^2\xi - \frac{1}{2\eta(\tau^2+\xi^{-1})}\big[\underbrace{(1+\tau^2\xi)(\delta-\sigma^2\xi-1) + 1}_{=0}\big]\\
&= \frac{\delta}{2}\log\Big(\frac{\sigma^2\xi}{\delta}\Big) + \frac{1}{2}\log\Big(\frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}\Big) + \frac{1}{2}\log(2\pi) - \frac{\tau_\ast^2}{2(\tau^2+\xi^{-1})} + \frac{\delta}{2} -\sigma^2\xi,
\end{align*}
where $\xi$ is given by (\ref{eq:consistent_xi}). This is previously proved rigorously in Theorem 3.4 of \cite{barbier2021performance}, with change of variable $c = \rho - q = \delta\xi^{-1} - \sigma^2$ therein. The same reference also shows that the limiting MSE is
\begin{align*}
\mse(g;g^\ast) \equiv \lim_{d\rightarrow\infty} d^{-1}\E_{g^\ast} \pnorm{\av{\btheta}_g - \btheta^\ast}{}^2 = \frac{\sigma^2\tau^4 + \delta\xi^{-2}\tau_\ast^2}{\delta(\xi^{-1} + \tau^2)^2 - \tau^4}.
\end{align*}
In the replica notation, this corresponds to $q + \tau_\ast^2- 2m$, given by (\ref{eq:replica_parameter}).
\end{remark}




==> singleparticle.tex <==
\section{Proof of Theorem \ref{thm:dmft_entrywise}}


\subsection{Refined leave-one-out analysis}

We introduce some further notation. For any $\cJ \subset [d]$ and $k\in[d]$ such that $k\notin \cJ$, let $\X_{(\cJ)}$ be $\X$ with columns in $\cJ$ set to 0, and $\X_{(k,\cJ)}$ with additional the $k$th column both set to $0$. Let $\y_{(\cJ)} = \X_{(\cJ)}\btheta^\ast + \beps$ and $\y_{(k,\cJ)} = \X_{(k,\cJ)}\btheta^\ast + \beps$. Analogous to the leave-one-out dynamic in (\ref{eq:leave_col_out}), consider the following leave-two-out dynamic:
\begin{align}\label{eq:leave_two_col_out}
\notag\btheta^{t+1}_{(k,\cJ)} &= \btheta^{t}_{(k,\cJ)} - \gamma\Big[\beta\X_{(k,\cJ)}^\top(\X_{(k,\cJ)}\btheta^{t}_{(k,\cJ)} - \y_{(k,\cJ)}) - s(\btheta^{t}_{(k,\cJ)}, \hat{\alpha}^{t}_{(k,\cJ)})\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma})\in \R^{d},\\
\hat{\alpha}^{t+1}_{(k,\cJ)} &= \hat{\alpha}^{t}_{(k,\cJ)} + \gamma \cG\Big(\hat{\alpha}^t_{(k,\cJ)}, \sP(\btheta^{t}_{(k,\cJ)})\Big),
\end{align}
with initialization $\hat\alpha^0_{(k,\cJ)} = \hat\alpha^0$ same as in (\ref{eq:leave_col_out}), and $(\btheta^0_{(k,\cJ)})_\ell = \theta^0_\ell$ if $\ell \notin \cJ \cup \{k\}$ and 0 otherwise.
\begin{lemma}\label{|em:loo_linfty_error}
Suppose Assumptions \ref{assump:model}, \ref{assump:prior}, and \ref{assump:gradient} hold. For any positive integer $T$, there exists some $C > 0$ depending on $T$ (and other problem parameters) such that for any $0\leq t\leq T$, 
\begin{align}
&\max_{\cJ\subset[d], k\in [d]:k\notin \cJ} \E\Big[\big|\e_k^\top (\btheta^{t} - \btheta^{t}_{(\cJ)}) \big|^q|\theta^0_\cJ, \theta^\ast_\cJ\Big] \leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^{q/2}}, \label{eq:loo_linfty}\\
&\max_{\cJ\subset[d], k\in [d]: k\notin \cJ} \E\Big[\pnorm{\hat{\alpha}^t - \hat{\alpha}_{(\cJ)}^t - \hat{\alpha}_{(k)}^t + \hat{\alpha}^t_{(k,\cJ)}}{}^q|\theta^0_\cJ, \theta^\ast_\cJ \Big] \leq \frac{(C + K_\gamma \exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast}{} + 1)^q}{d^q}, \label{eq:alpha_lto_l2} \\
&\max_{\cJ\subset[d], k\in [d]: k\notin \cJ}\E\Big[\Big(\sum_{\ell\in[d]:\ell\neq k,\ell\notin \cJ} \Big(\e_\ell^\top \big(\btheta^{t} - \btheta^{t}_{(k)} - \btheta^{t}_{(\cJ)} + \btheta^{t}_{(k,\cJ)}\big)\Big)^2\Big)^{q/2}|\theta^0_\cJ, \theta^\ast_\cJ\Big] \leq \frac{(C + K_\gamma \exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast}{} + 1)^q}{d^{q/2}} \label{eq:lto_l2}.
\end{align}
\end{lemma}
\begin{proof}
We prove by induction the in-probability versions of (\ref{eq:loo_linfty})-(\ref{eq:lto_l2}). The baseline case for $t=0$ holds by definition. Suppose the above claims hold up to some $t\geq 0$, and we will establish them for $t+1$. 

\noindent\textbf{Bound of (\ref{eq:loo_linfty})} For any $\cJ\subset[d]$ with fixed cardinality, we have
\begin{align*}
\btheta^{t+1} &= \btheta^t - \gamma\beta \X^\top (\X\btheta^t - \y) + \gamma s(\btheta^t,\hat\alpha^t) + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}), \\
\btheta^{t+1}_{(\cJ)} &= \btheta^t_{(\cJ)} - \gamma\beta \X_{(\cJ)}^\top (\X_{(\cJ)}\btheta^t_{(\cJ)} - \y_{(\cJ)}) + \gamma s(\btheta^t_{(\cJ)},\hat\alpha^t_{(\cJ)}) + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}). 
\end{align*}
Let $\bar{\X}_{(\cJ)} \in \R^{n\times (d-|\cJ|)}$ be $\X$ with columns in $\cJ$ removed. Then for any $k\in[d]$ such that $k\notin \cJ$, we have
\begin{align*}
\e_k^\top (\btheta^{t+1} - \btheta^{t+1}_{(\cJ)}) &= \underbrace{\e_k^\top (I - \gamma\beta\X^\top \X) (\btheta^t - \btheta^t_{(\cJ)})}_{(I)} - \gamma\beta \underbrace{\e_k^\top (\X^\top \X - \X_{(\cJ)}^\top \X_{(\cJ)})\btheta^t_{(\cJ)}}_{(II)} + \gamma\beta \underbrace{\e_k^\top(\X^\top \y - \X_{(\cJ)}^\top \y_{(\cJ)})}_{(III)}\\
&\quad + \gamma\underbrace{\big(s(\theta^t_k,\hat\alpha^t) - s((\btheta^t_{(\cJ)})_k,\hat\alpha^t_{(\cJ)})\big)}_{(IV)}.
\end{align*}
For $(I)$, we have
\begin{align*}
|(I)| &\leq |\e_k^\top (\btheta^t - \btheta^t_{(\cJ)})| + C\gamma\Big|\x_k^\top \X (\btheta^t - \btheta^t_{(\cJ)})\Big| \leq (1+C\gamma\pnorm{\x_k}{}^2)|\e_k^\top (\btheta^t - \btheta^t_{(\cJ)})| + \gamma\Big|\sum_{\ell\in[d]:\ell\neq k} (\x_k^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)})\Big|\\
&\leq  (1+C\gamma\pnorm{\x_k}{}^2)|\e_k^\top (\btheta^t - \btheta^t_{(\cJ)})| + \gamma\Big|\sum_{\ell\in[d]:\ell\neq k} (\x_k^\top \x_\ell) \e_\ell^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})\Big|\\
&\quad + \gamma\Big|\sum_{\ell\in[d]:\ell\neq k} (\x_k^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)})\Big|.
\end{align*}
By the induction hypothesis, the first term satisfies $\E[(1+C\gamma\pnorm{\x_k}{}^2)^q|\e_k^\top (\btheta^t - \btheta^t_{(\cJ)})|^q] \leq C/d^{q/2}$. The second term equals $\gamma \cdot \x_k^\top \bar{\X}_{(k)} (\bar{\btheta}^t_{(k)} - \bar{\btheta}^t_{(k,\cJ)})$, where $\bar{\X}_{(k)} \in \R^{n\times (d-1)}$ denotes $\X$ minus its $k$th column, and $\bar{\btheta}^t_{(k)}, \bar{\btheta}^t_{(k,\cJ)} \in \R^{d-1}$ represent $\btheta^t_{(k)}, \btheta^t_{(k,\cJ)}$ without their $k$th component. Since $\x_k$ is independent of $\bar{\X}_{(k)}, \bar{\btheta}^t_{(k)}, \bar{\btheta}^t_{(k,\cJ)}$, we have $\x_k^\top \bar{\X}_{(k)} (\bar{\btheta}^t_{(k)} - \bar{\btheta}^t_{(k,\cJ)}) | \bar{\X}_{(k)} \stackrel{d}{=} \N(0, d^{-1}\pnorm{\bar{\X}_{(k)} (\bar{\btheta}^t_{(k)} - \bar{\btheta}^t_{(k,\cJ)})}{}^2)$, where by Lemma \ref{lem:loo_error}, we have $\E\pnorm{\bar{\X}_{(k)} (\bar{\btheta}^t_{(k)} - \bar{\btheta}^t_{(k,\cJ)})}{}^q \leq C$. Hence we conclude that 
\begin{align*}
\E\Big|\sum_{\ell\in[d]:\ell\neq k} (\x_k^\top \x_\ell) \e_\ell^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})\Big|^q \leq C/d^{q/2}.
\end{align*}
Let $\bar{\X}_{(k,\cJ)} \in \R^{n\times (d-1-|\cJ|)}$ be $\X$ minus its column $i$ and columns in $\cJ$, and $\tilde{\btheta}^t, \tilde{\btheta}^t_{(\cJ)}, \tilde{\btheta}^t_{(k)}, \tilde{\btheta}^t_{(k,\cJ)}\in\R^{d-1-|\cJ|}$ be $\btheta^t, \btheta^t_{(\cJ)}, \btheta^t_{(k)}, \btheta^t_{(k,\cJ)}$ minus component $i$ and components in $\cJ$. Then the last term satisfies
\begin{align*}
\Big|\sum_{\ell\in[d]:\ell\neq k} (\x_k^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)})\Big| &\leq \sum_{\ell \in \cJ}|\x_k^\top \x_\ell | \Big|\e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)})\Big|\\
&\quad + \Big|\x_k^\top \bar{\X}_{(k,\cJ)}(\tilde{\btheta}^t - \tilde{\btheta}^t_{(\cJ)} - \tilde{\btheta}^t_{(k)} + \tilde{\btheta}^t_{(k,\cJ)})\Big|.
\end{align*}
By bound (\ref{eq:loo_expectation_5}) ahead, we have $\E|\x_j^\top \x_i |^q \big|\e_i^\top (\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)})\big|^q \leq C/d^{q/2}$, and 
\begin{align*}
\Big|\x_k^\top \bar{\X}_{(k,\cJ)} (\tilde{\btheta}^t - \tilde{\btheta}^t_{(\cJ)} - \tilde{\btheta}^t_{(k)} + \tilde{\btheta}^t_{(k,\cJ)})\Big| &\leq \pnorm{\x_k}{}\pnorm{\X}{\op} \cdot \pnorm{\tilde{\btheta}^t - \tilde{\btheta}^t_{(\cJ)} - \tilde{\btheta}^t_{(k)} + \tilde{\btheta}^t_{(k,\cJ)}}{},
\end{align*}
which implies, by the induction hypothesis, that $\E \Big|\x_k^\top \bar{\X}_{(k,\cJ)}(\tilde{\btheta}^t - \tilde{\btheta}^t_{(\cJ)} - \tilde{\btheta}^t_{(k)} + \tilde{\btheta}^t_{(k,\cJ)})\Big|^q \leq C/d^{q/2}$. In summary, we have $\E|(I)|^q \leq C/d^{q/2}$. 

To bound $(II)$, we apply $\X = \X_{(\cJ)} + \X_\cJ\bE_\cJ^\top$ to obtain $\X^\top \X - \X_{(\cJ)}^\top \X_{(\cJ)} = \X_{(\cJ)}^\top \X_\cJ\bE_\cJ^\top + \bE_\cJ \X_\cJ^\top \X_{(\cJ)} + \bE_\cJ \X_\cJ^\top \X_{\cJ} \bE_\cJ^\top$, so
\begin{align*}
|(II)| = \Big|\e_k^\top (\X_{(\cJ)}^\top \X_\cJ\bE_\cJ^\top + \bE_\cJ \X_\cJ^\top \X_{(\cJ)} + \bE_\cJ \X_\cJ^\top \X_{\cJ} \bE_\cJ^\top) \btheta^t_{(\cJ)}\Big| \leq \pnorm{\X_\cJ^\top \x_k}{}|\bE_\cJ^\top \btheta^t_{(\cJ)}|, 
\end{align*}
which, by standard concentration and bound (\ref{eq:loo_expectation_5}), implies that $\E|(II)|^q \leq C/d^{q/2}$.  For $(III)$, since $\X^\top \y - \X_{(\cJ)}^\top \X_{(\cJ)} = \X^\top \X_\cJ \theta^\ast_\cJ + \bE_\cJ(\X_\cJ^\top \X\btheta^\ast - \X_\cJ^\top \X_\cJ \theta^\ast_\cJ + \X_\cJ^\top \beps)$, we have the same bound $\E|(III)|^q = \E|\x_k^\top \X_\cJ\theta^\ast_\cJ|^q \leq C/d^{q/2}$. Lastly, by Assumption \ref{assump:prior} we have $|(IV)| \leq C|\e_k^\top (\btheta^t - \btheta^t_{(\cJ)})| + |\hat\alpha^t - \hat\alpha^t_{(\cJ)}|$, hence $\E|(IV)|^q \leq C/d^{q/2}$ via Lemma \ref{lem:loo_error} and the induction hypothesis. Combining the above bounds yields that $\E|\e_k^\top (\btheta^{t+1} - \btheta^{t+1}_{(\cJ)})|^q \leq C/d^{q/2}$, which concludes the induction for (\ref{eq:loo_linfty}).


\noindent\textbf{Bound of (\ref{eq:lto_l2})} Note that for some $(\tilde{\alpha}, \tilde{\btheta})$ (resp. $(\check{\alpha}, \check{\btheta})$) on the segment connecting $(\hat\alpha^t, \btheta^t)$ and $(\hat\alpha^t_{(\cJ)}, \btheta^t_{(\cJ)})$ (resp. $(\hat\alpha^t_{(k)}, \btheta^t_{(k)})$ and $(\hat\alpha^t_{(k,\cJ)}, \btheta^t_{(k,\cJ)})$), it holds that
\begin{align*}
\hat\alpha^{t+1} - \hat\alpha^{t+1}_{(\cJ)} &= \hat\alpha^t - \hat\alpha^t_{(\cJ)} + \gamma \Big(\cG(\hat\alpha^t, \sP(\btheta^t))  - \cG(\hat{\alpha}^t_{(\cJ)}, \sP(\btheta^t_{(\cJ)}))\Big)\\
&= \hat\alpha^t - \hat\alpha^t_{(\cJ)} + \gamma \nabla_\alpha \cG(\tilde{\alpha}, \sP(\tilde{\btheta}))^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)}) + \gamma\nabla_{\btheta} \cG(\tilde{\alpha}, \sP(\tilde{\btheta}))^\top (\btheta^t - \btheta^t_{(\cJ)}), \\
\hat\alpha^{t+1}_{(k)} - \hat\alpha^{t+1}_{(k,\cJ)} &= \hat\alpha^t_{(k)} - \hat\alpha^t_{(k,\cJ)} + \gamma \Big(\cG(\hat\alpha^t_{(k)}, \sP(\btheta^t_{(k)}))  - \cG(\hat{\alpha}^t_{(k,\cJ)}, \sP(\btheta^t_{(k,\cJ)}))\Big)\\
&= \hat\alpha^t_{(k)} - \hat\alpha^t_{(k,\cJ)} + \gamma \nabla_\alpha \cG(\check{\alpha}, \sP(\check{\btheta}))^\top (\hat{\alpha}^t_{(k)} - \hat{\alpha}^t_{(k,\cJ)}) + \gamma\nabla_{\btheta} \cG(\check{\alpha}, \sP(\check{\btheta}))^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}).
\end{align*}
Consequently, we have
\begin{align*}
\pnorm{\hat\alpha^{t+1} - \hat\alpha^{t+1}_{(\cJ)} - \hat\alpha^{t+1}_{(k)} + \hat\alpha^{t+1}_{(k,\cJ)}}{} &\leq \pnorm{\hat\alpha^{t} - \hat\alpha^{t}_{(\cJ)} - \hat\alpha^{t}_{(k)} + \hat\alpha^{t}_{(k,\cJ)}}{} + C \underbrace{\Big|\Big(\nabla_\alpha \cG(\tilde{\alpha}, \sP(\tilde{\btheta})) - \nabla_\alpha \cG(\check{\alpha}, \sP(\check{\btheta})) \Big)^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)})\Big|}_{(I)}\\
&\quad + C\underbrace{\pnorm{\nabla_\alpha \cG(\check{\alpha}, \sP(\check{\btheta}))}{} \pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)} - \hat\alpha^{t}_{(k)} + \hat\alpha^{t}_{(k,\cJ)}}{}}_{(II)}\\
&\quad + C\underbrace{\Big|\Big(\nabla_{\btheta} \cG(\tilde{\alpha}, \sP(\tilde{\btheta})) - \nabla_{\btheta} \cG(\check{\alpha}, \sP(\check{\btheta})) \Big)^\top (\btheta^t - \btheta^t_{(\cJ)})\Big|}_{(III)}\\
&\quad + C\underbrace{\Big|\nabla_{\btheta} \cG(\check{\alpha}, \sP(\check{\btheta}))^\top \Big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\Big) \Big|}_{(IV)}.
\end{align*}
Note that $\pnorm{\tilde\alpha - \check\alpha}{} \leq Cd(\alpha)$ and $\pnorm{\tilde\btheta - \check\btheta}{}\leq Cd(\btheta)$, where
\begin{align}\label{eq:dalpha_dtheta}
\notag d(\alpha) &:= \pnorm{\hat\alpha^t - \hat\alpha^t_{(\cJ)}}{} \vee \pnorm{\hat\alpha^t - \hat\alpha^t_{(k)}}{} \vee  \pnorm{\hat\alpha^t_{(k)} - \hat\alpha^t_{(k,\cJ)}}{},\\
d(\btheta) &:= \pnorm{\btheta^t - \btheta^t_{(\cJ)}}{} \vee \pnorm{\btheta^t - \btheta^t_{(k)}}{} \vee  \pnorm{\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}}{},
\end{align}
which satisfies $\E[d^q(\alpha)| \theta^0_\cJ, \theta^\ast_\cJ] \leq (C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q/d^{q/2}$ and $\E[d^q(\btheta)| \theta^0_\cJ, \theta^\ast_\cJ] \leq (C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$ by Lemma \ref{lem:loo_error}. Then by Assumption \ref{assump:gradient}, $(I)$ satisfies
\begin{align*}
\E[|(I)|^q | \theta^0_\cJ, \theta^\ast_\cJ] &\leq C\E\Big[\pnorm{\nabla_\alpha^2 \cG_1(\alpha, \sP(\btheta))}{\op}^qd(\alpha)^{2q} + \pnorm{\nabla_\alpha\nabla_{\btheta} \cG_1(\alpha, \sP(\btheta))}{\op}^qd(\alpha)^q d(\btheta)^q|\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\leq (C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^{2q}/d^q.
\end{align*}
Term $(II) \leq C\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)} - \hat\alpha^{t}_{(k)} + \hat\alpha^{t}_{(k,\cJ)}}{}$. Next we have $(III) \leq C\max_{k\in[K]}\pnorm{\nabla_\alpha\nabla_{\btheta}\cG_k(\alpha,\sP(\btheta))}{F}d(\alpha)d(\btheta) + \pnorm{\nabla_{\btheta}^2 \cG_k(\alpha,\sP(\btheta))}{\op}d(\btheta)^2$, so
\begin{align*}
\E[|(III)|^q|\theta^0_\cJ, \theta^\ast_\cJ] &\leq C\E\Big[\pnorm{\nabla_\alpha\nabla_{\btheta} \cG_1(\alpha, \sP(\btheta))}{\op}^qd(\alpha)^{q}d(\btheta)^q + \pnorm{\nabla^2_{\btheta} \cG_1(\alpha, \sP(\btheta))}{\op}^qd(\btheta)^{2q}|\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\leq (C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^{2q}/d^q.
\end{align*}
Lastly $(IV)$ satisfies
\begin{align*}
(IV) &\leq \Big|\nabla_{\theta_\cJ} \cG(\check{\alpha}, \sP(\check{\btheta})) \cdot \bE_\cJ^\top  \Big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\Big)\Big|\\
&\quad + \Big|\partial_{\theta_k} \cG(\check{\alpha}, \sP(\check{\btheta})) \cdot \e_k^\top  \Big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\Big)\Big|\\
&\quad + \Big|\partial_{\btheta \backslash \theta_k, \theta_\cJ} \cG(\check{\alpha}, \sP(\check{\btheta}))^\top \Big(\tilde{\btheta}^t - \tilde{\btheta}^t_{(\cJ)} - \tilde{\btheta}^t_{(k)} + \tilde{\btheta}^t_{(k,\cJ)}\Big)\Big|,
\end{align*}
where we recall that $\tilde{\btheta}^t, \tilde{\btheta}^t_{(\cJ)}, \tilde{\btheta}^t_{(k)}, \tilde{\btheta}^t_{(k,\cJ)}\in\R^{d-1-|\cJ|}$ are $\btheta^t, \btheta^t_{(\cJ)}, \btheta^t_{(k)}, \btheta^t_{(k,\cJ)}$ minus component $k$ components in $\cJ$. Again by Assumption \ref{assump:gradient} and the bound (\ref{eq:loo_expectation_5}), the first two terms satisfy
\begin{align*}
&\E\Big[\Big|\nabla_{\theta_\cJ} \cG(\check{\alpha}, \sP(\check{\btheta})) \cdot \bE_\cJ^\top  \Big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\Big)\Big|^q |\theta^0_\cJ, \theta^\ast_\cJ\Big] \leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q},\\
&\E\Big[\Big|\partial_{\theta_k} \cG(\check{\alpha}, \sP(\check{\btheta})) \cdot \e_k^\top  \Big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\Big)\Big|^q |\theta^0_\cJ, \theta^\ast_\cJ\Big] \leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q}, 
\end{align*}
and by the same assumption and the induction hypothesis, the last term satisfies
\begin{align*}
\E\Big[\Big|\partial_{\btheta \backslash \theta_i, \theta_j} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top \Big(\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}\Big)\Big|^q |\theta^0_\cJ, \theta^\ast_\cJ\Big] &\leq \E\Big[\pnorm{\nabla_{\btheta} \cG(\check{\alpha}, \sP(\check{\btheta}))}{}\pnorm{\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}}{}|\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\leq \frac{(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q}.
\end{align*}
Combining the bounds of $(I)$-$(IV)$ yields the desired conclusion. 

\noindent\textbf{Bound of (\ref{eq:lto_l2})} We have
\begin{align*}
\btheta^{t+1} - \btheta^{t+1}_{(\cJ)} &= (I - \gamma\beta\X^\top \X)(\btheta^t - \btheta^t_{(\cJ)}) - \gamma\beta (\X^\top \X - \X_{(\cJ)}^\top \X_{(\cJ)})\btheta^t_{(\cJ)}+ \gamma\beta (\X^\top \y - \X_{(\cJ)}^\top \y_{(\cJ)})\\
&\quad + \gamma \diag(\partial_\theta s(\btheta^t_{(k,\cJ)}, \hat{\alpha}^t_{(k,\cJ)})) (\btheta^t - \btheta^t_{(\cJ)}) + \Delta^t_1,  
\end{align*}
where $\Delta^t_1 = s(\btheta^t,\hat{\alpha}^t) - s(\btheta^t_{(\cJ)}, \hat{\alpha}^t_{(\cJ)}) - \diag(\partial_\theta s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k,\cJ)}))(\btheta^t - \btheta^t_{(\cJ)})$. Similarly,
\begin{align*}
\btheta^{t+1}_{(k)} - \btheta^{t+1}_{(k,\cJ)} &= (I - \gamma\beta\X_{(k)}^\top \X_{(k)})(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}) - \gamma\beta (\X_{(k)}^\top \X_{(k)} - \X_{(k,\cJ)}^\top \X_{(k,\cJ)})\btheta^t_{(k,\cJ)} + \gamma\beta (\X^\top_{(k)} \y_{(k)} - \X_{(k,\cJ)}^\top \y_{(k,\cJ)})\\
&\quad + \gamma \diag(\partial_\theta^2 \log g(\btheta^t_{(k,\cJ)};\hat{\alpha}^t_{(k,\cJ)})) (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}) + \Delta^t_2, 
\end{align*}
where $\Delta^t_2 =  s(\btheta^t_{(k)}, \hat{\alpha}^t_{(k)}) - s(\btheta^t_{(k,\cJ)}, \hat{\alpha}^t_{(k,\cJ)}) - \diag(\partial_\theta s(\btheta^t_{(k,\cJ)}, \hat{\alpha}^t_{k,\cJ}))(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})$. This implies that
\begin{align}\label{eq:ltw_decompose}
\notag&\btheta^{t+1} - \btheta^{t+1}_{(\cJ)} - (\btheta^{t+1}_{(k)} - \btheta^{t+1}_{(k,\cJ)}) = \Big(I - \gamma\beta\X^\top \X + \gamma \diag(\partial_\theta s(\btheta^t_{k,\cJ}, \hat\alpha^t_{k,\cJ}))\Big)\big(\btheta^{t} - \btheta^{t}_{(\cJ)} - (\btheta^{t}_{(k)} - \btheta^{t}_{(k,\cJ)})\big)\\
\notag&\quad - \gamma\beta \underbrace{(\X^\top \X - \X_{(k)}^\top \X_{(k)})(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})}_{(I)} - \gamma\beta\underbrace{\Big[(\X^\top \X - \X_{(\cJ)}^\top \X_{(\cJ)})\btheta^{t}_{(\cJ)} - (\X_{(k)}^\top \X_{(k)} - \X_{(k,\cJ)}^\top \X_{(k,\cJ)})\btheta^t_{(k,\cJ)}\Big]}_{(II)}\\
&\quad + \gamma\beta\underbrace{\Big((\X^\top \y - \X_{(\cJ)}^\top \y_{(\cJ)}) - (\X^\top_{(k)} \y_{(k)} - \X_{(k,\cJ)}^\top \y_{(k,\cJ)})\Big)}_{(III)} + \underbrace{\Delta^t_1 - \Delta^t_2}_{(IV)}.
\end{align}
To bound $(I)$, we have $\X^\top \X - \X_{(k)}^\top \X_{(k)} = \X_{(k)}^\top \x_k \e_k^\top + \e_k \x_k^\top \X_{(k)} + \e_k\e_k^\top \pnorm{\x_k}{}^2$, so
\begin{align*}
\pnorm{(I)}{} &= \Big|(\X_{(k)}^\top \x_k \e_k^\top + \e_k\x_k^\top \X_{(k)} + \e_k\e_k^\top \pnorm{\x_k}{}^2) (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}) \Big|\\
&\leq 2\pnorm{\X}{\op}\pnorm{\x_k}{}|\e_k^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})| + \big|\x_k^\top \X_{(k)}(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})\big|.
\end{align*}
By the induction hypothesis, the first term satisfies
\begin{align*}
\E\Big[\pnorm{\X}{\op}^q\pnorm{\x_k}{}^q|\e_k^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})|^q | \theta^0_\cJ, \theta^\ast_\cJ\Big] \leq \frac{(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{}+1)^q}{d^{q/2}}.
\end{align*}
%\begin{align*}
%\E\Big[\pnorm{\X}{\op}^2\pnorm{\x_j}{}^2|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})|^2\Big] \vee \E\Big[\pnorm{\x_j}{}^4 \big|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})\big|^2\Big] \leq C\log d/d.
%\end{align*}
For the second term, using independence between $\x_k$ and $\X_{(k)}, \btheta^t_{(k)}, \btheta_{(k,\cJ)}$, Rosenthal's inequality \cite[Theorem 15.11]{boucheron2013concentration}, and Lemma \ref{lem:loo_error}, we have
\begin{align*}
\E\Big[\big|\x_k^\top \X_{(k)}(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})\big|^q |\theta^0_\cJ, \theta^\ast_\cJ\Big] &\leq C\E\Big[(\pnorm{\X_{(k)}(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})}{}/\sqrt{d})^q|\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\leq \frac{(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{}+1)^q}{d^{q/2}}
\end{align*} 

To bound $(II)$, we use $\X^\top \X - \X_{(\cJ)}^\top \X_{(\cJ)} = \X_{(\cJ)}^\top \X_\cJ \bE_\cJ^\top + \bE_\cJ \X_\cJ^\top \X_{(\cJ)} + \bE_\cJ \X_\cJ^\top \X_\cJ \bE_\cJ^\top$ and $\X_{(k)}^\top \X_{(k)} - \X_{(k,\cJ)}^\top \X_{(k,\cJ)} = \X_{(k,\cJ)}^\top\X_\cJ\bE_\cJ^\top + \bE_\cJ\X_\cJ^\top\X_{(k,\cJ)} + \bE_\cJ \X_\cJ^\top \X_\cJ \bE_\cJ^\top$, hence
\begin{align*}
(II) = \underbrace{\X_{(\cJ)}^\top \X_\cJ \bE_\cJ^\top \btheta^t_{(\cJ)} - \X_{(k,\cJ)}^\top\X_\cJ\bE_\cJ^\top \btheta^t_{(k,\cJ)}}_{(II_1)} + \underbrace{\bE_\cJ \X_\cJ^\top \X_{(\cJ)} \btheta^t_{(\cJ)} - \bE_\cJ\X_\cJ^\top\X_{(k,\cJ)}\btheta^t_{(k,\cJ)}}_{(II_2)} + \underbrace{\bE_\cJ \X_\cJ^\top \X_\cJ \bE_\cJ^\top  (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})}_{(II_3)}.
\end{align*}
Using $\X_{(k,\cJ)} = \X_{(\cJ)} - \x_k\e_k^\top$, we have $\pnorm{(II_1)}{} = \pnorm{\X_{(\cJ)}^\top \X_\cJ\bE_\cJ^\top (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})+ \e_k \x_k^\top \X_\cJ \bE_\cJ^\top \btheta^t_{(k,\cJ)}}{} \leq \pnorm{\X}{\op}^2\pnorm{\bE_\cJ^\top (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})}{} + \pnorm{\X_\cJ^\top \x_k}{}\pnorm{\bE_\cJ^\top \btheta^t_{(k,\cJ)}}{}$, hence we have the desired bound for $\E[\pnorm{(II_1)}{}^q|\theta^0_\cJ, \theta^\ast_\cJ]$ by the induction hypothesis (\ref{eq:loo_linfty}), standard concentration, and bound (\ref{eq:loo_expectation_5}). %we have
%\begin{align*}
%\pnorm{(II_1)}{} \leq \pnorm{\X}{\op}\pnorm{\x_i}{} |\e_i^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\x_j^\top \x_i| |\e_i^\top \btheta^t_{(i,j)}| = O_P(1/\sqrt{d}).
%\end{align*}
Next we have $(II_2) = \bE_\cJ \X_\cJ^\top \X_{(\cJ)} (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)}) + \bE_\cJ \X_\cJ^\top \x_k \e_k^\top \btheta^t_{(k,\cJ)}$, hence $\pnorm{(II_2)}{} \leq \pnorm{\X_\cJ^\top \X_{(\cJ)} (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})}{} + \pnorm{\X_\cJ^\top \x_k}{}|\e_k^\top \btheta^t_{(k,\cJ)}|$, and the desired bound holds for $\E[\pnorm{(II_2)}{}^q|\theta^0_\cJ, \theta^\ast_\cJ]$ by independence of $\X_\cJ$ with $\X_{(\cJ)},\btheta^t_{(\cJ)},\btheta^t_{(k,\cJ)}$, Lemmas \ref{lem:loo_error} and bound (\ref{eq:loo_expectation_5}).
%, we have
%\begin{align*}
%\pnorm{(II_2)}{} \leq  |\x_i^\top \X_{(i)} (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\x_i^\top \x_j||\e_j^\top \btheta^t_{(i,j)}| = O_P(1/\sqrt{d}).
%\end{align*}
A similar bound holds for $(II_3)$, so we conclude the desired bound for $\E[\pnorm{(II)}{}^q|\theta^0_\cJ, \theta^\ast_\cJ]$.

To bound $(III)$, direct calculation shows that $(III) = \bE_\cJ \X_\cJ^\top \x_k \theta^\ast_k + \e_k \x_k^\top \X_\cJ \theta^\ast_\cJ$, hence we have the desired bound similar to $(II)$ above. For $(IV)$, it suffices to show that
\begin{align}\label{eq:Delta_linfty_bound}
\max_{\ell\in[d]:\ell\neq k,\ell \notin \cJ} \E\Big[|\e_\ell^\top (\Delta^t_1-\Delta^t_2)|^q |\theta^0_\cJ, \theta^\ast_\cJ\Big]\leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q}. 
\end{align}
To this end, we write $\Delta_1 = \Lambda^1 + \Lambda^2 + \Lambda^3$, where
\begin{align*}
\Lambda^1 &= s(\btheta^t, \hat{\alpha}^t) - s(\btheta^t_{(\cJ)}, \hat{\alpha}^t) - \diag(\partial_\theta s(\btheta^t_{(\cJ)},\hat{\alpha}^t))(\btheta^t - \btheta^t_{(\cJ)}),\\
\Lambda^2 &= \Big(\diag(\partial_\theta s(\btheta^t_{(\cJ)},\hat{\alpha}^t)) - \diag(\partial_\theta s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k,\cJ)}))\Big)(\btheta^t - \btheta^t_{(\cJ)}),\\
\Lambda^3 &= s(\btheta^t_{(\cJ)}, \hat{\alpha}^t) - s(\btheta^t_{(\cJ)},\hat{\alpha}^t_{(\cJ)}),
\end{align*}
and similarly $\Delta_2 = \Gamma^1 + \Gamma^2 + \Gamma^3$, where
\begin{align*}
\Gamma^1 &= s(\btheta^t_{(k)}, \hat{\alpha}^t_{(k)}) - s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k)}) - \diag(\partial_\theta s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k)}))(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}),\\
\Gamma^2 &= \Big(\diag(\partial_\theta s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k)})) - \diag(\partial_\theta s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k,\cJ)}))\Big)(\btheta^t_{(k)} - \btheta^t_{(k,\cJ)}),\\
\Gamma^3 &= s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k)}) - s(\btheta^t_{(k,\cJ)},\hat{\alpha}^t_{(k,\cJ)}).
\end{align*}
To prove the desird claim, it suffices to show that
\begin{align*}
&\max_{\ell\in[d]:\ell\neq k,\ell \notin \cJ} \E\Big[\Big( |\e_\ell^\top \Lambda^1| +  |\e_\ell^\top \Lambda^2| + |\e_\ell^\top \Gamma^1| + |\e_\ell^\top \Gamma^2|+ |\e_\ell^\top (\Lambda^3 - \Gamma^3)| \Big)^q |\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\quad\leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q}. 
\end{align*}
We only prove the claim for $\Lambda^1$ and $\Lambda^2$, and the claims for $\Gamma^1, \Gamma^2$ follow from similar arguments. To see the claim for $\Lambda^1$, we have by Assumption \ref{assump:prior} that
\begin{align*}
\big|\e_\ell^\top \Lambda^1\big| &= \Big|s((\btheta^t)_\ell,\hat{\alpha}^t) - s((\btheta^t_{(\cJ)})_\ell, \hat{\alpha}^t) - \partial_\theta s((\btheta^t_{(k,\cJ)})_\ell;\hat{\alpha}^t))\e_\ell^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})\Big|\\
&\leq C(|\e_\ell^\top (\btheta^t - \btheta^t_{(k,\cJ)})| + |\e_\ell^\top (\btheta^t_{(\cJ)} - \btheta^t_{(\cJ,k)})|)\cdot |\e_\ell^\top (\btheta^t_{(k)} - \btheta^t_{(k,\cJ)})|, 
\end{align*}
so the claim follows from the induction hypothesis. For $\Lambda^2$, we have by Assumption \ref{assump:prior} that
\begin{align*}
\big|\e_\ell^\top \Lambda^2\big| &= \Big|\partial_\theta s((\btheta^t_{(\cJ)})_\ell,\hat{\alpha}^t)) - \partial_\theta s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(k,\cJ)})\Big| |\e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)})|\\
&\leq C\big(|\e_\ell^\top (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})| + \pnorm{\hat{\alpha}^t - \hat{\alpha}_{(k,\cJ)}^t}{}\big)\cdot |\e_\ell^\top (\btheta^t - \btheta^t_{(\cJ)})|,
\end{align*}
so the conclusion follows from the induction hypothesis and Lemma \ref{lem:loo_error}. To handle $\Lambda^3$ and $\Gamma^3$, we have
\begin{align*}
\e_\ell^\top (\Lambda^3 - \Gamma^3) &= \Big(s((\btheta^t_{(\cJ)})_\ell,\hat{\alpha}^t) - s((\btheta^t_{(\cJ)})_\ell,\hat{\alpha}^t_{(\cJ)})\Big) - \Big(s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(k)}) - s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(k,\cJ)})\Big)\\
&= \underbrace{\Big[s((\btheta^t_{(\cJ)})_\ell,\hat{\alpha}^t) - s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t) - s((\btheta^t_{(\cJ)})_\ell,\hat{\alpha}^t_{(\cJ)}) + s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(\cJ)})\Big]}_{U_1}\\
&\quad + \underbrace{\Big[s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t) - s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(\cJ)}) - s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(k)}) + s((\btheta^t_{(k,\cJ)})_\ell,\hat{\alpha}^t_{(k,\cJ)})\Big]}_{U_2}. 
\end{align*}
Let us bound $U_1$ and $U_2$ separately. For $U_1$, there exist $\tilde{\theta}$ and $\check{\theta}$ that lie in the segment between $(\btheta^t_{(\cJ)})_\ell$ and $(\btheta^t_{(k,\cJ)})_\ell$ such that
\begin{align*}
U_1 = \Big(\partial_\theta s(\tilde{\theta}, \hat{\alpha}^t) -  \partial_\theta s(\check{\theta}, \hat{\alpha}^t_{(\cJ)})\Big) \cdot \e_\ell^\top(\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)}), 
\end{align*}
hence by Assumption \ref{assump:prior} we have
\begin{align*}
|U_1| \leq C(|\e_\ell^\top (\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})| + \pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)}}{}) \cdot |\e_\ell^\top(\btheta^t_{(\cJ)} - \btheta^t_{(k,\cJ)})|, 
\end{align*}
so we have the desired bound for $\E[|U_1|^q|\theta^0_\cJ, \theta^\ast_\cJ]$ by the induction hypothesis and Lemma \ref{lem:loo_error}. For $W_2$, there exist some $\tilde{\alpha}$ (resp. $\check{\alpha}$) that lies on the segment connecting $(\hat{\alpha}^t, \hat{\alpha}^t_{(\cJ)})$ (resp. $(\hat{\alpha}^t_{(k)}, \hat{\alpha}^t_{(k,\cJ)})$) such that
\begin{align*}
U_2 &= \nabla_\alpha s((\btheta^t_{(k,\cJ)})_\ell,\tilde{\alpha})^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)}) - \nabla_\alpha s((\btheta^t_{(k,\cJ)})_\ell;\check{\alpha})^\top (\hat{\alpha}^t_{(k)} - \hat{\alpha}^t_{(k,\cJ)})\\
&= \Big(\nabla_\alpha s((\btheta^t_{(k,\cJ)})_\ell,\tilde{\alpha}) - \nabla_\alpha s((\btheta^t_{(k,\cJ)})_\ell,\check{\alpha})\Big)^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)}) \\
&\quad + \nabla_\alpha s((\btheta^t_{(k,\cJ)})_\ell;\check{\alpha})^\top\Big(\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)} - \hat{\alpha}^t_{(k)} + \hat{\alpha}^t_{(k,\cJ)}\Big)\\
&\leq C\pnorm{\nabla_\alpha^2 s(\theta,\alpha)}{\op} d(\alpha)^2 + \pnorm{\nabla_\alpha s(\theta,\alpha)}{F} \pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(\cJ)} - \hat{\alpha}^t_{(k)} + \hat{\alpha}^t_{(k,\cJ)}}{}.
\end{align*}
Here we recall the definition of $d(\alpha)$ in (\ref{eq:dalpha_dtheta}), so by the subsequent bound on $d(\alpha)$ and the induction hypothesis, we have the desired bound for $\E[|U_2|^q|\theta^0_\cJ, \theta^\ast_\cJ]$. This concludes the bound (\ref{eq:Delta_linfty_bound}), which further implies that 
\begin{align*}
\E\Big[\Big(\sum_{\ell\in[d]:\ell\neq k,\ell\notin\cJ} |\e_\ell^\top (\Delta^t_1-\Delta^t_2)|^2\Big)^{q/2}|\theta^0_\cJ,\theta^\ast_\cJ\Big] \leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q/2}.
\end{align*}
%This concludes that $\e_k^\top (\Lambda^3 - \Gamma^3)$ and hence $\e_k^\top (IV)$ are both $O_P(1/d)$ for any $k\neq i,j$, implying $\sum_{k\in[d]:k\neq i,j} (\e_k^\top (IV))^2 = O_P(1/d)$. 

Combing back to (\ref{eq:ltw_decompose}), we conclude that
\begin{align*}
&\E\Big[\Big(\sum_{\ell\in[d]:\ell\neq k,\ell\notin\cJ} \Big(\e_\ell^\top \big(\btheta^t - \btheta^t_{(\cJ)} - \btheta^t_{(k)} + \btheta^t_{(k,\cJ)}\big)\Big)^2\Big)^{q/2}|\theta^0_\cJ, \theta^\ast_\cJ\Big]\\
&\leq \E\Big[\pnorm{(I)}{}^q + \pnorm{(II)}{}^q + \pnorm{(III)}{}^q + \Big(\sum_{\ell\in[d]:\ell\neq k,\ell\notin\cJ} |\e_\ell^\top (\Delta^t_1-\Delta^t_2)|^2\Big)^{q/2}|\theta^0_\cJ,\theta^\ast_\cJ\Big]\\
&\leq \frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^q/2},
\end{align*}
completing the induction for (\ref{eq:lto_l2}).
\end{proof}


\subsection{Entrywise convergence of discrete Langevin dynamic}




\begin{proposition}\label{prop:entrywise_discrete_approx}
Suppose Assumptions \ref{assump:model}-\ref{assump:gradient} hold. Recall the discrete DMFT system in (\ref{eq:dmft_theta_discrete1})-(\ref{eq:dmft_alpha_discrete1}). For any fixed $m\in \Z$, $\cJ\subset[d]$ with fixed cardinality, and $\xi^0_\cJ = \{\xi^0_j\}_{j\in\cJ}, \xi^\ast_\cJ = \{\xi^\ast_j\}_{j\in\cJ}$, it holds as $n,d\rightarrow\infty$ that
\begin{align*}
W_2\Big(\sP(\{\theta^0_j, \ldots, \theta^m_j\}_{j\in \cJ} | (\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0_\cJ, \xi^\ast_\cJ)), \otimes_{j\in \cJ}\sP(\bar{\theta}^{t_0}_\gamma, \ldots, \bar{\theta}^{t_m}_\gamma) | (\bar{\theta}^0, \theta^\ast) = (\xi^0_j, \xi^\ast_j)\Big)  \rightarrow 0,
\end{align*}
where the laws on both sides are taken over all the randomness.
\end{proposition}
\begin{proof}
%Without loss of generality, we study the last coordinate of $\btheta^t$ denoted by $\mu^t$, and we write $\btheta^t = (\bar{\btheta}^{t}, \mu^t)$ with $\bar{\btheta}^t \in \R^{d-1}$. We also write $\X = [\bar{\X}, \x]$ where $\x\in\R^n$ denotes the last column of $\X$, and $\{b^t\}$ denoting the last component of $\{\b^t\}$. Then it holds that
Let $\X_{(\cJ)} \in \R^{n\times d}$ denote $\X$ with columns in $\cJ$ set to 0. Then for any $j\in \cJ$,  
\begin{align}\label{eq:single_expansion_main}
\notag\theta_j^{t+1} &= \theta^t_j - \gamma\beta \sum_{\ell \in \cJ} (\x_j^\top \x_\ell)\theta^t_\ell - \gamma\beta\x_j^\top (\X_{(-\cJ)}\btheta^t - \y) + \gamma s(\theta^t_j,\hat{\alpha}^t) + \sqrt{2}(b^{(t+1)\gamma}_j - b_j^{t\gamma})\\
\notag&= \theta^t_j - \gamma\beta \sum_{\ell \in \cJ} (\x_j^\top \x_\ell)\theta^t_\ell - \gamma\beta\x_j^\top (\X_{(\cJ)}\btheta^t_{(\cJ)} - \y_{(\cJ)}) - \gamma\beta \x_j^\top \big(\X_{(\cJ)}(\btheta^t - \btheta^t_{(\cJ)}) + \y_{(\cJ)} - \y\big) \\
\notag&\quad + \gamma s(\theta^t_j,\hat\alpha^t) + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma})\\
\notag&= \theta^t_j - \gamma\delta\beta (\theta^t_j - \theta^\ast_j) - \gamma\beta \sum_{\ell\in\cJ:\ell\neq j} (\x_j^\top \x_\ell)(\theta^t_\ell - \theta^\ast_\ell) -  \gamma\beta\x_j^\top (\X_{(\cJ)}\btheta^t_{(\cJ)} - \y_{(\cJ)}) - \gamma\beta \x_j^\top \X_{(\cJ)}(\btheta^t - \btheta^t_{(\cJ)})\\
&\quad + \gamma s(\theta^t_j,\hat\alpha^t) + \sqrt{2}(b_j^{(t+1)\gamma} - b_j^{t\gamma}) - \gamma\beta(\theta^t_j - \theta^\ast_j)\cdot (\pnorm{\x_j}{}^2 - \delta).
\end{align}
Here $\btheta^t_{(\cJ)}$ is the leave-column-out dynamic defined in (\ref{eq:leave_col_out}), and we write $\bar{\btheta}^t_{(\cJ)} \in \R^{d-|\cJ|}$ as its sub-vector with indexed by $[d]\backslash \cJ$. 

Let $\bar{\btheta}^t \in \R^{d-|\cJ|}$ (resp. $\bar{\b}^t$) denote the sub-vector of $\btheta^t$ (resp. $\b^t$) indexed by $[d]\backslash \cJ$, and similarly $\bar{\X}\in \R^{n\times (d-|\cJ|)}$ denote sub-matrix of $\X$ removing the columns in $\cJ$. Let us now expand $\X_{(\cJ)}(\btheta^t - \btheta^t_{(\cJ)}) = \bar{\X}(\bar{\btheta}^t - \bar{\btheta}^t_{(\cJ)})$. We have
\begin{align*}
\bar{\btheta}^{t+1} = \Big(I - \gamma\beta \bar{\X}^\top \bar{\X}\Big)\bar{\btheta}^t - \gamma\beta \bar{\X}^\top (\X_{\cJ} \btheta^t_{\cJ} - \y) + \gamma s(\bar{\btheta}^t, \hat{\alpha}^t) + \sqrt{2}(\bar{\b}^{(t+1)\gamma} - \bar{\b}^{t\gamma}),\\
\bar{\btheta}^{t+1}_{(\cJ)} = \Big(I - \gamma\beta \bar{\X}^\top \bar{\X}\Big)\bar{\btheta}^t_{(\cJ)} - \gamma\beta\bar{\X}^\top (-\y_{(\cJ)}) + \gamma s(\bar{\btheta}^t_{(\cJ)}, \hat{\alpha}^t_{(\cJ)}) + \sqrt{2}(\bar{\b}^{(t+1)\gamma} - \bar{\b}^{t\gamma}),
\end{align*}
which implies that
\begin{align*}
\bar{\btheta}^{t+1}  - \bar{\btheta}^{t+1}_{(\cJ)} &= \Big(I - \gamma\beta\bar{\X}^\top \bar{\X}\Big)(\bar{\btheta}^t  - \bar{\btheta}^t_{(\cJ)}) - \gamma\beta \bar{\X}^\top \X_{\cJ}(\btheta^t_{\cJ} - \btheta^\ast_{\cJ}) + \gamma \diag(\partial_\theta s(\bar{\btheta}^t_{(\cJ)},\hat\alpha^t_{(\cJ)}))(\bar{\btheta}^t - \bar{\btheta}^t_{(\cJ)}) + \gamma \Delta_t\\
&= \underbrace{\Big(I - \gamma\beta\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta s(\bar{\btheta}^t_{(\cJ)},\hat\alpha^t_{(\cJ)}))\Big)}_{\Omega^t \in \R^{(d-|\cJ|) \times (d-|\cJ|)}} (\bar{\btheta}^t  - \bar{\btheta}^t_{(\cJ)}) - \gamma\beta \bar{\X}^\top \X_{\cJ}(\btheta^t_{\cJ} - \theta^\ast_{\cJ}) + \gamma \Delta_t,
\end{align*}
where $\Delta_t = s(\bar{\btheta}^t, \hat\alpha^t) - s(\bar{\btheta}^t_{(\cJ)}, \hat\alpha^t_{(\cJ)}) - \diag(\partial_\theta s(\bar{\btheta}^t_{(\cJ)},\hat\alpha^t_{(\cJ)})) (\bar{\btheta}^t - \bar{\btheta}^t_{(\cJ)})$. Iterating the above identity yields that
\begin{align*}
\bar{\btheta}^{t+1}  - \bar{\btheta}^{t+1}_{(d)} = \Omega^t \ldots \Omega^0 \underbrace{(\bar{\btheta}^0 - \bar{\btheta}^0_{(d)})}_{=0} + \sum_{\ell=0}^t \Omega^t \ldots \Omega^{\ell+1} \Big(-\gamma\beta \bar{\X}^\top \X_{\cJ} (\btheta^\ell_{\cJ} - \btheta^\ast_{\cJ}) + \gamma \Delta_\ell\Big),
\end{align*}
where we understand $\Omega^t \ldots \Omega^{\ell+1} = I_{d-|\cJ|}$ for $\ell = t$. Plugging the above identity into (\ref{eq:single_expansion_main}), we have
\begin{align*}
\theta^{t+1}_j &= \theta^t_j - \gamma\delta\beta (\theta^t_j - \theta^\ast_j) + \gamma s(\theta^t_j, \hat{\alpha}^t) + (\gamma\beta)^2 \sum_{\ell=0}^t \x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x_j \cdot(\theta^\ell_j - \theta^\ast_j) - \gamma\beta\x_j^\top (\bar{\X}\bar{\btheta}^t_{(\cJ)} - \y_{(\cJ)})\\
&\quad + \sqrt{2}(b^{(t+1)\gamma}_j - b_j^{t\gamma}) + (\gamma\beta)^2 \sum_{\ell=0}^t\sum_{k\in \cJ: k\neq j} \x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x_k \cdot(\theta^\ell_k - \theta^\ast_k)   - \gamma\beta(\theta^t_j - \theta^\ast_j)\cdot (\pnorm{\x_j}{}^2 - \delta)\\
&\quad - \gamma^2\beta\sum_{\ell=0}^t \x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell - \gamma\beta \sum_{\ell\in\cJ:\ell\neq j} (\x_j^\top \x_\ell)(\theta^t_\ell - \theta^\ast_\ell).
\end{align*}
Recall from (\ref{eq:dmft_theta_discrete1}) that the $\theta$-dynamic in the discrete DMFT system takes the form (with simplified notation introduced after (\ref{eq:dmft_response_rho})):
\begin{align}\label{eq:dmft_theta_single}
\theta^{t+1} &= \theta^t - \gamma\delta\beta (\theta^t - \theta^\ast) + \gamma s(\theta^t,\alpha^t) + \gamma\sum_{\ell=0}^t \bar{R}_\eta^\gamma(t,\ell)(\theta^\ell - \theta^\ast) + \gamma u^t_\gamma + \sqrt{2}(b^{(t+1)\gamma}_\gamma - b^{t\gamma}_\gamma).
\end{align}
Recall that $\xi^0_{\cJ} = \{\xi^0_j\}_{j\in\cJ}$ and $\xi^\ast_{\cJ} = \{\xi^\ast_j\}_{j\in \cJ}$. We now construct a coupling of the conditional laws $\sP(\{\theta^1_j,\ldots,\theta^{t+1}\}_{j\in \cJ}| \theta^0_{\cJ} = \xi^0_{\cJ}, \theta^\ast_{\cJ} = \xi^\ast_{\cJ})$ and $\otimes_{j\in \cJ}\sP(\theta^1,\ldots,\theta^{t+1}| \theta^0 = \xi^0_j, \theta^\ast = \xi^\ast_j)$, where for the latter law we denote $(u^t_\gamma, b^{t\gamma}_\gamma)$ in (\ref{eq:dmft_theta_single}) as $(u^{t,(j)}_\gamma, b^{t\gamma,(j)}_\gamma)$, and denote its realization as
 \begin{align*}
\theta^{t+1,(j)} &= \theta^{t,(j)} - \gamma\delta\beta (\theta^{t,(j)} - \theta^\ast) + \gamma s(\theta^{t,(j)},\alpha^t) + \gamma\sum_{\ell=0}^t \bar{R}_\eta^\gamma(t,\ell)(\theta^{\ell,(j)} - \theta^\ast) + \gamma u^{t,(j)}_\gamma + \sqrt{2}(b^{(t+1)\gamma,(j)}_\gamma - b^{t\gamma,(j)}_\gamma),
\end{align*}
with initialization $\theta^0$. Note that conditioning on $\theta^0,\theta^\ast$, the only random quantities in the above process are $(u^{t,(j)}_\gamma, b^{t\gamma,(j)}_\gamma)$, so it suffices to specify the realizations of $(u^{t,(j)}_\gamma, b^{t\gamma,(j)}_\gamma), j\in \cJ$ within the probability space that generates $\{\btheta^t\}$.
\begin{itemize}
\item In (\ref{eq:dmft_theta_single}), we take $b^{t\gamma,(j)}_\gamma = b_j^{t\gamma}$.
\item Let $\tilde{u}^t_j = -\beta\x_j^\top (\bar{\X}\bar{\btheta}^t_{(\cJ)} - \y_{(\cJ)})$ for each $j\in \cJ$, which by definition of $(\btheta^t_{(\cJ)}, \y_{(\cJ)})$ is independent of $\theta^0_{\cJ},\theta^\ast_{\cJ}$. %Using independence between $\x$ and $\bar{\X}, \btheta^t_{(d)}, \y_{(d)}$, we have $\E[\tilde{u}^t\tilde{u}^s|\X_{(d)}, \y_{(d)}] = \delta\beta^2 n^{-1}(\bar{\X}\bar{\btheta}^t_{(d)} - \y_{(d)})^\top (\bar{\X}\bar{\btheta}^s_{(d)} - \y_{(d)})$, where
By Lemma \ref{lem:loo_error} and the DMFT characterization Theorem \ref{thm:dmft_approx}, we have for any $0\leq r,s \leq t$ that conditioning on $(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})$,
\begin{align*}
\frac{\beta^2}{d} (\bar{\X}\bar{\btheta}^r_{(\cJ)} - \y_{(\cJ)})^\top (\bar{\X}\bar{\btheta}^s_{(\cJ)} - \y_{(\cJ)}) \rightarrow_{a.s.} C_\eta^\gamma(r,s) = \delta\beta^2\E(\eta^r + w^\ast - \eps)(\eta^s + w^\ast - \eps) = \E[u^ru^s].
\end{align*}
By Lemma \ref{lem:cond_gaussian}, we may then construct a coupling $\{\{u^{s,(j)}_\gamma\}_{j\in \cJ},\{\tilde{u}^s_j\}_{j\in \cJ}\}$, $0\leq s\leq t$ such that $\{u^{s,(j)}_\gamma\}_{j\in \cJ}$ are i.i.d. across $j\in\cJ$ and $\max_{0\leq s\leq t} \E(\tilde{u}^s_j - u_\gamma^{s,(j)})^2 \rightarrow 0$ as $n,d\rightarrow\infty$ (note that for any $0\leq s\leq t$, the required uniform integrability of $\frac{1}{\sqrt{d}}\pnorm{\bar{\X}\bar{\btheta}^s_{(\cJ)} - \y_{(\cJ)}}{}$ follows from the bound (\ref{eq:loo_expectation_2}).
\end{itemize}
Next note that by the analysis subsequent to (\ref{eq:loo_approximation}), it holds that, conditioning on $(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})$, $\E\Big[\big(\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x -\frac{1}{\gamma\beta^2}\bar{R}_\eta^\gamma(t,\ell)\big)^2|(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})\Big] \rightarrow 0$ (in fact the quantity under expectation is independent of $(\theta^0_{\cJ}, \theta^\ast_{\cJ})$), hence with the above coupling, we have $\sum_{j\in\cJ}\E[\pnorm{(\theta^0_j,\ldots,\theta_j^{t+1}) - (\theta^{0,(j)}, \ldots, \theta^{t+1,(j)})}{}^2| (\theta^0_j, \theta^\ast_j) = (\theta^0, \theta^\ast) = (\xi^0_j,\xi^\ast_j), j\in\cJ] \rightarrow 0$ provided that
\begin{align*}
\E\Big[|\theta^t_j - \theta^\ast_j|^2\cdot |\pnorm{\x_j}{}^2 - \delta|^2 \big| (\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})\Big] &\rightarrow 0, \quad j\in \cJ,\\
\E\Big[ \big(\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x_k \cdot(\theta^\ell_k - \theta^\ast_k)\big)^2|(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})\Big]^2 &\rightarrow 0, \quad 0\leq\ell\leq t, \quad j,k\in \cJ, j\neq k,\\
\E\Big[\big((\x_j^\top \x_k)(\theta^t_k - \theta^\ast_k)\big)^2|(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})\Big] &\rightarrow 0, \quad j,k\in \cJ, j\neq k,\\
\quad \E\Big[|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell|^2\big|(\theta^0_{\cJ}, \theta^\ast_{\cJ}) = (\xi^0_{\cJ}, \xi^\ast_{\cJ})\Big] &\rightarrow 0, \quad 0\leq \ell \leq t.
\end{align*}
The first three claim hold by standard concentration and the bound (\ref{eq:loo_expectation_5}).
%moment bound 
%\begin{align}\label{eq:single_entry_moment}
%\max_{j\in\cJ}\max_{t\leq \floor{T/\gamma}} \E[|\theta^t_j|^q | \theta^0_{\cJ}, \theta^\ast_{\cJ}] \leq \big(C+K_{\gamma}\exp(-c\sqrt{d})\big)(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q,
%\end{align}
%obtained by combining (\ref{eq:loo_expectation_3}) and Lemma \ref{lem:theta_loo_constant}. 
For the last claim, we decompose $\Delta_\ell = \Delta_\ell^1 + \Delta_\ell^2 + \Delta_\ell^3$, where
\begin{align*}
\Delta_\ell^1 &= s(\bar{\btheta}^\ell,\hat{\alpha}^\ell) - s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell) - \diag(\partial_\theta s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell))(\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(\cJ)}),\\
\Delta_\ell^2 &= \Big(\diag(\partial_\theta s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell)) - \diag(\partial_\theta s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell_{(\cJ)}))\Big)(\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(\cJ)}),\\
\Delta_\ell^3 &= s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell) - s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell_{(\cJ)}).
\end{align*}
For $\Delta_\ell^1$, we have $\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^1 \leq \pnorm{\x}{}\prod_{s=\ell+1}^t \pnorm{\Omega^s}{\op} \pnorm{\Delta_\ell^1}{}$, where $\pnorm{\Omega^s}{\op} \leq 1+C\gamma(\pnorm{\X}{\op}^2 + 1)$, and
\begin{align*}
\pnorm{\Delta_\ell^1}{}^2 \leq \sum_{j:j\notin \cJ} \pnorm{\partial_\theta^2 s(\theta,\alpha)}{\infty}^2 (\theta^\ell_j - (\btheta^\ell_{(\cJ)})_j)^4 \leq d\pnorm{\partial_\theta^2 s(\theta,\alpha)}{\infty}^2 \pnorm{\bar{\btheta}^\ell - \bar{\btheta}_{(d)}^\ell}{\infty}^4,
\end{align*}
hence $\E\Big[|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^1|\big|^2 (\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0,\xi^\ast)\Big] \rightarrow 0$
by Lemma \ref{|em:loo_linfty_error}. For $\Delta_\ell^2$, we similarly have $\pnorm{\Delta_\ell^2}{} \leq \pnorm{\partial_\theta \nabla_\alpha s(\theta,\alpha)}{\infty}\pnorm{\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)}}{}\pnorm{\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(\cJ)}}{}$, which implies $\E\Big[|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^2|\big|^2 (\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0,\xi^\ast)\Big] \rightarrow 0$ by Lemma \ref{lem:loo_error}. For $\Delta^3_\ell$, we have
\begin{align*}
\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^3 &= \x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\nabla_\alpha s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell_{(\cJ)}) (\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)})\\
&\quad + \x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\nabla_\alpha^2 s(\bar{\btheta}^\ell_{(\cJ)}, \tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)})^{\otimes 2}, 
\end{align*}
where $\tilde{\alpha}^\ell$ lies on the segment connecting $\hat\alpha^\ell$ and $\hat\alpha^\ell_{(\cJ)}$, and we understand $\nabla_\alpha^2 s(\bar{\btheta}^\ell_{(\cJ)},\tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)})^{\otimes 2}$ as the standard tensor product from $\R^{d-|\cJ|}\times \R^K \times \R^K$ and $\R^K \times \R^K$ to $\R^{d-|\cJ|}$. For the first term, using independence between $\x_j$ and $\bar\X, \{\Omega^\ell\}, \bar{\btheta}^\ell_{(\cJ)}, \hat{\alpha}^\ell_{(\cJ)}$, it is easy to argue that for each $k\in [K]$, $\E\Big[\big|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\partial_{\alpha_k} s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell_{(\cJ)})\big|^q\Big] \leq C + K_\gamma\exp(-c\sqrt{d})$, hence by Lemma \ref{lem:loo_error}, we have 
\begin{align*}
\E\Big[|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \nabla_\alpha s(\bar{\btheta}^\ell_{(\cJ)},\hat{\alpha}^\ell_{(\cJ)}) (\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)})|^2|(\theta^0_\cJ,\theta^\ast_\cJ) = (\xi^0_\cJ, \xi^\ast_\cJ)\Big] \leq \big(C + K_\gamma(-c\sqrt{d})\big)(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)/\sqrt{d} \rightarrow 0.
\end{align*}
On the other hand, we have
\begin{align*}
\Big|\x_j^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\nabla_\alpha^2 s(\bar{\btheta}^\ell_{(\cJ)}, \tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)})^{\otimes 2}\Big| \leq \sqrt{d}\cdot\pnorm{\x_j}{}\pnorm{\X}{\op}\prod_{s=\ell+1}^t \pnorm{\Omega^s}{\op}\pnorm{\nabla_\alpha^2 s(\theta,\alpha)}{\op}\pnorm{\hat\alpha^\ell - \hat\alpha^\ell_{(\cJ)}}{}^2.
\end{align*}
Hence by Lemma \ref{lem:loo_error}, its second moment converges to zero. The proof is complete.
\end{proof}

\begin{lemma}\label{lem:cond_gaussian}
For any fixed positive integers $k,m$, suppose $\x_1,\ldots,\x_k \overset{i.i.d.}{\sim} \N(0, I_d/d)$ and $\r^1, \ldots, \r^m$ are $m$ random vectors independent of $\x_1,\ldots,\x_k$ such that, for some p.s.d. matrix $\Sigma \in \R^{m\times m}$,  $\frac{1}{d} (\r^i)^\top \r^j \rightarrow_{a.s.} \Sigma_{ij}$ for any $i,j\in[m]$. Suppose that for each $i,j\in [m]$, $(\r^i)^\top \r^j/d$ is uniformly integrable (as a sequence of random variables indexed by $d$). Then 
\begin{align*}
W_2^2\big(\sP((\x_j^\top \r^1, \ldots, \x_j^\top \r^m)_{j=1}^k), \N^{\otimes k}(0,\Sigma)\big) \rightarrow 0
\end{align*}
as $d\rightarrow\infty$.
\end{lemma}
\begin{proof}
%Consider probability-1 event on which $\frac{1}{d} (\r^i)^\top \r^j \rightarrow_{a.s.} \Sigma_{ij}$ for any $i,j\in[m]$. 
Define the matrix $\bR := [\r^1; \ldots; \r^m] \in \R^{m\times d}$, and $\tilde{\bR} := \sqrt{d} \cdot \Sigma^{1/2}((\bR \bR^\top)^{1/2})^\dagger \bR \in \R^{m\times d}$, where $((\bR \bR^\top)^{1/2})^\dagger$ denotes the pseudo-inverse of $(\bR \bR^\top)^{1/2}$. Let $\X = [\x_1,\ldots,\x_k] \in \R^{d\times k}$ be independent of $\bR$ and $\tilde{\bR}$, then the law $\sP((\x_j^\top \r^1, \ldots, \x_j^\top \r^m)_{j=1}^k)$ (resp. $\N^{\otimes k}(0,\Sigma)$) can be realized as $\bR \X$ (resp. $\tilde{\bR}\X$), and
\begin{align*}
W_2^2\big(\sP(\sP((\x_j^\top \r^1, \ldots, \x_j^\top \r^m)_{j=1}^k), \N^{\otimes k}(0,\Sigma)\big) \leq \E \pnorm{(\bR - \tilde{\bR})\X}{}^2 = \frac{k}{d}\E \pnorm{\bR - \tilde{\bR}}{F}^2 = k\cdot\E\pnorm{(\frac{1}{d}\bR\bR^\top)^{1/2} - \Sigma^{1/2}}{F}^2.
\end{align*}
Since $d^{-1}\bR\bR^\top \rightarrow_{a.s.} \Sigma$, we also have $(d^{-1}\bR\bR^\top)^{1/2} \rightarrow_{a.s.} \Sigma^{1/2}$, and the desired in-expectation bound follows from the uniform integrability of $\pnorm{(\frac{1}{d}\bR\bR^\top)^{1/2}}{F}^2$.
\end{proof}

\subsection{Entrywise discretization error of Langevin dynamic}

Consider the dynamic $\{\btheta^t_\gamma, \hat{\alpha}^t_\gamma\}_{t\in \R_+}$ defined in (\ref{eq:discrete_langevin}). For any $j\in[d]$, we denote the $j$th component of $\btheta^t$ (resp. $\btheta^t_\gamma$) as $\theta^t_j$ (resp. $\theta^t_{\gamma,j}$).

\begin{proposition}\label{prop:entrywise_langevin_discretize}
Assume the conditions of Theorem \ref{thm:dmft_entrywise}. Fix $m\in\Z_+$, $\tau_1,\ldots,\tau_m \in \R_+$, and $\cJ\subset[d]$ with $|\cJ| = O(1)$. Then for any fixed $\xi^0_\cJ = \{\xi^0_j\}_{j\in \cJ}$ and $\xi^\ast_\cJ = \{\xi^\ast_j\}_{j\in \cJ}$, as $\gamma\rightarrow 0$, 
\begin{align*}
\limsup_{n,d\rightarrow\infty} W_1\Big(\sP(\{\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j\}_{j\in \cJ} | (\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0_\cJ, \xi^\ast_\cJ)), \sP(\{\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}\}_{j\in \cJ} | (\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0_\cJ, \xi^\ast_\cJ))\Big) \rightarrow 0.
\end{align*}
\end{proposition}

\subsubsection{An intermediate result}

\begin{lemma}\label{lem:l4_bound}
Control $\sum_{j=1}^d |\theta^t_j - \theta^t_{\gamma,j}|^4$. 
\end{lemma}
\begin{proof}
Throughout the proof, we use $\E^\circ$ as a shorthand for $\E[\cdot|\theta^0_\cJ,\theta^\ast_\cJ]$.
By definition, we have
\begin{align*}
\theta^t_j - \bar{\theta}^t_{\gamma,j} &= \underbrace{\int_{\floor{t}}^t \Big[-\beta \x_j^\top(\X\btheta^s - \y) + s(\theta^s_{j}, \hat\alpha^s)\Big] \d s}_{(I_j)}\\
&\quad + \underbrace{\int_0^{\floor{t}} \Big[-\beta \x_j^\top \X(\btheta^s - \bar\btheta^s_{\gamma}) + \big(s(\theta^s_{j}, \hat\alpha^s_j) - s(\bar{\theta}^s_{\gamma,j}, \bar{\widehat\alpha}^s_{\gamma,j})\big)\Big]\d s}_{(II_j)} + b^t_j - b^{\floor{t}}_j. 
\end{align*}
It is easy to verify that $\sup_{t\in[0,T]}\E^\circ[d^{-1}\sum_{j=1}^d |b^t_j - b^{\floor{t}}_j|^4] \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. To bound $(I)$, we have by Assumption \ref{assump:prior} that
\begin{align*} 
\Big|-\beta \x_j^\top(\X\btheta^s - \y) + s(\theta^s_{j}, \hat\alpha^s)\Big| &\leq C\Big(\pnorm{\x_j}{}^2 |\theta^s_j| + |\x_j^\top \X_{(j)}\btheta^s_{(j)}| + |\x_j^\top \X_{(j)}(\btheta^s - \btheta^s_{(j)})| + |\x_j^\top \y| + |s(0,0)| + |\theta^s_j| + \pnorm{\hat\alpha^s}{}\Big)\\
&\leq C\Big((\pnorm{\x_j}{}^2 + 1) |\theta^s_j| + |\x_j^\top \X_{(j)}\btheta^s_{(j)}| + \pnorm{\X}{\op}^2\pnorm{\btheta^s - \btheta^s_{(j)}}{} + |\x_j^\top \y|  + \pnorm{\hat\alpha^s}{} + 1\Big),
\end{align*}
where $\btheta^t_{(j)}$ is defined in (\ref{def:leave_col_out_cont}). By independence between $\x_j$ and $\X_{(j)}\btheta^s_{(j)}$, and Lemma \ref{lem:loo_error_continuous}, it is easy to verify that $\E^\circ[|-\beta \x_j^\top(\X\btheta^s - \y) + s(\theta^s_{j}, \hat\alpha^s)|^q] \leq C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$, which further implies that
\begin{align*}
\E^\circ\Big[\frac{1}{d}\sum_{j=1}^d (I_j)^4\Big] \leq Ch(\gamma)(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4,
\end{align*}
for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. To bound $(II_j)$, we have for $t\in[0,T]$ that
\begin{align*}
|(II_j)| &\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2) |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| + C\pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + C|\x_j^\top \X_{(j)} (\btheta^s - \bar{\btheta}^{s}_\gamma)|\Big] \d s\\
&\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 \leq 10\delta}) |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| \d s + \int_0^t  C|\x_j^\top \X_{(j)} (\btheta^s - \bar{\btheta}^{s}_\gamma - \btheta^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)})|\d s\\
&\quad + \int_0^T \Big[C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| + C\pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + C|\x_j^\top \X_{(j)} (\btheta^s_{(j)} - \bar{\btheta}^{s}_{\gamma,(j)})|\Big] \d s \\
&\leq C\int_0^t \Big( |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| + \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_\gamma - \btheta^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)})}{}\Big) \d s\\
&\quad + \underbrace{\int_0^T C\Big[\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| + \pnorm{\X}{\op}^2\bm{1}_{\pnorm{\X}{\op} \geq 4(1+\delta)}\pnorm{\btheta^s - \bar{\btheta}^{s}_\gamma - \btheta^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)}}{}}\\
&\quad \underbrace{+ \pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + C|\x_j^\top \X_{(j)} (\btheta^s_{(j)} - \bar{\btheta}^{s}_{\gamma,(j)})|\Big]\d s}_{A_j(T)}.
%&\quad\quad \underbrace{+ C\pnorm{\X}{\op}^2\pnorm{\bar\btheta^s_\gamma - \bar\btheta^{\floor{s}}_\gamma - \bar\btheta^s_{\gamma,(j)} + \bar\btheta^s_{\gamma,(j)}}{}\Big] \d s + \sqrt{2}\sup_{t\in[0,T]} |b^t_j - b^t_{\gamma,j}|}_{A_j(T)}.
\end{align*}
By standard concentration, Lemma \ref{lem:l2_discretization_expectation}, and the independence between $\x_j$ and $\X_{(j)}(\btheta^s_{(j)} - \bar{\btheta}^{s}_{\gamma,(j)})$, it is easy to show that $\E^\circ[A_j^4(T)] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4$ for each $j\in[d]$. 

\end{proof}

%\begin{lemma}\label{lem:entrywise_bound}
%For any fixed $T$, there exists some $C > 0$ depending on $T$ (and other problem parameters) such that $\max_{j\in[d]}\max_{0\leq t\leq T} \E |\theta^t_j|^2 \leq C$.
%\end{lemma}
%\begin{proof}
%%Fix $T \in \Z_+$. Consider the event $\mathcal{E} = \{\max_{j\in[d]}\pnorm{\x_j}{}\leq C_0, \pnorm{\X}{\op} \leq C_0, \max_{j\in[d]} |\x_j^\top \y| \leq C_0, \max_{0\leq t \leq T }\max_{j\in[d]} \langle\pnorm{\btheta^t - \btheta^t_{(j)}}{}\rangle \leq C_0\}$. By Lemma \ref{lem:loo_error}, for large enough $C = C(T)$, the event $\cal{E}$ holds almost surely as $n,d\rightarrow\infty$. Note that for any $j\in[d]$, 
%By definition, we have
%\begin{align*}
%\theta^{t+1}_j = \theta^t_j - \frac{\gamma}{\sigma^2} \x_j^\top \X\btheta^t + \frac{\gamma}{\sigma^2} \x_j^\top y + \gamma\partial_\theta \log g(\theta^t_j;\hat{\alpha}^t) + \sqrt{2}(b^{(t+1)\gamma}_j - b^{t\gamma}_j),
%\end{align*}
%so by Assumption \ref{assump:prior} and the almost sure bound $\max_{0\leq t \leq T}\pnorm{\hat\alpha^t}{} \leq C(T)$, we have
%\begin{align*}
%|\theta^{t+1}_j| \leq C\Big[(1+\pnorm{\x_j}{}^2 + \pnorm{\partial_\theta^2 \log g}{\infty})|\theta^t_j| + |\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t| + \pnorm{\x_j}{}^2|\theta^\ast_j| + |\x_j^\top (\bar{\X}_{(j)}\bar{\btheta}^\ast + \beps)| + 1\Big],
%\end{align*}
%where $\bar{\X}_{(j)}\in\R^{n\times (d-1)}$ denotes $\X$ minus its $j$th column, and $\bar{\btheta}^t, \bar{\btheta}^\ast\in\R^{d-1}$ denote $\btheta^t,\btheta^\ast$ minus their $j$th entry. It is clear that $\max_{j\in[d]}\E (\pnorm{\x_j}{}^2|\theta^\ast_j|)^2 \vee \max_{j\in[d]}\E|\x_j^\top (\bar{\X}_{(j)}\bar{\btheta}^\ast + \beps)|^2 \leq C$, while with $\bar{\btheta}^t_{(j)} \in \R^{d-1}$ denoting $\bar{\btheta}^t$ minus its $j$th entry, we have
%\begin{align*}
%\E|\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t|^2 \leq 2\Big(\E|\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t_{(j)}|^2 + \E|\x_j^\top \bar{\X}_{(j)} (\bar{\btheta}^t - \bar{\btheta}^t_{(j)})|^2\Big) \leq C,
%\end{align*}
%where we apply Lemma \ref{lem:loo_error}. The desired conclusion now follows from a simple induction.
%\end{proof}


\begin{lemma}
Fix $T > 0$ and $\gamma > 0$. Then for any $t\in[0,T]$, $\cJ\subset[d]$ with $|\cJ| = O(1)$, and $j\in[d]$, there exist constants $C,K_\gamma,c$ as specified in Lemma \ref{lem:loo_error} such that 
\begin{align*}
&\pnorm{\big(\btheta^t - \bar{\btheta}^t_\gamma - \btheta_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}\big)_{-j}}{}\\
&\leq C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}\d s + C\int_0^t |\theta^s_j - \bar{\theta}^s_{\gamma,j}|\d s + R(t),
\end{align*}
where $R(t)$ is such that $\sup_{t\in[0,T]} \E[R(t)^2|\theta^0_\cJ,\theta^\ast_\cJ] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4$.
\end{lemma}
\begin{proof}
Throughout the proof, we will use $\E^\circ$ as a shorthand for $\E[\cdot|\theta^0_\cJ, \theta^\ast_\cJ]$. We start with the definitions
\begin{align*}
\btheta^t - \bar{\btheta}^t_\gamma &= \int_{\floor{t}}^t [-\beta \X^\top (\X\btheta^s - \y) + s(\btheta^s, \hat\alpha^s)] \d s\\
&\quad + \int_0^{\floor{t}} -\beta \X^\top \X (\btheta^s - \btheta^{s}_\gamma) + \big[s(\btheta^s, \hat\alpha^s) - s(\btheta^{s}_\gamma, \hat\alpha^{s}_\gamma)\big]\d s + \sqrt{2}(\b^t - \b^{\floor{t}}),\\
\btheta_{(j)}^t - \bar{\btheta}^t_{\gamma,(j)} &= \int_{\floor{t}}^t [-\beta \X_{(j)}^\top (\X_{(j)}\btheta_{(j)}^s - \y_{(j)}) + s(\btheta^s_{(j)}, \hat\alpha^s_{(j)})] \d s\\
&\quad + \int_0^{\floor{t}} -\beta \X_{(j)}^\top \X_{(j)} (\btheta^s_{(j)} - \bar{\btheta}^{s}_{\gamma,(j)}) + \big[s(\btheta^s_{(j)}, \hat\alpha^s_{(j)}) -  s(\bar{\btheta}^s_{\gamma,(j)}, \bar{\widehat\alpha}^s_{\gamma,(j)})\big]\d s + \sqrt{2}(\b^t - \b^{\floor{t}}).
\end{align*}
For any $j\in[d]$, let $E_{(j)} \in \R^{(d-1)\times d}$ denote the identity matrix $I_d$ without its $j$th row. Then
\begin{align}\label{eq:second_order_decomp}
\notag&\Big(\btheta^t - \btheta^t_\gamma - \btheta_{(j)}^t + \btheta^t_{\gamma,(j)}\Big)_{-j}\\
\notag&= E_{(j)}\big(\btheta^t - \btheta^t_\gamma - \btheta_{(j)}^t + \btheta^t_{\gamma,(j)}\big)\\
\notag&= \underbrace{\int_{\floor{t}}^t E_{(j)}\Big[-\beta (\X^\top \X \btheta^s - \X_{(j)}^\top \X_{(j)}\btheta_{(j)}^s) + \beta (\X^\top \y - \X_{(j)}^\top \y_{(j)}) + s(\btheta^s, \hat\alpha^s) - s(\hat\btheta^s_{(j)}, \hat\alpha^s_{(j)})\Big]\d s}_{(I)}\\
\notag&+ \underbrace{\int_0^{\floor{t}} \Big[ -\beta E_{(j)}\Big((\X^\top \X - \X_{(j)}^\top \X_{(j)}) (\btheta^s - \bar{\btheta}^{s}_\gamma) + \X_{(j)}^\top \X_{(j)} (\btheta^s - \bar{\btheta}^s_{\gamma} - \btheta^s_{(j)} + \bar{\btheta}^s_{\gamma,(j)})\Big)} \\
&\quad \underbrace{+ E_{(j)}\Big(s(\btheta^s, \hat\alpha^s) - s(\bar{\btheta}^{s}_\gamma, \bar{\widehat\alpha}^{s}_\gamma) - s(\btheta^s_{(j)}, \hat\alpha^s_{(j)}) +  s(\bar{\btheta}^{s}_{\gamma,(j)}, \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big)\Big] \d s}_{(II)}.
\end{align}
We claim that 
\begin{align}\label{eq:bound_I}
\sup_{t\in[0,T]}\E^\circ[\pnorm{(I)}{}^2] \leq h(\gamma)(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2.
\end{align}
To see this, note that the first integrand satisfies
\begin{align*}
(i) := \pnorm{E_{(j)} (\X^\top \X\btheta^s - \X_{(j)}^\top \X_{(j)}\btheta^s_{(j)})}{} &\leq \pnorm{E_{(j)}(\X^\top \X - \X_{(j)}^\top \X_{(j)})\btheta^s}{} + \pnorm{E_{(j)}\X_{(j)}^\top \X_{(j)}(\btheta^s - \btheta^s_{(j)})}{}\\
&\leq \pnorm{E_{(j)} \X^\top \x_j \theta^s_j}{} + \pnorm{\X}{\op}^2\pnorm{\btheta^s - \btheta^s_{(j)}}{}, 
\end{align*}
so it follows from Lemma \ref{lem:loo_error} that $\sup_{s\in[0,T]}\E^\circ [(i)^2] \leq (C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2$. Similarly, $(ii) := \pnorm{E_{(j)}(\X^\top \y - \X_{(j)}^\top \y_{(j)})}{} = \pnorm{E_{(j)}\X^\top \x_j \theta^\ast_j}{}$, so we have $\sup_{s\in[0,T]}\E^\circ [(ii)^2] \leq C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2$. Lastly, $(iii) := \pnorm{E_{(j)}\big(s(\btheta^s, \hat\alpha^s) - s(\hat\btheta^s_{(j)}, \hat\alpha^s_{(j)})\big)}{} \leq C\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{} + \sqrt{d}\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{}$, so Lemma \ref{lem:loo_error} yields that $\E^\circ[(iii)^2] \leq (C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2$. By H\"older's inequality, this yields the claim (\ref{eq:bound_I}).

Next we bound $(II)$. Note that
\begin{itemize}
\item Since $E_{(j)}(\X^\top \X - \X_{(j)}^\top \X_{(j)}) = E_{(j)}(\X_{(j)}^\top \x_j\e_j^\top + \e_j \x_j^\top \X_{(j)} + \e_j\e_j^\top \pnorm{\x_j}{}^2) = E_{(j)}\X_{(j)}^\top \x_j\e_j^\top$, we have
\begin{align*}
&\biggpnorm{E_{(j)}(\X^\top \X - \X_{(j)}^\top \X_{(j)}) (\btheta^s - \bar{\btheta}^{s}_\gamma)}{} = \pnorm{E_{(j)}\X_{(j)}^\top \x_j (\theta^s_j - \bar{\theta}^{s}_{\gamma,j})}{}\\
&\leq \pnorm{\X}{\op}^2|\theta^s_j - \bar{\theta}^{s}_{\gamma,j}| \leq C|\theta^s_j - \bar{\theta}^s_{\gamma,j}| + \underbrace{\pnorm{\X}{\op}^2\bm{1}_{\pnorm{\X}{\op} \geq 4(1+\delta)}|\theta^s_j - \bar{\theta}^{s}_{\gamma,j}|}_{R(s)},
\end{align*}
where, by standard concentration and bound (\ref{eq:loo_expectation_5}), we have $\sup_{t\in[0,T]} \E^\circ [R^2(t)] \leq K_\gamma\exp(-c\sqrt{d})(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2$.
\item The second term satisfies 
\begin{align*}
&\pnorm{E_{(j)}\X_{(j)}^\top \X_{(j)} (\btheta^s - \btheta^s_{\gamma} - \btheta^s_{(j)} + \btheta^s_{\gamma,(j)})}{} =\pnorm{E_{(j)}\X_{(j)}^\top \X_{(j)} E_{(j)}^\top E_{(j)}(\bar{\btheta}^s - \bar{\btheta}^s_{\gamma} - \bar{\btheta}^s_{(j)} + \bar{\btheta}^s_{\gamma,(j)})}{}\\
&\leq \pnorm{\X}{\op}^2\pnorm{E_{(j)}^\top(\btheta^s - \bar{\btheta}^s_\gamma - \btheta_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)})}{}\\
&\leq C\pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^s_\gamma - \btheta_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)})}{} + \underbrace{\pnorm{\X}{\op}^2\bm{1}_{\pnorm{\X}{\op} \geq 4(1+\delta)}\pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^s_\gamma - \btheta_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)})}{}}_{R(s)},
\end{align*}
where $\sup_{t\in[0,T]}\E^\circ [R^2(t)] \leq K_\gamma\exp(-c\sqrt{d})(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2$.
%\item By Lemma \ref{lem:theta_decomp}, we have $\E^\circ\pnorm{\X_{(j)}^\top \X_{(j)} (\btheta^s_{\gamma} - \btheta^{\floor{s}}_{\gamma} - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)})}{}^2 \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$. 
\item For the last term, we have
\begin{align*}
E_{(j)}\Big(s(\btheta^s, \hat\alpha^s) - s(\btheta^s_{(j)}, \hat\alpha^s_{(j)})\Big) &= E_{(j)}\Big[\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha}))(\btheta^s - \btheta^s_{(j)}) + \nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) (\hat\alpha^s - \hat\alpha^s_{(j)})\Big],\\
E_{(j)}\Big(s(\bar{\btheta}^{s}_\gamma, \bar{\widehat\alpha}^{s}_\gamma) - s(\bar{\btheta}^{s}_{\gamma,(j)}, \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big) &= E_{(j)}\Big[\diag(\partial_\theta s(\check{\btheta}, \check{\alpha}))(\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}) + \nabla_\alpha s(\check{\btheta}, \check{\alpha}) ( \bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big],
\end{align*}
where $(\tilde\btheta, \tilde\alpha)$ lies on the segment connecting $(\btheta^s, \hat\alpha^s)$ and $(\btheta^s_{(j)}, \hat\alpha^s_{(j)})$, and $(\check\btheta, \check\alpha)$ lies on the segment connecting $(\bar{\btheta}^{s}_\gamma, \bar{\widehat\alpha}^{s}_\gamma)$ and $(\bar{\btheta}^{s}_{\gamma,(j)}, \bar{\widehat\alpha}^{s}_{\gamma,(j)})$. Consequently we have
\begin{align*}
&E_{(j)} \Big(s(\btheta^s, \hat\alpha^s) - s(\btheta^s_{(j)}, \hat\alpha^s_{(j)}) - s(\bar{\btheta}^{s}_\gamma, \bar{\widehat\alpha}^{s}_\gamma) - s(\bar{\btheta}^{s}_{\gamma,(j)}, \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big)\\
&= E_{(j)}\Big(\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha}))(\btheta^s - \btheta^s_{(j)}) - \diag(\partial_\theta s(\check{\btheta}, \check{\alpha}))(\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)})\Big)\\
&\quad + E_{(j)}\Big(\nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) ( \hat\alpha^s - \hat\alpha^s_{(j)}) - \nabla_\alpha s(\check{\btheta}, \check{\alpha}) (\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big)\\
&= \underbrace{E_{(j)}\Big(\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha})) - \diag(\partial_\theta s(\check{\btheta}, \check{\alpha}))\Big)(\btheta^s - \btheta^s_{(j)})}_{(i)} + \underbrace{E_{(j)}\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha}))\big(\btheta^s - \btheta^s_{(j)} - \bar\btheta^s_\gamma + \bar\btheta^s_{\gamma,(j)}\big)}_{(ii)}\\
&\quad + \underbrace{E_{(j)}\big(\nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) - \nabla_\alpha s(\check{\btheta}, \check{\alpha})\big)( \hat\alpha^s - \hat\alpha^s_{(j)})}_{(iii)} + \underbrace{E_{(j)}\nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) (\hat\alpha^s - \hat\alpha^s_{(j)} - \bar{\widehat\alpha}^s_\gamma + \bar{\widehat\alpha}^s_{\gamma,(j)})}_{(iv)}
%&\quad + \underbrace{\diag(\partial_\theta s(\check{\btheta}, \check{\alpha}))\Big(\bar\btheta^s_\gamma - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{\gamma,(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}\Big)}_{\Delta_1(s)} +  \underbrace{\nabla_\alpha s(\check{\btheta}, \check{\alpha})\Big(\hat\alpha^s_\gamma - \hat\alpha^{\floor{s}}_\gamma - \hat\alpha^s_{\gamma,(j)} + \hat\alpha^{\floor{s}}_{\gamma,(j)}\Big)}_{\Delta_2(s)}. 
\end{align*}
%This further implies that
%\begin{align*}
%&\pnorm{s(\bar{\btheta}^s, \hat\alpha^s) - s(\bar{\btheta}^s_{(j)}, \hat\alpha^s_{(j)}) - s(\bar{\btheta}^{\floor{s}}_\gamma, \hat\alpha^{\floor{s}}_\gamma) - s(\bar{\btheta}^{\floor{s}}_{\gamma,(j)}, \hat\alpha^{\floor{s}}_{\gamma,(j)})}{}\\
%&\leq \underbrace{\pnorm{\Big(\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha})) - \diag(\partial_\theta s(\check{\btheta}, \check{\alpha}))\Big)(\bar{\btheta}^s_\gamma - \bar{\btheta}^s_{\gamma,(j)})}{}}_{(i)} + \underbrace{\pnorm{\diag(\partial_\theta s(\tilde{\btheta}, \tilde{\alpha}))\big(\bar{\btheta}^s - \bar{\btheta}^s_{(j)} - \bar\btheta^s_\gamma + \bar\btheta^s_{\gamma,(j)}\big)}{}}_{(ii)}\\
%&\quad + \underbrace{\pnorm{\big(\nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) - \nabla_\alpha s(\check{\btheta}, \check{\alpha})\big)( \hat\alpha^s_\gamma - \hat\alpha^s_{\gamma,(j)})}{}}_{(iii)} + \underbrace{\pnorm{\nabla_\alpha s(\tilde{\btheta}, \tilde{\alpha}) (\hat\alpha^s - \hat\alpha^s_{(j)} - \hat\alpha^s_\gamma + \hat\alpha^s_{\gamma,(j)})}{}}_{(iv)} + \underbrace{\pnorm{\Delta_1(s)}{}}_{(v)} + \underbrace{\pnorm{\Delta_2(s)}{}}_{(vi)}. 
%\end{align*}
To bound $(i)$, note that for each $i\in [d]$ such that $i\neq j$, we have
\begin{align*}
|\tilde{\theta}_i - \check{\theta}_i| \leq |(\btheta^s)_i - (\btheta^s_{(j)})_i| + |(\btheta^s)_i - (\bar{\btheta}^{s}_{\gamma})_i| + |(\bar{\btheta}^{s}_{\gamma})_i - (\bar{\btheta}^{s}_{\gamma,(j)})_i|,
\end{align*}
and also
\begin{align*}
\pnorm{\tilde\alpha - \check\alpha}{} \leq \pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{} + \pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + \pnorm{ \bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma, (j)}}{}.
\end{align*}
For any $u\in\R^n$, let $\pnorm{u}{4} = (\sum_{i=1}^n |u_i|^4)^{1/4}$ denote its $\ell_4$ norm. Then the above display implies that
\begin{align*}
\pnorm{(i)}{} &\leq C\Big(\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4} + \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4} + \pnorm{E_{(j)}(\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)})}{4}\Big)\cdot \pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}\\
&\quad + C\Big(\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{} + \pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + \pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma, (j)}}{}\Big)\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{}.
\end{align*}
By Lemma \ref{lem:loo_error_continuous},
%analogous arguments to the proof of (\ref{eq:loo_linfty}) and (\ref{eq:loo_expectation_3}), we have
%\begin{align}\label{eq:loo_bound_continuous}
%\max_{k\in[d]:k\neq j}\sup_{s\in[0,T]} \E^\circ[|\e_k^\top (\btheta^s - \btheta^s_{(j)})|^q] \vee \E^\circ\Big[\Big(\frac{1}{\sqrt{d}}\pnorm{\btheta^s - \btheta^s_{(j)}}{}\Big)^q\Big] \vee \E^\circ[\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{}^q] \leq \frac{C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^{q/2}},
%\end{align}
%and
%\begin{align}\label{eq:single_bound_continuous}
%\E^\circ[|\theta^t_j|^q] \vee \max_{k\in[d]}\E^\circ[|(\btheta^t_{(j)})_k^q] \leq C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q,
%\end{align}
we have $\E^\circ[\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}^4] \rightarrow_{n,d\rightarrow \infty} 0$ for any fixed realizations of $(\theta^0_\cJ,\theta^\ast_\cJ)$. Similar arguments yield that, for any fixed realization of $(\theta^0_\cJ, \theta^\ast_\cJ)$, the following three quantities also vanish to $0$ as $n,d\rightarrow\infty$, 
\begin{align*}
\E^\circ [\pnorm{E_{(j)}(\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)})}{4}^2\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}^2], \E^\circ[\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{}^2\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{}^2],  \E^\circ[\pnorm{ \bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma, (j)}}{}^2\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{}^2 ], 
\end{align*}
and by Lemma \ref{lem:l2_discretization_expectation}, 
\begin{align*}
\limsup_{n,d\rightarrow\infty} \E^\circ[\pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{}^2 \pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{}^2] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4.
\end{align*}
In summary, we have $\pnorm{(i)}{} \leq C\pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s_\gamma - \btheta^s_{(j)})}{4}  + R(s)$ for some $R(s)$ such that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E^\circ [R^2(t)] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4$. Next by Assumption \ref{assump:prior}, we have 
\begin{align*}
\pnorm{(ii)}{} &\leq C\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)} - \bar\btheta^s_\gamma + \bar\btheta^s_{\gamma,(j)})}{},\\
\pnorm{(iii)}{} &\leq C(\pnorm{\tilde{\btheta} - \check{\btheta}}{} + \sqrt{d}\pnorm{\tilde\alpha - \check\alpha}{})\pnorm{\hat\alpha^s_\gamma - \hat\alpha^s_{\gamma,(j)}}{}\\
&\leq C\big(\pnorm{\btheta^s - \btheta^s_{(j)}}{} + \pnorm{\btheta^s - \bar{\btheta}^{s}_{\gamma}}{} + \pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}}{}\big)\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{}\\
&\quad + C\sqrt{d}\big(\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{} + \pnorm{\hat\alpha^s - \bar{\widehat\alpha}^{s}_\gamma}{} + \pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma, (j)}}{}\big)\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{},\\
\pnorm{(iv)}{} &\leq C\sqrt{d}\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)} - \bar{\widehat\alpha}^s_\gamma + \bar{\widehat\alpha}^s_{\gamma,(j)}}{},
%(v) &\leq C\pnorm{\bar\btheta^s_\gamma - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{\gamma,(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{},\\
%(vi) &\leq C\sqrt{d}\pnorm{\hat\alpha^s_\gamma - \hat\alpha^{\floor{s}}_\gamma - \hat\alpha^s_{\gamma,(j)} + \hat\alpha^{\floor{s}}_{\gamma,(j)}}{}.
\end{align*}
By similar arguments as above, we have $\limsup_{n,d\rightarrow\infty}\sup_{s \in [0,T]}\E^\circ[\pnorm{(iii)}{}^2] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4. $
Let us further bound the right side of $\pnorm{(iv)}{}$, namely, $\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)} - \bar{\widehat\alpha}^s_\gamma + \bar{\widehat\alpha}^s_{\gamma,(j)}}{}$. By definition, we have
\begin{align*}
\hat\alpha^t - \hat\alpha^t_{(j)} = \int_0^t \Big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)}))\Big)\d s, \quad \bar{\widehat\alpha}^t_{\gamma} - \bar{\widehat\alpha}^t_{\gamma,(j)} = \int_0^{\floor{t}} \Big(\cG(\bar{\widehat\alpha}^{s}_{\gamma}, \sP(\bar{\btheta}^{s}_{\gamma})) - \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))\Big)\d s,
\end{align*}
hence
\begin{align*}
\hat\alpha^t - \hat\alpha^t_{(j)} - \bar{\widehat\alpha}^t_{\gamma} + \bar{\widehat\alpha}^t_{\gamma,(j)} &= \int_{\floor{t}}^t  \Big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)}))\Big)\d s\\
&\quad + \int_0^{\floor{t}} \Big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)})) - \cG(\bar{\widehat\alpha}^{s}_{\gamma}, \sP(\bar{\btheta}^{s}_{\gamma})) + \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))\Big) \d s.
\end{align*}
To bound the first term, we have by Assumption \ref{assump:gradient} that $\pnorm{\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)}))}{} \leq C(\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)}}{} + \pnorm{\btheta^s - \btheta^s_{(j)}}{}/\sqrt{d})$, hence by the bound (\ref{eq:loo_bound_continuous}), we have
\begin{align*}
\E^\circ \Big[\Big(\int_{\floor{t}}^t  \Big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)}))\Big)\d s\Big)^2\Big] \leq \frac{Ch(\gamma)(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^2}{d}. 
\end{align*}
Next we bound the second term. Define
\begin{align*}
\Gamma_1(s) &:= \cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)})) - \nabla_\alpha \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\hat\alpha^s - \hat\alpha^s_{(j)}) - \nabla_{\btheta} \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\btheta^s - \btheta^s_{(j)}),\\
\Gamma_2(s) &:= \cG(\bar{\widehat\alpha}^{s}_\gamma, \sP(\bar{\btheta}^{s}_\gamma)) - \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)})) - \nabla_\alpha \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)})\\
&\quad - \nabla_{\btheta} \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}),
\end{align*}
then using Assumption \ref{assump:gradient}, we have
\begin{align*}
&\int_0^{\floor{t}} \Big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)})) - \cG(\bar{\widehat\alpha}^{s}_{\gamma}, \sP(\bar{\btheta}^{s}_{\gamma})) + \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))\Big) \d s\\
%&\leq \int_0^t \biggpnorm{\big(\cG(\hat\alpha^s, \sP(\btheta^s)) - \cG(\hat\alpha^s_{(j)}, \sP(\btheta^s_{(j)}))\big) - \big(\cG(\hat\alpha^{\floor{s}}_{\gamma}, \sP(\btheta^{\floor{s}}_\gamma)) - \cG(\hat\alpha^{\floor{s}}_{\gamma,(j)}, \sP(\btheta^{\floor{s}}_{\gamma,(j)}))\big)}{}\d s\\
&= \int_0^{\floor{t}} \biggpnorm{\Big(\nabla_\alpha \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\hat\alpha^s - \hat\alpha^s_{(j)}) + \nabla_{\btheta} \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\btheta^s - \btheta^s_{(j)}) + \Gamma_1(s)\Big)\\
&\quad  - \Big(\nabla_\alpha \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)}) + \nabla_{\btheta} \cG(\bar{\widehat\alpha}^{s}_{\gamma,(j)}, \sP(\bar{\btheta}^{s}_{\gamma,(j)}))^\top (\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}) + \Gamma_2(s)\Big)}{} \d s\\
&\leq \int_0^t \Big[C\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)} - \bar{\widehat\alpha}^{s}_\gamma + \bar{\widehat\alpha}^{s}_{\gamma,(j)}}{} + \frac{C}{\sqrt{d}}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)} - \bar{\btheta}^{s}_\gamma + \bar{\btheta}^{s}_{\gamma,(j)})}{} + \frac{C}{d}\big|\big(\btheta^s - \btheta^s_{(j)} - \bar{\btheta}^{s}_\gamma + \bar{\btheta}^{s}_{\gamma,(j)}\big)_j\big|\\
&\quad + \pnorm{\Gamma_1(s)}{} + \pnorm{\Gamma_2(s)}{}\Big] \d s\\
&\leq \int_0^t \Big(C\pnorm{\hat\alpha^s - \hat\alpha^s_{(j)} - \hat\alpha^{s}_\gamma + \hat\alpha^{s}_{\gamma,(j)}}{} + \frac{C}{\sqrt{d}}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)} - \bar{\btheta}^{s}_\gamma + \bar{\btheta}^{s}_{\gamma,(j)})}{}\Big) \d s\\
&\quad + \underbrace{\int_0^t \Big[\frac{C}{d}\big|\big(\btheta^s - \btheta^s_{(j)} - \bar{\btheta}^{s}_\gamma + \bar{\btheta}^{s}_{\gamma,(j)}\big)_j\big| + \pnorm{\Gamma_1(s)}{} + \pnorm{\Gamma_2(s)}{}\Big] \d s}_{R_2(t)}.
\end{align*}
We claim that for any positive integer $q\geq 2$, $\limsup_{n,d}\sup_{t\in[0,T]} \E^\circ [(\sqrt{d} \cdot R_2(t))^q] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. To see this, the bound for $\big|\big(\btheta^s - \btheta^s_{(j)} - \bar{\btheta}^{s}_\gamma + \bar{\btheta}^{s}_{\gamma,(j)}\big)_j\big|/\sqrt{d}$ follows from (\ref{eq:single_bound_continuous}) and (\ref{eq:loo_expectation_5}). For $\Gamma_2(t)$, we have by Assumption \ref{assump:prior} that 
\begin{align*}
\pnorm{\Gamma_2(t)}{} &\leq \pnorm{\nabla_\alpha^2 \cG(\alpha, \sP(\btheta))}{\op}\pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)}}{}^2 + \pnorm{\nabla_\alpha \nabla_{\btheta} \cG(\alpha, \sP(\btheta))}{\op}\pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)}}{}\pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}}{}\\
&\quad + \pnorm{\nabla_{\btheta}^2 \cG(\alpha, \sP(\btheta))}{\op}\pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}}{}^2\\
&\leq C\Big(\pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)}}{}^2 + \frac{1}{\sqrt{d}}\pnorm{\bar{\widehat\alpha}^{s}_\gamma - \bar{\widehat\alpha}^{s}_{\gamma,(j)}}{}\pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}}{} + \frac{1}{d} \pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)}}{}^2\Big), 
\end{align*}
hence we have by Lemma \ref{lem:loo_error} that $\sup_{t\in[0,T]} \E^\circ[(\sqrt{d}\pnorm{\Gamma_2(t)}{})^q] \rightarrow_{n,d\rightarrow\infty} 0$ for any fixed realizations of $\theta^0_\cJ, \theta^\ast_\cJ$. Using a similar argument, we also have $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E^\circ[(\sqrt{d}\pnorm{\Gamma_1(t)}{})^q] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$, proving the claim. Hence by a Gronwall argument, we have for any $t\in[0,T]$ that 
\begin{align*}
\sqrt{d}\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)} - \bar{\widehat\alpha}^t_\gamma + \bar{\widehat\alpha}^t_{\gamma,(j)}}{} \leq C\int_0^t \pnorm{E_{(j)}(\btheta^s - \btheta^{s}_{(j)} - \bar{\btheta}^s_{\gamma} + \bar{\btheta}^{s}_{\gamma,(j)})}{} \d s + R(t), 
\end{align*}
where $\limsup_{n,d}\sup_{t\in[0,T]} \E^\circ[R(t)^q] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$.

In summary ,we have shown that
\begin{align*}
&\pnorm{E_{(j)}\Big(s(\btheta^s, \hat\alpha^s) - s(\btheta^s_{(j)}, \hat\alpha^s_{(j)}) - s(\bar{\btheta}^{s}_\gamma, \bar{\widehat\alpha}^{s}_\gamma) - s(\bar{\btheta}^{s}_{\gamma,(j)}, \bar{\widehat\alpha}^{s}_{\gamma,(j)})\Big)}{}\\
&\leq C\pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s_\gamma - \btheta^s_{(j)})}{4} + C\int_0^s \pnorm{E_j(\btheta^{s'} - \btheta^{s'}_{(j)} - \bar{\btheta}^{s'}_\gamma + \bar{\btheta}^{s'}_{\gamma,(j)})}{}\d s' + R(s),
\end{align*}
for some $R(s)$ such that $\sup_{t\in[0,T]} \E^\circ[R(t)^2] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4$.
\end{itemize}

Combining the above three estimates, for term $(II)$ in (\ref{eq:second_order_decomp}), we have for every $t\in[0,T]$ that
\begin{align*}
|(II)| \leq C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^s_\gamma - \btheta_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)})}{}\d s + C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}\d s + C\int_0^t |\theta^s_j - \bar{\theta}^{s}_{\gamma,j}|\d s + R(t),
\end{align*}
where $\sup_{t\in[0,T]} \E^\circ[R(t)^2] \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^4$. Combining the above bound with the bound of $(I)$ in (\ref{eq:bound_I}), we have by (\ref{eq:second_order_decomp}) that
\begin{align*}
&\pnorm{E_{(j)}(\btheta^t - \bar{\btheta}^t_\gamma - \btheta_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)})}{}\\
&\leq C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^s_\gamma - \btheta_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)})}{}\d s + C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}\d s + C\int_0^t |\theta^s_j - \bar{\theta}^s_{\gamma,j}|\d s + R(t), 
\end{align*}
with the same guarantee on $R(t)$. By a Gronwall argument, we have for every $t\in[0,T]$ that
\begin{align*}
\pnorm{E_{(j)}(\btheta^t - \bar{\btheta}^t_\gamma - \btheta_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)})}{} \leq C\int_0^t \pnorm{E_{(j)}(\btheta^s - \bar{\btheta}^{s}_{\gamma})}{4}\pnorm{E_{(j)}(\btheta^s - \btheta^s_{(j)})}{4}\d s + C\int_0^t |\theta^s_j - \bar{\theta}^s_{\gamma,j}|\d s + R(t),
\end{align*}
completing the proof.
\end{proof}

\begin{lemma}\label{lem:l2_discretization_expectation}
Recall the processes $\{\bar{\btheta}^t_\gamma, \bar{\widehat\alpha}^t_\gamma\}_{t\in\R_+}$ in (\ref{eq:langevin_embedded}). Then for any $\gamma > 0$ and $T > 0$, integer $q\geq 2$, and $\cJ \subset [d]$ with $|\cJ| = O(1)$, there exist constants $C,K_\gamma,c$ as specified in Lemma \ref{lem:loo_error} such that 
\begin{align}
\E\Big[\Big(\frac{1}{\sqrt{d}}\pnorm{\btheta^t - \bar{\btheta}^{t}_\gamma}{}\Big)^q \vee \pnorm{\hat\alpha^t - \bar{\widehat\alpha}^{t}_\gamma}{}^q|\theta^0_\cJ, \theta^\ast_\cJ\Big] &\leq h(\gamma)(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q.
\end{align}
for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$.
\end{lemma}
\begin{proof}
This follows from the same analysis as in the proof of Lemma \ref{lem:langevin_discretize_error}, with an additional truncation step in the Gronwall argument as carried out in Lemma \ref{lem:l4_bound}. We omit the proof to avoid redundancy.
\end{proof}

Define the continuous-time version of the leave-column-out sequence in (\ref{eq:leave_col_out}): for any $\cJ \subset [d]$, let
\begin{align}\label{def:leave_col_out_cont}
\notag\btheta^t_{(\cJ)} &= \btheta^0_{(\cJ)} + \int_0^t \Big[-\beta\X_{(\cJ)}^\top (\X_{(\cJ)}\btheta^s_{\cJ} - \y_{(\cJ)}) + s(\btheta^s_{(\cJ)}, \hat\alpha^s_{(\cJ)})\Big] \d s + \sqrt{2}\b^t,\\
\hat\alpha^t_{(\cJ)} &= \hat\alpha^0 + \int_0^t \cG\Big(\hat\alpha^s_{(\cJ)}, \sP(\btheta^s_{(\cJ)})\Big)\d s, 
\end{align}
where $\theta^0_{(\cJ)}, \hat\alpha^0, \y_{(\cJ)}$ are the same as in (\ref{eq:leave_col_out}). The following lemma gives error bounds for $\{\btheta^t_{(\cJ)},\hat\alpha^t_{(\cJ)}\}_{t\in\R_+}$ analogous to those in Lemmas \ref{lem:loo_error} and \ref{|em:loo_linfty_error}.
\begin{lemma}\label{lem:loo_error_continuous}
For any integer $q\geq 2$, $T > 0$, $\cJ\subset [d]$ with $|\cJ|\leq L$, there exist constants $C,c$ as specified in Lemma \ref{lem:loo_error} such that
\begin{align}
\sup_{t\in[0,T]}\E\Big[\Big(\pnorm{\btheta^s - \btheta^s_{(\cJ)}}{} + \sqrt{d}\pnorm{\hat\alpha^s - \hat\alpha^s_{(\cJ)}}{}\Big)^q|\theta^0_\cJ,\theta^\ast_\cJ\Big]&\leq C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q, \label{eq:loo_bound_continuous}\\
\sup_{t\in[0,T]}\max_{j\in[d]}\E[(|\theta^t_j| + \pnorm{\hat\alpha^t}{})^q|\theta^0_\cJ,\theta^\ast_\cJ] &\leq C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q \label{eq:single_bound_continuous},\\
\max_{k\in[d]:k\notin \cJ}\sup_{t\in[0,T]} \E[|\e_k^\top (\btheta^s - \btheta^s_{(\cJ)})|^q|\theta^0_\cJ,\theta^\ast_\cJ] &\leq \frac{C(\pnorm{\theta^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^{q/2}}\label{eq:loo_infty_bound_continuous}.
\end{align}
\end{lemma}
\begin{proof}
The proof is similar to that of Lemmas \ref{lem:loo_error} and \ref{|em:loo_linfty_error}, and we omit it to avoid redundancy.
\end{proof}



\subsubsection{Proof of Proposition \ref{prop:entrywise_langevin_discretize}}
\begin{proof}
Let $\E^\circ$ denote expectation conditioning on $(\theta^0_\cJ, \theta^\ast_\cJ) = (\xi^0_\cJ, \xi^\ast_\cJ)$. It suffices to bound, for each $j\in\cJ$, $\E^\circ\big[\pnorm{(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}) - (\theta^{\tau_1}_{j},\ldots, \theta^{\tau_m}_{j})}{}^2\big] = \sum_{\ell=1}^m \E^\circ \big[(\theta^{\tau_\ell}_j - \theta^{\tau_\ell}_{\gamma,j})^2\big]$.
Recall the discretized Brownian motion $\{\b^t_\gamma\}_{t\in\R_+}$ defined in (\ref{eq:hd_BM_linear}). Let $\bar{\X}\in\R^{n\times (d-1)}$ denote $\X$ minus its $j$th column, and $\bar{\btheta}^t, \bar{\btheta}^t_\gamma \in \R^{d-1}$ denote $\btheta^t, \btheta^t_\gamma$ minus the $j$th entry. By definition, we have 
\begin{align*}
\theta^t_j &= \theta^0_j + \int_0^t \Big(-\beta\big(\pnorm{\x_j}{}^2 \theta^s_j + \x_j^\top \bar{\X} \bar{\btheta}^s - \x_j^\top \y\big) + s(\theta^s_j,\hat\alpha^s)\Big)\d s + \e_j^\top \b^t,\\
\theta^t_{\gamma,j} &= \theta^0_j + \int_0^t \Big(-\beta\big(\pnorm{\x_j}{}^2 \theta^{\floor{s}}_{\gamma,j} + \x_j^\top \bar{\X} \bar{\btheta}^{\floor{s}}_\gamma - \x_j^\top \y\big) + s(\theta^{\floor{s}}_{\gamma,j}, \hat\alpha^{\floor{s}}_{\gamma})\Big)\d s + \e_j^\top \b^t_\gamma,
\end{align*}
Then by Assumption \ref{assump:prior}, we have
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| &\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2) |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| + C\pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} + C|\x_j^\top \bar{\X} (\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma)|\Big] \d s + \sqrt{2}|\e_j^\top (\b^t - \b^t_\gamma)|\\
&\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 \leq 10\delta}) |\theta^s_j - \theta^{s}_{\gamma,j}| \d s + \int_0^t  C|\x_j^\top \bar{\X} (\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)})|\d s + \underbrace{\int_0^T C\pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} \d s}\\
&\quad + \underbrace{\int_0^T \Big[C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| + (1+ 10C\delta) |\theta^s_{\gamma,j} - \theta^{\floor{s}}_{\gamma,j}| + C|\x_j^\top \bar{\X} (\bar{\btheta}^s_{(j)} - \bar{\btheta}^{\floor{s}}_{\gamma,(j)})|\Big] \d s + \sqrt{2}\sup_{t\in[0,T]} |b^t_j - b^t_{\gamma,j}|}_{A_1(T)}\\
&\leq \int_0^t (C + 10C\delta) |\theta^s_j - \theta^{s}_{\gamma,j}| \d s + \int_0^t C\pnorm{\X}{\op}^2 \pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{} \d s + A_1(T).
\end{align*}
We may further decompose the middle term as
\begin{align*}
\pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{} \leq \pnorm{\bar{\btheta}^s - \bar{\btheta}^{s}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)}}{} + \pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{},
\end{align*}
where by Lemma \ref{lem:theta_decomp}, we have for any $t\in[0,T]$ that
\begin{align*}
\int_0^t \pnorm{\bar{\btheta}^s - \bar{\btheta}^{s}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)}}{} \d s \leq \exp(CT)CT\pnorm{\X}{\op}^2  \int_0^t |\theta^s_j - \theta^s_{\gamma,j}|\d s + \tilde{R}(t),
\end{align*}
for some $\tilde{R}(t)$ such that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E \tilde{R}^2(t) \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. Hence by a similar truncation argument as above applied to $\pnorm{\X}{\op}$, we conclude that for any $t\in[0,T]$, 
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| \leq C\int_0^t |\theta^s_j - \theta^s_{\gamma,j}|\d s + A_1(T) + A_2(T), 
\end{align*}
for some $A_2(T)$ such that $\limsup_{n,d\rightarrow\infty} \E A_2^2(T) \leq h(\gamma)$. By a Gronwall argument, this further implies
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| \leq \exp(Ct)(A_1(T) + A_2(T)), \quad \forall t\in[0,T]. 
\end{align*}
It remains to bound $\E^\circ A_1^2(T)$, which satisfies
\begin{align*}
\E^\circ A_1^2(T) &\leq C \E^\circ\Big(\int_0^T \pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| \d s\Big)^2 + C \E^\circ\Big(\int_0^T |\theta^s_{\gamma,j} - \theta^{\floor{s}}_{\gamma,j}| \d s\Big)^2 + C\E^\circ\Big(\int_0^T \pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} \d s\Big)^2\\
&\quad + C\E^\circ \Big(\int_0^T |\x_j^\top \bar{\X} (\bar{\btheta}^s_{(j)} - \bar{\btheta}^{\floor{s}}_{\gamma,(j)})| \d s\Big)^2 + C\E^\circ\sup_{t\in[0,T]} |b^t_j - b^t_{\gamma,j}|^2 := \sum_{i=1}^5 \zeta_i.
\end{align*}
By standard concentration and bound (\ref{eq:single_entry_moment}), the term $\zeta_1$ is bounded by $K_\gamma\exp(-c\sqrt{d})(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$.  For term $\zeta_2$, we have
\begin{align*}
|\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| &\leq C\gamma\Big(\pnorm{\x_j}{}^2 |\theta^{\floor{s}}_{\gamma,j} - \theta^\ast_j| + \big|\x_j^\top \bar{\X} (\bar\btheta^{\floor{s}}_{\gamma} - \bar{\btheta}^\ast)| + |\x_j^\top\beps|\Big) + \sqrt{2} \sup_{t\in [0,T]} |b^t_j - b^{\floor{t}}_j| + |b^t_j - b^{\ceil{t}}_j|\\
&\leq C\gamma\Big(\pnorm{\x_j}{}^2 |\theta^{\floor{s}}_{\gamma,j} - \theta^\ast_j| + \big|\x_j^\top \bar{\X} (\bar\btheta^{\floor{s}}_{\gamma,(j)} - \bar{\btheta}^\ast)| + \pnorm{\x_j}{}\pnorm{\X}{\op}\pnorm{\btheta^{\floor{s}}_\gamma - \btheta^{\floor{s}}_{\gamma,(j)}}{} + |\x_j^\top\beps|\Big)\\
&\quad + \sqrt{2} \sup_{t\in [0,T]} |b^t_j - b^{\floor{t}}_j| + |b^t_j - b^{\ceil{t}}_j|,
\end{align*}
where $\{\btheta^t_{\gamma,(j)}\}_{t\in\R_+}$ is defined in (\ref{eq:cont_time_loo_col}), and $\bar{\btheta}^t_{\gamma,(j)} \in \R^{d-1}$ denotes it without the $j$th entry. By independence between $\x_j$ and $\bar{\X}, \btheta^{\floor{s}}_{\gamma,(j)}$, the 1-dimensional version of Lemma \ref{lem:BM_maximal}, and Lemma \ref{lem:loo_error}, we conclude that $\zeta_2\vee \zeta_5 \leq h(\gamma)(C+K_\gamma \exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$. Next by the bound (\ref{eq:combine_alpha_theta_bound}) and a simple truncation argument, and bound (\ref{eq:alpha_discrete_error}), it holds that $\zeta_3 \leq h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. Lastly, $\zeta_4$ is also bounded by some $h(\gamma)(C+K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$ by independence between $\x_j$ and $\bar{\X}, \bar{\btheta}^s_{(j)}, \bar{\btheta}^{\floor{s}}_{\gamma,(j)}$, and bound (\ref{eq:combine_alpha_theta_bound}) and a simple truncation argument. We therefore conclude that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E^\circ |\theta^t_j - \theta^t_{\gamma,j}|^2 \leq h(\gamma)(\pnorm{\xi^0_\cJ}{} + \pnorm{\xi^\ast_\cJ}{} + 1)^2$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$, as desired.
%Let $\X_{(j)} \in \R^{n\times d}$ be $\X$ with its $j$th column set to zero, $\y_{(j)} = \X_{(j)}\btheta^\ast + \eps$, and $\{\btheta^t_{(j)}\}_{t\in\R_+} \subset \R^d$ be the continuous leave-one-column-out dynamic defined by
%\begin{align*}
%\btheta^t_{(j)} = \btheta^0 + \int_0^t \Big[-\frac{1}{\sigma^2}\X_{(j)}^\top (\X_{(j)} \btheta^s_{(j)} - \y_{(j)}) + \partial_\theta \log g(\btheta^s_{(j)})\Big]\d s + \sqrt{2}\b^t.
%\end{align*}
%Let $\{\btheta^t_{\gamma,(j)}\}_{t\in\R_+}$ be defined similarly, and $\bar{\btheta}^t_{(j)}, \bar{\btheta}^t_{\gamma,(j)}\in\R^{d-1}$ be $\btheta^t_{(j)}, \btheta^t_{\gamma,(j)}$ without the $j$th entry.  
\end{proof}

%\begin{lemma}\label{lem:theta_decomp}
%Assume the conditions of Theorem \ref{thm:dmft_entrywise}. For any fixed $T > 0$, there exists some function $h(\gamma) = h(\gamma;T) \rightarrow 0$ as $\gamma \rightarrow 0$ such that
%\begin{align*}
%\sup_{t\in[0,T]}\E\Big[\pnorm{\btheta^t_\gamma - \btheta^{\floor{t}}_\gamma - \btheta^t_{\gamma,(j)} + \btheta^{\floor{t}}_{\gamma,(j)}}{}^q|\theta^0_\cJ, \theta^\ast_\cJ\Big] &\leq h(\gamma)(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q, \\
%\sup_{t\in[0,T]}\E\Big[\pnorm{\hat\alpha^s_\gamma - \hat\alpha^{\floor{s}}_\gamma - \hat\alpha^s_{\gamma,(j)} + \hat\alpha^{\floor{s}}_{\gamma,(j)}}{}^q|\theta^0_\cJ, \theta^\ast_\cJ\Big] &\leq h(\gamma)\frac{(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q}{d^{q/2}}.
%\end{align*}
%\end{lemma}
%\begin{proof}
%We first expand $\pnorm{\btheta^{s}_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^{s}_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{}$. By definition, we have
%\begin{align*}
%\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma &= (s-\floor{s})\Big[-\beta\X^\top(\X\btheta^{\floor{s}}_\gamma - \y) + s(\btheta^{\floor{s}}_\gamma, \hat\alpha^{\floor{s}}_{\gamma})\Big] + \sqrt{2}(\b^{s}_\gamma - \b^{\floor{s}}_\gamma),\\
%\btheta^s_{\gamma,(j)} - \btheta^{\floor{s}}_{\gamma,(j)} &= (s-\floor{s})\Big[-\beta\X_{(j)}^\top(\X_{(j)}\btheta^{\floor{s}}_{\gamma,(j)} - \y_{(j)}) + s(\btheta^{\floor{s}}_{\gamma,(j)}, \hat\alpha^{\floor{s}}_{\gamma,(j)})\Big] + \sqrt{2}(\b^{s}_{\gamma} - \b^{\floor{s}}_{\gamma}),
%\end{align*}
%which implies that
%\begin{align*}
%\pnorm{\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{} &\leq C\gamma \Big(\pnorm{(\X^\top \X - \X_{(j)}^\top \X_{(j)})\btheta^{\floor{s}}_{\gamma,(j)}}{} + \pnorm{\X}{\op}^2\pnorm{\btheta^{\floor{s}}_{\gamma} - \btheta^{\floor{s}}_{\gamma,(j)}}{}\\
%&\quad + \pnorm{\hat\alpha^{\floor{s}}_{\gamma} - \hat\alpha^{\floor{s}}_{\gamma,(j)}}{} + \pnorm{\X^\top \y - \X_{(j)}^\top \y_{(j)}}{}\Big).
%\end{align*}
%By bounds (\ref{ineq:loo_1}), (\ref{ineq:loo_2}), and the conclusion of Lemma \ref{lem:loo_error}, we conclude that $\E[\pnorm{\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{}^q|\theta^0_\cJ, \theta^\ast_J] \leq h(\gamma)(C + K_\gamma\exp(-c\sqrt{d}))(\pnorm{\xi^0_\cJ}{} + \pnorm{\theta^\ast_\cJ}{} + 1)^q$. For the second claim, a similar argument along with Assumption \ref{assump:gradient} yield
%\begin{align*}
%\pnorm{\hat\alpha^s_\gamma - \hat\alpha^{\floor{s}}_\gamma - \hat\alpha^s_{\gamma,(j)} + \hat\alpha^{\floor{s}}_{\gamma,(j)}}{} \leq C\gamma\Big(\pnorm{\hat\alpha^{\floor{s}}_\gamma - \hat\alpha^{\floor{s}}_{\gamma,(j)}}{} + \pnorm{\btheta^{\floor{s}}_\gamma - \btheta^{\floor{s}}_{\gamma,(j)}}{}/\sqrt{d}\Big),
%\end{align*}
%hence the claim again follows from Lemma \ref{lem:loo_error}.
%\end{proof}



\subsection{Completing the proof}
Using a similar tightness argument as in the proof of Theorem \ref{thm:dmft_approx}, it suffices to show that for any fixed integer $m$, $\tau_1,\ldots,\tau_m\in\R_+$, and $j\in[d]$, it holds that $W_1(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)) \rightarrow 0$ as $n,d\rightarrow\infty$. To this end, we have for any $\gamma > 0$ that
\begin{align*}
&W_1\Big(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big) \leq  W_1\Big(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}, \theta^\ast_j)\Big)\\
&+ W_1\Big(\sP(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}, \theta^\ast_j), \sP(\bar{\theta}^{\tau_1}_{\gamma},\ldots, \bar{\theta}^{\tau_m}_{\gamma}, \theta^\ast)\Big) + W_1\Big(\sP(\bar{\theta}^{\tau_1}_{\gamma},\ldots, \bar{\theta}^{\tau_m}_{\gamma}, \theta^\ast), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big).
\end{align*}
The desired conclusion follows by taking first $\limsup_{n,d\rightarrow\infty}$ and then $\gamma \rightarrow 0$, applying Propositions \ref{prop:entrywise_discrete_approx}, \ref{prop:entrywise_langevin_discretize}, and Lemma \ref{lem:dmft_discretization_error}.

%Recall that $\bR_{\theta}(t,s) = \big(\E[\partial_j P_{t-s} e_k(\btheta^s)]\big)_{j,k=1}^d$, where the expectation is taken with respect to the Brownian motion in $\{\btheta^t\}$. We will show that for any bounded and continuous $h(\cdot)$, 
%\begin{align*}
%\int_0^t \frac{1}{d}\Tr \bR_\theta(t,s)h(s)\d s \rightarrow \int R_\theta(t,s)h(s) \d s. 
%\end{align*}
%Define the following two perturbed processes on $[0,T]$: for each $j\in[d]$ and $\eps > 0$, 
%\begin{align*}
%\btheta^{t,(j,\eps)} &= \btheta^0 + \int_0^t \Big(-\frac{1}{\sigma^2}\X^\top (\X \btheta^{s,(j,\eps)} - \y) - f'(\btheta^{s,(j,\eps)}) + \eps \e_jh(s)\Big)\d s + \sqrt{2}\b^t,\\
%\tilde{\btheta}^{t,(j,\eps)} &= \btheta^0 + \int_0^t \Big(-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{\floor{s},(j,\eps)} - \y) - f'(\tilde{\btheta}^{\floor{s},(j,\eps)}) + \eps \e_jh(\floor{s})\Big)\d s + \sqrt{2}\b^t. 
%\end{align*}
%Let $\{\btheta^t\}$ and $\{\tilde{\btheta}^t\}$ denote the unperturbed processes with $\eps = 0$. Note that at knots, 
%\begin{align*}
%\tilde{\btheta}^{(k+1)\gamma,(j,\eps)} = \tilde{\btheta}^{k\gamma,(j,\eps)} + \gamma\Big[-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{k\gamma,(j,\eps)} - \y) - f'(\tilde{\btheta}^{k\gamma,(j,\eps)}) + \eps \e_jh(k\gamma)\Big] + \sqrt{2}(\b^{(k+1)\gamma} - \b^{k\gamma}).
%\end{align*}
%Since $\int_0^t d^{-1}\Tr \bR_\theta(t,s)\d s = \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j]$, we have
%\begin{align*}
%\Big|\int_0^t d^{-1}\Tr \bR_\theta(t,s)\d s - \int R_\theta(t,s)h(s) \d s\Big| \leq (I) + (II) + (III),
%\end{align*}
%where
%\begin{align}
%(I) &= \Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j] - \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big|,\\
%(II) &= \Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big|
%\end{align}
%\textbf{Bound of $(I)$} We start with
%\begin{align*}
%\Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j] - \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big| \leq \frac{1}{d}\sum_{j=1}^d\E\Big|\partial_\eps|_{\eps = 0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{t,(j,\eps)}_j\Big|,
%\end{align*}
%and let us bound the right side quantity. By definition, with
%\begin{align*}
%\W^{s} = -\frac{1}{\sigma^2}\X^\top \X - \diag\big(f''(\btheta^{s})\big), \quad \tilde{\W}^{s} = -\frac{1}{\sigma^2}\X^\top \X - \diag\big(f''(\tilde{\btheta}^{s})\big),
%\end{align*}
%we have
%\begin{align}\label{eq:theta_eps_der}
%\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} &= \int_0^t \Big( \W^{s}\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} + \e_jh(s)\Big)\d s,\\
%\partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)} &= \int_0^t \Big(\tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} + \e_jh(\floor{s})\Big)\d s.
%\end{align}
%This implies
%\begin{align*}
%&\pnorm{\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)}}{}\\
%&= \pnorm{\int_0^t \W^{s} \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} \d s - \int_0^t \e_j^\top \tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} \d s + \int_0^t \e_jh(s) \d s  - \int_0^t \e_j h(\floor{s}) \d s}{}\\
%&\leq \int_0^t \pnorm{(\W^{s} - \tilde{\W}^{s}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s + \int_0^t \pnorm{(\tilde{\W}^{s} - \tilde{\W}^{\floor{s}}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s\\
%&\quad + \int_0^t \pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)}{}\d s +  \int_0^t \pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}\big)}{}\d s
%\end{align*}
%For the first term,
%\begin{align*}
%\pnorm{(\W^{s} - \tilde{\W}^{s}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq \pnorm{\W^{s} - \tilde{\W}^{s}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq \pnorm{f'''}{\infty}\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq C\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty}, 
%\end{align*}
%using Lemma \ref{lem:discrete_estimate}. For the second term, we similarly have
%\begin{align*}
%\pnorm{(\tilde{\W}^{s} - \tilde{\W}^{\floor{s}}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq C\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{\infty}.
%\end{align*}
%For the third term, we have
%%\begin{align*}
%%&\Big|\e_j^\top\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)\Big|\\
%%&\leq \frac{1}{\sigma^2}\Big|\e_j^\top \X^\top \X \big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)\Big| + \pnorm{f''}{\infty}\Big|\partial_\eps|_{\eps = 0} \btheta_j^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}_j^{s,(j,\eps)}\Big|\\
%%&\leq \Big(\frac{\pnorm{\x_j}{}^2}{\sigma^2} + \pnorm{f''}{\infty}\Big) \Big|\partial_\eps|_{\eps = 0} \btheta_j^{s,(j,\eps)} - \partial_\eps|_{\eps = 0}\tilde{\btheta}_j^{s,(j,\eps)}\Big| + \underbrace{\Big|\x_j^\top \sum_{k:k\neq j}\x_k \big(\partial_\eps|_{\eps = 0} \btheta_k^{s,(j,\eps)} - \partial_\eps|_{\eps = 0}\tilde{\btheta}_k^{s,(j,\eps)}\big)\Big|}_{R_j^s}.
%%\end{align*}
%\begin{align*}
%\pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)}{} \leq \pnorm{\tilde{\W}^{\floor{s}}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}}{} \leq L\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}}{},
%\end{align*}
%where $L = \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$. For the fourth term, it is bounded by $\pnorm{\tilde{\W}^{\floor{s}}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}}{}$, where, since
%\begin{align*}
%\partial_\eps|_{\eps=0} \tilde{\btheta}^s = \partial_\eps|_{\eps=0} \tilde{\btheta}^{\floor{s}} + (s - \floor{s})\Big(\tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} + \e_jh(\floor{s})\Big),
%\end{align*}
%we have by Lemma \ref{lem:discrete_estimate} that $\pnorm{\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}}{} \leq C\gamma$. Together with the bound $\pnorm{\tilde{\W}^{\floor{s}}}{\op} \leq \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$, we have
%\begin{align*}
% \int_0^t \Big|\e_j^\top \tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}\big)\Big|\d s \leq C\gamma.
%\end{align*}
%Combining the above four bounds, we have
%\begin{align*}
%\pnorm{\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)}}{} &\leq L\int_0^t \sup_{u\leq s}\pnorm{\partial_\eps|_{\eps=0} \btheta^{u,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{u,(j,\eps)}}{}\d s\\
%&\quad + C\int_0^t \Big(\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty} + \pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{\infty}\Big)\d s + C\gamma.
%\end{align*} 
%Hence applying Lemma \ref{lem:gronwall} yields that for any $t\leq T$,
%\begin{align*}
%\Big|\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps=0} \tilde{\btheta}_j^{t,(j,\eps)}\Big| \leq e^{C_1t} \cdot\Big[ C_2\int_0^t \Big(|\btheta^s_j - \tilde{\btheta}^s_j| + |\tilde{\btheta}^{s}_j - \tilde{\btheta}^{\floor{s}}_j| + R_j^s\Big)\d s + C\gamma\Big],
%\end{align*}
%which further implies that
%\begin{align*}
%\sum_{j=1}^d\Big|\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps=0} \tilde{\btheta}_j^{t,(j,\eps)}\Big| \leq C\sqrt{d} \cdot \int_0^t \big(\pnorm{\btheta^s - \tilde{\btheta}^s}{} + \pnorm{\tilde{\btheta}^{s} - \tilde{\btheta}^{\floor{s}}}{} + \pnorm{\bR^s}{}\big)\d s + Cd\gamma,
%\end{align*}
%where $\bR^s = (R^s_1,\ldots, R^s_d)$.
%
%
%\begin{lemma}
%Control $\pnorm{\btheta^s - \tilde{\btheta}^s}{}$ and $\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{}$
%\end{lemma}
%\begin{proof}
%Since
%\begin{align*}
%\pnorm{\btheta^t}{} \leq \pnorm{\btheta^0}{} + \int_0^t \Big(\frac{1}{\sigma^2}\pnorm{\X^\top}{\op}^2 + \pnorm{f''}{\infty}\Big)\pnorm{\btheta^s}{}\d s + t\sqrt{d}|f'(0)| + \sqrt{2}\pnorm{\b^t}{},
%\end{align*}
%we have by Lemma \ref{lem:gronwall} that
%\begin{align*}
%\pnorm{\btheta^t}{} \leq e^{Lt}\Big[\pnorm{\btheta^0}{} + t\sqrt{d}|f'(0)| + \sqrt{2}\pnorm{\b^t}{}\Big],
%\end{align*}
%which implies that $\E\pnorm{\btheta^t}{}^2 \leq C(\pnorm{\btheta^0}{}^2 + d)$. A similar bound holds for $\E\pnorm{\tilde{\btheta}^t}{}^2$. Note that
%\begin{align*}
%\tilde{\btheta}^s = \tilde{\btheta}^{\floor{s}} + (s-\floor{s})\Big(-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{\floor{s}} - \y) - f'(\tilde{\btheta}^{\floor{s}}) \Big) + \sqrt{2}(\b^s - \b^{\floor{s}}),
%\end{align*}
%hence
%\begin{align*}
%\E\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{}^2 \leq C\gamma^2\Big(\pnorm{\X}{\op}^4 \E\pnorm{\tilde{\btheta}^{\floor{s}}}{}^2 + \pnorm{\X^\top \y}{}^2\Big) + C\gamma d \leq C\gamma(\pnorm{\btheta^0}{}^2 + \pnorm{\X^\top \y}{}^2 + d). 
%\end{align*}
%\end{proof}
%
%
%
%\begin{lemma}\label{lem:discrete_estimate}
%Fix any $T > 0$. Then there exist some $C > 0$ depending on $T, \pnorm{h}{\infty}$, such that for any $t \leq T$,
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \leq Ce^{Lt}
%\end{align*}
%\end{lemma}
%\begin{proof}
%Note that $\pnorm{\W^{s,(j)}}{\op} \leq L := \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$. For any fixed $T > 0$ and $t\leq T$, we have
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} &\leq \int_0^t L \pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s + \int_0^t |h(s)|\d s\\
%&\leq L\int_0^t \sup_{u\leq s}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \d s + C,
%\end{align*}
%where $C$ depends on $t$ and $\pnorm{h}{\infty}$. Applying Lemma \ref{lem:gronwall} to $t\mapsto \sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{}$, we obtain
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \leq Ce^{Lt}.
%\end{align*}
%\end{proof}





